A survey on Adversarial Recommender Systems: from Attack/Defense strategies to Generative Adversarial Networks

Latent-factor models (LFM) based on collaborative filtering (CF), such as matrix factorization (MF) and deep CF methods, are widely used in modern recommender systems (RS) due to their excellent performance and recommendation accuracy. However, success has been accompanied with a major new arising challenge: many applications of machine learning (ML) are adversarial in nature. In recent years, it has been shown that these methods are vulnerable to adversarial examples, i.e., subtle but non-random perturbations designed to force recommendation models to produce erroneous outputs. The goal of this survey is two-fold: (i) to present recent advances on adversarial machine learning (AML) for the security of RS (i.e., attacking and defense recommendation models), (ii) to show another successful application of AML in generative adversarial networks (GANs) for generative applications, thanks to their ability for learning (high-dimensional) data distributions. In this survey, we provide an exhaustive literature review of 74 articles published in major RS and ML journals and conferences. This review serves as a reference for the RS community, working on the security of RS or on generative models using GANs to improve their quality.

==> OLD_FILES/OLD2_Sec3.tex <==
\section{Adversarial Learning for GAN-based Recommendation}~\label{sec:GAN}
\yd{What we presented in Section~\ref{sec:security} dealt with a class of statistical models referred to as \dquotes{discriminative} models. In the context of classification, a discriminative model is a model that seeks to find the mapping $x \rightarrow y$ for a given input-label pair $(x,y)$, by learning the conditional probability $p(y|x)$ from the training data. The focus of the current section is on a novel class of \dquotes{generative} models, named \textit{generative adversarial networks} (GANs). A generative model is a model that seeks to find the mapping $y \rightarrow x$ by learning the conditional probability $p(x|y)$ from the data. For example, if $y$ indicates whether an item is appealing to a user, $p(y|x)$ would measure the probability --- or whether or not --- the user would like the product; instead $p(x|y=1)$ looks into the distribution of product features appreciated by the user and $p(x|y=0)$, the distribution of irrelevant product features for the user. Loosely speaking, a generative model cares about the \textit{generative} process behind data --- or product features (in the example) ---  to categorize the data instances. A discriminative model disregards the information about how the data were generated, it merely focuses on how to \textit{categorize} given data instances.}

\yd{GANs are a powerful class of generative models that use two networks --- trained simultaneously in zero-sum game --- with one network focused on data generation and the other centered on discrimination. The adversarial learning scheme --- or the the min-max game --- which lies in the heart of GANs empowers these ML models with phenomenal capabilities such as the ability to model high-dimensional distributions. As the result, these networks have been exploited to solve challenging problem in the computer vision. For instance in [xxx]~\felice{Which paper?} \yashar{Just add one good paper here, from a good venue CVPR or NIPS. I guess we have many papers addressing this.}, a GAN model is proposed to generate plausible looking scenes. The research in RS community has used the generalization (or in technical term data distribution capturing) potential of GANs as an opportunity to solve variety of tasks relevant to RS.}

\yd{In summary, it is important to distinguish between two different applications of AML in RS and in a general term:}

\begin{enumerate}
    \item \yd{Adversarial learning to study attacks on, and defenses of machine-learned RS models. This aspect is centred on the \dquotes{security} of recommender models. We discussed this aspect in Section~\ref{sec:security}.}
    \item  \yd{Adversarial learning scheme used in GANs, empowering them to generalize and learn the data distributions. We refer to this aspect the \dquotes{generative} potential of GANs, which have been exploited in the field of RS. The focus of the current section is on this aspect.}
\end{enumerate}

\yd{As it can be noted the term \dquotes{adversarial} inside generative adversarial networks refers to the learning scheme used by these models and \textit{not the application}. In other words, the application of GANs for RS covers variety of aspects not limited to the security of RS, as we will see in the subsequent sections.}


\begin{comment}
This model, as its name suggests,
is able to generate new data that closely resemble the examples used during training. The development of GANs has made possible one of the most
challenging problems in computer vision: image-to-image translation. Just as
language translation seeks to translate one sentence from one language to another without altering the meaning, image-to-image translation aims to map
an image from one domain to another, without losing information about the
content

The two models are trained together in a zero-sum game, adversarial, until the discriminator model is fooled about half the time, meaning the generator model is generating plausible examples.

They are used widely in image generation, video generation and voice generation.
\end{comment}

\subsection{Foundations of Generative Adversarial Networks (GANs)}


\begin{comment}
\yd{GANs are a special type of neural network models where
two networks are trained simultaneously, with one focused on
data (e.g., image) generation and the other centered on discrimination. The
adversarial training scheme has gained attention in both academia
and industry due to its usefulness in counteracting domain shift,
and effectiveness in generating new image samples. This model
has achieved state-of-the-art performance in many image generation tasks, including, for instance, text-to-image synthesis, style-transfer and image domain adaptation.}

Generative adversarial network (GAN) architecture is composed by two neural networks, pitting one against the other (thus the “adversarial”) in order to generate new, synthetic instances of data that can pass for real data. They are used widely in image generation, video generation and voice generation.

GANs were introduced in a paper by Ian Goodfellow and other researchers at the University of Montreal, including Yoshua Bengio, in 2014~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14}. Referring to GANs, Facebook’s AI research director Yann LeCun called adversarial training “the most interesting idea in the last 10 years in ML.”
\end{comment}

\yd{GAN are deep generative models proposed by Goodfellow et al.,~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14} in 2014. A GAN is composed by two components, a generator $\mathcal{G}$, and a discriminator $\mathcal{D}$. The generator works to capture the real data distribution to generate adversarial examples and fool the discriminator,  while the discriminator endeavors to distinguish the fake examples from real ones.
This competition, known as adversarial learning, ends when the components reach the Nash equilibrium. The GAN architecture is shown in Figure~\ref{fig:gan_architecture}.} 

\begin{definition}[Conventional Vanilla GAN]
\yd{\textit{Assume that we are given a dataset of $n$ input samples $x \in \mathcal{X}$, where $x \sim \mathbb{P}_{\mathcal{X}}$ and $\mathbb{P}_{\mathcal{X}}$ represents the probability distribution of the original data and suppose $z \in \mathcal{Z}$ denotes a sample from some latent space $\mathcal{Z}$. We are interested in sampling from $\mathbb{P}_{\mathcal{X}}$. The goal of GAN is to train the generator $\mathcal{G}$ to transform samples $z \sim \mathbb{P}_{\mathcal{Z}}$ into $g_{\theta}(z) \sim \mathbb{P}_{\theta}$ such that $ \mathbb{P}_{\theta} \approx \mathbb{P}_{\mathcal{X}}$. The role of the discriminator is to distinguish $\mathbb{P}_{\theta}$ and $\mathbb{P}_{\mathcal{X}}$ by training a classifier $f_{\phi}$. The training involves solving the following min-max objective}}
\begin{equation}
     \label{eq:gan_basic}
     \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z)))
\end{equation}

\yd{where $\theta$ and $\phi$ are model parameters of the discriminator and generator respectively, learned during the trained phase. Different distance measures $f_{\theta}$ lead to different GAN models, e.g., Vanilla GAN (based on Jensen-Shannon divergence)~\cite{DBLP:journals/nips/GoodfellowPMXWOCB14}, Wasserstein GAN (based on Wasserstein distance)~\cite{DBLP:journals/corr/ArjovskyCB17}, and Conditional GAN (based on class conditioning on both the generator and discriminator)~\cite{DBLP:journals/corr/MirzaO14}.}
\end{definition}

\begin{definition}[Conditional-GAN (CGAN)]
\yd{\textit{Conditional GAN is proposed by Mirza et al.,~\cite{DBLP:journals/corr/MirzaO14} in which the model extends the conventional vanilla GAN presented in Def. 3.1, by incorporating $c$ --- an extra condition information term --- on both the input of the generator $\mathcal{G}$ and the discriminator $\mathcal{D}$, thus conditioning them on this extra term}}
\begin{equation}
     \label{eq:gan_basic}
     \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x|c) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z|c)))
\end{equation}
\yd{\textit{where $c$ can represent any auxiliary information to the networks such as class labels, content features, data from other domains and so forth.}}
\end{definition}
%Generative algorithms can be classified into two classes: explicit density model and implicit density model.

%There exist two general ways of applying adversarial learning to recommender system:
%\begin{enumerate}
%    \item using the adversarial learning to study the \textit{security} of recommender models (see Section~\ref{sec:security})
%    \item using generative adversarial networks (GAN)-based recommender systems.
%\end{enumerate}

%GAN-based recommender systems are at the core of this section where the training of a GAN is based on the typical game theoretic scenario at the core of the adversarial learning for security purposes (i.e., the \textit{min-max  game}). 
%The difference is that, while the use of AML in security settings (e.g. Section~\ref{sec:security}) has the goal to study attack/ defense methods, in the case of GAN-based recommender models AML is the learning paradigm of the deep generative model. 
%Different applications of GAN-based recommender systems have been proposed to address different goals. 
%We reviews them in Section~\ref{subsec:Applications of GAN-based Recommendation}.

%\begin{figure}
%  \begin{subfigure}[b]{0.75\textwidth}
%    \includegraphics[width=0.9\textwidth]{Pictures/GAN_part1_crop.pdf}
%    \caption{Conventional vanilla GAN model}
%    \label{fig:1}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.75\textwidth}
%    \includegraphics[width=0.9\textwidth]{Pictures/GAN_part2_crop.pdf}
%    \caption{Conditional GAN model}
%    \label{fig:2}
%  \end{subfigure}
%  \caption{Schematic comparison of two well-known GAN models.}
%\end{figure}

\begin{figure}
    \includegraphics[width=0.85\textwidth]{Pictures/GAN_joint.pdf}
  \caption{Schematic comparison of two well-known GAN models: (a) conventional vanilla GAN with filled color and (b) Conditional GAN (which includes the dashed blue entities)}
  \label{fig:gan_architecture}

\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.85\textwidth]{Pictures/GAN_General.pdf}
%    \caption{Schematic video of a GAN. The input of the generator $G$ is a random noise vector z, where $ z \sim \mathcal{N}(\mu,\,\sigma^{2})$. Then, $z$ is mapped to a fake sample through the generator model function, $G(z)$. Real sample $x$ from ground-truth data distribution, and generated sample $G(z)$ are the input of the discriminator $D$, a binary classifier. $D$ classifies if the input sample is real rather than generated. The GAN reaches the convergence when $D$ cannot discriminate between $G(z)$ and $x$. At this point, $G$ has learned the ground-truth data distribution.}
%    \label{fig:gan_architecture}
%\end{figure}

\begin{comment}

GAN are \textit{generative} models, which learn the mapping from \textit{random noise} $\rightarrow$ \textit{real data} . This tends to be a difficult task for high-dimensional unstructured data such as images. In fact, for this reason GAN got fame originally for their ability to generate image that looked authentic to original images and then were applied on other high-dimensional data such text and audio. 

Research on ML/RecSys community has exploited the power of GAN networks not as a problem, i.e., sensitivity of CF-models against adversarial inputs , rather as an \textit{opportunity} to fine tune the quality of recommendation models. The core idea is to utilize a pair of models ($G$ and $D$) and allow a competition game between the models to occur with the objective that each one can push the other one to achieve its goal better. This novel notion of learning stands at sharp contrast with classical recommendation setting where only one model is in charge of all user preference inference. In the context of GAN-based CF, the two models have the following responsibilities: $G$ generates items that the user might favor and $D$ distinguishes between the distribution generated by $G$ and user's ground truth. Through a competitive iteration between $G$ and $D$ (the \textit{min-max  game}), $G$ will learn the actual distribution of user interest over items (user profile), which will then be used to provide more appealing recommendation to users.
\end{comment}

\subsection{GAN-based Recommendation Framework}\label{subsec:GAN_RF}
\yd{GANs have been successfully applied in start-of-the-at RS to learning recommendation models. Since the first pioneering GAN-based work IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} in 2017, we have witnessed a rapid adoption of these network architectures in many traditional and novel applications and domains. The attempt of this section is to provide a conceptual framework that will show how GANs are employed in RS domain and shed light on particularities and differences of GAN application in RecSys and ML. This section would continue by providing a survey of recent advances in GAN-based recommendation models.}
\vspace{3mm}\\
\noindent {\textbf{Historical background:}} 
\yd{Among the pioneering works that proposed a GAN framework for improving the utility of item recommendation in a CF scenario, it is worth mentioning IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18}. The former proposes a solution for CF based on MF whereas the second one proposed a graph-representation learning for the same problem. We discuss these two pioneering works in detail here (IRGAN) and in Section~\ref{subsec:GAN_CF_rec} (GraphGAN).}

%GraphGAN in more details in Section~\ref{subsec:Applications of GAN-based Recommendation}, while we start from IRGAN details to propose a high-level overview framework for GAN-based recommender systems.

\yd{A fundamental question in IR is: \dquotes{Given a query $q$ and a document ($d$), what is the probability that $d$ is relevant to $q$?}. The answer to this basic question constitutes the basis for document ranking in IR and has been answered under two different perspectives, the generative model and the the discriminative one:}

\begin{itemize}
    \item \yd{The \textbf{generative model} makes the underlying assumption that there exists a stochastic \textit{generative process} between $d$ and $q$. It then answers the above basic question in probabilistic sense, given by \dquotes{How to compute the probability of relevance $R$ for a given document $d$ with respect to a query $q$, or $p(R=r|d,q) = 1- p(R=\bar{r}|d,q)$?}. In text retrieval, two approaches are commonly adopted to estimate the probability $p \, (R=r|d,q)$, which are proven to be equivalent based on different parametrization of the likelihood under the Bayes rule. The first approach is the Robertson-Sparck Jones~\cite{DBLP:journals/ipm/Jones79} approach that models the probability of relevance in a forward manner $q \rightarrow d$ via factorization $p(R=r|d,q) = p(q|r) \,  p(d|q, r)$. It can be shown that this problem is equivalent to the naive Bayes model for classification in which for a given information need $q$, the goal is to classify the document into classes $r$ and $\bar{r}$. The second approach is based on language modeling paradigm~\cite{DBLP:conf/sigir/PonteC98}, that takes the reverse approach $d \rightarrow q$ via factorization $p(R=r|d,q) = p(d|r) p(q|d, r)$; it aims to generate query terms for a given document.
    \item The \textbf{discriminative model} uses a machine learning approach to answer the basic question in which documents and queries are jointly considered as features and the goal is to predict relevance in ML way by using a large amount of training data. Therefore the problem can be seen as $q + d \rightarrow d$. A prominent example of this approach is learning to rank (LTR) whose aim to is to learn the right ranking of documents (or items) given a representation of an information need (query or context).}
\end{itemize}

\yd{Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} presented a unified theory of generative and discriminative methodologies in IR under the GAN framework named IRGAN. The proposed system is validated for different tasks including item recommendation in which the query is constructed from user's historical interactions. During adversarial learning --- the min-max game --- the generator learns true distribution of relevant items as much as possible.  It turns out that this novel training idea results in more satisfactory accuracy in recommendation than optimizing the traditional pure discriminate loss functions based on pointwise, or pairwise, objectives.}\\

\noindent {\textbf{GAN-CF problem formulation and conceptual model:}}
\yd{The prominent recommendation models in the literature that successfully apply GAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17,DBLP:conf/aaai/WangWWZZZXG18} for CF task, utilize the two-player min-max game with objective function built on top of Eq.~\ref{eq:gan_basic}.}
\begin{definition}[The GAN-CF model]
\yd{\textit{Let $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items in a system, respectively. The training objective is given by}}
\begin{equation}
     \label{eq:irgan_basic}
      \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) = \, \mathbb{E}_{i \sim \mathbb{P}_{\mathcal{X}}(i|u)} \, \log f_{\phi}(i|u) + \mathbb{E}_{\hat{i} \sim \mathbb{P}_{\theta}(\hat{i}|u)} \log \, (1-f_{\phi}(\hat{i} | u))
\end{equation}
\yd{\textit{where $i$ is an item receiving implicit (or explicit) feedback by user $u$ (e.g., purchased) and $\hat{i}$ is a generated item. In IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the score functions in $\mathcal{G}$ and $\mathcal{D}$ are generally based on the \textit{sigmoid} function.}} 
\end{definition}
\yd{A few observations are important to be made here: (i) the output of generator $\mathcal{G}$ is a set of item indices deemed relevant to user $u$; (ii) both $\mathcal{G}$ and $\mathcal{D}$ are \textit{user-conditioned}, signifying that model parameters are learnt by considering \textbf{user's personalization}; (iii) the GAN-based CF works does use the noise term as input (to $\mathcal{G}$) as the goal is to generate one unique --- yet plausible --- item rather than a set of items. Figure~\ref{fig:GAN-CF} summarizes these aspects conceptually.} 

\noindent {\textbf{Discrete outcome and sampling strategies:}} 
\yd{The parameters in the GAN-CF model are learned in an end-to-end fashion. 
However, before we can take benefit of this training paradigm, the system needs to solve a critical issue that does not exist on original GAN presented in Def. 3.1. based on sampled noise signal. The generation of recommendation lists is a discrete sampling operation, i.e., performed over discrete candidate items, see Figure~\ref{fig:GAN-CF}. Thus, the gradients that are derived from the objective function in Eq.~\eqref{eq:irgan_basic} cannot be directly used to optimize the generator via gradient descent as happens in the original GAN formulation, where gradients are applied for differentiable values (e.g.,images and videos). To obtain differentiable sampling strategy in GAN-CF models, two sampling strategies are proposed in the literature based on reinforcement learning algorithm and the Gumbel-Softmax differentiable sampling procedure~\cite{DBLP:conf/nips/SuttonMSM99,DBLP:conf/iclr/JangGP17, DBLP:journals/eswa/SunWWY19}, summarized in Table~\ref{tbl:smple_strg}.}

\begin{table}
\caption{Key sampling strategies proposed for CF-GAN recommendation models}
\label{tbl:smple_strg}
\centering
\begin{tabular}{@{} lll @{}} 
\toprule
    \textbf{Method} & 
    \textbf{Key insight} & 
    \textbf{Formal description} \\  
    \midrule
    \begin{tabular}[l]{@{}l@{}}
    \small{REINFORCE} \\ 
    \small{\cite{DBLP:conf/nips/SuttonMSM99}}
    \end{tabular} & 
    \small{
    \begin{tabular}[l]{@{}l@{}}Optimize $G$ with $K$ discrete \\ items $\hat{i}_k$.\end{tabular}}
     & 
    \begin{minipage}{7cm}
    $ \nabla_{\theta} \simeq \frac{1}{K} \sum_{k=1}^{K} \nabla_{\theta} \log p_{\theta}(\hat{i}_k | u,r) \log (1-f_{\phi}(\hat{i}_k | u)))$
    \end{minipage} \\ [5pt] 
    \begin{tabular}[l]{@{}l@{}}
    \small{Gumbel-Softmax} \\\small{\cite{DBLP:conf/iclr/JangGP17, DBLP:journals/eswa/SunWWY19}}
    \end{tabular}
    & 
    \small{
    \begin{tabular}[l]{@{}l@{}}Approximate discrete items \\ through a continuous \\ differentiable estimator. \end{tabular}}
    & \begin{minipage}{7cm}
    $ v_k = \frac{\exp \left(\left(\log p_{\theta}\left(i_{k}| u, r\right)+g_{k}\right) / \tau\right)}{\sum_{j=1}^{K} \exp \left(\left(\log p_{\theta}\left(i_{j}| u, r\right)+g_{j}\right) / \tau\right)}$
    \end{minipage} \\ 
    \midrule
    \multicolumn{3}{l}{\small{\textit{In the Gumbel-Softmax formulation $g_k$ and $g_j$ represent sampled noise.}}} \\ \bottomrule
\end{tabular}
\end{table}
%\yashar{If I have missed other aspect, it would be insightful to add it here. I will link to Figure.}~\felice{I think it's ok!}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{Pictures/gan_cf_new.pdf}
%    \caption{GAN-based Recommendation Framework.}
    \caption{A conceptual view of GAN-CF incorporating GAN to address item recommendation task.}
    \label{fig:GAN-CF}
\end{figure}

%The work by IRGAN is the first attempt to integrate the above notions of relevance under the same roof by proposing a GAN-based IR model. In particular, a \textit{min-max  game} is played between a discriminative model responsible for discriminating ground-truth user-item recommendations and adversarially generated ones, and a generator model responsible for producing recommendations approximating the true distribution of relevant items as much as possible.

%\yd{Inspired by its algorithmic and architectural approach, we propose to summarize main GAN-based recommender models under a general framework, named \textit{GAN-based Recommendation Framework (GAN-RF)}. Figure~\ref{fig:GAN-RF} shows the architecture of the GAN-RF.} 

\begin{comment}
\subsubsection{GAN-RF: Model Formulation}~\label{subsubsec:ganfr_model_formulation}
We model GAN-RF with a \textit{conditional GAN} (CGAN)~\cite{DBLP:journals/corr/MirzaO14}, an important modification of the original generative model GAN that could regulate the data generation process by conditioning the model on additional information besides a random prior noise input.  In doing so, $G$ is user-conditioned (e.g., the user-id) such that it can generate \textbf{user-personalized} recommendations. 

Let $u$ be a user, $i$ be an item interacted by $u$ and $\hat{i}$ be a generated item. Taken a user-conditioned input $u$, $G$ generates relevant items trying to approximate the true relevance distribution $p_{\text { true }}(i | u, r)$, while $D$ tries to distinguish the generated relevant items from the real ones. We may represent the GAN-RF loss function as
\begin{equation}
     %\small
     \label{equation:gan-rf-j}
     J(\theta,\phi) =  \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
 \end{equation}
\felice{
\begin{equation}
     %\small
     \label{equation:gan-rf-j}
     J(\theta,\phi) =  \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
 \end{equation}
 }
while the min-max  game to train the generator and the discriminator is formally defined as:
\begin{equation}
     %\small
     \label{equation:gan-rf-formula}
     \arg \min _{\theta}\max _{\phi} J(\Theta,\Phi)
 \end{equation}
where $\theta$ parametrizes the generative data distribution $p_{\theta}(\hat{i} | u_{n}, r)$ of $G$, and $\phi$ parametrizes the discriminative function of $D$.  We omit the random noise $z$ in GAN-RF, which is used in the classic GAN formulation, since the generative retrieval process is a discrete item sampling (i.e., the generated relevant items), which is different from the deterministic generation based on the sampled noise signal in the original GAN.
\end{comment}

%\subsubsection{GAN-RF: Recommendation list sampling strategies }~\label{subsubsec:ganfr_discrete_item_sampling}




\begin{comment}
\begin{table}
\caption{Key sampling strategies proposed for CF-GAN recommendation models}
\centering
{\scalebox{0.70}
\begin{tabular}{@{} lll @{}} 
\toprule
    \textbf{Method} & 
    \textbf{Key insights} & 
    \textbf{Formal description} \\ 
    \midrule
    REINFORCE~\cite{DBLP:conf/nips/SuttonMSM99} & 
    \small{
    \begin{tabular}[l]{@{}c@{}}Optimize $G$ with $K$ discrete items ($\hat{i}_k$).\end{tabular}}

     & 
    \begin{minipage}{7cm}
    $ \nabla_{\theta} \simeq \frac{1}{K} \sum_{k=1}^{K} \nabla_{\theta} \log p_{\theta}(\hat{i}_k | u,r) \log (1-f_{\phi}(\hat{i}_k | u)))$
    \end{minipage} \\ [4pt]
    Gumbel-Softmax~\cite{DBLP:conf/iclr/JangGP17, DBLP:journals/eswa/SunWWY19} & 
    \small{
    \begin{tabular}[l]{@{}c@{}}Approximate discrete items through  \\ a continuous differentiable estimator. \end{tabular}}

    & \begin{minipage}{7cm}
    $ v_k = \frac{\exp \left(\left(\log p_{\theta}\left(i_{k}| u, r\right)+g_{k}\right) / \tau\right)}{\sum_{j=1}^{K} \exp \left(\left(\log p_{\theta}\left(i_{j}| u, r\right)+g_{j}\right) / \tau\right)}$
    \end{minipage} \\ 
    \bottomrule
    \multicolumn{3}{c}{\small{\textit{In the Gumbel-Softmax formulation $g_k$ and $g_j$ represent sampled noise from $Gumbel(0, 1) = -\log (-\log (Uniform(0,1)))$.}}} \hline
\end{tabular}}
\end{table}

\end{comment}

% \begin{itemize}
%     \item The \textbf{policy gradient based reinforcement learning algorithm} (REINFORCE)~\cite{DBLP:conf/nips/SuttonMSM99} optimizes $G$ to generate highly rewarded recommendation list. The gradient of the generator is derived as follows:
%         \begin{align*}
%             \nabla_{\theta} J&=\nabla_{\theta} \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u,r)}[\log (1-D_{\phi}(\hat{i} | u)))]\\
%             &=\nabla_{\theta} \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u,r)}[\log (1-D_{\phi}(\hat{i} | u)))]\\
%             &=\sum_{m=1}^{M} \nabla_{\theta} p_{\theta}(\hat{i}_m | u,r) \log (1-D_{\phi}(\hat{i}_m | u))\\
%             &=\sum_{m=1}^{M} p_{\theta}(\hat{i}_m | u,r) \nabla_{\theta} \log p_{\theta}(\hat{i}_m | u,r) \log (1-D_{\phi}(\hat{i}_m | u)))\\
%             &=\mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u,r)}[\nabla_{\theta} \log p_{\theta}(\hat{i} | u,r) \log (1-D_{\phi}(\hat{i} | u)))]\\
%             &\simeq \frac{1}{K} \sum_{k=1}^{K} \nabla_{\theta} \log p_{\theta}(\hat{i}_k | u,r) \log (1-D_{\phi}(\hat{i}_k | u)))
%         \end{align*}
% where the sampling approximation of discrete items is performed in the last step in which $\hat{i}_k$ is the $k$-th relevant item sampled from the current version of the generative function $p_{\theta}(\hat{i} | u,r)$.

% This method suffers of instability in  gradient estimating for G's parameter optimization in the case of a large set of items~\cite{DBLP:conf/sigir/WangYZGXWZZ17} since the variation of the gradients increases linearly with number of items~\cite{DBLP:conf/icml/RezendeMW14}. The next approach propose a solution that solves this problem.

%         \item The \textbf{Gumbel-Softmax differentiable sampling procedure} is an alternative solution to the policy gradient to solve the non-differentiation problem of discrete inputs proposed in Sun et al.~\cite{DBLP:journals/eswa/SunWWY19}. It adopts the Gumbel-Softmax estimator~\cite{DBLP:conf/iclr/JangGP17} to approximate discrete examples through a continuous distribution to make the sampling procedure  differentiable thus allowing the update of $G(\Theta)$.
        
%         Gumbel-Softmax distribution is a continuous approximation to a multinomial distribution parameterized in terms of the softmax function.
%         \begin{equation}\label{eq:vk-gumbel}
%             v_k = \frac{\exp \left(\left(\log p_{\theta}\left(i_{k}| u, r\right)+g_{k}\right) / \tau\right)}{\sum_{j=1}^{K} \exp \left(\left(\log p_{\theta}\left(i_{j}| u, r\right)+g_{j}\right) / \tau\right)}
%         \end{equation}
            
%         In the previous equation $g_k$ and $g_j$ represent sampled noise from $Gumbel(0, 1) = -\log (-\log (Uniform(0,1)))$
% \end{itemize}

\subsection{GAN-based Recommendation Models: State of the Art}\label{subsec:Applications of GAN-based Recommendation}
\yashar{ XXX I AM FOCUSED HERE XXX}
\yd{In this section, we focus on the novel trend of AML research --- GAN-based Recommendation --- applied to various domains. We have identified a total of 45 papers that integrate GAN in order to accomplish a particular RS-related task. We can classify these tasks according to:} 

%A total of \felice{45} studies were found to identify novel recommender models that integrate GAN in order to accomplish different tasks. We identified five main recommendation task in the literature that use adversarial learning in a GAN-based recommendation approach:
\begin{enumerate}
    \item Collaborative Recommendation
    \item Context-aware Recommendation
    \item Cross-domain Recommendation
    \item Complementary Recommendation
\end{enumerate}
\yd{In the following, we review each of these application scenarios in detail. We present Table~\ref{tbl:gan-approaches} to summarize the proposed models under different recommendation tasks with additional implementation details.}
%We review these five classes in the subsequent sections.  For simplicity, we have created Table~\ref{tbl:gan-approaches} to summarize the proposed models under different recommendation tasks with additional implementation details. 
\input{Tables/gan_rs.tex}

\subsubsection{Collaborative Recommendation}
\label{subsec:GAN_CF_rec}
\yashar{We should provide an introduction here, here is a try}
\yd{GANs have been shown powerful in generating relevant recommendations --- in particular using the CF approach --- and be able to successively compete with state-of-the-art models in the field of RS. We have identified the following reasons for the potential of GANs in RS: (i) they are able to generalize well and learn unknown user preference distributions and thus be able to model user preference in complex settings (e.g., IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18}); (ii) they are capable of generate more negative samples than random samples in pairwise learning tasks (e.g., APL~\cite{DBLP:journals/eswa/SunWWY19}, DASO~\cite{DBLP:conf/ijcai/FanD0WTL19}) and (iii) they can be used for data augmentation (e.g., AugCF~\cite{DBLP:conf/kdd/WangYWNHC19}  and RAGAN~\cite{DBLP:conf/www/ChaeKKC19}).}

%generalize and learn the datadistributions


% From the pioneering works that proposed a GAN framework for improving utility of item recommendation scenario under CF, we should highlight IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18}, with the difference that the former proposes the solution for CF based on MF whereas the second one proposed a graph-representation learning for the same problem. We discuss these works in more details in the following.

% In~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, Wang et. al. present a unified theory of generative and discriminative methodologies in IR under the GAN framework named IRGAN. An important question in IR is: \dquotes{Given a query ($q$) and a document ($d$), what is the probability that $d$ is relevant to $q$?}. The answer to this basic question constitutes the basis for document ranking in IR and has been answered under two schools of thinking: i)the generative model and the ii)the discriminate model described in the following:

% \begin{itemize}
%     \item The \textbf{generative model} makes the underlying assumption is that there exists a stochastic \textbf{generative process} between $d$ and $q$. It then answers the above basic question in probabilistic terms by stating that it is equivalent to this question \dquotes{what is the probability of relevance, i.e., $p(R=r|d,q) = 1- p(R=\bar{r}|d,q)$?}. In text retrieval, two approaches are commonly used to estimate $p(R=r|d,q)$, which can be seen equivalent based on different parametrization of the likelihood under the Bayes rule; the first is the Robertson-Sparck Jones~\cite{DBLP:journals/ipm/Jones79} approach which aim to model the probability of relevance in a forward manner as $q arrow d$ via factorization $p(R=r|d,q) = p(q|r) p(d|q, r)$. It can be shown that this problem becomes equivalent to the naive Bayes model for classification in which for a given information need $q$, the goal is to classify the document into classes $r$ and $\bar{r}$. The second is the language modeling approach~\cite{DBLP:conf/sigir/PonteC98} which takes the reverse approach $d arrow q$ via factorization $p(R=r|d,q) = p(d|r) p(q|d, r)$, and aims to generate query terms for a given document.
%     \item The \textbf{discriminative model} uses a machine learning approach to answer the basic question in which documents and queries are jointly considered as features and the goal is to predict relevance in ML way by using large amount of training data. Therefore the problem can be seen as $q+d arrow d$. A significant example of this approaches are learning to rank (LTR) models whose aim to is the learn right ranking of documents (or items) given a representation of an information need (query or context). 
% \end{itemize}

% The work by IRGAN is presumably the first attempt to integrate the above notions of relevance under the same roof by proposing a GAN-based IR model. In particular a min-max  game is proposed composed of a discriminative model responsible for discriminating ground-truth user-item recommendations from generated ones and a generator responsible for producing recommendations approximating the true distribution of relevant items as much as possible. The authors finally demonstrate the application of IRGAN for \textit{web search}, \textit{item recommendation} and \textit{question answering} tasks. 
% \yashar{@Felice: to connect it to RS, could we add one more sentence how this links with item recommendation? Thanks}



\setlength{\parindent}{15pt} \yd{[\textbf{IRGAN}] As presented in Section~\ref{subsec:GAN_RF}, IRGAN --- the work by Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} --- is presumably the first attempt to integrate generative and dicriminative approach to IR under the same roof by proposing a GAN-based IR model. The authors demonstrate the application of IRGAN for web search, item recommendation and question answering tasks.} 

\setlength{\parindent}{15pt} \yd{[\textbf{GraphGAN}] In~\cite{DBLP:conf/aaai/WangWWZZZXG18}, the authors proposed GraphGAN, which employs GAN to perform graph representation learning (a.k.a. network embedding). Graph-based analysis are becoming increasingly popular in recent years due to their ubiquity in real-world problems such as modelling user preference for item recommendation as well as social graphs in social media (SM) networks, co-occurrence graph in linguistics, citation graph in research, knowledge graph and so forth. The central idea of network embedding is to represent each entity (e.g., node) in a graph with a lower-dimensional latent vector of features to facilitate tasks within the network and prediction over entities. For example, the features of the latent vector embedding can allow a system to perform prediction for supervised tasks and, at the same time, the distance between node embedding vectors can serve as a useful measure in unsupervised tasks. GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18} can be viewed as a similar approach with IRGAN, with the difference that GraphGAN proposed a graph-representation learning for the MF-based CF. Here queries are nodes in the graph and the goal of $G$ is to imitate as much as possible the ground-truth  connectivity distribution over vertices $p_{true}(v|v_c)$ and $D$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$ where \yashar{I will in this part}}

\begin{comment}
In~\cite{DBLP:conf/aaai/WangWWZZZXG18}, the authors proposed GraphGAN, which employs GAN to perform graph representation learning (a.k.a. network embedding). Graph-based analysis are becoming increasingly popular in recent years due to their ubiquity in real-world problems such as modelling user preference for item recommendation as well as social graphs in social media (SM) networks, co-occurrence graph in linguistics, citation graph in research, knowledge graph and so forth. A real-world information graph can consist of millions to billions of nodes and edges and uncovering relationship among all these entities can allow conducting various complex inference over the entire graph. The central idea of network embedding is to represent each entity (e.g., node) in a graph with a lower-dimensional latent vector of features to facilitate tasks within the network and prediction over entities. For example, the features of the latent vector embedding can allow a system to perform prediction for supervised tasks and, at the same time, the distance between node embedding vectors can serve as a useful measure in unsupervised tasks. GraphGAN proposes a similar idea to IRGAN, where queries are nodes in the graph and the goal of $G$ is to imitate as much as possible the ground-truth  connectivity distribution over vertices $p_{true}(v|v_c)$ and $D$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$\tommaso{spend a few words to introduce $v$ and $v_c$}. 

\end{comment}

\setlength{\parindent}{15pt} \yd{[\textbf{GAN-HNBR}] From an application perspective, GAN-based graph representation, have been applied for different  domains of recommenders, e.g., for personalized citation recommendation (i.e., recommending research papers for citation) by using a content-based and author-based representation~\cite{DBLP:conf/ismis/ZhangYCD18}  or learning heterogeneous bibliographic network representation (HBNR)~\cite{DBLP:conf/aaai/CaiHY18}. As for GAN-HNBR, the role of GAN component is to infer the optimal representation of a bibliographic network consisting of heterogeneous vertex content features (e.g., papers, authors, manuscripts) into a common shared latent space and applying personalized recommendation on the obtained representation.}

%Various other GAN-based CF models have been proposed following the works by IRGAN and GraphGAN. 
% \yashar{Here we can add some overall information LATER: often these proposal are different based on the fact if}

\setlength{\parindent}{15pt} \yd{[\textbf{CFGAN}] CFGAN is introduced in \cite{DBLP:conf/cikm/ChaeKKL18}, which improves one of weakness in IRGAN, as claimed by authors. Indeed, the main problem in IRGAN is that the generator produces each time a single item index %\yashar{Felice is it single item index or item indices?} 
that is discrete in nature. This is different from original GAN framework by authors, in which the output of $G$ is an image (i.e., a vector). The generation of discrete item indices by $G$ can lead to poor sampling of items from the pool of available alternatives (i.e., samples exactly identical to ground-truth) resulting in a deterioration of the performance of $G$ and $D$ (instated of improvement) over time after the min-max game is performed between them. By introducing vector-wise adversarial learning and testing it quantitatively over a series of experiments/datasets, the authors show the improvement of CFGAN over IRGAN and GraphGAN baselines. As an example, for P@20 and the Ciao dataset this improvement is approximately $100\%$  with respect to IRGAN (0.45 v.s. 0.23) and $160\%$ compared with GraphGAN (0.45 v.s. 0.17), which seems to be significantly on the high side.}

\setlength{\parindent}{15pt} \yd{[\textbf{AE-GAN]}} In~\cite{8525831} the authors propose an auto-encoder-based GAN. The authors identify a problem in conventional MF-based approach which is linear and difficult to capture the non-linear  subtle latent factors underlying user-item interactions. In the the proposed approach, an auto-encoder takes the role of $G$ to model the underlying distribution of user preference over items.  
%\yashar{shouldn't we add one sentence about auto-encoder, why it can be powerful?}

\setlength{\parindent}{15pt} \yd{[\textbf{VAE-GAN]}} An adversarial variational auto-encoder (VAE) is adopted in~\cite{8663730} where the authors propose the usage of a GAN to regularize variational autoencoder by imposing an arbitrary prior on the latent representation (uses implicit feedback). A similar work can be found in ~\cite{DBLP:conf/icde/TongLZSC19, DBLP:conf/cikm/LeeSM17} which exploits a VAE to enhance the robustness of adversarial examples. The author furthermore present the Wasserstein Distance with gradient penalty.

Other issues of IRGAN such as sparsity causing gradient vanishing and update instability, and discrete value preventing a training to optimize using gradient descent are addressed in \cite{DBLP:conf/flairs/CostaD19}. The proposed solution is named convolutional adversarial latent factor model (CALF) which employ a CNN to learn correlations between embeddings and Rao-Blackwell sampling to deal with discrete values optimizing CALF.  The authors of \cite{DBLP:conf/ijcai/WuLMZZG19} propose a solution to improve diversity of CF-based recommendation with GAN based on personalized diversification. We will better review this paper later. 

In~\cite{DBLP:conf/ijcnn/WangZC019} the authors propose to improve the recommendation performance in a pairwise scenario by proposing lambda rank~\cite{DBLP:conf/cikm/YuanGJCYZ16} function into the adversarial learning of the proposed GAN-based CF framework.

A variant of Variational Autoencoder is introduced in \cite{DBLP:conf/ijcai/YuZCX19} to address the limited expressiveness of the inference model and latent features which reduces the generalization performance of the model. The proposed solution, named Adversarial Variational Autoencoders (VAEGAN), is a more expressive, and flexible, model that better approximates the posterior distribution by combining VAEs and GAN. They are the first to propose the application of Adversarial Variational Bayes (AVB)~\cite{DBLP:conf/icml/MeschederNG17} to compute the adversarial training. 


%\textbf{Improve Beyond-Accuracy Aspect}
% \yashar{Newly added}
%The success of recommendation algorithms is commonly measured by how well they are capable of making predictions of high-relevance items to a target user, i.e., items that users will likely click, buy or listen. The earliest research on MRS were focused on promoting this perspective through improving \textit{recommendation accuracy}. However, too much personalization, i.e., excessive pandering to user's existing musical taste can harm the development of curiosity and personal growth in users. The extreme case of this aesthetic concern is described as the \dquotes{filter bubble} effect, which refers to the scenario where as the result of excessive personalization of content geared toward users' individual preference, personalization services (web SE and RS) reduce diversity of the information presented and lead to partial information blindness (i.e., filter bubbles). 

\subsubsection{Context-aware Recommendation}
%\begin{comment}
%A body of existing works has focused on improving the POI
%recommendation performance by exploiting various implicit context features embedded in check-ins, such as their spatial informa- tion [13, 14, 17]; semantics [9]; social relations [5, 11, 36]; temporal characteristics [18, 33]; and sequential dependence [6, 19, 27, 35]
%\end{comment}
Although long-term preference modelling has proven to be effective in several domains~\cite{DBLP:conf/kdd/BerkovskyF15}, recent research indicates that user preference are highly variable based on user's context, e.g., time, location and mood~\cite{DBLP:conf/recsys/KompanKB17}. Context provides background of \textit{user objective} for using the system and can be used to generate more relevant recommendations.

\qquad \textit{Temporal-aware Recommendation:}
% \felice{Revised - Newly Added}
In real applications, users' preferences change over time and modeling such \textit{temporal evolution} is needed for effective recommendation. While long-term preferences of users change slowly, their \textit{short-term preferences} can be seen more dynamic and changing more rapidly. Predicting short-term user preference has been recently studied in the context of \textit{session-based} and \textit{sequential recommendations}. A temporal extension of SVD++ towards the modeling of temporal dynamic,  named TimeSVD++, has been proposed by Koren~\cite{DBLP:journals/cacm/Koren10} in 2010. However, it has been proved that the structure of time-aware inputs (e.g., click-logs, session) are effectively modelled by recurrent neural network (RNN).
For instance, Hidasi et al.~\cite{DBLP:journals/corr/HidasiKBT15} proposed to model the sequential user clicks to output session-based recommendation with a GRU-gated recurrent unit; while Wu et al.~\cite{DBLP:conf/wsdm/WuABSJ17} proposed to integrate an LSTM model, to capture both the user and the item temporal evolution, and MF to model  stationary preferences. 

Inspired by the accuracy improvements of IRGAN different GAN-based models have been combined in temporal frameworks to boost the recommendation performance in sequence-aware recommendation tasks. 

In~\cite{DBLP:conf/recsys/BharadhwajPL18}, the authors propose to incorporate in a single framework both the temporal modelling capabilities of RNN and the latent feature modelling power of the \textit{min-max  game}. The proposed framework, named RecGAN, implements both the generator a the discriminator with the Gated Recurrent Unit (GRU)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}, in order to make $G$ capable to predict a sequence of relevant items based on the dynamic evolution of user's preferences.

Differently from RecGAN that implements only a RNN cell to capture the dynamic evolution of user's behaviour, Zhao et al.~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, 8643032} propose to combine MF and RNN in an adversarial recommendation framework to model respectively long and short-term user-item associations. The proposed framework, named PLASTIC, adopts MF and LSTM cells into $G$ to generate the sequence-aware recommendation list for a given user, while a Siamese Network learns to distinguish the generated ones from real ones in a pair-wise learning setting.

An integration of a streaming recommender systems based on key-value memory networks~\cite{DBLP:conf/www/ZhangSKY17} with a generative adversarial network (instead of a random sampler) is presented in \cite{DBLP:conf/kdd/WangYHLWH18} to generate more informative negative examples used by the recommender models to learn users' preference in a pairwise settings. The motivation of this particular GAN application originates from the fact that random sampling strategies are static and scarcely contribute towards the training of the recommender model. Instead, adversarial learning includes the generation of adaptive and informative samples that the authors experimentally evaluated to improve the training effectiveness and the recommendation accuracy of the model.


GAN-based solution for sequence-aware RS has also been proposed in conjunction with Reinforcement Learning (RL) techniques. In~\cite{DBLP:conf/icml/Chen0LJQS19}, the authors propose to model the behavior temporal evolution and the RL reward function of a user through the adversarial learning of GAN. The core idea of the proposed framework, named GAN-user-model, is to model user's behavior evolution via a min-max  formulation. 


\qquad \textit{Geographical-aware Recommendation:} A relevant application of contextual information is point-of-interest (POI) recommendation. 
In~\cite{DBLP:conf/ijcai/0061W0Y19}, the authors propose \textit{Geo-ALM}, a GAN-based recommender where $G$ is used to generate more informative negative samples to be coupled with positive (real) ones to train $D$ under a pairwise learning setting. The proposed model firstly integrates both $G$ and $D$ with geographical features (e.g., the number of nearest POIs, and the size of the region containing a POI) in order to fuse geographical constraints in the min-max  game. 

A proposal to learn user-latent representations in a generative way is presented in \cite{DBLP:conf/www/0002YZTZW19}. The idea is inspired by the advances of recommendation performance under GAN-based framework. The main novelty of the proposed framework, \textit{Adversarial POI Recommendation} (APOIR), is the use of POIs geographical features and the users' social relations into the reward function used to optimize the $G$. The reward function acts like a contextual-aware regularizer of $G$, that is the component of APOIR used to POI recommendation task. 


%\begin{comment}
%\felice{Need to be revised because taken from old technical version}
%Zhou \textit{et al.}~\cite{DBLP:conf/www/0002YZTZW19} focuses on ~\hltask{location-based recommendation systems} to suggest point-of-interest (POI) to users. The authors address the ~\hltask{lack of formal models to understand user check-in behavior} which can lead to poor recommendation performance. They propose a novel GAN-based POI recommendation model, named \hlmethod{Adversarial POI Recommendation} (APOIR), for learning the user check-in model in a generative way, rather than extracting them with baseline approaches, such as MF, Context Embedding and Pairwise Ranking, in order to boost the recommendation performance.
%The generative process is used to model the relationship between a user $u$ and the set of POIs, where a POI is $i$. The underlying distribution of the user preferences over POIs is learned by classical min-max  game between a generator $G$ and a discriminator $D$ explained in Section~\ref{subsec:GAN-based CF}. Similarly to IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the authors employ a reward policy based on \textit{Geographical rewards}, e.g. the distance between POIs, and \textit{Social rewards}, e.g. the POIs visited by user's friends, which works as a regularizer to the recommended POIs from the generator $G$.
%They evaluate APOIR on public location-based social network datasets and compare it to several state-of-the-art models. The results demonstrate the effectiveness of APOIR approach in improving POI recommendation.

%Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} investigate \hltask{query recommendation systems} in order to improve the suggestion performance by understanding and modeling user search intents accurately. The authors propose a novel model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), that provides query suggestions considering the sequential search queries issued by the user and and his the history of clicks on last suggestions. Similarly to APR~\cite{DBLP:conf/sigir/0001HDC18}, they employ an adversarial training stage during the training of CFAE by injecting adversarial examples built by adding adversarial perturbations of item embeddings.~\felice{It is necessary to define in a Section the procedure user to create adversarial perturbations. They use FSGM}
%Experiments on a e-shopping domain dataset demonstrate that adversarial training on CFAN not only significantly \textit{improve the robustness} of the model but also outperforms the baseline methods for the task of query suggestion.
%\end{comment}

\subsubsection{Cross-domain Recommendation}
% \felice{STABLE- Done by \textbf{Yashar}}
Cross-domain recommender models are designed to compute recommendations for items belonging to a single domain, for example in media streaming platforms, Netflix recommends movies/TV series to its consumers while Lasts.Fm offers song and music-album recommendations. Items belonging to a certain domain share characteristics and attributes, which are intrinsically similar. The development of \textit{domain-specific} recommendation models allows the designer to study these characteristics separately.

However, single-domain recommendation can face numerous challenges. The first refers to the well-known cold-start problem, which happens when insufficient interactions or preference scores exist in the considered domain. The second relies on the fact users' interests and needs span across different application areas and large e-commerce sites, like Amazon or Ebay, store users' preference scores related to products/services of various domains - from books and products to online movies and music. As companies strive to increase the diversity of products or services to users, cross-domain recommendation can help such companies to increase sale productivity by offering personalized cross-selling or bundle recommendations for items from multiple domains~\cite{cantador2015cross}. A third aspect relates to the idea of discovering relationships for images related to different domains. For example, can machine achieve a human-level understanding to choose a suit jacket with pants or shoes in the same style to wear? The central problem here is to find a mapping function from one domain to another domain~\cite{DBLP:journals/corr/abs-1812-06229}. Recently, the generative power of GANs has been used to tackle this problem as a conditional image generation problem, i.e., to generate an image in one domain given another image in the other domain~\cite{DBLP:conf/cvpr/IsolaZZE17}. In the following we review different research works applying GAN-based approaches to various cross-domain recommendations tasks: 

In~\cite{DBLP:conf/bigcomp/JoJCJ19}, the authors propose a cross-domain GAN to generate fashion designs from the sceneries. In the proposed hypothetical scenario, the user can specify via a query her POI to visit (e.g., mountain, beach, etc.) together with keywords describing a season (i.e., spring, summer, fall, and winter). The core idea is to automatically generate fashion items (e.g., clothes, handbags, and shoes) whose effective features (i.e., style) match the the natural scenery specified by the user. For instance, the system can recommend a collection of fashion items that look cool/bright for visiting a beach in summer even though the true preference of the user is black-style clothes. The role of GAN is to learn associations between scenery and fashion images. In the field of ML and Computer Vision, the problem is termed as \dquotes{style transfer} or \dquotes{image to image translation} problem~\cite{DBLP:conf/cvpr/GatysEB16}. %\yashar{stable}

An effective cross-domain recommendation system relies on \textit{capturing both similarities and difference among features of domains} and leveraging them for improving recommendation quality in multiple domains. Single-domain algorithms have difficulty in uncovering the specific characteristics of each domain. To solve this problem some approaches extract latent features of the domains by a separate network~\cite{DBLP:conf/www/LianZXS17,DBLP:journals/tmm/MinBXH15}. Although these approaches might be successful in capturing characteristic features of each domain, they do not establish the similarity between features of multiple domains. With the goal to extract both homogeneous and divergent features in multiple domains, in~\cite{DBLP:journals/corr/abs-1812-06229} the authors propose generic cross domain recommendation system. The system takes the user interaction history (click vector) in each domain as input, maps each vector to shared latent space via the help of two autoencoders (AE) and then uses a generator to remap the latent representation to click vectors. The main novelty of this work lies on building/linking shared latent space between domains, which in turn facilitates \textit{domain-to-domain} translation. In particular, the former is realized by enforcing a weight-sharing constraint related to variational auto-encoders, i.e., the encoder-generator pair $\{E_A, G_A\}$ and $\{E_B, G_B\}$\footnote{The wights sharing is done on the last few layers of encoders $\{E_A, E_B\}$ and first few layers generators $\{G_A, G_B\}$ which are in charge of encoding and decoding high-level representations of the input click vectors.} and using cycle-consistency (CC) as a weight-sharing constraint. Finally two separate adversarial discriminators are employed to determine whether the translated vectors are realistic. The final system is called VAE-GAN-CC network. It is worth mentioning that the proposed system extends the unsupervised Image-to-Image Translation Network (UNIT) \cite{DBLP:conf/nips/LiuBK17} for RS and is thus named Domain-to-Domain Translation Model (D2D-TM). %\yashar{stable}
         
A possible solution for cross-domain recommendation is to rely on \textit{domain linkage} based on \textit{user-} and \textit{item-overlap}. Four types of relationships are identified in SoA literature in cross-domain recommendation~\cite{DBLP:conf/icdm/CremonesiTT11}: i) no overlap, ii) user-overlap, iii) item-over lap and (iv) user and item overlap. CF models can function in all these cases, except for the first case. Therefore, the existence of an overlap is the key enabler to obtain an effective recommendations with a classic CF strategy. However, in many real applications a limited overlap between domains may exist, hindering CF functioning. Such approaches have been proposed to deal with  the  \textit{domain overlap  issue} in  a  more  flexible  way such as by approaches that build/measure \dquotes{characteristics}  that  are  shared  by  the  user/item  profiles in  the different  domains (often via a latent representation). Although effective, in face of heterogeneity of domains,  number of shared characteristic between domain can be small~\cite{fernandezcross}.  
         
%To address the above issues or generally, in~\cite{DBLP:journals/corr/abs-1903-10794} the author propose an approach to solve the challenging issues in cross-domain recommendation - the problem of data sparsity and unbalancedeness via \textit{integration of transfer learning with adversarial learning}. Transfer learning is a ML task \yashar{citation}, whose goal is to transfer knowledge learned in a source domain and use it to improve the learning in the target domain and has been mentioned applied to solve cross-domain problem~\cite{fernandezcross}.  
         
         
        %  \yashar{I am here REVISING}

\subsubsection{Complementary Recommendation}
% \felice{working here}

Complementary Recommendation (Com) is a novel challenging task that points to suggest complementary items to customers. A very intuitive application domain is the fashion domain. For instances, given a red top (i.e., upper garment), the recommender model may recommend a selection of bottoms (e.g., trousers) in a complementary way.  Novel solutions have been proposed to address the problem of recommending complementary items by using adversarial-based approaches.


Huynh \textit{et al.}~\cite{DBLP:conf/eccv/HuynhCTA18} address the problem of recommending complementary items for a given item based on visual features. They develop an unsupervised learning approach for Complementary Recommendation using Adversarial Feature Transform (CRAFT), by learning the co-occurrence of item pairs in real images. The proposed method does not generate new images but it learns to generate features of the complementary items conditioned on the query item. 
% \begin{figure}[h]
%   \includegraphics[width=0.6\linewidth]{Pictures/CRAFT.png}
%   \caption{Architecture for the CRAFT framework. The transformer component is trained to generate the target features conditioned on the source features and a sampled noise vector.}
%   \label{fig:CRAFT}
% \end{figure}

The generator $G$ acts like a feature transformer to transform the source feature $s_{q}$ into a complementary target feature $\hat{t_{q}}$ by playing a \textit{min-max  game} with a discriminator $D$ that aims to classify feature pairs as real ($s_{i}$, $t_{i}$) or synthetic ($s_{q}$, $\hat{t_{q}}$).
Similar to Equation~\eqref{equation:gan-rf-j}, the objective function is

\begin{equation}
    \label{eq:craft}
    %\small
    J(\theta, \phi) = \mathbb{E}_{(s_{i}, t_{i}) \sim p_{c}} \log D_{\phi}(s_{i}, t_{i})+\mathbb{E}_{z \sim p_{z}, s_{q} \sim p_{s}} \log (1-D_{\phi}(s_{q}, G_{\theta}(s_{q}, z)))
\end{equation}

where $p_{z}$ and $p_{s}$ are the probability distribution function of the random noise and the source feature.
Recommendations are built on a nearest neighbor search of $\hat{t_{q}}$ on the subspace with pre-indexed target features $t_{i}$.
CRAFT has been tested by experienced users who gave positive feedback on the goodness of complementary recommendations.

Inspired by advances in image generation by class labels or by texts, and image transformation between different domains, Kang \textit{et al.}~\cite{DBLP:conf/icdm/KangFWM17}, Shih \textit{et al.}~\cite{DBLP:conf/aaai/ShihCLS18}, Lin \textit{et al.}~\cite{Yang2018FromRT} and Kumar and Das Gupta~\cite{DBLP:journals/corr/abs-1906-05596} propose GAN-based~\cite{DBLP:journals/corr/RadfordMC15} solutions for the generation of compatible items in the fashion domain.

\cite{DBLP:conf/icdm/KangFWM17} is the first publication where the Generative Adversarial Networks are used in Fashion Domain recommendation to generate item images based on user preferences. For instance, given a user and an item category, they propose a model to generate new images (i.e., clothing items) that are most consistent with user's preferences. In this paper, the authors adapt the Bayesian Personalized Ranking (BPR) to include item image content via a Siamese network in a Deep Visually-aware Bayesian Personalized Ranking method, called DVBPR. Then, this model is combined with a GAN-based framework to generate images that are consistent with user's personal taste. Iteratively, the generator learns a low dimensional latent code, which generates an item image that maximizes a personal objective value. 
Inspired by LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}, the overall objective function is
\begin{equation}
    \small
    \label{eq:dvbpr_gan_objective}
    J = \mathbb{E}_{\mathbf{x}, c \sim p_{true}(x, c)} [D(\mathbf{x}, c) - 1]^{2} + 
        \mathbb{E}_{c \sim p(c), z \sim p(z)} [D(G(z, c), c)]^{2}
\end{equation}
where $x$ is a image of the training dataset, $c$ is the category of the image $x$, and $z$ is a random noise vector. Given a user $u$ and a category $c$, the authors propose to synthesize personalized images by optimizing a user preference score
\begin{equation}
    \small
    \widehat{\delta}(u, c) = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} ( \widehat{r}_{u, e} )
    = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} \big(r_{u, e}-\eta D(e, c) \big)
\end{equation}
 where $r_{u,e}$ is the user score assigned to a generated new image and $\eta$ controls the trade-off between preference score and image quality. Generated images are quantitatively compared with real images using the preference score (mean objective value), inception score~\cite{DBLP:conf/nips/SalimansGZCRCC16} and Opposite SSIM~\cite{DBLP:conf/icml/OdenaOS17}. This comparison shows above all improvement on preference score with respect to non-GAN based images. At the same time, the qualitative comparison demonstrates that the generated images are realistic and plausible, yet they are quite different from any images in the original dataset --they have common shape and color profiles, but quite different styles. 

Shih \textit{et al.} propose a Compatibility Learning Framework by using a \hlmethod{Metric-regularized Conditional Generative Adversarial Network} (MrCGAN) to pursue the item generation task. The proposed model is composed of a compatibility learning component and a DCGAN~\cite{DBLP:journals/corr/RadfordMC15}-based component, MrCGAN, that is regularized on a compatibility metric learnt in the first component. Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18} they conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines. 
\\The authors of~\cite{Yang2018FromRT} addresses the same problem settings by proposing a novel fashion clothing framework composed of two parts: a clothing recommendation model based on BPR combined with visual features and a clothing complementary item generation based on DCGAN. Particularly, the generation component takes in input a piece of clothing recommended successfully in the recommendation model and generates clothing images of other categories (top, bottom or shoes) to build up a set of complementary items. They evaluate GAN performance with three indexes: \textit{Inception} score related to the quality of the generated image~\cite{DBLP:conf/nips/SalimansGZCRCC16}, \textit{Opposite SSIM} related to the diversity~\cite{DBLP:conf/icml/OdenaOS17}, and a proposed \textit{Compatibility index} to measure the compatibility of the generated set of complementary items. They compare the model with DCGAN as there are not baseline methods for such comparison. %~\futureworks{Can be interesting to focus on this field and try to propose new models a a baseline way to compare images?}.
A similar approach has been proposed also in~\cite{DBLP:journals/corr/abs-1906-05596}, to generate bottom fashion item paired with a given top item.


% \felice{Need to be revised}

% \qquad \textit{GAN-based Attacks on RS}\\
% They propose a framework for generating \hltask{shilling profiles} which, when incorporated in the training of a recommendation system, can achieve an adversarial intent, while remaining \textbf{indistinguishable from real user profiles}. The generation is mapped with a GAN-based framework where the Discriminator is the recommender model and the generator is the component that tries ot imitate the real distribution of users by looking to manipulate the recommendations.

\begin{comment}
\subsubsection{Other applications}

\qquad \textit{Privacy Protection}\\
Attribute inference attacks are emerging issues to user privacy in recommender systems domain~\cite{DBLP:conf/recsys/WeinsbergBIT12, DBLP:conf/cikm/Otterbacher10}. The attacker aims to infer a user's private attributes (e.g., gender, sexual orientation, political and religion views) via leveraging its public data (e.g., in recommender systems, it could be the list of rated items).

Recognising existing defense methods against attribute inference attacks are either computationally intractable or computationally tractable - but they add a large amount of noise to a user's public data; Jia \textit{et al.}~\cite{jia2018attriguard} propose ~\hlmethod{AttriGuard} a computationally tractable defense mechanism that adds small noise. The proposed defense method works in two phases. Firstly, it finds such minimum adversarial noise to evade the attacker's classifier. through an optimized version of \textit{evasion attack} developed by Papernot \textit{et al.}~\cite{DBLP:conf/eurosp/PapernotMJFCS16}, named \hlmethod{Policy-Aware Noise Finding Algorithm} (PANDA). Then, AttriGuard randomly selects one of the adversarial noise found previously to mislead the attacker's inference. The authors evaluate AttriGuard and compare it with existing defenses using a real-world dataset. Results demonstrate that the proposed evasion attack outperforms existing ones (FGSM, JSMA~\cite{DBLP:conf/eurosp/PapernotMJFCS16} and C\&W), and the proposed defense mechanism, AttriGuard, is effective at defending against attribute inference attacks. Otherwise it adds significantly smaller noise to users' public data than existing defenses.

Resheff \textit{et al.}~\cite{DBLP:conf/icpram/ResheffESS19} addresses the problem setting of the \hltask{leakage of private information} in recommender systems. The proposed privacy-adversarial framework in addition to eliminating such leakage it helps to guarantee fairness of results.
Inspired by the Domain Adversarial Training~\cite{DBLP:series/acvpr/GaninUAGLLML17}, the proposed method points to construct a user representation from which the private information can not be read out. This is achieved by training the model with an additive loss for the privacy protection.
This is achieved by application of the gradient reversal trick~\cite{DBLP:series/acvpr/GaninUAGLLML17} which leads to the following update rule for user embedding $p_{u}$:
\begin{equation}
    \small  
    \label{eq:panda_optimization}
    p_{u} \leftarrow p_{u}-\alpha\left[\frac{\partial \mathcal{L}_{recsys}}{\partial p_{u}}
    - 
    \lambda \sum_{i} \frac{\partial \mathcal{L}_{private_{i}}}{\partial p_{u}}\right]
\end{equation}
where $\alpha$ is the learning rate, $\lambda$ is the adversarial learning rate, and $ \mathcal{L}_{recsys}$ and $\mathcal{L}_{private_{i}}$ are the loss function of the recommender model and the adversarial privacy-protection component appended to the recommender model. Experiments on movie recommendation domain show the effectiveness of the proposed method in reducing the leakage of user's personal data.


\end{comment}


% \subsection{Potential Limitations of GAN for Recommender System}

% \begin{itemize}
%     \item GAN Convergence problem caused by Discrete Items (AML is studied for continuous). A first solution in res-sys has been proposed in IRGAN. The authors address the non-differentiation problem for the optimization of the generator with the policy gradient strategy (REINFORCE)~\cite{DBLP:conf/nips/SuttonMSM99}. Results show that the variance of its policy gradients explodes with a huge number of items~\cite{DBLP:conf/icml/RezendeMW14}, like for the input data of a real-world recommender models (e.g., Amazon catalog had millions of items). Recently, Gumbel-Softmax was proposed to overcome these limitations. It introduces a continuous distribution on the simplex that can approximate categorical samples, whose parameter gradients can be easily computed via the reparameterization trick. This approach has been successfully used in~\cite{DBLP:journals/eswa/SunWWY19, DBLP:conf/kdd/WangYWNHC19, DBLP:journals/corr/abs-1909-03529}  with a demonstrated improvement in the adversarial training procedure. In~\cite{DBLP:conf/flairs/CostaD19} the authors adopts Rao-Blackwell sampling procedure~\cite{DBLP:conf/icml/LiuRTJM19} to reduce the high variance of the gradient.
% \end{itemize}


% \input{Plots/OpenChallenges.tex}     
% \input{Plots/Domain.tex}  
\input{Tables/Recommender_Models.tex}



==> OLD_FILES/OLD3_Sec3.tex <==
\section{Adversarial Learning for GAN-based Recommendation}~\label{sec:GAN}
\yd{What we presented in Section~\ref{sec:security} dealt with a class of statistical models referred to as \dquotes{discriminative} models. In the context of classification, a discriminative model is a model that seeks to find the mapping $x \rightarrow y$ for a given input-label pair $(x,y)$, by learning the conditional probability $p(y|x)$ from the training data. The focus of the current section is on a novel class of \dquotes{generative} models, named \textit{generative adversarial networks} (GANs). A generative model is a model that seeks to find the mapping $y \rightarrow x$ by learning the conditional probability $p(x|y)$ from the data. For example, if $y$ indicates whether an item is appealing to a user, $p(y|x)$ would measure the probability --- or whether or not --- the user would like the product; instead $p(x|y=1)$ looks into the distribution of product features appreciated by the user and $p(x|y=0)$, the distribution of irrelevant product features for the user. Loosely speaking, a generative model cares about the \textit{generative} process behind data --- or product features (in the example) ---  to categorize the data instances. A discriminative model disregards the information about how the data were generated, it merely focuses on how to \textit{categorize} given data instances.}

\yd{GANs are a powerful class of generative models that use two networks --- trained simultaneously in zero-sum game --- with one network focused on data generation and the other centered on discrimination. The adversarial learning scheme --- or the the min-max game --- which lies in the heart of GANs empowers these ML models with phenomenal capabilities such as the ability to model high-dimensional distributions. As the result, these networks have been exploited to solve challenging problem in the computer vision. For instance in~\cite{DBLP:conf/cvpr/KarrasLA19}, a GAN model is proposed to transfer style plausible looking scenes. The research in RS community has used the generalization (or in technical term data distribution capturing) potential of GANs as an opportunity to solve variety of tasks relevant to RS.}

\yd{In summary, it is important to distinguish between two different applications of AML in RS and in a general term:}

\begin{enumerate}
    \item \yd{Adversarial learning to study attacks on, and defenses of machine-learned RS models. This aspect is centred on the \dquotes{security} of recommender models. We discussed this aspect in Section~\ref{sec:security}.}
    \item  \yd{Adversarial learning scheme used in GANs, empowering them to generalize and learn the data distributions. We refer to this aspect the \dquotes{generative} potential of GANs, which have been exploited in the field of RS. The focus of the current section is on this aspect.}
\end{enumerate}

\yd{As it can be noted the term \dquotes{adversarial} inside generative adversarial networks refers to the learning scheme used by these models and \textit{not the application}. In other words, the application of GANs for RS covers variety of aspects not limited to the security of RS, as we will see in the subsequent sections.}

\subsection{Foundations of Generative Adversarial Networks (GANs)}

\yd{GAN are deep generative models proposed by Goodfellow et al.,~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14} in 2014. A GAN is composed by two components, a generator $\mathcal{G}$, and a discriminator $\mathcal{D}$. The generator works to capture the real data distribution to generate adversarial examples and fool the discriminator,  while the discriminator endeavors to distinguish the fake examples from real ones.
This competition, known as adversarial learning, ends when the components reach the Nash equilibrium. The GAN architecture is shown in Figure~\ref{fig:gan_architecture}.} 

\begin{definition}[Conventional Vanilla GAN]
    \yd{\textit{Assume that we are given a dataset of $n$ input samples $x \in \mathcal{X}$, where $x \sim \mathbb{P}_{\mathcal{X}}$ and $\mathbb{P}_{\mathcal{X}}$ represents the probability distribution of the original data and suppose $z \in \mathcal{Z}$ denotes a sample from some latent space $\mathcal{Z}$. We are interested in sampling from $\mathbb{P}_{\mathcal{X}}$. The goal of GAN is to train the generator $\mathcal{G}$ to transform samples $z \sim \mathbb{P}_{\mathcal{Z}}$ into $g_{\theta}(z) \sim \mathbb{P}_{\theta}$ such that $ \mathbb{P}_{\theta} \approx \mathbb{P}_{\mathcal{X}}$. The role of the discriminator is to distinguish $\mathbb{P}_{\theta}$ and $\mathbb{P}_{\mathcal{X}}$ by training a classifier $f_{\phi}$. The training involves solving the following min-max objective}}
    \begin{equation}
         \label{eq:gan_basic}
         \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z)))
    \end{equation}
    
    \yd{where $\theta$ and $\phi$ are model parameters of the discriminator and generator respectively, learned during the trained phase. Different distance measures $f_{\theta}$ lead to different GAN models, e.g., Vanilla GAN (based on Jensen-Shannon divergence)~\cite{DBLP:journals/nips/GoodfellowPMXWOCB14}, Wasserstein GAN (based on Wasserstein distance)~\cite{DBLP:journals/corr/ArjovskyCB17}, and Conditional GAN (based on class conditioning on both the generator and discriminator)~\cite{DBLP:journals/corr/MirzaO14}.}
\end{definition}

\begin{definition}[Conditional-GAN (CGAN)]
    \yd{\textit{Conditional GAN is proposed by Mirza et al.,~\cite{DBLP:journals/corr/MirzaO14} in which the model extends the conventional vanilla GAN presented in Def. 3.1, by incorporating $c$ --- an extra condition information term --- on both the input of the generator $\mathcal{G}$ and the discriminator $\mathcal{D}$, thus conditioning them on this extra term}}
    \begin{equation}
         \label{eq:gan_basic}
         \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x|c) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z|c)))
    \end{equation}
    \yd{\textit{where $c$ can represent any auxiliary information to the networks such as class labels, content features, data from other domains and so forth.}}
\end{definition}

\begin{figure}
    \includegraphics[width=0.85\textwidth]{Pictures/GAN_joint.pdf}
  \caption{Schematic comparison of two well-known GAN models: (a) conventional vanilla GAN with filled color and (b) Conditional GAN (which includes the dashed blue entities)}
  \label{fig:gan_architecture}
\end{figure}

\subsection{GAN-based Recommendation Framework}\label{subsec:GAN_RF}

\yd{GANs have been successfully applied in start-of-the-at RS to learning recommendation models. Since the first pioneering GAN-based work IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} in 2017, we have witnessed a rapid adoption of these network architectures in many traditional and novel applications and domains. The attempt of this section is to provide a conceptual framework that will show how GANs are employed in RS domain and shed light on particularities and differences of GAN application in RecSys and ML. This section would continue by providing a survey of recent advances in GAN-based recommendation models.}
\vspace{3mm}\\
\noindent {\textbf{Historical background:}} 
\yd{Among the pioneering works that proposed a GAN framework for improving the utility of item recommendation in a CF scenario, it is worth mentioning IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18}. The former proposes a solution for CF based on MF whereas the second one proposed a graph-representation learning for the same problem. We discuss these two pioneering works in detail here (IRGAN) and in Section~\ref{subsec:GAN_CF_rec} (GraphGAN).}

\yd{A fundamental question in IR is: \dquotes{Given a query $q$ and a document ($d$), what is the probability that $d$ is relevant to $q$?}. The answer to this basic question constitutes the basis for document ranking in IR and has been answered under two different perspectives, the generative model and the the discriminative one:}

\begin{itemize}
    \item \yd{The \textbf{generative model} makes the underlying assumption that there exists a stochastic \textit{generative process} between $d$ and $q$. It then answers the above basic question in probabilistic sense, given by \dquotes{How to compute the probability of relevance $R$ for a given document $d$ with respect to a query $q$, or $p(R=r|d,q) = 1- p(R=\bar{r}|d,q)$?}. In text retrieval, two approaches are commonly adopted to estimate the probability $p \, (R=r|d,q)$, which are proven to be equivalent based on different parametrization of the likelihood under the Bayes rule. The first approach is the Robertson-Sparck Jones~\cite{DBLP:journals/ipm/Jones79} approach that models the probability of relevance in a forward manner $q \rightarrow d$ via factorization $p(R=r|d,q) = p(q|r) \,  p(d|q, r)$. It can be shown that this problem is equivalent to the naive Bayes model for classification in which for a given information need $q$, the goal is to classify the document into classes $r$ and $\bar{r}$. The second approach is based on language modeling paradigm~\cite{DBLP:conf/sigir/PonteC98}, that takes the reverse approach $d \rightarrow q$ via factorization $p(R=r|d,q) = p(d|r) p(q|d, r)$; it aims to generate query terms for a given document.}
   
    \item \yd{The \textbf{discriminative model} uses a machine learning approach to answer the basic question in which documents and queries are jointly considered as features and the goal is to predict relevance in ML way by using a large amount of training data. Therefore the problem can be seen as $q + d \rightarrow d$. A prominent example of this approach is learning to rank (LTR) whose aim to is to learn the right ranking of documents (or items) given a representation of an information need (query or context).}
\end{itemize}

\yd{Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} presented a unified theory of generative and discriminative methodologies in IR under the GAN framework named IRGAN. The proposed system is validated for different tasks including item recommendation in which the query is constructed from user's historical interactions. During adversarial learning --- the min-max game --- the generator learns true distribution of relevant items as much as possible.  It turns out that this novel training idea results in more satisfactory accuracy in recommendation than optimizing the traditional pure discriminate loss functions based on pointwise, or pairwise, objectives.}\\

\noindent {\textbf{GAN-CF problem formulation and conceptual model:}}
\yd{The prominent recommendation models in the literature that successfully apply GAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17,DBLP:conf/aaai/WangWWZZZXG18} for CF task, utilize the two-player min-max game with objective function built on top of Eq.~\ref{eq:gan_basic}.}
\begin{definition}[The GAN-CF model]
    \yd{\textit{Let $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items in a system, respectively. The training objective is given by}}
    \begin{equation}
         \label{eq:irgan_basic}
          \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) = \, \mathbb{E}_{i \sim \mathbb{P}_{\mathcal{X}}(i|u)} \, \log f_{\phi}(i|u) + \mathbb{E}_{\hat{i} \sim \mathbb{P}_{\theta}(\hat{i}|u)} \log \, (1-f_{\phi}(\hat{i} | u))
    \end{equation}
    \yd{\textit{where $i$ is an item receiving implicit (or explicit) feedback by user $u$ (e.g., purchased) and $\hat{i}$ is a generated item. In IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the score functions in $\mathcal{G}$ and $\mathcal{D}$ are generally based on the \textit{sigmoid} function.}} 
\end{definition}
\yd{A few observations are important to be made here: (i) the output of generator $\mathcal{G}$ is a set of item indices deemed relevant to user $u$; (ii) both $\mathcal{G}$ and $\mathcal{D}$ are \textit{user-conditioned}, signifying that model parameters are learnt by considering \textbf{user's personalization}; (iii) the GAN-based CF works does use the noise term as input (to $\mathcal{G}$) as the goal is to generate one unique --- yet plausible --- item rather than a set of items. Figure~\ref{fig:GAN-CF} summarizes these aspects conceptually.} 

\noindent {\textbf{Discrete outcome and sampling strategies:}} 
\yd{The parameters in the GAN-CF model are learned in an end-to-end fashion. 
However, before we can take benefit of this training paradigm, the system needs to solve a critical issue that does not exist on original GAN presented in Def. 3.1. based on sampled noise signal. The generation of recommendation lists is a discrete sampling operation, i.e., performed over discrete candidate items, see Figure~\ref{fig:GAN-CF}. Thus, the gradients that are derived from the objective function in Eq.~\eqref{eq:irgan_basic} cannot be directly used to optimize the generator via gradient descent as happens in the original GAN formulation, where gradients are applied for differentiable values (e.g.,images and videos). To obtain differentiable sampling strategy in GAN-CF models, two sampling strategies are proposed in the literature based on reinforcement learning algorithm and the Gumbel-Softmax differentiable sampling procedure~\cite{DBLP:conf/nips/SuttonMSM99,DBLP:conf/iclr/JangGP17, DBLP:journals/eswa/SunWWY19}, summarized in Table~\ref{tbl:smple_strg}.}

\input{Tables/sampling_strategy}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{Pictures/gan_cf_new2.pdf}
    \caption{A conceptual view of GAN-CF incorporating GAN to address item recommendation task.}
    \label{fig:GAN-CF}
\end{figure}

\subsection{GAN-based Recommendation Models: State of the Art}\label{subsec:Applications of GAN-based Recommendation}
\yd{In this section, we focus on the novel trend of AML research --- GAN-based Recommendation --- applied to various domains. We have identified a total of 47 papers that integrate GAN in order to accomplish a particular RS-related task. We can classify these tasks according to:} 
\input{Tables/gan_rs.tex}

\begin{enumerate}
    \item Collaborative Recommendation
    \item Context-aware Recommendation
    \item Cross-domain Recommendation
    \item Fashion Recommendation
\end{enumerate}
\yd{In the following, we review each of these application scenarios in detail. Table~\ref{tbl:gan-approaches} to summarize the proposed models providing insights about the constituting bulling bollocks of the GAN model.}
\vspace{-2mm}
\subsubsection{Collaborative Recommendation}\label{subsec:GAN_CF_rec}
%\yashar{We should provide an introduction here, here is a try}
\yd{GANs have been shown powerful in generating relevant recommendations --- in particular using the CF approach --- and be able to successively compete with state-of-the-art models in the field of RS. We have identified the following reasons for the potential of GANs in RS: (i) they are able to generalize well and learn unknown user preference distributions and thus be able to model user preference in complex settings (e.g., IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18}); (ii) they are capable of generate more negative samples than random samples in pairwise learning tasks (e.g., APL~\cite{DBLP:journals/eswa/SunWWY19}, DASO~\cite{DBLP:conf/ijcai/FanD0WTL19}) and (iii) they can be used for data augmentation (e.g., AugCF~\cite{DBLP:conf/kdd/WangYWNHC19}  and RAGAN~\cite{DBLP:conf/www/ChaeKKC19}).}

\setlength{\parindent}{15pt} \yd{[\textbf{IRGAN}] As presented in Section~\ref{subsec:GAN_RF}, IRGAN --- the work by Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} --- is presumably the first attempt to integrate generative and dicriminative approach to IR under the same roof by proposing a GAN-based IR model. The authors demonstrate the application of IRGAN for web search, item recommendation and question answering tasks.} 

\setlength{\parindent}{15pt} \yd{[\textbf{GraphGAN}] In~\cite{DBLP:conf/aaai/WangWWZZZXG18}, H. Wang et al., propose GraphGAN --- a graph-based representation learning --- (a.k.a. network embedding) for CF recommendation. Graph-based analysis are a booming research in recent years due to their ubiquity in real-world problems such as modeling user preference for item recommendation as well as social graphs in social media (SM) networks, co-occurrence graph in linguistics, citation graph in research, knowledge graph and so forth. The central idea of network embedding is to represent each entity in a graph with a lower-dimensional latent representation to facilitate tasks within the network and prediction over entities. For example, such latent representation can allow to perform prediction for supervised tasks or the distance between node embedding vectors can serve as a useful measure in unsupervised tasks. GraphGAN can be viewed as a graph-based representation of IRGAN, where queries/items are \textit{nodes} of the graph. For a given node $v_c$, the objective of $\mathcal{G}$ is to learn the ground-truth connectivity distribution over vertices $p_{true}(v|v_c)$, whereas $\mathcal{D}$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$. GraphGan furthermore proposes the graph softmax as $\mathcal{G}$ --- instead of traditional softmax --- which appears to boost the computational efficiency of training (graph sampling and embedding learning) performed by  $\mathcal{G}$.}

%generator's role (i.e., drawing samples and learn graph embedding).

%GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18} can be viewed as a similar approach with IRGAN, with the difference that GraphGAN proposed a graph-representation learning for the MF-based CF. Here queries are nodes in the graph and the goal of $\mathcal{G}$ is to imitate as much as possible the ground-truth  connectivity distribution over vertices $p_{true}(v|v_c)$ and $\mathcal{D}$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$ where \yashar{I will in this part}

\setlength{\parindent}{15pt} \yd{[\textbf{GAN-HNBR}] From an application perspective, GAN-based graph representation have been also applied in more niche domains of RS including personalized citation recommendation. The goal is to recommend research articles for citation by using a content-based and author-based representation~\cite{DBLP:conf/ismis/ZhangYCD18} or learning heterogeneous bibliographic network representation (HBNR). In~\cite{DBLP:conf/aaai/CaiHY18} Cai et al., propose GAN-HNBR --- a GAN-based citation recommendation model --- that can learn the optimal representation of a bibliographic network consisting of heterogeneous vertex content features such as papers and authors into a common shared latent space and provide personalized citation recommendation.}


\setlength{\parindent}{15pt} \yd{[\textbf{CFGAN}] CFGAN is introduced in~\cite{DBLP:conf/cikm/ChaeKKL18}, to address a problem with \textit{discrete items} in IRGAN, where $\mathcal{G}$ produces at each iteration a single item index, which is a discrete entity in nature. This is different from the original GAN in the CV domain in which the output of $\mathcal{G}$ is an image (i.e., a vector). The generation of discrete item indices by $\mathcal{G}$ results in a poor sampling of items from the pool of available alternatives (i.e., samples identical to ground-truth) deteriorating the performance of $\mathcal{G}$ and $\mathcal{D}$ --- instated of improvement --- during the min-max training iteration. CFGAN introduces \textit{vector-wise
training} in which $\mathcal{G}$ generates continuous-valued vectors to avoid misleading $\mathcal{D}$, which in turn improves the performance of both $\mathcal{G}$ and $\mathcal{D}$. The authors show the improvement of CFGAN over IRGAN and GraphGAN baselines. As an example, with regards to P@20 on the Ciao dataset, the improvement is $100\%$  for CFGAN vs. IRGAN (0.45 v.s. 0.23) and $160\%$ for CFGAN vs. GraphGAN (0.45 v.s. 0.17), which turns to be a significant improvement of the recommendation accuracy.} 
% CFGAN can be easily extended to learn from and generatethe rating data, even though it was also proposed to perform CFbased on implicit feedback dataset. 


%By introducing vector-wise adversarial learning and testing it quantitatively over a series of experiments/datasets, the authors show the improvement of CFGAN over IRGAN and GraphGAN baselines. As an example, along with P@20 on the Ciao dataset, the improvement is approximately $100\%$  with respect to IRGAN (0.45 v.s. 0.23) and $160\%$ compared with GraphGAN (0.45 v.s. 0.17), which turns to be a significantl improvement of the recommendation accuracy.}

\setlength{\parindent}{15pt} \yd{[\textbf{Chae et al.,}] In ~\cite{8525831}, Chae et al. propose an auto-encoder-based GAN, in which an auto-encoder(AE), as $\mathcal{G}$ models the underlying distribution of user preference over items. The primary motivation behind this work is the conventional GAN-based MF-based approaches are linear. Instead, the proposed system can generate non-linear latent factor model and uncover more complex relationships in the underlying use item interaction matrix.}


%which is linear and difficult to capture the non-linear  subtle latent factors underlying user-item interactions. In the the proposed approach, an auto-encoder takes the role of $\mathcal{G}$ to model the underlying distribution of user preference over items.

% on-linear latent factors, would bring more impressive recommendation results

\setlength{\parindent}{15pt} \yd{[\textbf{VAE-GAN]} An adversarial variational auto-encoder (VAE) is adopted in~\cite{8663730}, where the authors propose the usage of a GAN to regularize VAE by imposing an arbitrary prior on the latent representation (based on implicit feedback). A similar work can be found in~\cite{DBLP:conf/icde/TongLZSC19, DBLP:conf/cikm/LeeSM17}, which exploits a VAE to enhance the robustness of adversarial examples. The author furthermore present the Wasserstein Distance with gradient penalty.} %\tbc

\setlength{\parindent}{15pt} \yd{[\textbf{CALF]} Other issues of IRGAN such as sparsity causing gradient vanishing and update instability and discrete value preventing a training to optimize using gradient descent are addressed in~\cite{DBLP:conf/flairs/CostaD19}. The proposed solution is named convolutional adversarial latent factor model (CALF), which employ a CNN to learn correlations between embeddings and Rao-Blackwell sampling to deal with discrete values optimizing CALF.}

\setlength{\parindent}{15pt} \yd{[\textbf{PD-GAN]} The authors of~\cite{DBLP:conf/ijcai/WuLMZZG19} propose a solution to improve diversity of CF-based recommendation with GAN based on personalized diversification.} 

%We will better review this paper later. 

\setlength{\parindent}{15pt} \yd{[\textbf{LambdaGAN]} In~\cite{DBLP:conf/ijcnn/WangZC019}, the authors Wang et al., propose LambdaGAN --- a GAN model with lambda ranking strategy --- that improves the recommendation performance in a pairwise ranking setting by proposing lambda rank~\cite{DBLP:conf/cikm/YuanGJCYZ16} function into the adversarial learning of the proposed GAN-based CF framework.}

\setlength{\parindent}{15pt} \yd{[\textbf{VAEGAN]} A variant of VAE is introduced in~\cite{DBLP:conf/ijcai/YuZCX19} to address the limited expressiveness of the inference model and latent features, which reduces the generalization performance of the model. The proposed solution, named adversarial variational autoencoder GAN (VAEGAN), is a more expressive, and flexible model that better approximates the posterior distribution by combining VAEs and GAN. This work is one of first work to propose the application of adversarial variational Bayes (AVB)~\cite{DBLP:conf/icml/MeschederNG17} to perform the adversarial training.} 


\subsubsection{Context-aware Recommendation}
\yd{Although long-term preference modeling has proven to be effective in several domains~\cite{DBLP:conf/kdd/BerkovskyF15}, recent research indicates that users' preferences are highly variable based on the user's context, e.g., time, location, and mood~\cite{DBLP:conf/recsys/KompanKB17}. Context provides the background of \textit{user objective} for using the system and can be used to generate more relevant recommendations.}

\noindent \yd{\textbf{Temporal-aware Recommendation:}
In real applications, users' preferences change over time and modeling such \textit{temporal evolution} is needed for effective recommendation. While long-term preferences of users change slowly, their \textit{short-term preferences} can be seen as more dynamic and changing more rapidly. Predicting short-term user preference has been recently studied in the context of \textit{session-based} and \textit{sequential recommendations}. A temporal extension of SVD++ towards the modeling of temporal dynamic,  named TimeSVD++, has been proposed by Koren~\cite{DBLP:journals/cacm/Koren10} in 2010. It has also been reported that the structure of time-aware inputs (e.g., click-logs, session) are effectively modelled by recurrent neural network (RNN).
For instance, Hidasi et al.~\cite{DBLP:journals/corr/HidasiKBT15} proposed to model the sequential user clicks to output session-based recommendation with a GRU-gated recurrent unit; while Wu et al.~\cite{DBLP:conf/wsdm/WuABSJ17} proposed to integrate an LSTM model, to capture both the user and the item temporal evolution, and MF to model stationary preferences. Inspired by the accuracy improvements of IRGAN, GAN-based models have been combined in temporal frameworks to boost the recommendation performance in sequence-aware recommendation tasks.} 

\setlength{\parindent}{15pt} \yd{[\textbf{RecGAN}] In~\cite{DBLP:conf/recsys/BharadhwajPL18}, the authors propose to incorporate in a single framework both the temporal modeling capabilities of RNN and the latent feature modeling power of the \textit{min-max  game}. The proposed framework, named RecGAN, implements both the generator and the discriminator with the Gated Recurrent Unit (GRU)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}, in order to make $\mathcal{G}$ capable of predicting a sequence of relevant items based on the dynamic evolution of user's preferences.}

\setlength{\parindent}{15pt} \yd{[\textbf{PLASTIC \& LSIC}] Differently from RecGAN that implements only a RNN cell to capture the dynamic evolution of user's behaviour, Zhao et al.~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, 8643032} propose to combine MF and RNN in an adversarial recommendation framework to model respectively long and short-term user-item associations. The proposed framework, named PLASTIC, adopts MF and LSTM cells into $\mathcal{G}$ to account for varying aspect of both users and item,  while a two-input Siamese network --- built manually by using a MF and RNN --- as $\mathcal{D}$ encodes both the \textit{long-term} and \textit{session-based information} in the pair-wise scenario.}

\setlength{\parindent}{15pt} \yd{[\textbf{NMRN-GAN}] Recent studies have endorsed creating close-to-observed negatives samples adversarially are capable of improving the user and item representation. In~\cite{DBLP:conf/kdd/WangYHLWH18}, Wang et al., introduce \textit{GAN-based negative sampling} for streaming recommendation. Instead of using a random sampling strategy, which is static and hardly contributes towards the training of the recommender model, adversarially generated negative samples are more informative. NMRN-GAN uses a key-value memory network~\cite{DBLP:conf/www/ZhangSKY17} to keep the model's long-term and short-term memory combined with a GAN-based negative sampling strategy to create more instructive negative samples and improve the training effectiveness and the quality of the recommendation model.}

%An integration of a streaming recommender systems based on key-value memory networks~\cite{DBLP:conf/www/ZhangSKY17} with a generative adversarial network (instead of a random sampler) is presented in \cite{DBLP:conf/kdd/WangYHLWH18} to generate more informative negative examples used by the recommender models to learn users' preference in a pairwise settings. The motivation of this particular GAN application originates from the fact that random sampling strategies are static and scarcely contribute towards the training of the recommender model. Instead, adversarial learning includes the generation of adaptive and informative samples that the authors experimentally evaluated to improve the training effectiveness and the recommendation accuracy of the model.

\setlength{\parindent}{15pt} \yd{[\textbf{GAN-CQDN}] GAN-based solution for sequence-aware recommendation has been proposed in conjunction with reinforcement learning (RL), to model the dynamic of user's status and long-term performance. In~\cite{DBLP:conf/icml/Chen0LJQS19}, the authors Chen et al., propose GAN-CQDN, an RL-based recommender system that exploits GAN to model user behavior dynamics and learn her reward function. The advantages of using GAN is that it improves the representation of the user profile, improves the reward function according to the learned user profile and accommodates online changes for new users.} 
%\yashar{Felice, we should name this paper: GAN-CQDN}

%In~\cite{DBLP:conf/icml/Chen0LJQS19}, the authors propose to model the behavior temporal evolution and the RL reward function of a user through the adversarial learning of GAN. The core idea of the proposed framework, named GAN-user-model, is to model user's behavior evolution via a min-max  formulation. 
\noindent \yd{\textbf{Geographical-aware Recommendation:}  A relevant application of contextual information is point-of-interest (POI) recommendation. }\yashar{add a few more words here}


\setlength{\parindent}{15pt} \yd{[\textbf{Geo-ALM}] In~\cite{DBLP:conf/ijcai/0061W0Y19}, the authors propose Geo-ALM, a GAN-based POI recommender that integrates geographical features (POI and region features) with a GAN to achieve (better) POI recommendation. In the proposed system, $\mathcal{G}$ improves the random negative sampling approach in the pairwise POI recommendation scenario that leads to better representation of user and items and enhances recommendation quality with respect to state of the art models.}

%where $\mathcal{G}$ is used to generate more informative negative samples to be coupled with positive (real) ones to train $\mathcal{D}$ under a pairwise learning setting. The proposed model firstly integrates both $\mathcal{G}$ and $\mathcal{D}$ with geographical features (e.g., the number of nearest POIs, and the size of the region containing a POI) in order to fuse geographical constraints in the min-max  game.

\setlength{\parindent}{15pt} \yd{[\textbf{APOIR}] Inspired by the advances of POI recommendation performance under GAN-based framework, Zhou et al., propose adversarial point-of-interest recommendation (APOIR)~\cite{DBLP:conf/www/0002YZTZW19} to learn user-latent representations in a generative manner. The main novelty of the proposed framework is the use of POIs' geographical features and the users' social relations into the reward function used to optimize the $\mathcal{G}$. The reward function acts like a contextual-aware regularizer of $\mathcal{G}$, that is the component of APOIR in the proposed POI recommendation model.}

\subsubsection{Cross-domain Recommendation}
\yashar{To make it balanced with previous section, this introduction could be a bit shortened by Tommaso}
\yd{Cross-domain recommender models are designed to compute recommendations for items belonging to a single domain; for example, in media streaming platforms, Netflix recommends movies/TV series to its consumers while Lasts.Fm offers songs and music-album recommendations. Items belonging to a specific domain share characteristics and attributes, which are intrinsically similar and domain-specific recommendation models allow the designer to study these characteristics individually. However, \textit{single-domain} recommendation face numerous challenges. First, refers to the well-known \textit{cold-start} problem, when insufficient interactions exist in the considered domain. Second, users' interests and needs span across different application areas and large e-commerce sites, like Amazon or Ebay, store users' preference scores related to products/services of various domains - from books and products to online movies and music. As companies strive to increase the diversity of products or services to users, cross-domain recommendation can help such companies to increase sale productivity by offering personalized cross-selling or bundle recommendations for items from multiple domains~\cite{cantador2015cross}. The third aspect is a novel research idea related to discovering relationships between item (e.g., images) of two different domains. For example, can machine achieve a human-level understanding to recommend a fashion item (domain A) consistent with user taste/style in another domain such as media or visual scenery (domain B)? The central problem here is to find a mapping function from one domain to another domain~\cite{DBLP:journals/corr/abs-1812-06229}. Recently, the generative power of GANs has been used to tackle this problem as a conditional image generation problem, i.e., to generate an image in one domain given another image in the other domain~\cite{DBLP:conf/cvpr/IsolaZZE17}. In the following we review different research works applying GAN-based approaches to various cross-domain recommendations tasks: }

\setlength{\parindent}{15pt} \yd{[\textbf{FR-DiscoGAN}]
In~\cite{DBLP:conf/bigcomp/JoJCJ19}, the authors propose a cross-domain GAN to generate fashion designs from the sceneries. In the proposed hypothetical scenario, the user can specify via a query her POI to visit (e.g., mountain, beach) together with keywords describing a season (i.e., spring, summer, fall, and winter). The core idea is to automatically generate fashion items (e.g., clothes, handbags, and shoes) whose useful features (i.e., style) match the the natural scenery specified by the user. For instance, the system can recommend a collection of fashion items that look cool/bright for visiting a beach in summer even though the true preference of the user is black-style clothes. The role of GAN is to learn associations between scenery and fashion images. In the field of ML and Computer Vision, the problem is termed as \dquotes{style transfer} or \dquotes{image to image translation} problem~\cite{DBLP:conf/cvpr/GatysEB16}.} 
%\yashar{@Felice: this paper we do not have in the Table.}

\setlength{\parindent}{15pt} \yd{[\textbf{VAE-GAN-CC}]
An effective cross-domain recommendation system relies on \textit{capturing both similarities and differences} among features of domains and exploiting them for improving recommendation quality in multiple domains. Single-domain algorithms have difficulty in uncovering the specific characteristics of each domain. To solve this problem, some approaches extract latent features of the domains by a separate network~\cite{DBLP:conf/www/LianZXS17,DBLP:journals/tmm/MinBXH15}. Although these approaches might be successful in capturing characteristic features of each domain, they do not establish the similarity between features of multiple domains. To extract both homogeneous and divergent features in multiple domains, in~\cite{DBLP:journals/corr/abs-1812-06229} Nguyen et al., propose a generic cross-domain recommendation system that takes as input the user interaction history (click vector) in each domain,  maps the vectors to a shared latent space using two AEs and then uses $\mathcal{G}$ to remap the underlying latent representation to click vectors. The main novelty of this work lies in building/linking shared latent space between domains, which in turn facilitates \textit{domain-to-domain} translation. In particular, the former is realized by enforcing a weight-sharing constraint related to variational auto-encoders, i.e., the encoder-generator pair $\{\mathcal{E}_A, \mathcal{G}_A\}$ and $\{\mathcal{E}_B, \mathcal{G}_B\}$ and using cycle-consistency (CC) as a weight-sharing constraint. Finally, two separate adversarial discriminators are employed to determine whether the translated vectors are realistic. The final system is called VAE-GAN-CC network, which extends the unsupervised image-to-image translation network in the CV domain~\cite{DBLP:conf/nips/LiuBK17} for RS applications and is thus named domain-to-domain translation model (D2D-TM).} 
   %      \footnote{The wights sharing is done on the last few layers of encoders $\{E_A, E_B\}$ and first few layers generators $\{G_A, G_B\}$ which are in charge of encoding and decoding high-level representations of the input click vectors.}
% \yashar{We are going to remove this into since it has no backup paper. Will add CnGAN or DASO instead} A possible solution for cross-domain recommendation is to rely on \textit{domain linkage} based on \textit{user-} and \textit{item-overlap}. Four types of relationships are identified in SoA literature in cross-domain recommendation~\cite{DBLP:conf/icdm/CremonesiTT11}: i) no overlap, ii) user-overlap, iii) item-over lap and (iv) user and item overlap. CF models can function in all these cases, except for the first case. Therefore, the existence of an overlap is the key enabler to obtain an effective recommendations with a classic CF strategy. However, in many real applications a limited overlap between domains may exist, hindering CF functioning. Such approaches have been proposed to deal with  the  \textit{domain overlap  issue} in  a  more  flexible  way such as by approaches that build/measure \dquotes{characteristics}  that  are  shared  by  the  user/item  profiles in  the different  domains (often via a latent representation). Although effective, in face of heterogeneity of domains,  number of shared characteristic between domain can be small.  

\yd{
\setlength{\parindent}{15pt} [\textbf{DASO}]
Inspired by the efficacy of \textit{adversarial negative sampling} techniques proposed in~\cite{DBLP:conf/kdd/WangYHLWH18}, Fan et al.~\cite{DBLP:conf/ijcai/FanD0WTL19} address the limitation of typical negative sampling in the \textit{social recommendation} domain in transferring users' information from social domain to item domain. The proposed deep adversarial social recommendation (DASO) system, harnesses the power of adversarial learning to dynamically generate difficult negative samples for \textit{user-item} and \textit{user-user pairs}, to guide the network to learn better user and item representations. The authors validate the effectiveness of the system compared with the state of the art pairwise ranking and GAN-based models.}

%To evaluate the performance, the authors compared DASO with BPR, SBPR~\cite{DBLP:conf/cikm/ZhaoMK14}, DeepSoR~\cite{DBLP:conf/aaai/FanLC18}, GraphRec~\cite{DBLP:conf/www/Fan0LHZTY19} and IRGAN. Comprehensive experiments on two real-world datasets show the effectiveness of their model


\yd{\setlength{\parindent}{15pt} [\textbf{CnGAN}]
Perera et al., in~\cite{DBLP:conf/www/PereraZ19}, propose GAN for cross-network (CnGAN) to address one of the significant shortcomings of cross-network recommendation concerning \textit{non-overlapping users}  missing preference scores. These users exist in the source domain but not in the target domain, and thus, their preferences about items in the target domain are not available. In the proposed work, $\mathcal{G}$ learns the mapping of user preferences from \textit{target to source} and generate more \textit{informative preferences} on the source domain. $\mathcal{D}$ uses the synthetically generated preferences (generated from $\mathcal{G}$) to provide recommendations for users who only have interactions on the target network (not overlapped users). The authors also propose two novel loss functions --- a content-wise and a user-wise loss function --- to guide the min-max training process better. The author validate the effectiveness of the system against state-of-the-art models both in terms of accuracy and beyond-accuracy measures (novelty, diversity).}

%While Vanilla GAN models are typically used to generate real-like samples from random noise vectors, CnGAN aims to \textit{learn} a specific mapping from target to source network in order to \textit{move} the encoding of non-overlapped users in a latent space that encodes global implicit information of another domain (source network). 
%The discriminator uses the synthetically generated preferences (generated from $G$) to provide recommendations for users who only have interactions on the target network (not overlapped users). The authors evaluate CnGAN against TimePop, TBKNN~\cite{Campos:2010:STK:1869652.1869655}, TDCN~\cite{DBLP:conf/mm/PereraZ17} showing outperforming results in terms of accuracy, novelty and diversity.
\vspace{-5mm}


\subsubsection{Fashion Recommendation}
\yd{Most conventional RS --- such as CF or CBF --- are not suitable for application in the fashion domain due to unique characteristics hidden in this domain. For instance, people do not follow the crowd blindly when buying clothes or do not buy a fashion item twice~\cite{DBLP:conf/waim/ShaWZFZY16}. Furthermore, each person --- in particular women ---  would like to look different than the others. Another aspect is related to notion of \textit{complementary} relationship for recommending a personalized fashion outfit. It is natural for humans to establish a sense of relationship between products based on their visual appearance. Traditional visual CBF (and hybrid) models are centered around the notion of similarity (or alternativeness), e.g., seeking to answer the question \dquotes{which shirt matches this shirt more?}. Instead, complementary relationship seeks to answer the question \dquotes{given a red top (upper garment), which pairs of trousers (bottom garment) matches it --- as an outfit --- in a complementary way?}. Recently, GAN-based models have shown promising performance for outfit recommendation, being able to compete with state-of-the-art fashion recommendation models in the field, such as Siamese-base networks [] and [xxx]. Finally, another exciting application of GANs are related to exploit the \textit{generative power of GANs} to synthesize real-looking fashion clothes. This aspect can inspire the aesthetic appeal/curiosity of costumer and designers and motivates them to explore the space of
potential fashion styles.}

%The complementary recommendation task is a new and challenging problem popularized in the context of fashion recommendation.

\setlength{\parindent}{15pt} \yd{[\textbf{CRAFT}] Huynh et al.,~\cite{DBLP:conf/eccv/HuynhCTA18} address the problem of recommending complementary fashion items for a given fashion based on visual features by using an adversarial process that resembles GAN and uses a conditional feature transformer as $\mathcal{G}$ and a discriminator, $\mathcal{D}$. One main distinction between this work and the prior literature is that the <input, output> pair for $\mathcal{G}$ are both features (here features are extracted using pre-trained CNNs~\cite{DBLP:conf/aaai/SzegedyIVA17}), instead of <image, image> or hybrid types such as <image, features> explored in numerous previous works~\cite{DBLP:conf/iccv/ZhuFULL17,DBLP:conf/cvpr/VolpiMSM18}. This would allow the network to learn the relationship between items directly on the feature space, spanned by the features extracted. The proposed system is named complementary recommendation using adversarial feature transform (CRAFT) since in the model, $\mathcal{G}$ acts like a feature transformer that --- for a given query product image $q$ --- it maps the source feature $s_{q}$ into a complementary target feature $\hat{t}_{q}$ by playing a min-max game with $\mathcal{D}$ that aims to classify fake/real features. For training, the system relies on learning the co-occurrence of item pairs in real images. In summary, the proposed method does not generate new images; instead it learns how to generate features of the complementary items conditioned on the query item. CRAFT has been tested by experienced users who gave positive feedback on the goodness of complementary recommendations.}

%\yashar{Since we emphasize in the following, please check the above paper uses pre-trained CNN not an End-to-end model.}~\felice{Thery extract the feature from a pre-trained network and they they append these features which are the input of a features transformer (the generator) the component that is learned in the model. But the first feature extraction is done from a pre-trained model}

\setlength{\parindent}{15pt} \yd{[\textbf{DVBPR}] Deep visual Bayesian personalized ranking (DVBPR)~\cite{DBLP:conf/icdm/KangFWM17} is presumably one of the first works that exploit the \textit{visual generative power of the GAN} in the fashion recommendation domain. It aims to generate clothing images based on user preferences. Given a user and a fashion item category (e.g., tops, t-shirts, and shoes), the proposed system generates new images --- i.e., clothing items --- that are consistent with the user's preferences. The contributions of this work are two-fold: first, it builds and end-to-end learning framework based on the Siamese-CNN framework. Instead of using the features extracted in advance, it constructs an end-to-end system that turns out to improve the visual representation of images. Second, it uses a GAN-based framework to generate images that are consistent with the user's personal taste. Iteratively, $\mathcal{G}$ learns to generate a product image integrating a \textit{user preference maximization objective}, while $\mathcal{D}$ tries to distinguish crafted images from real ones. Generated images are quantitatively compared with real images using the preference score (mean objective value), inception score~\cite{DBLP:conf/nips/SalimansGZCRCC16}, and opposite SSIM~\cite{DBLP:conf/icml/OdenaOS17}. This comparison shows improvement in preference prediction in comparison with non-GAN based images. At the same time, the qualitative comparison demonstrates that the generated images are realistic and plausible, yet they are quite different from any images in the original dataset --they have standard shape and color profiles, but quite different styles.} %\yashar{Please check quantitative and qualitative, SSIM is a metric that matches human visual system.}
%~\felice{\textbf{From the paper}: Evaluation of Generated Images: Next, our goal is to quantitatively compare real versus generated images. As we stated in Section IV-A, we use the mean objective value (i.e., eq. 6), inception score [39] and Opposite SSIM [36], [40] to evaluate how well images match user preferences, image quality, and diversity, respectively.}

%We extended previous work on visually-aware recommendation using an end-to-end learning approach based on the Siamese-CNN framework. This leads to substantially more accurate performance than methods that make use of pretrained representations. We then used the framework of Generative Adversarial Networks to learn the distribution of fashion images and generate novel fashion items that maximize users’ preferences. This framework can be used in a variety of recommendation scenarios, to explore the space of possible fashion items, to modify e

%it is defined by the category extracted from the CNN,
%Complementary Recommendation is a novel challenging task that points to suggest complementary items to customers. A very intuitive application domain is the fashion domain. For instances, given a red top (i.e., upper garment), the recommender model may recommend a selection of bottoms (e.g., trousers) in a complementary way.  Novel solutions have been proposed to address the problem of recommending complementary items by using adversarial-based approaches. Kang et al. [38] do not directly use the features extracted in advance, but instead construct an end-to-end model by CNNs.

% \yashar{xxx: could we mention the type of features? is it CNN or AE feature?}\felice{CNN, I have put a reference to the cnn that they have used}\yashar{Thanks. is it pre-trained CNN? I assumed and added this term. if it learned, remove plz.}~\felice{Pre-trained}

% \yashar{This part will check later}
% It is worthwhile mentioning that inspired by advances in image generation by class labels or by texts, and image transformation between different domains, Kang \textit{et al.}~\cite{DBLP:conf/icdm/KangFWM17}, Shih \textit{et al.}~\cite{DBLP:conf/aaai/ShihCLS18}, Lin \textit{et al.}~\cite{Yang2018FromRT} and Kumar and Das Gupta~\cite{DBLP:journals/corr/abs-1906-05596} propose GAN-based~\cite{DBLP:journals/corr/RadfordMC15} solutions for the generation of compatible items in the fashion domain.\yashar{till here}


%Our architecture resembles traditional GAN designs with two main components: a conditional feature transformer and a discriminator


%They develop an unsupervised learning approach for Complementary Recommendation using Adversarial Feature Transform (CRAFT), by learning the co-occurrence of item pairs in real images. The proposed method does not generate new images but it learns to generate features of the complementary items conditioned on the query item. The generator $\mathcal{G}$ acts like a feature transformer to transform the source feature $s_{q}$ into a complementary target feature $\hat{t_{q}}$ by playing a \textit{min-max  game} with a discriminator $\mathcal{D}$ that aims to classify feature pairs as real ($s_{i}$, $t_{i}$) or synthetic ($s_{q}$, $\hat{t_{q}}$).

% We define an adversarial process to train a conditional generative adversarial network that can learn the joint distribution of item pairs by observing samples from the real distribution, i.e., image features of co-occurring items.

%Similar to Equation~\eqref{equation:gan-rf-j}, the objective function is
%\begin{equation}
%    \label{eq:craft}
%    J(\theta, \phi) = \mathbb{E}_{(s_{i}, t_{i}) \sim p_{c}} \log D_{\phi}(s_{i}, t_{i})+\mathbb{E}_{z \sim p_{z}, s_{q} \sim p_{s}} \log (1-D_{\phi}(s_{q}, G_{\theta}(s_{q}, z)))
%\end{equation}
%where $p_{z}$ and $p_{s}$ are the probability distribution function of the random noise and the source feature.
%Recommendations are built on a nearest neighbor search of $\hat{t_{q}}$ on the subspace with pre-indexed target features $t_{i}$.
%CRAFT has been tested by experienced users who gave positive feedback on the goodness of complementary recommendations.



%Inspired by LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}, the overall objective function is
%\begin{equation}
%    \small
%    \label{eq:dvbpr_gan_objective}
%    J = \mathbb{E}_{\mathbf{x}, c \sim p_{true}(x, c)} [D(\mathbf{x}, c) - 1]^{2} + 
%        \mathbb{E}_{c \sim p(c), z \sim p(z)} [D(G(z, c), c)]^{2}
%\end{equation}
%where $x$ is a image of the training dataset, $c$ is the category of the image $x$, and $z$ is a random noise vector. Given a user $u$ and a category $c$, the authors propose to synthesize personalized images by optimizing a user preference score
%\begin{equation}
%    \small
%    \widehat{\delta}(u, c) = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} ( \widehat{r}_{u, e} )
%    = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} \big(r_{u, e}-\eta D(e, c) \big)
%\end{equation}
%where $r_{u,e}$ is the user score assigned to a generated new image and $\eta$ controls the trade-off between preference score and image quality.
\setlength{\parindent}{15pt} \yd{[\textbf{MrCGAN}] Shih et al.,~\cite{DBLP:conf/aaai/ShihCLS18} propose a compatibility learning framework that allows the user to visually explore candidate \textit{compatible prototypes} (e.g., a white T-shirt and a pair of blue-jeans). The system uses metric-regularized conditional GAN (MrCGAN) to pursue the item generation task. It takes as the input a projected prototype (i.e., the transformation of a query image in the latent "Compatibility Space") and produces as the output a synthesized image of a compatible item (the authors consider a compatibility notions based on the complementary of the query item across different catalogue categories.). Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18}, the authors conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines.}
% 
% \yashar{@Felice: could we specify for xxx what do they refer with the notion of prototype? is it real or in latent space? for yyyy it would be good to know if they consider similarity, complementary or both. Thanks}

%The proposed model is composed of a compatibility learning component and a DCGAN~\cite{DBLP:journals/corr/RadfordMC15}-based component, MrCGAN, that is regularized on a compatibility metric learnt in the first component. Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18} they conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines.



% We propose modeling the asymmetric and many-to-many relationship of compatibility by learning a Compatibility Family of representation and prototypes with an end-to-end system and the novel Projected Compatible Distance function. The learned Compatibility Family achieves more accurate recommendation results when compared with the state-ofthe-art Monomer method (He, Packer, and McAuley 2016) on real-world datasets. Furthermore, the learned Compatibility Family resides in a meaningful Compatibility Space and can be seamlessly coupled with our proposed MrCGAN model to generate images of compatible items. The generated images validate the capability of the Compatibilty Family in modeling many-to-many relationships. Furthermore, when compared with other approaches for generating compatible images, the proposed MrCGAN model is significantly more preferred in our user surveys


\setlength{\parindent}{15pt} \yd{[\textbf{Yang et al.,} \& \textbf{$c^+$GAN}] Yang et al., in~\cite{Yang2018FromRT} address the same problem settings of MrCGAN~\cite{DBLP:conf/aaai/ShihCLS18} by proposing a fashion clothing framework composed of two parts: a clothing recommendation model based on BPR combined with visual features and a clothing complementary item generation based GAN. Notably, the generation component takes in input a piece of clothing recommended in the recommendation model and generates clothing images of other categories (i.e., top, bottom, or shoes) to build up a set of complementary items. The authors follow a similar qualitative and quantitative evaluation procedure as DVBPR~\cite{DBLP:conf/icdm/KangFWM17} and further propose a \textit{compatibility index} to measure the compatibility of the generated set of complementary items. A similar approach has also been proposed also in [\textbf{$c^+$GAN}]~\cite{DBLP:journals/corr/abs-1906-05596}, to generate bottom fashion item paired with a given top item.}


%\yashar{Do we want to say any technical word about how the generation is done?}~\felice{Probably we can simply say they follow the experimental protocol of that paper.}
%They evaluate GAN performance with three indexes: \textit{Inception} score related to the quality of the generated image~\cite{DBLP:conf/nips/SalimansGZCRCC16}, \textit{Opposite SSIM} related to the diversity~\cite{DBLP:conf/icml/OdenaOS17}, and a proposed \textit{Compatibility index} to measure the compatibility of the generated set of complementary items. \yashar{This paper is very similar to previous paper ~\cite{DBLP:conf/icdm/KangFWM17} in terms of evaluation metrics, please check.}~\felice{We can omit it and put the reference with the previous one} They compare the model with DCGAN as there are not baseline methods for such comparison. 




 %   \item \textbf{Users preferences Learning with Generative Adversarial Networks}  A interesting task is to generate more plausible user-rating profiles that can be used to improve recommendation performance above all in cold-user scenario. An interesting possible open directions may be to train a generator on domain with a huge amount of profiles and use it to enrich the source dataset that suffers of cold problem.
 %   \item  \textbf{Strength the difference between Adversarial Machine Learning and Generative Adversarial Networks} We think that the application of AML in rec sys need a unified view and categorization In this work, we have raised up the misunderstood of mixing GAN recommender under normal AML setting (attack/defense). We consider important to remark such division.  
 
% As the literature on AML for security emerged in the context of ML

% Adversarial examples created for image classificationtask are empowered based on continuous real-valued representation of image data (i.e., pixelvalues), but in RS, the raw values are user, item IDs and ratings that are discrete in nature.Perturbing these discrete entities is infeasible since it may lead to changing the semantic of theinput, e.g., loosely speakingI D+δcan result in a new userI D. Therefore, existing adversarialattacks in the field of ML are not transferable to the RS problems trivially. Furthermore, in thecontext of attacks against vision tasks, the perturbations often need to be “human-imperceptible”or “inconspicuous” (i.e., may be visible but not suspicious) [124]. How can we capture thesenuances for designing attacks in RS remains as a challenge.


%The application of GAN in recommendation scenario has been demonstrated to be effective in generating more informative negative samples, as data augmenter components and to compute cross-domain and complementary recommendations in a novel way thanks to the capability of transfer learning capabilities of GAN models. 
\begin{comment}
\begin{itemize}
    \item \textbf{Further Explore AML attack/defense approaches.} Is it possible to extend AML state-of-the-art attacks/defense in recommendation scenarios considering the differences between a classical classification task and the recommendation task? In Section 2, we have mentioned that perturbing a pixel images (continuous domain) does change the semantic of the image (human-imperceptible image alteration), while modifying users' profiles completely change the semantic of their behaviors.
    \item \textbf{Security of Content-RS Recommendation} Another interesting open direction is the investigation of the impact of adversarial perturbation on content-based, or hybrid, recommender models. Music, images and video deep features are widely used in modern recommenders and a deep study on alterations due to adversarial attack (and possible defense) can be really interesting.
    \item  \textbf{Definition of Attack Threat Model}
    We miss a common evaluation approach for attacking/defending scenarios. For instance, it is important to define a common attacker threat model (inspired by~\cite{DBLP:journals/corr/abs-1902-06705}) in order to define at priori the attacker knowledge and capabilities to make the attack (or defense) reproducible and comparable with novel proposal.
    \item\textbf{ Explainable Recommendation}  We mention also that there are not works that point to interpret recommendation results variation after attack, or after adversarial training. 
    \item \textbf{Move the attention towards Beyond Accuracy effect in Recommendation}  What is the impact of adversarial learning in other metrcis? For now we have found problem that works almost on hit ratio and nDCG, but what is the effect on other metric? Can be used adversarial learning to alter (in positive, and negative way) other perspective of evaluation?. 
    \item \textbf{Scalability and Stability of Learning }We identify the need to further explore the stability learning problems which have been already identified as a big problem when the GAN-RS are applied in real scenarios with huge catalogue. A initial point of study may be the study of novel GAN models proposed in computer vision (e.g., WGAN 3, LSGAN 27, and BEGAN 4).
    \item \textbf{Users preferences Learning with Generative Adversarial Networks}  A interesting task is to generate more plausible user-rating profiles that can be used to improve recommendation performance above all in cold-user scenario. An interesting possible open directions may be to train a generator on domain with a huge amount of profiles and use it to enrich the source dataset that suffers of cold problem.
    \item  \textbf{Strength the difference between Adversarial Machine Learning and Generative Adversarial Networks} We think that the application of AML in rec sys need a unified view and categorization In this work, we have raised up the misunderstood of mixing GAN recommender under normal AML setting (attack/defense). We consider important to remark such division. 


    
    
\end{itemize}
\end{comment}

%\emph{Multi-modal recommender systems.}
%\pc{not sure about this}
%Given that media items are described by multiple modalities, xxxx

%\emph{Leveraging additional interaction types.} 
%Generally, in the context of recommender systems leveraging multimedia content, xxx

%\emph{Considering the impact of user interfaces.} 

==> OLD_FILES/OLD_Sec2_Foundations.tex <==
\section{Characterizing Recommendation Models based on Adversarial-Machine Learning}

\subsection{Inputs, Outputs, Adversarial Tasks, and Problem Formalization}

This section is used to explain how is generally integrated an Adversarial Component in a recommendation framework.

\qquad\textit{Inputs. } The main inputs of an adversarial-based recommender system are the same of a classic recommender system. Inputs can be both user-related and item-related. \yashar{We can also state it as URM-based or going beyond the URM. For the former we have interactions, explicit or implicit. For the latter, we have user-contributed side information such as tag, review, comments and user-contributed multimedia. We can think about it.} User-related input are ratings, reviews, tags and any type of additional content that a user can upload in the recommender system. User-generated inputs are really important in an adversarial scenario because a malicious use of AML may be based on the injection of adversarial-user-generated content with the goal to manipulate the recommendation engine. Item-related inputs are also very important in an adversarial scenario. Depending on the domain, additional information on products, and services might be used by the adversarial-component to learn item-features exploitable in really challenging recommendation area such as complementary recommendations and cross-domain recommendations. 
% Generally, such forms of input data are partially available in practical applications and, by looking to the type and quantity of inputs, we will see different AML usage in recommender systems..


\qquad\textit{Outputs. } The output of adversarial-based recommender system is related to classical recommendation tasks. 
AML in recommendation task has different applications:
\begin{itemize}
    \item List of Applications
\end{itemize}


% The output is mainly the traditional "item-ranking" recommendation. Otherwise, there are works where there are other types of outputs. For example there are publications on complementary recommendations, where the recommended output is a complementary products, generally in fashion domain; and works in sequence-aware recommendations, where the output is the next probable chosen item.  


% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{Pictures/FigureGeneralArchitecture.pdf}
%     \caption{High-level Overview of Adversarial-Aware Recommendation Problems.}
%     \label{fig:GeneralFraamework}
% \end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=\linewidth]{Pictures/AdvReg_MF.png}
      \caption{Adversarial Regularized rec. model}
      \label{fig:sub1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.62\linewidth]{Pictures/GAN_model.png}
      \caption{GAN-based rec. model}
      \label{fig:sub2}
    \end{subfigure}
    \caption{General framework for AML-RS}
    \label{fig:test}
\end{figure}

\qquad\textit{Adversarial Tasks. }\label{sec:AdversarialTasks} 
Different adversarial tasks in recommendation scenario can be identified in the literature. 
Firstly, we identify the most intuitive adversarial task which is the use of AML to attack the system. Attacks point to worse the recommendation performance of the system. Note that these attacks are different from the well-known shilling attacks ~\cite{DBLP:journals/air/GunesKBP14} on recommender system and we will describe such differences in Section~\felice{subsubsec:AdversarialAttacks}.
Secondly, we analyze the defence task with AML techniques which is strictly related to the first one. It is interesting to note that mostly each work on attacks proposes also a countermeasure to attacks. See Section~\felice{subsubsec:DefenseMechanism} for further explanation.
Finally, the most interesting application of adversarial machine learning is related in improving recommendation performances. This advances in performances are mostly achieved thanks to a \textit{minimax game} played between the adversarial component and the recommender engine. Here, the adversarial component tries to minimize the effectiveness of the system, while the recommender engine works to maximize its objectives. At the end of this game both the \textit{adversarial component} and the pure \textit{recommender engine} contribute to the output generation which depends on the type of desired output, such as recommendation list, complementary and sequential. Section~\felice{subsubsec:ImproveRecommendation} focuses on this topic.



\qquad\textit{Problem Formalization. } Adopting the formalism of IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and \cite{DBLP:journals/corr/abs-1810-00069}~\felice{Survey-On-ADV}, we can describe the problem at a more formal level as follows.

Without loss of generality, let us consider the following information items ${i_{1}, ...,i_{M}}$. We have a set of user profile ${u_{1}, ..., u_{N}}$. For a given query $u_{n}$, we have a set of relevant items labelled, the size of which is much smaller than the total number of items M.

\felice{Here we can define some formalism used in our survey!!!}

%\section{Foundation and Key Challenges of AML in RS}\label{sec:literature}

Before we jump into the core of this survey, we focus on a brief overview to the bases of recommender system, deep learning techniques and adversarial machine learning. 
\textbf{Figure ~\felice{fig:example}} gives a high-level overview of the problem, its inputs, outputs, and a general task associate with the integration of an adversarial component in a recommender system. In general, the ordering of the objects can be relevant both with respect to the inputs and to the outputs. We will discuss these aspects in more detail next.

\subsection{Foundations of Adversarial Machine Learning}
We collected the list of survey publications related to adversarial machine learning advances. Searching strategy is based on the results of "adversarial survey" and "adversarial overview" search strings done on DBLP. 
\textbf{The robustness of a neural collaborative algorithm to adversarial perturbations is defined as its capacity against perturbations}
\felice{need paraphrasing- Taken from~\cite{DBLP:conf/www/ParkC19}}
Then, Goodfellow et al. hypothesized that the vulnerability of the models come from the linear nature in the models~\cite{DBLP:journals/corr/GoodfellowSS14}.
That is, the adversarial perturbation in each dimension adds up to a great change in the output due to some extent of linearity in the models. Goodfellow et al. also suggested to train a model by learning adversarial examples as well as original examples, where the adversarial examples were generated with the proposed fast gradient sign method. The trained model was reported more robust to adversarial examples. Adversarial examples and adversarial training are surveyed in .
The earlier adversarial training approaches required labels of examples, and this is not ideal for semi-supervised learning where there are much more unlabeled data than labeled data. Miyato et al.~\cite{DBLP:journals/pami/MiyatoMKI19} proposed virtual adversarial training, where labels are not required to generate adversarial examples. With its strength in semi-supervised learning, it has been applied to semi- supervised text classification [22] and image classification [23]
\felice{...till here}
\felice{need paraphrasing ... Taken By Deep Learning Goodfellow}
Goodfellow et al.~\cite{DBLP:journals/corr/GoodfellowSS14} showed that one of the primary causes of these adversarial examples is excessive linearity. Neural networks are built out of
primarily linear building blocks. In some experiments the overall function they
implement proves to be highly linear as a result. These linear functions are easy
to optimize. Unfortunately, the value of a linear function can change very rapidly
if it has numerous inputs. If we change each input by $\epsilon$, then a linear function with weights $w$ can change by as much as $\epsilon||w||_{1}$, which can be a very large
amount if $w$ is high-dimensional. Adversarial training discourages this highly
sensitive locally linear behavior by encouraging the network to be locally constant
in the neighborhood of the training data. This can be seen as a way of explicitly
introducing a local constancy prior into supervised neural nets.
Adversarial training helps to illustrate the power of using a large function
family in combination with aggressive regularization. Purely linear models, like
logistic regression, are not able to resist adversarial examples because they are
forced to be linear. Neural networks are able to represent functions that can range
from nearly linear to nearly locally constant and thus have the flexibility to capture
linear trends in the training data while still learning to resist local perturbation.
The assumption motivating this approach is that different classes usually lie
on disconnected manifolds, and a small perturbation should not be able to jump
from one class manifold to another class manifold.
\felice{...till here}
\textit{It was found in ~\cite{DBLP:journals/corr/SzegedyZSBEGF13} that several machine learning models, including modern state-of-the-art neural networks, fail with adversarial examples. A slight adversarial perturbation in the original input was enough to fake the models, meaning that the models classify the adversarial example into a wrong class with high confidence. Then, Goodfellow et al. hypothesized that the vulnerability of the models come from the linear nature in the models [9]. That is, the adversarial perturbation in each dimension adds up to a great change in the output due to some extent of linearity in the models. Goodfellow et al. also suggested to train a model by learning adversarial examples as well as original examples, where the adversarial examples were generated with the proposed fast gradient sign method. The trained model was reported more robust to adversarial examples. 
The earlier adversarial training approaches required labels of examples, and this is not ideal for semi-supervised learning where there are much more unlabeled data than labeled data. Miyato etal. [24] proposed virtual adversarial training, where labels are not required to generate adversarial examples. With its strength in semi-supervised learning, it has been applied to semi-supervised text classification [22] and image classification [23].}

\textit{Key-points for this section:}
\begin{enumerate}
    \item Brief Introduction of Adv ML 
    \item Explain Adversarial Attack/Defense evolution 
    \item Definition of key aspects:
    \begin{enumerate}
        \item Attacks: Adversarial Attack(\textbf{GAN}), Adversarial Examples Generation: [Type: L-BFGS, \textbf{FGSM}, Jacobian Based Method, \textbf{C\&W}] [Perturbation Selection: Perturb all the input dimensions, Perturb a selected input dimensions]
        \item Defense: \textbf{Adversarial Training}, Gradient Hiding, \textbf{Defensive Distillation}, Feature Squeezing, Ensemble
        \item \textbf{minimax} games and its effect of performance. [Improve a \textbf{classifier}, \textbf{Transfer} Distribution in a Generator, Generate New Data]
        \begin{itemize}
            \item             GAN FOR CONTINUOUS DATA In the original GAN [13], the objective is:
            \begin{equation}
            \label{equation:gan}
            \small
                J(\theta, \phi)=\mathbb{E}_{\boldsymbol{x} \sim p_{\text { data }}(\boldsymbol{x})}[\log D_{\phi}(\boldsymbol{x})]+\mathbb{E}_{\boldsymbol{z} \sim p_{\boldsymbol{z}}(\boldsymbol{z})}[\log (1-D_{\phi}(G_{\theta}(\boldsymbol{z})))]
            \end{equation}
            where the θ-parameterized generator $G_{\theta}$ and the $\phi$-parameterized discriminator $D_{\phi}$ play a minimax game. The generator is formulated to the data instance x, and the discriminator is formulated as a as a deterministic neural net that maps a noise vector $\boldsymbol{z} \sim p_{\boldsymbol{z}}$ sigmoid-based binary classifier:
            \begin{equation}
                \small
                \label{equation:gan_d}
                        D_{\phi}(x)=\sigma\left(f_{\phi}(x)\right)=\frac{1}{1+\exp \left(-f_{\phi}(x)\right)}
                 \end{equation}
             where $f_{\phi}(x)$ could be any scoring function to calculate the logit value of the sigmoid.
        \end{itemize}
    \end{enumerate}
\end{enumerate}


Note that there are numerous advanced model emerging each year, here we only briefly listed some important ones.






\subsection{How do we collect the papers?}\label{subsec:howCollect}

To identify the relevant publications that constitute the state of the art on the topic of adversarial learning in recommender systems, we mainly relied on publications indexed in major computer science bibliography databases namely DBLP\footnote{\url{https://dblp.uni-trier.de/}} and Scopus\footnote{\url{https://www.scopus.com}}. In addition, realizing the fact that many top-tiers venues also publish related works, which may not be necessarily indexed in the above databases, we we also gathered a number of related publications
by searching directly through Google Scholar.\footnote{\url{https://scholar.google.it/}} Our search strategy was composed of two main stages: 
\begin{enumerate}
\item relevant publication collection, 
\item filtering and preparing the final list.
\end{enumerate} 
~\felice{YYYY I AM HERE YYYYY}\\
We collected also referenced publications in the yet selected ones.
As for the first stage, we queried the term \dquotes{adversarial recommend} in the above-mentioned indexing services. While search in DBLP returns publications containing the query term in the \textit{title}, the search results from Scopus and Google Scholar return publications containing the query \textit{both in the tile and the content}, thereby all-together forming a complete list of identified research works. We collected all resulting publications from DBLP (43 papers)~\felice{Updated 22 October 2019} and 15 papers obtained from Scopus and Google Scholar search. In the second stage, we went through all the collected research works and removed all obviously irrelevant works. These for instance could include works that used AML for an application different than RS (e.g., in Computer Vision) or clearly out of scope topics (e.g., xxx)~\felice{?}.
We mostly turned our attention to conference-level and journal publications published in top conferences and to a lesser extent to workshop publications or works published in entry-level venues. Some of the considered journals and conferences include: the ACM Conference on Recommender Systems (RecSys),\footnote{\url{http://www.recsys.acm.org}}, the International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR),\footnote{\url{http://www.sigir.org}}, the ACM International WSDM Conference~\footnote{http://www.wsdm-conference.org/}, the International World Wide Web Conference (TheWebConference) and 
nternational Joint Conferences on Artificial Intelligence (IJCAI)~\footnote{https://www.ijcai.org/}.~\yashar{update}~\felice{Done!}

Given the recentness and originality of the topic, most of the identified research works are published between years 2017 to 2019. In table~\felice{Need It}, we provide some statistics about the reviewed research papers. While we do not claim that the final list of publications identified by our selection approach is exhaustive, we strongly believe that this literature review provides an overall picture of the most recent advances, trends on the topic and shed light on what we believe are the most pressing goals of AML application in RS, and useful insights for to both industrial practitioners and academic researchers. \yashar{Other search strategies should be clearly mentioned here}

\yashar{Here we can create a table and briefly provide some statistics, e.g., the final number of papers reviewed, average/min year of publications and maybe mostly used venue e.g, top 5}~\felice{Totally agree (it depends on the space)}

\subsection{Related Surveys.}
To put this survey into context, we identified the following related overview and survey articles, and explain in which ways the article at hand connects to and extends earlier work. 
\yashar{@Felice: Here we need to describe the most relevant surveys}~\felice{There aren't survey on this topic. I think we can drop off (comment) this paragraph for now and decide later if we have enough space to add it.}
\\Identified surveys:
\begin{itemize}
 \item Wild Patterns: Ten Years After the Rise of Adversarial Machine Learning~\cite{DBLP:journals/corr/abs-1712-03141} 
 \item Threat of Adversarial Attacks on Deep Learning in Computer Vision: A Survey~\cite{DBLP:journals/access/AkhtarM18}
 \item A survey on Adversarial Attacks and Defenses in Text~\cite{DBLP:journals/corr/abs-1902-07285}
 \item Recent Progress on Generative Adversarial Networks (GANs): {A} Survey~\cite{DBLP:journals/access/PanYYKYZ19}
 \item A survey of practical adversarial example attacks~\cite{DBLP:journals/cybersec/SunTZ18}
 \item How Generative Adversarial Networks and Their Variants Work: An Overview~\cite{DBLP:journals/csur/HongHYY19}
 \item Generative Adversarial Networks: An Overview~\cite{DBLP:journals/spm/CreswellWDASB18}
\end{itemize}




\input{Tables/abbreviations.tex}

\subsection{Contribution of this survey.}
\yashar{sure, we can finalize it toward the end of the work.}\\
~\felice{We need to paraphrase some parts. This part is only an example}
The objective of this study is to altogether audit writing on the advances of antagonistic AI based recommender framework. It gives a display which per users can rapidly comprehend and venture into the field of profound learning based proposal.
This study establishes the frameworks to encourage developments in the region of recommender framework and tap into the extravagance of this exploration zone. This review serves the analysts, professionals, and teachers who are keen on recommender framework, with the expectation that they will have a harsh rule with regards to picking the profound neural systems to tackle proposal main jobs.
\\
To summarize, the key contributions of this survey are three-folds: (1) We conduct a systematic review for recommendation models integrated with adversarial learning modules and propose a classification scheme to position and organize the current work; (2) We provide an overview and summary for the state-of-the-arts. (3) We discuss the challenges and open issues, and identify the new trends and future directions in this research field to share the vision and expand the horizons of adversarial machine learning based recommender system research.

The remaining of this article is organized as follows: Section 2 introduces the preliminaries for XXXXXXX. Section 3 presents our classification framework and then gives detailed introduction to the state-of-the-art. Section 4 discusses the challenges and prominent open research issues. Section 5 concludes the paper









==> OLD_FILES/OLD_Sec3OLD_Categorization.tex <==
\section{Categorization of Adversarial-based Recommender System}\label{section3}
% \yashar{Preparing the stable version. Will be pushed soon after completion.}

\begin{itemize}
    \item Categorization based on goal/challenges: (Section~\ref{sec:goal_catag},~Table~\ref{tab:CatTaskChalDom}, Fig~\ref{plt:openchallenge})
    \begin{itemize}
        \item Improve utility of CF recommendation
        \item Improve beyond-accuracy aspect
    \end{itemize}
    
    \item Categorization based on domain: (Section~\ref{sec:domain_catag},~Table~\ref{tab:CatTaskChalDom}, Fig~\ref{plt:domain})
    \begin{itemize}
        \item Media \& Entertainment 
        \item E-Product
        \item Social Computing
        \item Others

    \end{itemize}
        \item Technical categorization: (Section~\ref{sec:technical_catag})

    \begin{itemize}
        \item Based on GAN model and usage
        \item Based GAN-Disc type
        \item Based on learning type
        \item Based on training paradigm
    \end{itemize}
\end{itemize}


\subsection{Categorization based on the goal/challenges}\label{sec:goal_catag}



\subsubsection{Improve Utility of collaborative recommendation}
\label{subsec:util_CF}
% \yashar{New as the final version}
In the past two decades, we have witnessed a noteworthy advancement in design and deployment of various CF models. A prominent class of CF methods is \textit{model-based CF}, which learns a prediction model from the user rating matrix (URM) and use it at the prediction time to generate recommendation for a given user. Generally, these models can be differentiated based on two design-aspect considerations~\cite{DBLP:conf/ijcai/0001DWTTC18}: (i) how user and items are represented by the model and (ii) how the interaction between the user and item representations is described. We provide a few examples here, matrix factorization (MF) is the principal type of model-based CF, which assumes that there exists a linear relation between latent features (aka embedding) of users and item described via their inner product. BPR-MF learns MF by using a pairwise loss function which enforces positive items precede negative items in the ranking list. NeuroCF and DeepMF learn the latent representation via DNNs. \cite{DBLP:conf/ijcai/WangTWL15}  exploit hierarchical structures of users and items for recommendation.





~\cite{DBLP:conf/ijcai/0001DWTTC18} combines neural and tree-based method to obtain explainable recommendation.

The most recent approach and the one we focus here is the one based on adversarial training to learn CF models (such as MF).



% \yashar{till here}

Collaborative filtering (CF) models have been the principal choice of many online services and academic research due to their good recommendation quality. CF models rely solely on user item interaction matrix  (urm) and leverage the correlations encoded among interaction patterns of users (user-based CF) or items (item-based CF) in order to generate recommendations. By taking into account the collective behavior of other users, these models have been shown to be capable of generating a plausible representation of users' needs/preferences commonly measured in terms of top-$k$ recommendation accuracy.

% \yashar{added new} 
Matrix factorization (MF) is the principal type of model-based CF, which assumes that there exists a linear relation between latent features (aka embeddings) of users and item and models it via their inner product.
%


% \yashar{added the following...} 
We can classify (CF) recommendation models according to the types of objective functions used for training the model as \textit{pointwise}, \textit{pairwise} and \textit{listwise}~\cite{DBLP:journals/corr/HidasiKBT15}. Pointwise focuses on individual preference scores (e.g., RMSE) or ranking of items (e.g., MRR, cross-entropy) and the loss function is designed so as to maximize the utility of relevant items (i.e., higher preference scores or lower ranking). Pairwise loss function (such as BPR~\cite{DBLP:conf/uai/RendleFGS09} adopts a relative approach by taking into the account pairs of (positive, negative) and enforcing to place positive items in a lower-ordered position compared to the the negative items. Listwise considers the utility (preference score or ranking) of all items in the list and compares it with the ideal one. This loss function can directly predict the ranking and avoid the noise introduced as the results of prediction/aggregation in pointwise raking however it is often computationally more expensive.\footnote{Note that we can regard CF models based on pointwise loss function as \textit{rating-oriented} and the other two case as \textit{ranking-oriented}.} Examples of CF models that are trained based on these loss, we can name of SLIM, CADE (pointwise), BPR-MF (pairwise) and listCF (listwise).
% \yashar{pureSVD?}~\felice{Generally not used} \yashar{ok, I don't think it is a huge problem if we just name it here for the sake of completeness}
% \yashar{Felice, I added information like this. Please check and add the models to Table with citations if we are not going to cite them here.}~\felice{I would like to add on that table all the models that are directly interested by adversarial stuff because it will be too big if we insert a description for all the model named also for 'simple' related work.}


%\yashar{@Felice, please mention some examples: }~\felice{ Factorization Machine (FM)~\cite{DBLP:conf/icdm/Rendle10} generalizes MF to capture associations between features inside high dimensional sparse datasets with. } \yashar{FM extends MF by allowing side information, therefore it is not a pure CF model. Furthermore, in FM one can allow high-order interaction, I am not sure if it is always linear. Here we would like to contrast two CF approaches: i) linear models (the one modelling interactions between latent feature linear like MF) and ii) non-linear models (such as DNN, still CF but modelling interactions between latent features non-linearly). See some examples of linear ones below commented.}~\felice{Where? I think we should put models that are useful for the type of model discussed in the survey like BPR-MF, VBPR or FM which are used in different applications with AML} 


%BiasedMF , SVD++ [20], and PMF [29] on the rating prediction task, and WRMF
%[15], BPR [34], PureSVD [7], SLIM [30], CLiMF [36], and FISM }


Having reached a level of maturity in terms of recommendation accuracy, attempts to further improve the performance of CF methods have been followed on several directions by the research community. These approaches differ from each other based on the data they use as input (pure urm or urm plus side information), the machine learning model architecture (classical v.s. deep) or the core problem formulation (classical v.s. adversarial-learning). The first popular research direction is to use of \textit{side-information beyond the urm}~\cite{DBLP:journals/csur/ShiLH14}, for example by using item description information such as textual metadata (e.g., movie cast, product review, artist information)~\cite{DBLP:conf/recsys/NingK12,DBLP:conf/recsys/VasileSC16} or information extracted directly from the signal (images or audio)~\cite{DBLP:journals/umuai/DeldjooDCECSIC19,DBLP:conf/nips/OordDS13}. These approaches can be used to alleviate cold-start (CS) issues such as data sparsity or new/item user problem, which impede the performance of CF models. Based on the unique nature of side information in different domains, different hybrid CF strategies are designed commonly referred by \textit{CF models using side information} on items or users~\cite{DBLP:journals/csur/ShiLH14}. 

Another popular trend, which is booming in recent years, are recommendation based on deep neural networks (DNNs). DNNs have been show to achieve remarkable prediction accuracy for visual recognition task in presence of vast amount of training data and high computational resources (high-speed CPUs/GPUs). One of the main strength of deep-CF models is that they can uncover a non-relationship between latent factors of user and items giving them an advantage over MF approaches, which make a linearity assumption for the aforementioned factor, which may not be an accurate assumption in complex recommendation scenarios presumably. Examples of Deep-CF approaches include: CDL, CVAE,  AutoRec, CDAE,  NCF. See Table \ref{recommendermodels} for further information. 

% \yashar{Felice I have mentioned Deep-CF make sure this is correct for these examples. Also let's link to Table 4}~\felice{I have left only the ones that are mentioned or used under adversarial settings. Then I think we don't need here citation because these are e in the Table4}\yashar{Just make sure they are not hybrid and if they are mention that. Sure about citation, please remove.}~\felice{Done!}

%\felice{such as CDL~\cite{DBLP:journals/corr/WangWY14}, CVAE~\cite{DBLP:conf/kdd/LiS17}, Mult-VAE~\cite{DBLP:conf/www/LiangKHJ18}, AutoRec~\cite{DBLP:conf/www/SedhainMSX15}, SpectralCF~\cite{DBLP:conf/recsys/ZhengLJZY18}, CDAE~\cite{DBLP:conf/wsdm/WuDZE16},  NCF~\cite{DBLP:conf/www/HeLZNHC17}} \yashar{Please change abit the names, they look exactly similar to the paper CFGAN. See intro Para 2 of paper CFGAN. Just update the list a bit if possible.}~\felice{Done!}

Despite the efficacy of deep-CF models, recently it has been reported that they can be highly vulnerable in presence adversarial perturbations~\cite{DBLP:conf/sigir/0001HDC18, DBLP:conf/sigir/YuanYB19, DBLP:conf/ijcnn/YuanYB19, 8618394, DBLP:journals/tmm/DuFYXCT19, DBLP:conf/recsys/ChenL19} that can corrupt the performance of these models. Adversarial samples are meticulously modified information crafted to mandate a desired output, or alter the normal output, for an illegitimate purpose (e.g., market penetration, reduce trust in the provider). In the context of ML, this meticulous objective can be realized by attempting to fool a desired model to classify the input on a class different from the authentic class~\cite{DBLP:journals/ieeesp/McDanielPC16} (e.g., spams that can sidestep a spam filter) and in the context of recommendation(e.g., reduce the predicted score of an unrated item to a victim user, nuke the possibility of an entire group of items to be recommended~\cite{DBLP:conf/recsys/Christakopoulou19}

% 
% \yashar{@Felice: can you give a similar example for recsys}~\felice{}.

For instance, in ~\cite{DBLP:conf/sigir/0001HDC18} authors demonstrate that MF model optimized by BPR is not robust and is vulnerable to adversarial perturbations on its parameters; in ~\cite{DBLP:journals/tmm/DuFYXCT19} and ~\cite{DBLP:conf/sigir/YuanYB19} authors reveal respectively vulnerabilities at adversarial perturbations of two state-of-the-art deep models for recommendations, FNCF and CDAE.  In fact, adversarial attacks in the form of shilling attacks were shown to be effective to undermine the performance of recommendation much longer ago~\cite{DBLP:conf/recsys/MehtaHN07}. However, what make shilling attacks different from AML-based attack, the one we focus in this survey, is that classical shilling profiles have been built with \textit{hand-engineered} techniques (e.g. set the rating of the target item with a minimum/maximum value, and fill the rest of the shilling user profile with ratings sampled from normal distribution to mimic the ground-truth rating distribution~\cite{DBLP:conf/dexa/OMahonyHS02}), while AML-based attacks user \textit{machine-learning} optimization techniques to address the adversarial intent~\cite{DBLP:conf/recsys/Christakopoulou19}.


% \yashar{could we add a sentence here?}~\felice{}


We identified two main paradigms that adversarial machine learning has been used in recommender system for different application scenarios: \\
(1) GAN-based Models \\
(2) Adversarial learning without GAN 


\noindent{\textit{GAN-Based Approaches:}} The research on ML/RecSys community has used the power of GAN networks not as a problem (i.e., sensitivity of CF-models against adversarial inputs), rather as an \textit{opportunity} to fine tune the quality of recommendation models. The core idea is to utilize a pair of models ($G$ and $D$) and allow a competition game between the models to occur with the objective that each can push the other to achieve it goal better. This novel notion of learning stands at shark contrast with classical recommendation setting where only one model is in charge of all user preference inference. In the context of GAN-based CF, the two models have the following responsibilities: $G$ to generate items that the user might favor and $D$ to distinguish between the distribution generated by $G$ and user's ground truth. Through a competitive iteration between $G$ and $D$ (known as minimax game), $G$ will learn the actual distribution of user interest over items (user profile), which can be used to provide more appealing recommendation to users.

From the pioneering works that proposed a GAN framework for improving utility of item recommendation scenario under CF, we should highlight IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18}, with the difference that the former proposes the solution for CF based on MF whereas the second one proposed a graph-representation learning for the same problem. We discuss these works in more details in the following:

In~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, Wang et. al. present a unified theory of generative and discriminative methodologies in IR under the GAN framework named IRGAN. An important question in IR is: \dquotes{Given a query ($q$) and a document ($d$), what is the probability that $d$ is relevant to $q$?}. The answer to this basic question constitutes the basis for document ranking in IR and has been answered under two schools of thinking: i)the generative model and the ii)the discriminate model described in the following:

\begin{itemize}
    \item The \textbf{generative model} makes the underlying assumption is that there exists a stochastic \textbf{generative process} between $d$ and $q$. It then answers the above basic question in probabilistic terms by stating that it is equivalent to this question \dquotes{what is the probability of relevance, i.e., $p(R=r|d,q) = 1- p(R=\bar{r}|d,q)$?}. In text retrieval, two approaches are commonly used to estimate $p(R=r|d,q)$, which can be seen equivalent based on different parametrization of the likelihood under the Bayes rule; the first is the Robertson-Sparck Jones~\cite{DBLP:journals/ipm/Jones79} approach which aim to model the probability of relevance in a forward manner as $q \rightarrow d$ via factorization $p(R=r|d,q) = p(q|r) p(d|q, r)$. It can be shown that this problem becomes equivalent to the naive Bayes model for classification in which for a given information need $q$, the goal is to classify the document into classes $r$ and $\bar{r}$. The second is the language modeling approach~\cite{DBLP:conf/sigir/PonteC98} which takes the reverse approach $d \rightarrow q$ via factorization $p(R=r|d,q) = p(d|r) p(q|d, r)$, and aims to generate query terms for a given document.
    \item The \textbf{discriminative model} uses a machine learning approach to answer the basic question in which documents and queries are jointly considered as features and the goal is to predict relevance in ML way by using large amount of training data. Therefore the problem can be seen as $q+d \rightarrow d$. A significant example of this approaches are learning to rank (LTR) models whose aim to is the learn right ranking of documents (or items) given a representation of an information need (query or context). 
\end{itemize}

The work by IRGAN is presumably the first attempt to integrate the above notions of relevance under the same roof by proposing a GAN-based IR model. In particular a minimax game is proposed composed of a discriminative model responsible for discriminating ground-truth user-item recommendations from generated ones and a generator responsible for producing recommendations approximating the true distribution of relevant items as much as possible. \yashar{To make it different with the information I gave before, maybe we can at least mention what $G$ and $D$ models are?} The authors finally demonstrate the application of IRGAN for \textit{web search}, \textit{item recommendation} and \textit{question answering} tasks. \yashar{@Felice: to connect it to RS, could we add one more sentence how this links with item recommendation? Thanks}

In~\cite{DBLP:conf/aaai/WangWWZZZXG18}, the authors proposed GraphGAN, which employs GAN to perform graph representation learning (aka network embedding). Graph-based analysis are becoming increasingly popular in recent years due their ubiquity in real-world problems such as modelling user preference for item recommendation as well as social graphs in SM networks, co-occurrence graph in linguistics, citation graph in research, knowledge graph and so forth. A real-world information graph can consist of millions to billions of nodes and edges and uncovering relationship among all these entities can allow conducting various complex inference over the entire graph. The central idea of network embedding is to represent each entity (e.g., node) in a graph with a lower-dimensional latent vector of to facilitate tasks within network and prediction over entities. For example, the features of the latent vector embedding can allow to perform prediction for supervised tasks or the distance between node embedding vectors can serve as a useful measure in unsupervised tasks. GraphGAN proposes a similar idea to IRGAN, where queries are nodes in the graph and the goal of $G$ is to imitate as much as possible the ground-truth  connectivity distribution over vertices $p_{true}(v|v_c)$ and $D$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$. 

From a technical perspective, GAN-based graph representation, have been applied in different application domains of recommenders, e.g., for personalized citation recommendation (i.e., recommending research papers for citation) by using a content-based and author-based representation~\cite{DBLP:conf/ismis/ZhangYCD18}  or learning heterogeneous bibliographic network representation (HBNR)~\cite{DBLP:conf/aaai/CaiHY18}. As for GAN-HNBR, the role of GAN component is to infer the optimal representation of a bibliographic network consisting of heterogeneous vertex content features (e.g., papers, authors, manuscripts) into a common shared latent space and applying personalized recommendation on the obtained representation.

%These methods use graphs to model each feature of the article, but an adjacency graph represents only between the relationship of two features. The graph model ignores the potential relationship between features as an entirety. In this paper, heterogeneous information network is suggested to represent the relationship between characteristics of articles, which retains the structure of the real-world article network

% \input{Tables/gan_basic.tex}

\begin{table}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|l|l|}
\hline
GAN name &Year &\multicolumn{9}{c|}{Generator Model} & \multicolumn{8}{c|}{Discriminator Model} & \multicolumn{3}{l|}{Rec Goal} \\ \hline
& & \multicolumn{3}{c|}{Linear} & \multicolumn{6}{c|}{Non-Linear} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \rotatebox{90}{CF util } & \rotatebox{90}{div} & \rotatebox{90}{CA} \\ \hline
& & \rotatebox{90}{MF} &  &  & \rotatebox{90}{MLP} & \rotatebox{90}{CNN} & \rotatebox{90}{AE} & \rotatebox{90}{VAE} & \multicolumn{2}{c|}{RNN} &  &  &  &  &  &  &  &  &  &  &  \\ \hline
& &  &  &  &  &  &  &  & \rotatebox{90}{LSTM} & \rotatebox{90}{GRU} &  &  &  &  &  &  &  &  &  &  &  \\ \hline
IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} &2017 & \cmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &\cmark   &  &  \\ \hline
GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18} &2018 & \cmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &\cmark   &  &  \\ \hline
CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18} &2018 & \cmark &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &\cmark   &  &  \\ \hline
\end{tabular}
\end{table}


% \yashar{ XXX I AM HERE REVISING XXX}

Various other GAN-based CF models have been proposed following the works by IRGAN and GraphGAN. 
% \yashar{Here we can add some overall information LATER: often these proposal are different based on the fact if}

In~\cite{DBLP:conf/cikm/ChaeKKL18} the authors propose CFGAN which improves one of weakness in IRGAN, as claimed by authors. The main problem in IRGAN is that the generator produces each time a single item index \yashar{Felice is it single item index or item indices?} that is discrete in nature. This is different from original GAN framework by authors, in which the output of $G$ is an image (i.e., a vector). The generation of discrete item indices by $G$ can lead to poor sampling of items from the pool of available alternatives (i.e., samples exactly identical to ground-truth) resulting in deterioration of the performance of $G$ and $D$ (instated of improvement) over time after the min-max game is performed between them. By introducing vector-wise adversarial learning and testing it quantitatively over a series of experiments/datasets, the authors show the improvement of CFGAN over IRGAN and GraphGAN baselines. As an example, for P@20 and the Ciao dataset this improvement is approximately $100\%$ for with respect to IRGAN (0.45 v.s. 0.23) and $160\%$ for compared with GraphGAN (0.45 v.s. 0.17), which seems to be significantly on the high side.
% \yashar{XXX I AM HERE REVISING XXX}

% \felice{XXXXX Look at this comparison of IRGAN/GraphGAN (idea from pag2 of~\cite{DBLP:journals/corr/abs-1909-03529}):\\ IRGAN and GraphGAN address the  differentiation problem on discrete data by utilizing Policy Gradient (REINFORCE). In~\cite{DBLP:conf/icml/RezendeMW14} authors evidence that with a huge set of items (e.g., millions) the variance of the estimated gradients explodes and, because of the gradient strategy suffers from large variance, the adversarial learning becomes unstable.
% A solution at this issue is based on Gumbel-Softmax function~\cite{DBLP:conf/iclr/JangGP17, DBLP:conf/iclr/MaddisonMT17}, which estimates a multinomial distribution like a continuous distribution thanks to a reparametrization with a continuous and differentiable softmax function. Then, its is possible to perform gradient descent.}

In~\cite{8525831} the authors propose an auto-encoder-based GAN. The authors identify a problem in conventional MF-based approach which is linear and difficult to capture the non-linear, subtle latent factors
underlying user-item interactions. The proposed approach an auto-encoder takes the role of $G$ to model the underlying distribution of user preference over items.  \yashar{shouldn't we add one sentence about auto-encoder, why it can be powerful?}

In~\cite{8663730}  the authors propose an adversarial variational auto-encoder, which uses GAN to regularize variational autoencoder by imposing an arbitrary prior on the latent representation (uses implicit feedback). A similar work can be found in ~\cite{DBLP:conf/icde/TongLZSC19, DBLP:conf/cikm/LeeSM17} which a VAE to enhance the robustness of adversarial examples. The author furthermore present the Wasserstein Distance with gradient penalty.

In~\cite{DBLP:conf/flairs/CostaD19} the authors propose an approach to address other issues of IRGAN, sparsity causing gradient vanishing and update instability and discrete value preventing ad training to optimize using gradient descent. The proposed solution is named convolutional adversarial latent factor model (CALF) which employ a CNN to learn correlations between embeddings and Rao-Blackwell sampling to deal with discrete values optimizing CALF. 


In~\cite{DBLP:conf/ijcai/WuLMZZG19} the authors propose a solution to improve diversity of CF-based recommendation with GAN based on personalized diversification. We would review this paper in section xxx. 

% ~\felice{New Papers ADDED on CF - 22 October 2019}

In~\cite{DBLP:conf/ijcnn/WangZC019} the authors propose to improve the recommendation performance in a pairwise scenario by proposing lambda rank~\cite{DBLP:conf/cikm/YuanGJCYZ16} function into the adversarial learning of the proposed GAN-based CF framework.

In~\cite{DBLP:conf/ijcai/YuZCX19} the authors propose a variant of Variational Autoencoder to address the limited expressiveness of the inference model and latent features which reduces the generalization performance of the model. The proposed solution, named Adversarial Variational Autoencoders (VAEGAN), is a more expressive, and flexible, model that better approximate the posterior distribution by combining VAEs and GANs. They are the first to propose the application of Adversarial Variational Bayes (AVB)~\cite{DBLP:conf/icml/MeschederNG17} to compute the the adversarial training. 

\noindent{\textit{Non-GAN based AdL Training:}}

\subsection{Improve Beyong-Accuracy Aspect}

% \yashar{Newly added}
The success of recommendation algorithms is commonly measured by how well they are capable of making predictions of high-relevance items to a target user, i.e., items that users will likely click, buy or listen. The earliest research on MRS were focused on promoting this perspective through improving \textit{recommendation accuracy}. However, too much personalization, i.e., excessive pandering to user's existing musical taste can harm the development of curiosity and personal growth in users. The extreme case of this aesthetic concern is described as the \dquotes{filter bubble} effect, which refers to the scenario where as the result of excessive personalization of content geared toward users' individual preference, personalization services (web SE and RS) reduce diversity of the information presented and lead to partial information blindness (i.e., filter bubbles). 

\subsection{Categorization based on the domain}\label{sec:domain_catag}

\subsection{Technical categorization}\label{sec:technical_catag}

\input{Tables/CategoryChallangeDomainBase.tex}
\input{Plots/OpenChallenges.tex}     
\input{Plots/Domain.tex}  
\input{Tables/Recommender_Models.tex}





\begin{comment}

\subsubsection{Attack on RS}

\yd{As stated before, attacks on RS models follow the same categorization provided in xxx, based on data poisoning attacks and evasion attacks. }

\yd{Data poisoning attacks in RS are performed via shilling profile injection that aim to target the performance of rating-based CF in matrix completion task. Given a URM $M$ with $n$ real users and $m$ items, the goal is to augment a fraction of malicious users $\lfloor{\alpha n} \rfloor$ to $M$ ($\alpha << 1$) in which each malicious user profile can contain ratings to a maximum number of $C$ items. The ultimate goal is to harvest recommendation outcomes toward a illegitimate benefit, e.g., pushing some targeted items into the top-$K$ list of users for market penetration. Shilling attacks against RS have a established literature and their development face two main milestones: first, since the early of 2000s, where the focus of literature was focused on building hand-crafted fake profiles whose rating assignment follow different strategy according to random, popular, love-hate, bandwagon attacks among others~\cite{DBLP:journals/air/GunesKBP14}; the second research direction started in 2016 when the first ML-optimized attack was proposed by Li et al.~\cite{DBLP:conf/nips/LiWSV16} on factorization-based RS. This  work reviews a novel type of data poisoning attack that applies the adversarial learning paradigm for generate poisoning input data. We present the framework for robust adversarial recommendation in section~\ref{subsec:adv_techn} for a deeper understanding on the concept.} 


\yashar{I will rephrase the following a bit but the content is good enough.}
Data poisoning attacks in RS follow two main research directions. In the early of 2000s, hand-engineered attacks, named also \textit{shilling attacks}, have been deeply analyzed~\cite{DBLP:journals/air/GunesKBP14}, and are based on a real creation and insertion of fake users in a recommender system who start to add rating following different attack strategies (i.e., random, popular, bandwagon attacks [XXX]). The second research direction started in the second half of the 10s when the first ML optimized attack was proposed by Li et al.~\cite{DBLP:conf/nips/LiWSV16} on factorization-based RS. The current work review a novel type of data poisoning attacks that applies the adversarial learning paradigm for generate poisoning input data. In the below section~\ref{subsubsec:adv_learning}, we present the foundation of adversarial learning to prepare the reader to a full understanding of its application in recommendation tasks. \yashar{till here, end of rephrase}

\yashar{I will rephrase the following a bit but the content is good enough.}
Starting from this first foundation it is already important to underline that in the case of AML in RS the attacker can not apply pure \textit{evasion attacks} because of recommender models do not work as a classical classifier. Indeed, a huge amount of work on the security of recommender systems relate to data poisoning attacks where an adversary may modify inputs of a recommendation system to degrade its performances.} 

A variety of principal AML attack methods have been recently reviewed by Akhtar et al. in~\cite{akhtar2018threat}: L-BFGS~\cite{DBLP:journals/corr/SzegedyZSBEGF13} that firstly formalized adversarial example generation under a minimization framework, fast gradient sign method~\cite{DBLP:journals/corr/GoodfellowSS14} that generates adversarial perturbations in the direction of loss function gradients, Jacobian based method~\cite{DBLP:conf/eurosp/PapernotMJFCS16} that estimates the output's variability to the variation of input feature dimensions and modifies the most impactful features until it alters the classification; and C\&W attack~\cite{DBLP:conf/sp/Carlini017} that solves an optimization problem to find malicious perturbed images. These methods represent the state-of-the-art of adversarial attacks in deep learning and a huge amount of works have been published in computer vision domain. Since the already claimed problem setting of recommender system on the fact that users and items are mostly discrete inputs, the literature review in RS has shown a prominent use of a modified version of FGSM in the case of recommendation task. Section~\ref{subsec:adv_techn} focuses on describing a general adversarial threat model in recommendation settings. \yashar{till here, end of rephrase}



\subsubsection{Defense Mechanism.}\label{subsubsec:defence_strategies}


Latest advancements in defence strategies prove that several state-of-the-art machine learning algorithms can be broken easily in shocking ways. Difference countermeasures for adversarial examples follow two types
of defence \textit{reactive} and \textit{proactive} strategies~\cite{DBLP:journals/tnn/YuanHZL19}. While the first strategy recognises adversarial examples after the training of an ML model, the second one makes the model more robust to adversarial examples before their generation. Reactive countermeasures are not present in recommender system domain, while proactive approaches have been successfully explored starting from the work by Xiangnan He et al.~\cite{DBLP:conf/sigir/0001HDC18} in 2018, that, for the first time, applied \textbf{adversarial training} to make BPR-MF more robust to adversarial examples. 

Adversarial training, also known as adversarial regularization, is the training procedure that includes generated adversarial into the training data in order to make use of them during the training of the model. Goodfellow et al.~\cite{DBLP:journals/corr/GoodfellowSS14} showed that adversarial training improves the robustness of DNN~\cite{DBLP:conf/iclr/TramerKPGBM18, DBLP:conf/aaai/Sankaranarayanan18} as well as might provide its regularization and improve the accuracy performance~\cite{DBLP:conf/emnlp/WuBR17}. 
The central idea is to enhance model's robustness such that the adversarial noise has a smaller impact on the model's prediction by ensuring that the model to preserve the same recommendation quality for true inputs as well as perturbed ones. All mentioned publications demonstrate the effectiveness of this defense mechanism with a consistent improvement of performances when the model is adversarially-trained or not.
Section~\ref{subsec:adv_techn} provides a comprehensive formulation and description of adversarial training in recommendation scenario.

The application of other proactive defence mechanisms like the \textit{defensive distillation}~\cite{DBLP:conf/sp/PapernotM0JS16}. Defensive distillation is an effective training for obtaining robust collaborative filtering models based on defensive distillation has been proposed in~\cite{DBLP:journals/tmm/DuFYXCT19} inspired by ~\cite{DBLP:journals/corr/HintonVD15, DBLP:conf/cvpr/GongTLMFFY15}. It is also interesting to observe that the same approach has been also proposed by Papernot et al.~\cite{DBLP:journals/corr/PapernotM17, DBLP:conf/sp/PapernotM0JS16}  as a defensive mechanism against adversarial examples crafting methods in computer vision domain.

\subsection{Optimization Framework for Robust Adversarial Recommendation}\label{subsec:adv_techn}
Here we introduce an high level framework to summarize the application of Adversarial Learning in the security of recommendation tasks.

%\subsubsection{Adversarial Recommendation Framework (Adv-RF)}
One of the successful application of AML for attack/ defence scenarios in RS is to perturb users and items input embeddings in and through an adversarial attack method.
Motivated by the evaluation protocol and experimental framework introduced by Xiangang He et al.~\cite{DBLP:conf/sigir/0001HDC18}, we propose the following adversarial framework to address the attack/ defence security issues to evaluate the robustness performance under adversarial settings.  



Let $L({\Delta})$ the objective function (to be minimized) of a recommender model where $\Theta$ are the model parameters (e.g., the users and items embedding of MF), where we consider non-linear recommender models~\felice{We should define better the fact of non-linearity because it makes the optimization problem intractable }.

The first step is to define the verify the effectiveness of adversarial perturbation on embedding with respect to random perturbations. The generation of adversarial perturbations $\Delta_{adv}$ differs form the classical adversarial learning perturbation in Equation~\ref{eq:eq_minim} (i.e., the goal is to fail the classifier) aims to maximize the recommender model objective function $L({\Omega})$:

\begin{equation}
    \small
    \label{eq:adv_perturbation}
    \Delta_{adv}=\arg \max _{\Delta, \| \Delta| | \leq \epsilon} \mathcal{L}(X|\Omega+\Delta)
\end{equation}
where $\epsilon$ controls the magnitude of adversarial perturbations, $|| \cdot ||$ denotes the $L_{2}$ norm, $\Omega$ is the fixed set of the current model parameters, and $X$ denotes the set of training instances.

The optimization problem in Eq.~\ref{eq:adv_perturbation} to get the $\Delta$ is an intractable problem. To the extent of our knowledge, the FGSM is the first method for generating adversarial examples which has been used in the recommender system domain among the state-of-the-art approaches presented in Section~\ref{subsubsec:adv_learning}.

The common solution of is the linearization of the problem in Eq.~\ref{eq:adv_perturbation} round $\Delta$. The adversarial perturbation is the obtained as:
\begin{equation}
    \small
    \label{eq:fgsm_adv_perturbations}
    \Delta_{adv}=\epsilon \frac{\Pi}{\|\Pi\|} \quad \text { where } \quad \Pi=\frac{\partial \mathcal{L}(X|\Omega+\Delta)}{\partial \Delta}
\end{equation}

If the experimental results of the proposed attack on the recommender model demonstrate that adversarial perturbations have a huge impact on the recommendation performance (see Section XXX for the evaluation protocol), then it is necessary to enhance the robustness of the model. To address this task \textbf{adversarial (re)training} has been widely used in recommendation scenario between the state-of-the-art defense strategies present in the AML literature and briefly introduced in Section~\ref{subsubsec:defence_strategies}.

The \textbf{adversarial (re)training} strategy, also known as \textbf{adversarial regularization}, consists in generating adversarial examples and inject them into the training dataset during the training stage. The training strategy to make robust a recommender system under adversarial perturbations is formulated as a minimax game between an adversary, who tries to generate the best adversarial perturbation to alter recommendation performance, and a defender, who tries to protect the recommendation performance. This minimax game pattern is at the core of the defence strategies for recommender models, and it is the core of the training of adversarial deep generative models reviewed in Section~\ref{sec:GAN}. Formally, the error function of the adversarial framework for RS is defined as follow:
\begin{equation}
    \label{eq:j_apr}
    \small
    L_{AML-RS}(X | \Omega) = \mathcal{L}(X | \Omega)+\lambda \mathcal{L}(X | \Omega+\Delta_{adv})
\end{equation}
where $\mathcal{L}(X|\Omega+\Delta)$ works as a adversarial regularization component to enhance the robustness of the model. 

The adversarial (re)training is formalized as:
\begin{equation}
    \small
    \label{eq:minmax_apr}
    \arg \min _{\Omega} \max _{\Delta,| | \Delta| | \leq \epsilon} \mathcal{L}(X | \Omega)+\lambda \mathcal{L}(X|\Omega+\Delta)
\end{equation}
where the minimax game is formally represented by the fact that the model parameters ($\Omega$) learning acts as to minimize the error function, while the generation of adversarial perturbations ($\Delta$) acts to maximize it.

\subsection{Applications}\label{subsec:alb_recc}


Xiangnan He et al.~\cite{DBLP:conf/sigir/0001HDC18} are the first to propose adversarial learning framework for recommendation. The proposed model, called \textit{Adversarial Personalized Ranking (APR)}, examines the robustness of BPR-MF with respect to adversarial perturbation on users and items embedding of a BPR-MF~\cite{DBLP:conf/uai/RendleFGS09}. The authors firstly verify the success of using the \textbf{adversarial (re)training} as a defence against adversarial perturbations and demonstrate the competitive results in applying adversarial training on BPR-MF.

Tang et al.~\cite{8618394} put under adversarial framework another BPR model, VBPR. They proposed to use adversarial training to enhance the robustness of VBPR under adversarial perturbations on the deep latent feature of items' images extracted by DNN (e.g., ResNet50~\cite{DBLP:conf/cvpr/HeZRS16}).The proposed system,  Adversarial Multimedia Recommendation (AMR), does not train the recommender model and the feature extractor in and end-to-end way because of overfitting issues in training the DNN and the recommender model simultaneously leaving the proposal of an end-to-end solution as an open challenges.

Yuan, F. et al.~\cite{DBLP:conf/sigir/YuanYB19, DBLP:conf/ijcnn/YuanYB19} use the adversarial training framework for neural network-based recommendation models. Expressly, they verified the enhancement in robustness after applying the minimax optimization algorithm not only on the users' embeddings of a collaborative denoising auto-encoder (CDAE)~\cite{DBLP:conf/wsdm/WuDZE16} but also on the hidden layers of the autoencoder after they gave proof of evidence on the negligible influence of adversarial perturbations on the overall performance.

Chen and Li~\cite{DBLP:conf/recsys/ChenL19} combine tensor factorization and adversarial learning to improve the robustness of pairwise interaction tensor factorization (PITF)~\cite{DBLP:conf/wsdm/RendleS10} in context-aware recommendation. Comparison with standard tensor models in tag recommendations demonstrates that also the adversarial framework outperforms state-of-the-art tensor-based recommenders.

Park et al.~\cite{DBLP:conf/www/ParkC19} address the vulnerability of MF to adversarial examples by perturbing directly the input of the recommender model.The proposed generation approach works for both discrete and continuous input by adding the adversarial perturbation directly on the input vector (e.g., one-hot encoding user-id, or the frequency of bough items) and then multiplying it by the embedding matrix. Then, the authors proposed to improve adversarial training with an adversarial sampling strategy by generating virtual adversarial example~\cite{DBLP:journals/pami/MiyatoMKI19} (i.e., the process for generating adversarial examples without labels). 

Du et al.~\cite{DBLP:journals/tmm/DuFYXCT19} approach security issues for \textbf{C\&W  attacks}~\cite{DBLP:conf/sp/Carlini017}, one of the most effective attack methods where adversaries have the full knowledge of the target model (i.e., white-box settings). The authors proposed to make more robust neural network-based collaborative filtering models (e.g., NCF~\cite{DBLP:conf/www/HeLZNHC17}) by using \textbf{knowledge distillation}~\cite{DBLP:journals/corr/HintonVD15} instead of the adversarial (re)training. 
The framework integrates the knowledge distillation-from a teacher network to a student one- with the injection of additive adversarial noise at training time. Experiments demonstrated that this system enhance the robustness of the treated recommender model.

Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} propose a novel recommender model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), to provide query suggestions considering the sequential search queries issued by the user and and his the history of clicks.
The authors employ additional adversarial (re)training epochs (i.e., adding adversarial perturbations on item embeddings) to improve the robustness of the model. 
\begin{itemize}
    \item Adversarial Mahalanobis Distance-based Attentive Song Recommender for Automatic Playlist Continuation. (SIGIR2019),
    \item Domain adaptation in display advertising: an application for partner cold-start.
\end{itemize}

\end{comment}


==> OLD_FILES/OLD_Sec3_Categorization_old.tex <==
\section{Categorization of Adversarial-based Recommender System}
This section will provide a qualitative-oriented overview of adversarial-based publications.
The first section focuses on the categorization of publications based on the adversarial tasks introduced in Section~\ref{sec:AdversarialTasks}. The next one is an analysis of works to obtain a better understanding respect to open challenges. Finally, we present a categorizations base on Domains. All these categorizations are based on Table~\ref{tab:CatTaskChalDom}.

\input{Tables/CategoryChallangeDomainBase.tex}


\subsection{Categorization based on Adversarial-Goal}\label{subsec:CategorizationbasedonAdversarialGoal}


    We recognized three primary objectives in the academic literature that can be accomplished with the use of adversarial machine learning techniques in various application scenarios:
    \begin{enumerate}[label={(\arabic*)}]
        \item \textbf{Adversarial Attack} 
        \item \textbf{Defense Mechanism} 
        \item \textbf{Improve Recommendation}
    \end{enumerate}
    We will discuss these three main goals in detail in the next. 

    \subsubsection{Adversarial Attacks}\label{subsubsec:AdversarialAttacks}
    The core idea of adversarial machine learning is to add small adversarial perturbation on dataset input, e.g. images, to fool a classifier~\cite{DBLP:journals/corr/SzegedyZSBEGF13}. The creation of adversarial examples gains a lot of attention in computer vision and malware detection domain since the birth of AML \textit{[We can cite adv paper here]} with surprisingly advances in few years. 
    
    Attacking a classifier is a common malicious application of AML in the computer vision domain. This goal is not directly applicable to recommendation domain since recommender systems are generally used for finding some\textbackslash{all} good items~\cite{DBLP:reference/sp/2015rsh} for the user.
    Looking to the main goal of a RS, an adversary may attack it to affect its recommendation behavior with different goals. A yet explored goal in the literature is to inject fake user profiles into CF-RS in order to push/nuke a segment of products to yield poor recommendations for his competitors~\textquotesingle items (nuke) while attempting to secure positive recommendations for his own (push), or to reduce the trust to the system, e.g. e-commerce site. 
    Gunes \textit{et al.}~\cite{DBLP:journals/air/GunesKBP14} and Burke \textit{et al.}~\cite{DBLP:reference/sp/BurkeOH15} surveyed about shilling attacks in collaborative filtering algorithms by giving a comprehensive overview about shilling attack types, detection schemes and robust algorithms.
    This malicious behaviour of an adversary is not under the analysis of this survey because it does not use AML techniques.
    % ~\felice{@yashar: We should have a section before this on where we explain in brief the Adversarial Attack techniques [FGSM, JSFM, C\&W]} \yashar{Preferably try to describe these models with less requirements to know these techniques. Maybe we could mention in simple words the common characteristics of them. Then you can cite future sections using command (cf. Sec~\ref{xxx}) for detailed discussion.}
    
    This section is referred to the set of adversarial attacks where adversaries exploit the system's sensitivity to adversarial gradients to produce adversarial noise capable to lead to fail the recommender model. The state-of-the-art generation of adversarial examples from the computer vision domain is infeasible in recommendation domain, since recommender models have discrete inputs data, e.g. the user-item matrix, to make recommendations. In fact, the application of adversarial noise on discrete features may destroy the semantic of data has shown in ~\cite{DBLP:conf/sigir/0001HDC18}.
    
    Starting from these limitations, typical applications of AML attacks in the literature include the generation of adversarial noise as model parameter perturbations~\cite{DBLP:conf/sigir/0001HDC18, advcol19sigir, DBLP:journals/corr/abs-1809-07062} 
    % by exploiting the Fast-Gradient Method proposed int Goodfellow et al.~\cite{DBLP:journals/corr/GoodfellowSS14}
    , the crafting of adversarial fake user profiles in a GAN-based framework~\cite{DBLP:journals/corr/abs-1809-08336}
    and the generation of adversarial example using the state-of-the-art adversarial attack~\cite{DBLP:journals/tmm/DuFYXCT19}.
    % C\&W attacks~\cite{DBLP:conf/sp/Carlini017} by.
    
    % \felice{@Yashar: Shall we discuss more here? I can write a little bit more on the last internal categorization of attacks' without giving information on techniques but by concerning the goal of each paper} \yashar{For the first version, it seems good. I would suggest to move on next sections, in the second review we can work on improving the quality. Let's try to compile all the papers here first, it is a very good progress if we can review briefly the papers from the goal perspective.}
    
    \subsubsection{Defense Mechanism}\label{subsubsec:DefenseMechanism}
    
    The defense against adversarial perturbations in a recommender model is another potential goal that can be accomplished by adversarial-based recommender model to improve its robustness. Robustness is the stability of the recommendation in the presence of fake information, typically inserted on purposes to influence the recommendation\cite{DBLP:reference/sp/BurkeOH15}. Previously explored publications on adversarial attacks  on recommendations demonstrate the effectiveness of adversarial malicious purposes on recommender models, which can be sabotaged with a marked worsening of their accuracy performances. \\
    A substantial amount of research in AML provides some practical defense mechanisms used to block these adversarial attacks which are used in recommendation scenarios.
    
    Then, publications on adversarial attacks propose also defense strategies. We can distinguish between two types of applied defense mechanism that comes directly from AML literature: Adversarial Training and Distillation Network.
    \begin{itemize}
        \item \textit{Adversarial Training.} 
            Towards the goal of learning more robust models to adversarial perturbations on model parameters \cite{DBLP:conf/sigir/0001HDC18, DBLP:journals/corr/abs-1808-05361, advcol19sigir, DBLP:conf/www/ParkC19, DBLP:journals/corr/abs-1809-07062} propose to perform an adversarial training by learning with a modified objective function that takes into account adversarial perturbations. The central idea is to enhance model's robustness such that the adversarial noise has a smaller impact on the model's prediction by ensuring that the model to preserve the same recommendation quality for true inputs as well as perturbed ones. All mentioned publications demonstrate the effectiveness of this defense mechanism with a consistent improvement of performances when the model is adversarially-trained or not. \\
            \textit{Limitations.}
            It is important to note that all these works point to apply adversarial noise on the model parameters and not directly on the input. \cite{DBLP:journals/corr/abs-1809-07062} sustains that the intuitive solution is to apply perturbations directly to model inputs but it does not implement this solution for a tricky training of the recommender system (Input Feature Extractor + Recommender Model). Furthermore, Xiangnan \textit{et al.}~\cite{DBLP:conf/sigir/0001HDC18} claim that to add noises in the input layer is irrational because it will change the semantics of the input.
        \item \textit{Defensive Distillation}
            An effective training for obtaining robust collaborative filtering models based on defensive distillation has been proposed in~\cite{DBLP:journals/tmm/DuFYXCT19} inspired by ~\cite{DBLP:journals/corr/HintonVD15, DBLP:conf/cvpr/GongTLMFFY15}. It is also interesting to observe that the same approach has been also proposed by Papernot et al.~\cite{DBLP:journals/corr/PapernotM17, DBLP:conf/sp/PapernotM0JS16}  as a defensive mechanism against adversarial examples crafting methods in computer vision domain. 
        % \item \textit{Others}
        %     Adversarial Machine Learning: The Case of Recommendation Systems~\cite{DBLP:conf/spawc/TruongKE18}. ~\felice{@Yashar: I think that this paper is not so simple to classify under recommender system scenario what do you think?}
    \end{itemize}
    
    \subsubsection{Improve Recommendation Tasks}\label{subsubsec:ImproveRecommendation}
    
    \yashar{XXX I AM FOCUSED HERE AND DOING A DEEP REVIEW - LOCKED - All the commented sections are still there, will return them back. XXX}

\begin{enumerate}

        \item \textit{Personalization and long-term preference modelling}: Personalization lies at the heart of user-centered experience in modern Web applications. Catering a personalized recommendation service relies on accurate modeling of users' interests and needs. \textit{Long-term user preference modelling} is concerned with what the user will do over a long time horizon and serves as the basis for personalized recommendation services ... \\ \yashar{will connect to AdL after reading the papers} \\

        
        \item \textit{Context-awareness}: Although long-term preference modelling has proven to be effective in several domains~\cite{DBLP:conf/kdd/BerkovskyF15}, recent research indicates that user preference are highly variable based on user's context, e.g., time, location and mood~\cite{DBLP:conf/recsys/KompanKB17}. Context provides background of \textit{user objective} for using the system and together with long-term user preferences can be used to generate more relevant recommendations ... \\ \yashar{will connect to AdL after reading the papers} \\
        
        \item \textit{Short-term preference modelling and sequences.} 
        In real applications, user preference over items and items state per se change over time and modeling the \textit{temporal evolution} of the former two aspects is needed for effective recommendation. While long-term preferences of users change slowly,  \textit{short-term preference} of users can be seen more dynamic and changing more rapidly. Predicting short-term user preference has been recently studied in the context of \textit{session-based} and \textit{sequential recommendations} ...
        \yashar{will connect to AdL after reading the papers} \\
        
         \item \textit{Cross-domain or multi-domain recommendation}: Majority of recommendation approaches are designed to compute recommendations for items belonging to a single domain, for example in media streaming platforms, Netflix recommends movies/TV series to its consumers while Lasts.Fm offers song and music-album recommendations. Items belonging to a certain domain share characteristics and attributes, which are intrinsically similar. Development of \textit{domain-specific} recommendation models allow to study these characteristics separately.
         
         However, single-domain recommendation can face numerous challenges. The first refers to the well-known cold-start problem, which happens when insufficient interactions or preference scores exist in the considered domain. The second relies on the fact users' interests and needs span across different application areas and large e-commerce sites like Amazon or Ebay store users' preference scores related to products/services of various domains - from books and products to online movies and music. As companies strive to increase the diversity of products or services to users, cross-domain recommendation can help such companies to increase sale productivity by offering personalized cross-selling or bundle recommendations for items from multiple domains~\cite{cantador2015cross}. The third related aspect relates to the idea of discovering relationships for images related to different domains. For example, can machine achieve a human-level understanding to choose a suit jacket with pants or shoes in the same style to wear? The central problem here is to find a mapping function from one domain to another domain~\cite{DBLP:journals/corr/abs-1812-06229}. Recently, the generative power of GANs has been used to tackle this problem as a conditional image generation problem, i.e., to generate an image in one domain given another image in the other domain~\cite{DBLP:conf/cvpr/IsolaZZE17}. In the following we review different research works applying GAN- and AdL-based approaches to various cross-domain recommendations tasks: 
         
         In~\cite{DBLP:conf/bigcomp/JoJCJ19}, the authors propose a cross-domain GAN \textbf{to generate fashion designs from the sceneries}. In the proposed hypothetical scenario, the user can specify via a query her interest POI to visit (e.g., mountain, beach, etc.) together with keywords describing a season (i.e., spring, summer, fall, and winter). The core idea is to automatically generate fashion items (e.g., clothes, handbags, and shoes) whose affective features (i.e., style) match the the natural scenery specified by the user. For instance, the system can recommend a collection of fashion items that look cool/bright for visiting a beach in summer even though the true preference of user is black-style clothes. The role of GAN is to learn association between scenery and fashion images. In the field of ML and CV, the problem is terms as \dquotes{style transfer} or \dquotes{image to image translation} problem~\cite{DBLP:conf/cvpr/GatysEB16}. \yashar{stable}
         
        
         An effective cross-domain recommendation system relies on \textit{capturing both similarities and difference among features of domains} and leveraging them for improving recommendation quality in multiple domains. Single-domain algorithms have difficulty in uncovering the specific characteristics of each domain. To solve this problem some approaches extract latent features of the domains by a separate network~\cite{DBLP:conf/www/LianZXS17,DBLP:journals/tmm/MinBXH15}. Although these approaches might be successful in capturing characteristic features of each domain, they do not establish the similarity between features of multiple domains. With the goal \textbf{to extract both homogeneous and divergent features in multiple domains}, in~\cite{DBLP:journals/corr/abs-1812-06229} the authors propose generic cross domain recommendation system. The system takes the user interaction history (click vector) in each domain as input, maps each vector to shared latent space via the help of two autoencoders (AE) and then uses a generator to remap the latent representation to click vectors. The main novelty of this work lies on building/linking shared latent space between domains, which in turn facilitates \textit{domain-to-domain} translation. In particular, the former is realized by enforcing a weight-sharing constraint related to variational auto-encoders, i.e., the encoder-generator pair $\{E_A, G_A\}$ and $\{E_B, G_B\}$\footnote{The wights sharing is done on the last few years of encoders $\{E_A, E_B\}$ and first few layers generators $\{G_A, G_B\}$ which are in charge of encoding and decoding high-level representations of the input click vectors.} and using cycle-consistency (CC) as a weight-sharing constraint. Finally two separate adversarial discriminators are employed to determine whether the translated vectors are realistic. The final system is called VAE-GAN-CC network. It is mentioned that the proposed system extends the unsupervised Image-to-Image Translation Network (UNIT) \cite{DBLP:conf/nips/LiuBK17} for RS and is thus named Domain-to-Domain Translation Model (D2D-TM). \yashar{stable}
         
         An possible solution for cross-domain recommendation is to rely on \textit{domain linkage} based on \textit{user-} and \textit{item-overlap}. Four types of relationships are identified in SoA literature in cross-domain recommendation~\cite{DBLP:conf/icdm/CremonesiTT11}: i) no overlap, ii) user-overlap, iii) item-over lap and (iv) user and item overlap. CF models can function in all these cases, except the first case. Therefore, existence of -overlap- is the key enabler to obtain an effective recommendations with a classic CF strategy. However, in many real applications a limited overall between domain may exist, hindering CF functioning. As such approaches have been proposed to deal with  the  \textit{domain overlap  issue} in  a  more  flexible  way such as by approaches that build/measure \dquotes{characteristics}  that  are  shared  by  the  user/item  profiles in  the different  domains (often via a latent representation). Although effective, in face of heterogeneity of domains,  number of shared characteristic between domain can be small~\cite{fernandezcross}.  
         
         To address the above issues or generally, in~\cite{DBLP:journals/corr/abs-1903-10794} the author propose an approach to solve the challenging issues in cross-domain recommendation - the problem of data sparsity and imbalancedness via \textit{integration of transfer learning with adversarial learning}. Transfer learning is a ML task \yashar{citation}, whose goal is to transfer knowledge learned in a source domain and use it to improve the learning in the target domain and has been mentioned applied to solve cross-domain problem~\cite{fernandezcross}.  
         
         
         \yashar{I am here REVISING}

         
%It learns to adapt the user, item and user-item interaction representations from a source domain to a target domain in an unsupervised and adversarial fashion. Multiple generators and discriminators are designed to adver- sarially learn target generators for generating domain-invariant representations. Four RecSys-DAN instances, namely, UI- DAN, U-DAN, I-DAN, and H-DAN, are explored by con- sidering different scenarios characterized by the overlap of users and items in both unimodal and multimodal settings.
         

         
         
     %in practice due  to  the heterogeneity of domains, 
         
         %Nonetheless,assuming  a  memory-based  approach  to  CF,when  the  overlap  is  small,  user  and  item  similarities,  and  consequently  generated recommendations,  may  tend  to  be  inaccurate.  To  address  the  above  mentioned  no-overlap  situation,  we  have  to  develop  approaches  that  find  or  build  some  type  of explicit/implicit  relations  between  domains,  which  would  be  used  as  semantic  bridges connecting different domains in a recommender system
     
         
         %However, this methods suffers from the problem that
         

         
        %  \begin{figure}
        %      \centering
        %      \includegraphics[width=0.95 \linewidth]{Pictures/RecSys_DAN.png}
        %      \caption{Caption}
        %      \label{fig:catag_challenge}
        %  \end{figure}
         
         %issue with cross domain recommendation is cross-domain imbalancedness, meaning the number of users, items or interactions in source and target domain are imbalanced. 
         
         
         

          
         %is proposed to extract both homogeneous and divergent features among domain. \yashar{...} 
  
         
         %Conventional cross-domain models use the source domain as an external knowledge source to transfer knowledge from a source to the target domain. The source domain can be information from social networks or a search query \yashar{It is strange that they consider query as a domain}. However, this information also might be impossible to obtain n some application scenarios. 
         
         
         
         
         %solve the cold-start problem via a translation-based approach. In~\cite{DBLP:conf/webi/YiHQ18}, the works learns the transferable latent representations of users, items and user-item pairs across different product domains. (key concept transfer learning particularly domain adaptation). In  ~\cite{DBLP:conf/www/PereraZ19} the system generates user preferences for non-overlapped users. In ~\cite{DBLP:journals/corr/abs-1905-13160}proposed for social recommendation, transfers users' information between social domain and item domain using adversarial learning. 
        \item \textit{Diversity and Novelty}: The success of different recommendation models is commonly measured by how well they are capable of making predictions of high-relevance items to a target user, i.e., items that users will likely click, like or consume. For this reason, the earliest research on RS were focused on improving \textit{recommendation accuracy}. However, too much pandering to user's taste can hinder the development of curiosity and personal growth in users. The extreme case of this aesthetic concern is described as the \dquotes{filter bubble} effect, which refers to the scenario where as the result of excessive personalization of content geared toward users' individual preference, the personalization service (web search engine or recommender) reduces the diversity of the information presented and lead to partial information blindness, i.e., the filter bubbles. 

         
         %The availability of large-scale datasets such as DeepFash-ion (Liu et al., 2016) has fueled recent progress in applyingdeep learning to fashion tasks. 
         
        
         
         
         

        % Today, companies are striving to provide a diversity of products or services to users. For example, Amazon is not only e-commerce plat- form; it is also online movie and music platform. Therefore,
         
         %and large large e-commerce sites like Amazon and eBay consumers can have multiple feedbacks associated to different categories of products. The second refers to the idea of cross-selling or bundle recommendation when companies want to promote sale of the products. 
         
         
         
          %For example, it can not work well when a user hasno interaction in the considered domain or when companies wantto cross-sell their products.
         
         %large e-commerce sites like Amazon and eBay often store user
%feedback for items from multiple domains, and in social media users often express their tastes and interests for a variety of topics.
         
         %In reality we may want to leverage all the available user data provided in various systems and domains, in order to generate more encompassing user models and better recommendations
         %Users' interests and needs span across different application areas. RS can use this fact to improve recommendations in cold-start scenarios (where we lack information in one domain) and for cross-selling (a user in Amazon can have multiple shopping histories in Book, Health or Product domains) among others. A cross domain recommendation setting is the one which recommends users item from domain A by using his knowledge in domain B. 
         

             
             

         
         
         
         


\begin{comment}
% \begin{itemize}
%            \item To study the latent features behind \textit{static and dynamic evolution of users and items}~\cite{DBLP:conf/recsys/BharadhwajPL18}. \textbf{Proposed method RecGAN.}
%            \item Long-term v.s. session-based. While the former focuses on long-term modelling of user item interactions (changing slowly), the latter encodes the dynamic behavior of items (changing faster).  
%            \textbf{Proposed method PLASTIC. Trains generator as an agent of RL} Recommends next item to the user sequentially~\cite{DBLP:conf/ijcai/ZhaoWYGYC18}. On the same goal,~\cite{DBLP:conf/kdd/WangYHLWH18} propose a streaming recommender system based on neural memory networks using AdL. (ADL used for negative sampling)
%            \item Better negative sampling in Word2Vec scenario and thus in associated tasks Prod2Vec using for modelling user shopping activity~\cite{DBLP:conf/recsys/BharadhwajPL18} . \textbf{Proposed method GAN-Word2Vec.} In \cite{DBLP:conf/kdd/WangYHLWH18} they also used a GAN-framework for negative sampling.
%            \item playlist continuation, i.e., songs to add to a playlist~\cite{DBLP:conf/recsys/VaglianoGMS18}. Ad network is joined with an autoencoder. 
 %       \end{itemize}
\end{comment}


\end{enumerate}

%        Sub-goals: 
%        
        
    
  %  The most important goal of adversarial-based recommender system is to exploit AML techniques and properties to improve recommendation performances. This goal may be analyzed under different perspectives. In fact, Adversarial Machine Learning techniques are mostly used in a huge part of publications to improve performances in different open challenges such as item recommendations, complementary recommendations and cross-domain recommendation.
   % Moreover, we identify an important use of Adversarial techniques used to speed up efficiency and stability, in addition to a significant fraction of works on properties \textit{beyond the accuracy}, such as fairness, privacy, novelty and diversity.
   % Section~\ref{sec:TechnicalSection} will deal in the technical overview of different solutions.
    %We can identify the following categories of adversarial-based recommendation scenarios.
   % \begin{itemize}
%        \item \textit{Adversarial-learning as a Regularization Term.}
%        Adversarial learning can be used for better exploiting different content to optimize the recommender training. A typical application example could be the use of an adversarial component to generate negative examples which may fool the normal behavior of the system. The \textit{minimax game} between the adversarial component and the recommender model helps to enhance the capability of the system to capture a better representation of user preferences. 
        
 %       \item \textit{Using the Adversarial component to Generate Recommendations.}
  %      In a different scenario, the adversarial component is used like a generator of recommendation.
   %     A very meaningful example can be shown in complementary recommendation in fashion domain where the generator is used to generate complementary fashion product, e.f. given a shirt the generator will recommend a skirt. This usage is possible thanks to the ability of the adversarial component to capture the complementary data distribution at the end of the minimax game.
        
    %    \item \textit{Adversarial-learning to a Better Exploiting of Data.}
     %   Another common scenario is the use of Adversarial Learning for a better exploitation of different data-sources with the goal to use them in a single framework in order to capture better user preferences. For example, there are application scenarios where the adversarial learning is used to move users' ratings and users' review or tags in a common representation in order to make recommendations depending on more sources.
        
        % \item \textit{}
        % \item \textit{}
%    \end{itemize}


%\subsection{Categorization based on Open Challenge in Recommender Community}\label{subsection:Categorization based on Open Challenge in Recommender Community}
% \begin{comment}

%     In Section~\ref{subsec:CategorizationbasedonAdversarialGoal} we have discussed different objectives of adversarial-based recommender systems without looking the specific recommendation output. Furthermore, we consider very important to categorize all publications looking to their contribution to open challenges tasks in recommender system community.
%     We differentiate between next categories:
%     \begin{itemize}
%         \item Personalization. 
        
%         %~\felice{I can add a short definition from the Handbook} \yashar{if you want, you can do. But I can also initiate the goal and for reviewing the papers you can help.}
    
%         \item Sequences. Traditionally RS are designed to help users with the right information/product choices by learning \textit{long-term} preference models. Such recommendation 
%         Sub-goals: 
%         \begin{itemize}
%             \item To study the latent features behind \textit{static and dynamic evolution of users and items}~\cite{DBLP:conf/recsys/BharadhwajPL18}. \textbf{Proposed method RecGAN.}
%             \item Long-term v.s. session-based. While the former focuseson long-term modelling of user item interactions (changing slowly), the latter encodes the dynamic behavior of items (changing faster).  
%             \textbf{Proposed method PLASTIC. Trains generator as an agent of RL} Recommends next item to the user sequentially~\cite{DBLP:conf/ijcai/ZhaoWYGYC18}. On the same goal,~\cite{DBLP:conf/kdd/WangYHLWH18} propose a streaming recommender system based on neural memory networks using AdL. (ADL used for negative sampling)
%             \item Better negative sampling in Word2Vec scenario and thus in associated tasks Prod2Vec using for modelling user shopping activity~\cite{DBLP:conf/recsys/BharadhwajPL18} . \textbf{Proposed method GAN-Word2Vec.} In \cite{DBLP:conf/kdd/WangYHLWH18} they also used a GAN-framework for negative sampling.
%             \item playlist continuation, i.e., songs to add to a playlist~\cite{DBLP:conf/recsys/VaglianoGMS18}. Ad network is joined with an autoencoder. 
%         \end{itemize}
        
    
%         \item Context-awareness.
    
%         \item Cross-Domain Recommendation.
    
%         \item Complementary Recommendation.
        
%         \item Alleviating Cold Start
        
%         \item Improving Diversity \& Novelty
    
%         \item Improving Efficiency
%         \item Improving Privacy

    
%     \end{itemize}
%     Figure~\ref{plt:openchallenge} shows the number of research works that fall into the different categories.

% \end{comment}

% \input{Plots/OpenChallenges.tex}\label{plt:openchallenge}      
    
% Figure~\ref{plt:domain} shows in which application area succession mindful recommenders were explored. In the accompanying, we give instances of normal research works in every area.


% \subsection{Categorization based on Domain}\label{subsec:CategorizationbasedonDomain}
%     Figure~\ref{plt:domain} shows in which application domain adversarial-based recommenders have been proved. In the following, we explain a meaningful example of a publications in each domain.
%     % \input{Tables/GoalBasedCategorization.tex}
%     \input{Plots/Domain.tex}\label{plt:domain}
    
%     \qquad\textit{Media \& Entertainment} is the most examined domain with a huge amount of works on the movie domain, e.g., in ~\cite{DBLP:conf/sigir/WangYZGXWZZ17, DBLP:conf/ijcai/ZhaoWYGYC18} and ~\cite{DBLP:conf/cikm/ChaeKKL18}, where the general goal seems to be voted in improving the personalized recommendation. The consumption of M\&E content is also based on both long-term and short-term preferences. Such constraints are pursued by ~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:conf/recsys/BharadhwajPL18, DBLP:conf/kdd/WangYHLWH18}.
%     Interesting publications on the challenge of automatic playlist continuation~\cite{DBLP:conf/recsys/VaglianoGMS18, DBLP:journals/corr/abs-1906-03450} and content-based rating prediction~\cite{DBLP:conf/webi/YiHQ18} are addressed in this domain. Challenging work on long-term user behavior modelling  has been presented in ~\cite{DBLP:conf/icml/Chen0LJQS19}.

    
%     \qquad\textit{E-Products} is another mostly investigated domain of adversarial-based recommenders. A common problem settings is related on the generation of complementary recommendation in Fashion domain, e.g., ~\cite{DBLP:conf/eccv/HuynhCTA18, DBLP:journals/corr/abs-1711-02231, 2019arXiv190605596K } and~\cite{DBLP:journals/corr/abs-1711-02231} propose new frameworks.
%     E-Products websites sell generally products in different categories, e.g., Home \& Kitchen and Office Products~\cite{DBLP:journals/corr/abs-1903-10794}. In ~\cite{DBLP:journals/corr/abs-1903-10794,DBLP:journals/corr/abs-1812-06229, DBLP:conf/bigcomp/JoJCJ19}, authors mitigates the cold-start and sparsity problem by leveraging the knowledge from different domains. Other problem in the e-commerce domain is the next-basket recommendation~\cite{DBLP:journals/corr/abs-1805-08720}.
    
%     \qquad\textit{Social Computing} is a challenging application area with lots of interest from the industry, i.e., one of the most important conference in rec-sys community propose a challenge on this domain~\footnote{https://recsys.acm.org/recsys19/challenge/}. 
%     AML has been applied to predict the next location in POI recommendations~\cite{DBLP:conf/www/0002YZTZW19}, to improve image-based recommendation task in a Social Network like Pinterest~\footnote{} ~\cite{DBLP:journals/corr/abs-1809-07062}. Another problem setting is to improve recommendation by transferring preferences between different Social-network. For example,  ~\cite{DBLP:conf/www/PereraZ19,} proposes a adversarial-based solutions by generating user preferences on the Twitter source network for recommendations on the YouTube target network for not-overlapped users; and ~\cite{ DBLP:journals/corr/abs-1905-13160} works on transferring users' information from social domain to item domain.
    
%     \qquad\textit{Information-based} domain is mostly investigated in personalized citation-recommendations~\cite{DBLP:conf/aaai/CaiHY18, DBLP:conf/um/GalkeMVS18, DBLP:conf/ismis/ZhangYCD18}.
%     Other publications concern to query prediction during online search~\cite{DBLP:conf/www/LiLWZW19}, the improvement of long-tail performance in the question-info domain~\cite{DBLP:conf/cikm/KrishnanSSS18} and news-recommendations~\cite{DBLP:conf/icml/Chen0LJQS19}.
    


==> OLD_FILES/OLD_Sec4_A_GAN.tex <==
\section{ADVERSARIAL LEARNING BASED RECOMMENDATION: Technical Overview}\label{sec:TechnicalSection}

In this section, we firstly introduce the application of adversarial machine learning based recommendation models and then highlight state-of-the-art research prototypes, aiming to identify the most notable and promising advancement in recent years.~\felice{Need paraphrasing}\\
We focus on technical and architectural solution in recommender systems looking at the application of adversarial learning in a GAN-based framework and the use of adversarial learning as a regularization parameters.    

% \felice{Table Idea 1: A table where for each proposed model we can set:\\ TASK - Proposed Model - \textbf{Baseline} - \textbf{Metrics}}

% \felice{Table Idea 2: At the end of the chapter we can Put a Table with:\\ Goal - Paper Name - Dataset - Public Available - Metrics }

% \felice{Table Idea 3: Try to fix the Variable for the Formalism at create a TABLE with all the formula in a single table}



\subsection{GAN-based Solutions}
This Section focus on different application of Generative Adversarial Network in recommendation domain. As there are different uses of GAN which depend from the type of recommendation, we present different proposed framework 

\subsubsection{Collaborative Recommendation}

\qquad\textit{IRGAN}~\cite{DBLP:conf/sigir/WangYZGXWZZ17} is the pioneering work that proposes a GAN-based method in Recommender Systems. The authors address the \hltask{rating prediction} and item \hltask{recommendations} proposing a \hlmethod{minimax game} to combine the rating \textit{generative} process and the learning to rank \textit{discriminative} process.
They model the minimax game between the generative and discriminative model in a GAN-based approach, named IRGAN, looking at the conditional GAN (CGAN)~\cite{DBLP:journals/corr/MirzaO14} , as both $G$ and $D$ are user-conditioned take \textbf{user-personalization} into account.
The \textit{Generator} tries to generate relevant items by approximating the true relevance distribution over items, $p_{\text { true }}(i | u, r)$, while the \textit{Discriminator} tries to distinguish between the generated and the ground-truth relevant items.
Formally:
\begin{equation}
     \small
     \label{equation:irgan}
     J(\theta, \phi)= \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
 \end{equation}
where $\theta$ parameterized the generator $p_{\theta}(\hat{i} | u_{n}, r)$ and $\phi$-parameterized the discriminator $D_{\phi}$. The generator maps a conditioned user vector $u_{z}$, to a generated relevant item. \\
The discriminator is trained to maximize such an objective with the fixed generator $G_{\theta}$
\begin{equation}
    \label{equation:irgan_max_d}
    \phi^{*}=\arg \max _{\phi} J(\theta, \phi) = \arg \max _{\phi} J^{D}
\end{equation}
\begin{equation}
    \label{equation:irgan_d}
    J^{D} = \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
\end{equation}
while the generator is trained to minimize such an objective with the fixed discriminator $D_{\phi}$
\begin{equation}
    \small
    \theta^{*}=\arg \min _{\theta} J(\theta, \phi)=\arg \min _{\theta} \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
\end{equation}
and, as claimed in the original GAN paper~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14}
\begin{equation}
    \small
    \label{equation:irgan_min_g}
    \theta^{*} = \arg \min _{\theta} ( -  \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}(\hat{i} | u)))] ) = \arg \min _{\theta} J^{G}
\end{equation}
\begin{equation}
    \small
    \label{equation:irgan_g}
    J^{G} = - \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}(\hat{i} | u)))]
\end{equation}
Where $J_{D}$ and $J_{G}$ are the objective function~\footnote{We define the $J_{D}$ objective functions to be a maximization problem and $J_{G}$ a minimization problem.} of the GAN. \\
Note that they do not use the random noise variable $z$ like in classic GAN Eq.~\ref{equation:gan} since the goal is to generate a single, most plausible recommended item to a user rather than different relevant items.
As the sampling of $i$ is discrete, it cannot be directly optimised by gradient descent as in the original GAN formulation. Authors were the first to employ the \textit{policy-gradient based reinforcement learning} (REINFORCE)~\cite{DBLP:journals/ml/Williams92} to optimize the generator.
The authors empirically explores the effectiveness of the proposed method on the widely used matrix factorization~\cite{DBLP:journals/computer/KorenBV09} model in the movie domain with significant performance gains with respect to BPR~\cite{DBLP:conf/uai/RendleFGS09} and LambdaFM~\cite{DBLP:conf/cikm/YuanGJCYZ16}.
This work inspired a lot of new works to test GAN in Recommendation domain.

% CFGAN
\qquad Chae \textit{et al.} ~\cite{DBLP:conf/cikm/ChaeKKL18} address a qualitative problem in the IRGAN training algorithm. The authors identify the limitation of IRGAN and GraphGAN (see Section) in their \hltask{generation of discrete items} by verifying a worsening of recommendation performances when the number of epochs increase. As the training is further progressed, $G$ gets to sample frequently the items exactly same as those in ground truth. Since $D$ receives the same item index sometimes like a \textit{fake} element and sometimes like a \textit{ground-truth} one, it gets confused and, after few epochs, it starts to perform worse.
Beginning with such limitations, the authors propose a novel adversarial training, named \hlmethod{vector-wise training}, where $G$ \textit{generates real-valued vectors}. The proposed approach is named CFGAN, and it is based on a conditional GAN (CGAN). Formally, the important change compared to IRGAN overall objective function is in the $G$ Equation~\ref{equation:irgan_g}:
\begin{equation}
 \label{equation:cfgan_g}
 \small
 J^{G}=\mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}((\hat{i}\odot{e} ) | u))] = - \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}((\hat{i}\odot{e} ) | u))]
 % J^{G}=\sum_{n=1}^{N} \log (1-D_{\phi}((\hat{i}\odot{e_{n}} ) | u_{n}))
\end{equation}

\begin{equation}
 \label{equation:cfgan_d}
 \small
 J^{D}= \mathbb{E}_{i \sim p_{\text { true }}(i | u_{n}, r)}[\log D_{\phi}(i | u_{n})] + \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}((\hat{i}\odot{e} ) | u))]
 % J^{G}=\sum_{n=1}^{N} \log (1-D_{\phi}((\hat{i}\odot{e_{n}} ) | u_{n}))
\end{equation}
where $e$ in Eq.~\ref{equation:cfgan_g} is an $n$-dimensional vector specifying whether $u$ has purchased each item $\hat{i}$
% (eui =1) or not (eui =0),
and $\odot$ stands for element-wise multiplication. The main difference between CFGAN and the original GAN is element-wise multiplication in order to deal with the sparsity in ground-truth data that $G$ tries to mimic.
Experiments on different real-world datasets prove a significant improvement on different baseline methods ItemPop~\cite{DBLP:conf/recsys/CremonesiKT10}, BPR, FISM, CDAE and above all IRGAN and GraphGAN. 

\qquad Moreover, Chae \textit{et al.}~\cite{8525831, DBLP:journals/access/ChaeSK19} point out an issue regarding the employment of a linear model as the basic CF core of IRGAN because of non-ability to \hltask{capture non-linear interactions of users' and items'} latent factors to have better item-recommendations. Because of~\cite{DBLP:journals/access/ChaeSK19} is an extension of ~\cite{8525831} we deep in the extended one. Their main contribution is an advanced GAN-based CF framework, named \hlmethod{Collaborative Adversarial autoencoders} (CAAE), which is innovatively composed by three components: \textit{positive item generator} ($G$) , \textit{negative item generator} ($G^{\prime}$), and \textit{discriminator} ($D$). Generators are implemented with an autoencoder and the discriminator with BPR-MF~\cite{DBLP:conf/uai/RendleFGS09}.
Formally:
\begin{equation}
 \small
 \label{equation:cfgan2_d}
 J^{\mathcal{D}}= - \mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta} o r \hat{i} \sim p_{\theta^{\prime}}(\hat{i} | u)}[\log D_{\phi}(i, \hat{i} | u)]
\end{equation}
\begin{equation}
 \small
 \label{equation:cfgan2_g}
 J^{G}=\lambda \cdot \big( -\mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta}(\hat{i} | u)}[\log (1-D_{\phi}(i, \hat{i} | u))] \big) +(1-\lambda) \cdot  \mathcal{L}_{AE}
\end{equation}

\begin{equation}
 \small
 \label{equation:cfgan2_g_first}
 J^{G^{\prime}}=-\mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta^{\prime}}(\hat{i} | u)}[\log {D}(i, \hat{i} | u)) ]
\end{equation}
where $\mathcal{L}_{AE}$ in Eq.~\ref{equation:cfgan2_g} is the loss function of the autoencoder of the positive example generator, $\lambda$ parameterized its importance regard to generative loss function and $\theta^{\prime}$ is the set of model parameters of the second generator ($G^{\prime}$).
Note that the objective of $G^{\prime}$ is to help $D$ to \hlmethod{correctly discriminate} $G^{\prime}$ \textit{real} items from \textit{fake} items coming from $G^{\prime}$ to help $D$ to capture the difference between positive and negative items and $G$ to decrease the likelihood of generating items that the user may not prefer. Experiments on recommendation accuracy of CAAE framework with some well-known baselines demonstrate significant improvement on IRGAN and comparable performances on CFGAN.

\qquad Inspired by CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18}, a \hlmethod{GAN-based Rating Augmentation framework with \textit{bias treatment}}, named $RAGAN^{BT}$, has been proposed by Kim \textit{et al.}~\footnote{The same group of Authors of CFGAN} to alleviate the \hltask{data sparsity} problem in collaborative filtering (CF) by generating additional labeled data, which is called data augmentation. They propose a bias treatment to avoid $G$ from being biased towards high ratings in rating augmentation. This challenge is addressed by training the GAN on a modified version of original rating matrix where they add low ratings to the negative items.  
Formally, the objective function of generator and discriminator are the same in Equations~\ref{equation:cfgan_g} and ~\ref{equation:cfgan_d}.
After training of GAN is completed, the generated ratings on unrated items are used to augment the original rating matrix. 
They validate the effectiveness of $RAGAN^{BT}$ on four real-world datasets. The results demonstrate that the proposed data augmentation strategy outperforms the state-of-the-art CF models not only under basic top-N recommendations, but also under (i) \hltask{long-tail item} recommendations and (ii) recommendations to cold-start users. Compared models are: ItemPop, Item\textit{k}NN, SVD~\cite{DBLP:journals/computer/KorenBV09}, SVD++~\cite{DBLP:conf/kdd/Koren08}, AutoRec, PureSVD~\cite{DBLP:conf/recsys/CremonesiKT10} and Zero-Injection~\cite{DBLP:conf/icde/HwangPKLL16}.

The \hltask{long-tail phenomenon} in recommender performance is addressed also by \textit{Krishnan et al.}~\cite{DBLP:conf/cikm/KrishnanSSS18}. They propose and GAN-based approach to augment Neural Collaborative Filtering training to levy penalties when the recommender fails to identify suitable niche items for users, given their history and global item co-occurrence. 
The discriminator learns the inter-item association structure in the feedback data and correlates the generated niche item recommendations with popular items in the user's history. The generator must produce synthetic niche item recommendations that are correlated with the user's history. The effectiveness of the proposed method is evaluated on VAE and CDAE by measuring performance gains in niche-item on two real-world datasets. Results demonstrate that the proposed approach outperforms long-tail performances on the same model without the adversarial training. 

\qquad Sun \textit{et al.}~\cite{DBLP:journals/eswa/SunWWY19} address the problem settings of the \hltask{unstable and slow convergence adversarial training on a huge number of items}~\cite{DBLP:conf/sigir/WangYZGXWZZ17}. They propose (i) a GAN-based recommendation method, namely \hlmethod{Adversarial Pairwise Learning} (APL), for improving the training process of the adversarial model, by accelerating the convergence and enhancing the stability; and (ii) a \hlmethod{differentiable procedure}~\cite{DBLP:conf/iclr/JangGP17} to imitate the discrete item generation process and optimize APL with gradient descent directly instead of REINFORCE~\cite{DBLP:journals/ml/Williams92} used in most works (see Table~\felice{TABLE WITH STATISTICS ON TECHNIQUES}). 
The generator $G$ tries to imitate the observed item generation process and generate personalized items for each user; while the discriminator $D$ aims at learning a pairwise ranking function and determining the preferences of each user in preferring real items on generated ones. The novel component is related to the adoption of a Gumbel-Softmax~\cite{DBLP:conf/iclr/JangGP17} module that works as a bridge between $G$ and $D$. This implies that the GAN model is entirely differentiable, and the generator can be optimized with a standard back-propagation algorithm. 
The experiments on real-world datasets showed that (i) APL substantially enhances the convergence and stability of the adversarial learning process; (i) the differentiable item sampling procedure improves the stability of APL; (i) APL achieves state- of-the-art performance with respect to analyzed baseline models. Compared models are ItemPop, UIEM~\cite{DBLP:journals/eswa/NilashiIB18}, BPRMF, LambdaMF, AOBPR~\cite{DBLP:conf/wsdm/RendleF14}, IRGAN.

% QUI
\qquad Wu \textit{et al.}~\cite{DBLP:conf/ijcai/WuLMZZG19} propose to use the adversarial training to learn user's personal preference to items in a novel GAN-based recommender model, called \hlmethod{Personalized Diversity-promoting GAN} (PD-GAN), to generate recommendations that are as diverse and relevant as the ground-truth. Specifically, the authors implement the generator with the Determinantal Point Process (DPP) model~\cite{DBLP:journals/corr/abs-1709-05135} which captures the diversity and relevance of items. Experiments demonstrates the effectiveness of the proposed method in the item recommendation task compared against BPR.MF, IRGAN, MMR~\cite{DBLP:journals/sigir/CarbinellG17}, a canonical baseline for diversified ranking problems) and DPP, the state-of-the-art method for diversified recommendation.


\textit{Variational Autoencoder to Model Auxiliary Information.}

Lee \textit{et al.}~\cite{DBLP:conf/cikm/LeeSM17} and Zhang \textit{et al.}~\cite{8663730} propose for the first time the use of a Variational Autoencoder~\cite{DBLP:journals/corr/KingmaW13} as the generator in a GAN-based framework with the goal to take implicit feedback data into account for the top-\textit{n} recommendations.
Inspired by the adversarial process used in GAN, Lee \textit{et al.}~\cite{DBLP:conf/cikm/LeeSM17} propose a novel \hlmethod{VAE with Adversarial Regularization} (VAE-AR) framework to improve item recommendation. 
The basic idea is to merge two independent distributions of user-item interactions and auxiliary information in an unique model thanks to the capability of a Variational AutoEncoder to regularize another AutoEncoder through an adversarial \textit{minimax game}. Note that Variational AutoEncoders differ from Adversarial AutoEncoders, used for example in~\cite{DBLP:conf/webi/YiHQ18},. In fact, an AAE enforces prior knowledge on the latent variables of autoencoders, while a VAE regularize another VAE through its own inferred latent representations.  
The evaluation of recommendation performances on two publicly available datasets demonstrates a clear improvement on WRMF~\cite{DBLP:conf/icdm/HuKV08}, BPR~\cite{DBLP:conf/uai/RendleFGS09}, CDL~\cite{DBLP:conf/kdd/WangWY15}, CDAE~\cite{DBLP:conf/wsdm/WuDZE16}, CVAE~\cite{DBLP:conf/ijcnn/PandeyD17} and JMVAE~\cite{DBLP:conf/iclr/SuzukiNM17}. 

\qquad Tong \textit{et al.}~\cite{DBLP:conf/icde/TongLZSC19} implement the generator with a VAE in a collaborative scenario without implicit feedback.
They propose \hlmethod{Collaborative Generative Adversarial Network} (CGAN) model to enhance the recommendation performance and the robustness to adversarial examples by taking the advantage of the VAEs nonlinear nature in learning better aggregated posterior distribution from the given data and generate high-quality negative samples to fail the discriminator. Then, the author propose to alleviate the issue of unstable convergence and time-consuming training of classic GAN by using Improved Wasserstein GAN (WGAN-GP)~\cite{DBLP:conf/nips/GulrajaniAADC17}, which removes the log function and adds a gradient penalty term $ W_{pen}$ on the original critic loss. 
The objective functions of G and D are presented as follows:
\begin{equation}
    \label{eq:cf_vae_d}
    \small
    J^{D} = - \mathbb{E}_{i \sim p_{\text {true}}(i | u)}[D_{\phi}(i| u)] + \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u) }[D_{\phi}(\hat{i}| u)] + \lambda W_{pen}
\end{equation}

\begin{equation}
    \label{eq:cf_vae_g}
    \small
    J^{G}= \lambda \cdot \big(- \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u) }[D_{\phi}(\hat{i}| u)]\big) + (1 - \lambda) \cdot \mathcal{L}_{VAE}
\end{equation}
where $J^{D}$ is the WGAN-GP objective with the critic term, ${L}_{VAE}$ stands for the loss function of VAE, $\lambda$ parameterized its importance regard to generative loss function. Recommendations are built upon the reconstructed vector of user's ratings by the Variational AutoEncoder in the model.
Experimental evaluation on recommendation performances demonstrate advances on ItemPop, BPR-MF, CDAE, NeuMF~\cite{DBLP:conf/www/HeLZNHC17}, GraphGAN and IRGAN. Then, the authors demonstrate the effectiveness of the adversarial training by utilizing the Wasserstein distance with gradient penalty through an \textit{ablation study}.


\qquad Costa and Dolog~\cite{DBLP:conf/flairs/CostaD19} address the problem setting related to highly sparse data and discrete values when adversarial training is used in recommendation scenarios. The authors identify that \hltask{the policy gradient strategy is impractical in RS} with a large number of items because the variance of the estimated gradients increases linearly according to the number of items. In order to solve this challenge, they propose a novel model, named ~\hlmethod{Convolutional Adversarial Latent Factor} (CALF), that uses the  Rao-Blackwell sampling~\cite{DBLP:conf/icml/LiuRTJM19}. Inspired by He \textit{et al.}~\cite{DBLP:conf/ijcai/0001DWTTC18}, the authors introduce a novel convolutional layer in the generator and discriminator for processing the useful signal from the pairwise user-item interactions.
Experiments of CALF and other baseline models( AMF, IRGAN, CFGAN and CNCF~\cite{DBLP:conf/ijcai/0001DWTTC18}), demonstrate that the proposed model outperforms baseline models in the item recommendation task and the novel sampling strategy effectively improves adversarial training thanks to the reduction of the gradient variance.


\subsubsection{Hybrid Recommendation}
GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18} is the first \hltask{graph representation learning} framework which \hltask{models} generative models, that learn the underlying connectivity distribution in the graph to generate \textit{fake vertex}, and discriminative models, that detect whether a sampled vertex is real or fake; in a GAN way. The authors accomplish the item-recommendation task with a graph representation learning by modeling users and items as vertices and by mapping user-item interaction, e.g. ratings and implicit feedback, with an edge. top-\textit{n} recommendation list is built upon this graph after the training of the model. Since the formulation of minimax problem is the same of IRGAN in Section~\felice{subsec:GAN-based CF} we identify a main contribution in the an alternative neighbor-aware softmax for the generator named \hlmethod{graph softmax} with the goal to overcome the limitations of traditional softmax function: (i) lacking of graph structure because of equal treats of all vertices and (ii) inefficiency due the evaluation of softmax on every vertex.
\\They demonstrate better recommendation performance of GraphGAN by comparing it with other graph representation learning methods: DeepWalk~\cite{DBLP:conf/kdd/PerozziAS14}, LINE~\cite{DBLP:conf/www/TangQWZYM15}, node2vec~\cite{DBLP:conf/kdd/GroverL16}, and struc2vec~\cite{DBLP:conf/kdd/RibeiroSF17}. 

\qquad Han \textit{et al.}~\cite{DBLP:conf/aaai/CaiHY18} address the problem of graph-based \hltask{citation recommendation} when heterogeneous content information is associated with each vertex of the network.
They model each paper and author ($i$) as a vertex, the citation as the link ($r$) between vertices and the recommendation task as a \hltask{link prediction problem}. Note that this work is not under collaborative settings with a user-item matrix, but under a content-based setting with an item-item matrix.
The authors propose a GAN-based model, named GAN-HBNR, \hlmethod{to learn an effective feature representation that preserves both vertex content information and network structure information}. 
% Then, this latent representation can be applied to address the  recommendation task.
They employ an energy-based formulation for generative adversarial training, called EBGAN~\cite{DBLP:conf/iclr/ZhaoML17}, where the ground truth is a vertex vector concatenated with its content vector, encoded with \textit{Doc2Vec}~\cite{DBLP:conf/icml/LeM14}.
The discriminator of an EBGAN is implemented with an auto-encoder architecture. The energy function, the MSE, is trained to push down on the reconstruction error of the autoencoder when the input is the ground truth, and to push up when the discriminator input is the generated one. 
The recommendations are made by mapping real-data into the latent space of the trained autoencoder and by producing the recommendation list by taking the most similar ones.
\\Experimental studies verify the effectiveness of the proposed approach compared to DeepWalk, Line, Doc2Vec, TriDNR~\cite{DBLP:conf/ijcai/PanWZZW16} and Node2Vec~\cite{DBLP:conf/kdd/GroverL16}.
% ~\felice{Here I am not inserting any formalism because I don't know how many papers use EBGAN. If I will find a lot of paper I will introduce here the formalism}.
~\futureworks{\textbf{What do you think if we use SemAuto in the Decoder? We should exploit its explainability properties for cold-item}}


\qquad In~\cite{DBLP:conf/icdm/LiH018}, the authors addresses the task of \hltask{Tag-Aware Recommendation}~\cite{DBLP:journals/jcst/ZhangZZ11}.
Formally, the overall loss function is a combination of three components:
\begin{equation}
    \label{equation:TDGAN}
    \small
    J(\theta, \phi, \eta) = \lambda_{1} \cdot f_{1}(R_{\eta}(x)) + \lambda_{2} \cdot f_{2}(G_{\theta}(R_{\eta}(x))) +  \lambda_{3} \cdot f_{3}D_{\phi}((G_{\theta}(R_{\eta}(x))))
\end{equation}
where $\theta, \phi, \eta$ are the model parameters of $G$, $D$ and $R$, $x$ is the input user or item vector, $f_{1}$ measures the relevance scores of items $i$ to a given user $u$, $f_{2}$ is the reconstruction error of the re-generated vector $x$ and $f_{3}$ measures the discrepancy between genuine input and generated one. 
After training, the proposed model predicts results for recommendation by combining linearly the similarity between the extracted abstract from the tag-based profiles of users and items, from $R$, and the tag-based profiles reconstructed by $G$.
Experiments on music domain show better top-\textit{n} recommendation performances compared to baseline methods: CFA~\cite{DBLP:journals/ijon/ZuoZGJ16} and DSPR~\cite{DBLP:conf/ijcai/XuLCMM17}. Furthermore, the authors explore the impact of the discriminator $D$ to implement the adversarial strategy by demonstrating that, without this component, accuracy metrics go down in a significance way.

\qquad The authors of ~\cite{DBLP:conf/webi/YiHQ18} focus on \hltask{solving the sparsity problem} in order to get \hltask{higher recommendation quality} by exploting both user-ratings and user-generated reviews on items. They propose a GAN-based recommendation method, named \hlmethod{aae-RS}, by employing the \textit{minimax game} between the rating relations and review relations of users and items in order to merge the user-item ratings and reviews by making them indistinguishable. The proposed model, inspired by AAE~\cite{DBLP:journals/corr/MakhzaniSJG15}, is composed by three autoencoders, namely $G_{rev}$, $G_{u}$, and $G_{i}$, a discriminator $D$ and a predictor $P$. autoencoders map users' vectors, items' vectors, and users' reviews in a common latent space. The discriminator tries to maximize its ability to distinguish between the user-item vector, the ground truth, and the review vector, the fake sample, while autoencoders try to minimize the difference of the two vectors in an adversarial manner. The prediction is trained to predict a real-value rating given auser-item vector. Formally, the overall objective function is a linear combination of six components:
\begin{equation}
    \label{equation:aae-RS}
    \small
    J = \lambda_{1} \cdot \mathcal{L}_{adv} 
    +  \lambda_{2} \cdot \mathcal{L}_{rec_{rev}} 
    +  \lambda_{3} \cdot \mathcal{L}_{rec_u}
    +  \lambda_{4} \cdot \mathcal{L}_{rec_i} 
    +  \lambda_{5} \cdot \mathcal{L}_{rec_{rev+u+i}}
    +  \lambda_{6} \cdot \mathcal{L}_{pred}
\end{equation}
where $\mathcal{L}_{adv}$ is the adversarial loss, $\mathcal{L}_{rec_{rev}}$ is the reconstruction loss of $G_{rev}$, $\mathcal{L}_{rec_u}$ and $J_{rec_i}$ are the reconstruction losses respective of $G_{u}$ and $G_{i}$, $\mathcal{L}_{rec_{rev+u+i}}$ is the reconstruction loss among the representations of different latent vectors of the same pair of user and item and $\mathcal{L}_{pred}$ is the square loss between the predicted ratings and the real ratings. $\lambda_{j}, j= 1,...,6$ are hyper parameters to weight objective functions. Experiments on e-commerce datasets validate the superiority of aae-RS over HFT~\cite{DBLP:conf/recsys/McAuleyL13}, mDA-CF~\cite{DBLP:conf/cikm/LiKF15}, ConvMF-~\cite{DBLP:conf/recsys/KimPOLY16} and ReDa~\cite{DBLP:journals/nn/ZhuangZQSXH17}.

\qquad Chen \textit{et al.}~\cite{DBLP:journals/tois/ChenZXQZ19} address computational inefficiency of baseline recommendation with external knowledge in practical scenario, i.e. review-based recommendation, by proposing a teacher-student model, named \textit{Generalized Distillation Framework} (GDF). Particularly the use an \hlmethod{adversarial adaption strategy} in order to guarantee the \hltask{effectiveness of the knowledge distillation} from the teacher to the student models of GDF for better \hltask{recommendation performances}.
The minimax-game is played by the user-item prediction network, which works as the generator $G$; and a discriminator $D$. 
$D$ tries to distinguish between the ground truth, the review-embedded vector produced by the Teacher, and the fake example, the user-item embedding vector generated by the Student for fooling $D$. At the end of the game, the user-item prediction network is able to encode review-based user-item relevant information and it achieves better rating prediction as show in the experimental evaluation.

\qquad Rafailidis and Crestani~\cite{DBLP:conf/sigir/RafailidisC19} address the challenge on learning how reviews influence users' rating behaviors by proposing an \hlmethod{Adversarial Training approach for Review-based recommendations}, namely ATR. The proposed ATR model consists of two GANs, one for users' review generation , and the other for items' review generation; coupled with a matrix factorization to predict the ratings, by considering both the ground-truth and machine-generated reviews. The generator
The authors compare compare the proposed ATR model with the baseline PMF~\cite{DBLP:conf/nips/SalakhutdinovM07} model that ignores users’ reviews on items, the HFT model~\cite{DBLP:conf/recsys/McAuleyL13} and review-based deep learning strategies of DeepCoNN~\cite{DBLP:conf/wsdm/ZhengNY17}, TNET~\cite{DBLP:conf/recsys/CatherineC17} and TARMF~\cite{DBLP:journals/complexity/LinWHMCLC18}. Experimental evaluation shows that the proposed ATR model the proposed ATR model beats all the competitors thanks to the adversarial-based joint learning strategy that produces deep representations of reviews close to the user and item latent features.

\subsubsection{Contextual Recommendation}

Sequence-aware Recommender Systems are mostly studied in these years to emphasize the significance of modeling short-term and long-term temporal profiles behind temporal evolution of user preference and item state to make relevant suggestions. Different solutions are proposed under the adversarial-framework.

\textbf{Model Dynamics of User and Item Interactions.}\\

\qquad Bharadhwaj \textit{et al.}~\cite{DBLP:conf/recsys/BharadhwajPL18} address the problem to improve the effectiveness of RS by accurately ~\hltask{modelling temporal dynamics of user and item} under the GAN framework. Inspired by Recurrent Recommender Networks~\cite{DBLP:conf/wsdm/WuABSJ17} and IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the authors propose a \hlmethod{Recurrent Generative Adversarial Networks for Recommendation Systems}, named RecGAN, in order to exploit in a single framework both the temporal modelling capabilities of RNN and the latent feature modelling power of the \textit{minimax game}.
They implement both the generator a the discriminator with the Gated Recurrent Unit (GRU)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}, a RNN cell, in order to make $G$ capable to generate ratings for each user-item pair denoted by $(r|u, j, t)$. The overall objective function is formally defined
\begin{equation}
     \small
     \label{equation:recgan}
     J(\theta, \phi)= \mathbb{E}_{r \sim p_{\text { true }}(r | i, u, t)}[\log D_{\phi}(r | i, u, t)]+ \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (1-D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}
where $p_{\theta}(\hat{r} | i, u, t)$ is the rating distribution learned by the generator and $D_{\phi}(r | i, u, t)$ refers to the discriminator's prediction of the likelihood of $(r|i, j, t)$ being sampled from the true distribution $p_{\text { true }}(r | i, u, t)$.
\\Similarly to Equations~\ref{equation:irgan_d} and~\ref{equation:irgan_g}
\begin{equation}
     \small
     \label{equation:recgan_d}
     J^{D} = \mathbb{E}_{r \sim p_{\text { true }}(r | i, u, t)}[\log D_{\phi}(r | i, u, t)]+ \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (1-D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}
 \begin{equation}
     \small
     \label{equation:recgan_g}
     J^{G}= - \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}

The authors demonstrate that RecGAN outperforms various baselines model dealing with temporal aspects in two different RS domains, movie and food. The baseline models include PMF~\cite{DBLP:conf/nips/SalakhutdinovM07}, TimeSVD++~\cite{DBLP:journals/cacm/Koren10}, AutoRec~\cite{DBLP:conf/iconip/OuyangLRX14} and RRN~\cite{DBLP:conf/wsdm/WuABSJ17}.  


\qquad Similar to~\cite{DBLP:conf/recsys/BharadhwajPL18}, Zhao \textit{et al.}~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:journals/corr/abs-1712-09059} address the ~\hltask{long and short-term preference modelling} by leveraging the MF~\cite{DBLP:conf/nips/SalakhutdinovM07} and RNN approaches for top-\textit{n} recommendation using a GAN framework. They propose ~\hlmethod{Prioritizes Long And Short-Term Information in top-\textit{n} reCommendation} (PLASTIC) model in order to incorporate long-term interactions modelling of MF and short-term interactions modelling of RNN in a unique recommendation framework. The discriminator $D$ is implemented via a \hlmethod{Siamese Network} that incorporates MF and LSTM~\cite{DBLP:conf/wsdm/WuABSJ17} cell in a pair-wise scenario and learns to distinguish the real high-rated items in the training data from the recommendation list generated by the generator $G$. While the generator $G$ learns to maximize the probability of $D$ making a mistake by  generating top-\textit{n} recommendations produced using a MF model and re-ranked with LSTM cell.
The discriminator and generator objective function are formally defined as
\begin{equation}
    \small
    \label{equation:plastic_d}
    J^{D} =  
    \mathbb{E}_{i_{+}, i_{-} \sim p_{true}(i_{+}, i_{-} |u, t)}[\log D_{\phi}(i_{+}, i_{-} |u, t)] + 
    \mathbb{E}_{i_{+} \sim p_{true}(i_{+} |u, t), \hat{i} \sim p_{\theta}(\hat{i} | u, t)}[\log (1-D_{\phi}(i_{+}, \hat{i} | u, t)]
\end{equation}
\begin{equation}
    \small
    \label{equation:plastic_g}
    J^{G} =  
    - 
    \mathbb{E}_{i_{+} \sim p_{true}(i_{+} |u, t), \hat{i} \sim p_{\theta}(\hat{i} | u, t)}[\log (D_{\phi}(i_{+}, \hat{i} | u, t)]
\end{equation}
where $i_{+}$ is a positive item, $i_{-}$ is a randomly chosen negative item and $\hat{i}$ is the generated item by $G$ at time $t$ for the user $u$. Experiments on movie domains demonstrate that PLASTIC outperforms recommendation performance of BPR~\cite{DBLP:conf/uai/RendleFGS09}, PRFM~\cite{DBLP:conf/cikm/QiangLY13}, LambdaFM~\cite{DBLP:conf/cikm/YuanGJCYZ16}, RRN and IRGAN.

\qquad Chen \textit{et al.}~\cite{DBLP:conf/icml/Chen0LJQS19} work on the challenging application of \hltask{reinforcement learning (RL)} to RS to take into account the long-term user interest evolution and the influence of the recommender action for improving, for instance, users' long-term engagement with an online platform. Model-free reinforcement learning techniques suffer from (i) manually designed reward function which may not reflect a user's preference, and (ii) the need for collecting lots of user-data in order to learn a good-policy. Starting from these limitations, the authors propose a model-based RL framework where user behavior model and the associated reward function are learnt by with a GAN-based approach, called \textbf{GAN user model}.
The generator $G$ learns to mimic the user model by generating the user's next action in order to maximize his reward function, that is to minimize the discriminator. The discriminator $D$ acts as the reward function by maximizing its ability to distinguish between the user's actual actions and those generated by $G$. On completion of the \textit{minimax game}, the authors use the user model and the reward function as the simulation environment to obtain a recommendation policy in the RL framework. Experiments show important advances of the proposed approach in an offline on realistic domains.
% Main contributions of this framework are: (i)the user model and the reward function are learned in a consistent way with the user model; (ii) the learned reward carries out the RL policy in a more principled way, rather than the manually designed one; (ii) the learned user model allows us to perform model-based RL and online adaptation for new users to achieve better results.

\qquad Wang \textit{et al.}~\cite{DBLP:conf/kdd/WangYHLWH18} and Tanielian \textit{et al.}~\cite{DBLP:journals/corr/abs-1805-08720}, address limitations of baseline \hltask{adaptive negative sampling} methods used to improve recommendations and optimize the training of multi-class models with a huge set of output classes.
Wang \textit{et al.}~\cite{DBLP:conf/kdd/WangYHLWH18} focus on this problem setting in their proposed streaming recommender system, called \hlmethod{Neural Memory Recommender Networks} (NMRN). Inspired by KBGAN~\cite{DBLP:conf/naacl/CaiW18}, the authors propose a novel \hlmethod{GAN-based adaptive negative sampling method} with the aim of improving training efficiency much more than classic random and popularity-biased sampling methods which are not able to dynamic negative items. At the end of the \textit{minimax game} the generator is able to generate adversarial negative samples for each user.
They validate their statements with extensive experiments which show clear improvements compared to the classic streaming recommendation models and the proposed model NRMN without the GAN sampling.
Tanielian \textit{et al.}~\cite{DBLP:journals/corr/abs-1805-08720} address the same issues in the task of basket completion with learned embedding representations. Inspired by MaliGAN~\cite{DBLP:journals/corr/CheLZHLSB17}, the authors propose to solve these issues with a GAN-based sampling method, called ~\hlmethod{Adversarial Negative Sampling} that draws negative samples from a dynamic distribution that is by design more informative than the fixed distribution used in standard negative sampling. They introduce the new method in a novel basket completion model, namely \textbf{GAN-Word2Vec}. 
Experiments on two e-commerce datasets show better top-\textit{1} recommendations when GAN-Word2Vec is compared to classical Word2Vec approaches.

\qquad Zhou \textit{et al.}~\cite{DBLP:conf/www/0002YZTZW19} focus on ~\hltask{location-based recommendation systems} to suggest point-of-interest (POI) to users. The authors address the ~\hltask{lack of formal models to understand user check-in behavior} which can lead to poor recommendation performance. They propose a novel GAN-based POI recommendation model, named \hlmethod{Adversarial POI Recommendation} (APOIR), for learning the user check-in model in a generative way, rather than extracting them with baseline approaches, such as MF, Context Embedding and Pairwise Ranking, in order to boost the recommendation performance.
The generative process is used to model the relationship between a user $u$ and the set of POIs, where a POI is $i$. The underlying distribution of the user preferences over POIs is learned by classical minimax game between a generator $G$ and a discriminator $D$ explained in Section~\felice{XXX}. Similarly to IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the authors employ a reward policy based on \textit{Geographical rewards}, e.g. the distance between POIs, and \textit{Social rewards}, e.g. the POIs visited by user's friends, which works as a regularizer to the recommended POIs from the generator $G$.
They evaluate APOIR on public location-based social network datasets and compare it to several state-of-the-art models. The results demonstrate the effectiveness of APOIR approach in improving POI recommendation.


\qquad Lie \textit{et al.}~\cite{DBLP:conf/ijcai/0061W0Y19} work on the POI recommendation task looking at (i) the ineffectiveness of random sampling strategy for the selection of negative samples in the model training of a pairwise ranking approach, and (ii) a better use of geographical information to improve the recommendation performance. To address the above issues, they propose a novel adversarial-based approach, called \hlmethod{Geographical information based Adversarial Learning Model} (Geo-ALM), with the goal to combine the Adversarial Learning and geographical features, to craft high-quality unvisited POI for a given user (i.e., the negative samples), which helps the discriminator to improve its training performance. Empirical study demonstrate the effectiveness of the proposed model in POI recommendation task compared against different baseline POI recommender models.
The effective novelty on AML in RS is in the integration of geographical features into the adversarial learning mechanism.


Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} investigate \hltask{query recommendation systems} in order to improve the suggestion performance by understanding and modeling user search intents accurately. The authors propose a novel model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), that provides query suggestions considering the sequential search queries issued by the user and and his the history of clicks on last suggestions. Similarly to APR~\cite{DBLP:conf/sigir/0001HDC18}, they employ an adversarial training stage during the training of CFAE by injecting adversarial examples built by adding adversarial perturbations of item embeddings.~\felice{It is necessary to define in a Section the procedure user to create adversarial perturbations. They use FSGM}
Experiments on a e-shopping domain dataset demonstrate that adversarial training on CFAN not only significantly \textit{improve the robustness} of the model but also outperforms the baseline methods for the task of query suggestion.

\subsubsection{Cross-Domain Recommendation}

Cross-domain recommendation (CDR) offers recommendations in a target domain by exploiting knowledge from source domains. This recommender category has received much attention because it is a potential solution to mitigate the cold-start and sparsity problem.
% ~\futureworks{I think that this field is quite not explored in the domain of adv-recommender systems. It can be intriguing to think on an adversarial-based model to move information from a movie domain (e.g. Netflix) to a music domain (e.g. Last.fm) in an unsupervised way. Another idea can be to use domain2domain translation also in music recommendation itslef for playlist building (ropose interesting playlist in another genre,...) }

Inspired by e Unsupervised Image-to-image Translation (UNIT)~\cite{DBLP:conf/nips/LiuBK17}, Nguyen and Ishigaki~\cite{DBLP:journals/corr/abs-1812-06229} address the problems relating to the ~\hltask{difficulty to obtain similar features among different domains} and to ~\hltask{transfer the knowledge on a denser target domain $A$ into a source one $B$} for cross-domain recommendation by proposing a \hlmethod{VAE-GAN-CC} network.
to (i) extract both homogeneous and divergent features among domains, (ii) translate one domain to another and (iii) apply an end-to-end deep learning approach for CF-RS which only uses the user interaction history as input.
The proposed model is composed by two generative adversarial networks $GAN_{A}$ and $GAN_{B}$. The generator of each GAN is a VAE.
In their model, $VAE_{A}$ is the generator for domain A, while $VAE_{B}$ is related to domain B. For an input click vector $u_{A}$ $\in$ A, the $VAE_{A}$ first maps $u_{A}$ to a code in a latent space $Z$ via its encoder component. It then decodes a randomly perturbed version of the code to reconstruct the input click vector via the decoder.
The authors enforce a weight-sharing constraint between some layers of VAEs in order to learn domain-to-domain translation, e.g. 
Because of the weight-sharing of between the two VAE of each GAN, each generator generates a reconstructed user vector that can come from the same domain, or a different one. For instance, it is possible to translate a click vector $u_{A}$ in domain A to a click vector in domain B through applying $G_{B}$.
$G_{A}$ generates click vector ${u}_{AA}$ and ${u}_{BA}$ where ${u}_{BA}$ is the translation vector of the user vector in domain B to the domain A, $G_{A}$ generates click vector ${u}_{BB}$ and ${u}_{AB}$ where ${u}_{AB}$ is the translated version of $u_{A}$ in the domain $B$. 
$D_{A}$ is trained to output true for real click vectors sampled from $A$ domain and to output false for click vectors generated from $G_{A}$, $D_{B}$ works in the same way for the $B$ domain.
The overall objective function is composed by six components:
\begin{equation}
    \label{equation:domain2domain}
    \small
    J = \mathcal{L}_{VAE_{A}} + \mathcal{L}_{GAN_{A}} + \mathcal{L}_{CC_{AB}} + \mathcal{L}_{VAE_{B}} + \mathcal{L}_{GAN_{B}} + \mathcal{L}_{CC_{BA}}
\end{equation}
where $\mathcal{L}_{VAE_{A}}$ and $\mathcal{L}_{CC_{BA}}$ are the loss function of the cycle-consistency constraint for weight-sharing.
The trained generator $G_{A}$ is used to predict the user click vector in the domain $D$ given the vector in a domain $A$ and viceversa. 
Experiments on real-world domains, i.e. movie and e-commerce, demonstrate an improvement of ranking based metrics on CDL~\cite{DBLP:conf/kdd/WangWY15}, CCCFNET~\cite{DBLP:conf/www/LianZXS17}, Multi-VAE~\cite{DBLP:conf/www/LiangKHJ18} and APR~\cite{DBLP:conf/sigir/0001HDC18}.
% ${u}_{AA}=G_{A}({z}_{A} \sim q_{A}({z}_{A} | {u}_{A}))$ and ${u}_{B A}=G_{A}({z}_{{B}} \sim q_{B}({z}_{B} | {u}_{B}))$, where $z_{A}$ and $z_{B}$ are the latent representation of the encoders of $G_{A}$ and $G_{B}$ respectively, $q_{A}$ and $q_{B}$ are the distributions of $z_{A}$ and $z_{B}$.

Wang \textit{et al.}~\cite{8698453} address \hltask{data sparsity and data imbalance} problem setting in cross-domain recommender systems. Inspired by the last advances in adversarial domain adaptation like ADDA~\cite{DBLP:conf/cvpr/TzengHSD17} and Bi-LSTM model~\cite{DBLP:journals/tomccap/WangYM18}, they propose a \hlmethod{Discriminative Adversarial Networks for Cross-Domain Recommendation (RecSys-DAN)} method to learn domain indistinguishable representations of users, items and user-item pairs across different product domains in a unsupervised way.~\felice{They claim that RecSys-DAN can be viewed as the first work which explores the power of GAN in the context of cross- domain recommender systems.} They perform domain adaptation going from a \textit{source domain with several user-item preference values} to a \textit{target domain with no user-item preferences}.~\felice{The minimax game objective function is a little bit complicated to insert because it is based on 6 generators and 3 discriminators.}
The authors evaluate RecSys-DAN on multiple sets on e-shopping domain with different item and user interactions such as review text, product images and ratings different tasks. Results demonstrates competitive performance compared to baseline supervised methods for the rating prediction, even without explicit preferences.

D. Perera and R. Zimmermann~\cite{DBLP:conf/www/PereraZ19} propose a solution to address the limit in applying \hltask{cross-domain recommendations} to apply a GAN based model to generate missing source network preferences for non-overlapped users. The authors propose \hlmethod{CnGAN}, a novel GAN based model which includes a content loss function and user-based pairwise loss (BPR) function for the \textit{generator} and \textit{recommender} tasks.
The generator task learns the corresponding mapping from target to source network user preferences and generates auxiliary preferences on the source network thanks. While classic GAN models are typically used to generate real-like samples from random noise vectors, CnGAN aims to \textit{learn} a specific mapping from target to source network encoding in order to 'move' the encoding of not-overlapped users in a latent space that encodes global implicit information of another domain (source network). The novel content-loss is used to provide additional guidance for G to map users in the source space.~\felice{Not simple to explain... need more accuracy}
The recommender task uses the synthetically generated preferences to provide recommendations for users who only have interactions on the target network (not overlapped users). Experimental evaluation of CnGAN against single network (TimePop:), cross-network (TBKNN~\cite{Campos:2010:STK:1869652.1869655}, TDCN~\cite{DBLP:conf/mm/PereraZ17}, linear factorization and GAN based baselines demonstrate advances in terms of accuracy, novelty and diversity.

Inspired by \hlmethod{adversarial negative sampling} techniques proposed in~\cite{DBLP:conf/kdd/WangYHLWH18}, Fan \textit{et al}~\cite{DBLP:conf/ijcai/FanD0WTL19} address the limitation of typical negative sampling in \hltask{social recommendation} domain to transfer users' information from social domain to item domain. The proposed framework, namely \hlmethod{Deep Adversarial SOcial recommendation} (DASO), harnesses the power of adversarial learning to dynamically generate 'difficult' negative samples of user-item pairs and user-user pairs, to guide the framework in learning better user and item representations.
 Adversarial Learning used to learn better user representations from the social perspective and $\lambda$ is the parameter to control the relative importance of cycle-reconstruction $\mathcal{L}_{CC_{I,S}}$ used to bidirectional map between the social and the item domain. To evaluate the performance, the authors compared DASO with BPR, SBPR~\cite{DBLP:conf/cikm/ZhaoMK14}, DeepSoR~\cite{DBLP:conf/aaai/FanLC18}, GraphRec~\cite{DBLP:conf/www/Fan0LHZTY19} and IRGAN. Comprehensive experiments on two real-world datasets show the effectiveness of their model

Transferability properties of GAN have been exploited also by Sang-Young Jo \textit{et al.}~\cite{DBLP:conf/bigcomp/JoJCJ19}. They focus on addressing \hltask{fashion recommendation} challenge by proposing a recommendation system that takes into account the styles and patterns of sceneries pictures. Inspired by style-transfer ability of DiscoGAN~\cite{DBLP:conf/icml/KimCKLK17}, the authors employ a GAN-based framework to generate new fashion images with the styles from the sceneries. ~\felice{I think we can remove the analysis of this article}.
% RecSys2019
Aggarwal et al.~\cite{DBLP:conf/recsys/AggarwalYK19} address the challenge of using a much larger re-targeting data (source domain) for CTR prediction on cold users (target domain) by modelling it like a domain adaptation problem. Particularly, one of the two proposed method, Supervised Sub-domain Adaptation Neural Network (SDA-DANN) inspired by ~\cite{DBLP:journals/jmlr/GaninUAGLLML16} performs domain invariance through a class-wise based adversarial loss to leverage the prediction label information.

\subsubsection{Complementary Recommendation}
Complementary Recommendation (Com) is a novel challenging task that points to suggest complementary items to suggest new items to customers. A very intuitive application domain is the fashion domain. For instances, given a red top (i.e., upper garment), the recommender model may recommend a selection of bottoms (e.g., trousers) in a complementary way. 
\\Novel solutions have been proposed to address the problem of recommending complementary items by using adversarial-based approaches.


Huynh \textit{et al.}~\cite{DBLP:conf/eccv/HuynhCTA18} address the problem of ~\hltask{recommending complementary items} for a given item based on visual features. They develop an unsupervised learning approach for \hlmethod{Complementary Recommendation using Adversarial Feature Transform} (CRAFT), by learning the co-occurrence of item pairs in real images. The proposed method does not generate new images but it learns to generate features of the complementary items conditioned on the query item. 
\begin{figure}[h]
  \includegraphics[width=0.6\linewidth]{Pictures/CRAFT.png}
  \caption{Architecture for the CRAFT framework. The transformer component is trained to generate the target features conditioned on the source features and a sampled noise vector.}
  \label{fig:CRAFT}
\end{figure}

The generator $G$ acts like a feature transformer to transform the source feature $s_{q}$ into a complementary target feature $\hat{t_{q}}$ by playing a \textit{minimax game} with a discriminator $D$ that aims to classify feature pairs as real ($s_{i}$, $t_{i}$) or synthetic ($s_{q}$, $\hat{t_{q}}$).
Similar to Equation~\ref{equation:gan}, the objective function is
\begin{equation}
    \label{eq:craft}
    \small
    J(\theta, \phi) = \mathbb{E}_{(s_{i}, t_{i}) \sim p_{c}} \log D_{\phi}(s_{i}, t_{i})+\mathbb{E}_{z \sim p_{z}, s_{q} \sim p_{s}} \log (1-D_{\phi}(s_{q}, G_{\theta}(s_{q}, z)))
\end{equation}
where $p_{z}$ and $p_{s}$ are the probability distribution function of the random noise and the source feature.
Recommendation are built on a nearest neighbor search of $\hat{t_{q}}$ on the subspace with pre-indexed target features $t_{i}$.
CRAFT has been tested by experienced users whose who gave positive feedback on the goodness of complementary recommendations.

Inspired by advances in image generation by class labels or by texts, and image transformation between different domains, Kang \textit{et al.}~\cite{DBLP:conf/icdm/KangFWM17}, Shih \textit{et al.}~\cite{DBLP:conf/aaai/ShihCLS18}, Lin \textit{et al.}~\cite{Yang2018FromRT} and Kumar and Das Gupta~\cite{DBLP:journals/corr/abs-1906-05596} propose GAN-based~\cite{DBLP:journals/corr/RadfordMC15} solutions for the \hltask{generation of compatible items} in the fashion domain.

\cite{DBLP:conf/icdm/KangFWM17} is the first publication where the Generative Adversarial Networks are used in Fashion Domain recommendation to \hltask{generate item images based on user preferences}. For instance, given a user and an item category, they propose a model to generate new images (i.e., clothing items) that are most consistent with user's preferences. In this paper, the authors adapt the Bayesian Personalized Ranking (BPR) to include item image content via a Siamese network in a \hlmethod{Deep Visually-aware Bayesian Personalized Ranking} method, called DVBPR. Then, this model is combined with a GAN-based framework to generate images that are consistent with user's personal taste. Iteratively, the generator learns a low dimensional latent code, which generates an item image that maximizes a personal objective value. 
Inspired by LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}, the overall objective function is
\begin{equation}
    \small
    \label{eq:dvbpr_gan_objective}
    J = \mathbb{E}_{\mathbf{x}, c \sim p_{true}(x, c)} [D(\mathbf{x}, c) - 1]^{2} + 
        \mathbb{E}_{c \sim p(c), z \sim p(z)} [D(G(z, c), c)]^{2}
\end{equation}
where $\mathbb{x}$ is a image of the training dataset, $c$ is the category of the image $\mathbb{x}$ a $z$ is a random noise vector. Given a user $u$ and a category $c$, the authors propose to synthesize personalized images by optimizing a user preference score
\begin{equation}
    \small
    \widehat{\delta}(u, c) = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} ( \widehat{r}_{u, e} )
    = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} \big(r_{u, e}-\eta D(e, c) \big)
\end{equation}
where $r_{u,e}$ is the user score to a generated new image and $\eta$ controls the trade-off between preference score and image quality. Generated Images are quantitatively compared with real images using the preference score (mean objective value), inception score~\cite{DBLP:conf/nips/SalimansGZCRCC16} and Opposite SSIM~\cite{DBLP:conf/icml/OdenaOS17}. This comparison show above all improvement on preference score with respect to not-GAN based images. At the same time, the qualitative comparison demonstrates that the generated images are realistic and plausible, yet are quite different from any images in the original dataset—they have common shape and color profiles, but quite different styles. 

Shih \textit{et al.} propose a Compatibility Learning Framework by using a \hlmethod{Metric-regularized Conditional Generative Adversarial Network} (MrCGAN) to pursue the item generation task. The proposed model is composed of a compatibility learning component and a DCGAN~\cite{DBLP:journals/corr/RadfordMC15}-based component, MrCGAN, that is regularized on a compatibility metric learnt in the first component. Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18} they conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines. 
% \\The authors of~\cite{Yang2018FromRT} addresses the same problem settings by proposing a novel fashion clothing framework composed of two parts: a clothing recommendation model based on BPR combined with visual features and a clothing complementary item generation based on DCGAN. Particularly, the generation component takes in input a piece of clothing recommended successfully in the recommendation model and generates clothing images of other categories (top, bottom or shoes) to build up a set of complementary items. They evaluate GAN performance with three index: Inception score related to the quality of the generated image~\cite{DBLP:conf/nips/SalimansGZCRCC16}, Opposite SSIM related to the diversity~\cite{DBLP:conf/icml/OdenaOS17}, and a proposed \textit{Compatibility index} to measure the compatibility of the generated set of complementary items. They compare the model with DCGAN as there are not baseline methods for such comparison. ~\futureworks{Can be interesting to focus on this field and try to propose new models a a baseline way to compare images?}.
% A similar approach has been proposed also in~\cite{2019arXiv190605596K}, to generate bottom fashion item paired with a given top item.







==> OLD_FILES/OLD_Sec4_B_AdvReg.tex <==
\subsection{Adversarial Regularization}

Under CF models there is a huge set of publications that starting from an assessment of model vulnerability to adversarial perturbations then they propose adversarial-based optimization framework to enhance the robustness of a recommender model and thus improve its generalization performance.
We identify in \hlmethod{Adversarial Personalized Ranking} (APR)~\cite{DBLP:conf/sigir/0001HDC18} the first fundamental work inside this field. Lots of publications have taken inspiration from APR. 

\qquad Xiangnan \textit{et al.}~\cite{DBLP:conf/sigir/0001HDC18}, inspired by advances on adversarial machine learning in failing many state-of-the-art classifiers with \textit{adversarial examples}~\felice{We should have defined in Chapter 2(Definition Reference)}, are the first authors that explore adversarial learning methods on item recommendation. 
\\Recognising the in-feasibility of generating adversarial perturbations directly on the discrete features of a recommender model (i.e., user-id, item-id, ratings and other categorical values) they start by investigating the robustness of BPR-MF at perturbations on embedding parameters.
For adversarial perturbations, they define it as the perturbations that aim to maximize the objective function of BPR:
\begin{equation}
    \small
    \label{eq:adv_perturbation}
    \Delta_{adv}=\arg \max _{\Delta, \| \Delta| | \leq \epsilon} \mathcal{L}_{BPR}(X | \Omega+\Delta)
\end{equation}
where $\epsilon$ controls the magnitude of adversarial perturbations, $|| \cdot ||$ denotes the $L_{2}$ norm, $\Omega$ is a constant set denoting the current model parameters, and $X$ denotes the set of pairwise training instances.
Inspired by the Fast Gradient Sign Method (FGSM) proposed in Goodfellow \textit{et al.}~\cite{DBLP:journals/corr/GoodfellowSS14}, they approximate the objective function by linearizing it round $\Delta$. With this approximation and the max-norm constraint, the adversarial perturbation is
\begin{equation}
    \small
    \label{eq:fgsm_adv_perturbations}
    \Delta_{adv}=\epsilon \frac{\Gamma}{\|\Gamma\|} \quad \text { where } \quad \Gamma=\frac{\partial \mathcal{L}_{BPR}(X | \Omega+\Delta)}{\partial \Delta}
\end{equation}
and $ \mathcal{L}_{BPR}$ is the objective function of BPR.
The authors verify the existence of vulnerability to adversarial perturbations and develop \hlmethod{Adversarial Personalized Ranking} (APR), a novel adversarial learning framework for personalized ranking that leads to robust recommender models that are insensitive to such adversarial perturbations.
\\The authors define the objective function of adversarial personalized ranking as follows
\begin{equation}
    \label{eq:j_apr}
    \small
    J_{APR}(X | \Omega)=\mathcal{L}_{BPR}(X | \Omega)+\lambda \mathcal{L}_{BPR}(X | \Omega+\Delta_{adv})
\end{equation}
where $\mathcal{L}_{BPR}(X | \Omega+\Delta_{adv})$ is the \textit{adversarial term} that can be seen as the \textit{regularizer term} of the model to stabilize the classification function in BPR.
looking at Equation~\ref{eq:j_apr}, the training process of APR can be expressed as playing the typical \textit{minimax game} where the
learning algorithm for model parameters $\Omega$ is the \textbf{minimizing} player, and the procedure for getting perturbations $\Delta$ acts as the \textbf{maximizing} player, which aims to build the worst-case perturbations against the current model. The minimax game evidences that APR is a general learning framework which is model independent.  Formally.
\begin{equation}
    \small
    \label{eq:minmax_apr}
    \Omega^{*}, \Delta^{*}=\arg \min _{\Omega} \max _{\Delta,| | \Delta| | \leq \epsilon} \mathcal{L}_{BPR}(X | \Omega)+\lambda \mathcal{L}_{B P R}(X | \Omega+\Delta_{adv})
\end{equation}
The authors employ APR on user and item embedding vectors of BPR-MF in a novel adversarial regularized model named Adversarial Matrix Factorization (AMF). The predicted  model with adversarial perturbations is defined as 
\begin{equation}
    \small
    \label{eq:amf_adv}
    \textbf{r}_{u i} = (\mathbf{p}_{u}+\Delta_{u})^{T}(\mathbf{q}_{i}+\Delta_{i})
\end{equation}
where $\Delta_{u} \in \mathbb{R}^{K}$ and $\Delta_{i} \in \mathbb{R}^{K}$ denote the perturbation vector for user $u$ and item $i$, respectively.
They evaluate the proposed model with three publicly available datasets and verify that, by training MF with APR, the model becomes less sensitive to adversarial perturbations compared to that the same model without adversarial regularization. Then, the performance evaluation show that AMF achieves the best results in most cases in comparing its TOP@\textit{k} recommendations ($k=50, k=100$) with ItemPop, BPR-MF, CDAE, NeuMF and IRGAN.

Inspired by ~\cite{DBLP:conf/sigir/0001HDC18}, Feng \textit{et al.}~\cite{DBLP:conf/sigir/YuanYB19, DBLP:conf/ijcnn/YuanYB19} address the problem setting related to the impact of \hltask{adversarial noises on the model non-linearity} by proposing \hlmethod{Fine-Grained Adversarial Collaborative AutoEncoder} (FG-ACAE).
The authors employ an adversarial training on a modified version of collaborative denoising auto-encoder (CDAE) model~\cite{DBLP:conf/wsdm/WuDZE16} by adding adversarial perturbations on different hidden weights of CDAE. Similarly to Equation~\ref{eq:j_apr}, th objective function is
\begin{equation}
    \small
    J_{FG-ACAE}= \mathcal{L}_{CAE}(X,\Omega)+\sum_{i=1}^{S} \lambda_{i} \mathcal{L}_{CAE}(X, \Omega + \alpha_{i} \Delta_{i} )
\end{equation}
where $S$ is the set of CAE layers where adversarial noises are added, $\alpha_{i}$ denotes the noise coefficient, $\Delta_{i}$ denotes the additive adversarial noise, $\lambda_{i}$ controls the adversarial regularization strength.
The authors show salient improvements on performance and robustness by carrying out standard experiments on three different datasets with respect to highly competitive state-of-the-art recommendation models, ItemPop, BPR-MF, CDAE, JRL~\cite{DBLP:conf/cikm/ZhangACC17}, NeuMF, ConvNCF~\cite{DBLP:conf/ijcai/0001DWTTC18} and AMF.

Adversarial regularization has been also proposed in multimedia recommendation by Tang \textit{et al.}~\cite{8618394}. The authors introduce an adversary which adds adversarial perturbations on multimedia content with the aim of maximizing the Visual Bayesian Personalized Ranking (VBPR)~\cite{DBLP:conf/aaai/HeM16} loss function, the image-based recommender model under their study. They propose \hlmethod{Adversarial Multimedia Recommendation} (AMR) likewise the Adversarial Personalized Recommendation~\cite{DBLP:conf/sigir/0001HDC18}.
Similar to Equation~\ref{eq:amf_adv}, the rating prediction of the perturbed model is formulated as
\begin{equation}
    \small
    \label{eq:amr_adv}
    \textbf{r}_{u i} = \mathbf{p}_{u}^{T} \big(\mathbf{q}_{i}+ E \cdot (c_{i} + \Delta_{i})\big)
\end{equation}
where $c_{i} $ denotes the visual feature vector for item $i$, and $E$ converts the visual feature vector to latent space. The overall objective function, the general learning framework and the learning of the adversarial perturbations are respectively the same in Equation~\ref{eq:j_apr}, ~\ref{eq:minmax_apr} and ~\ref{eq:fgsm_adv_perturbations}.
Experiments on two real-world datasets demonstrate performance advances of AMR with respect to ItemPop, BPR-MF, MF-eALS~\cite{DBLP:conf/sigir/HeZKC16}, DUIF~\cite{DBLP:conf/iccv/GengZBC15} and VBPR.


Park \textit{et al.}~\cite{DBLP:conf/www/ParkC19} address the vulnerability to adversarial examples by proposing and adversarial sampling-based training to build robust models. Differently from IRGAN, they do not use a GAN to generate examples, but they generate adversarial examples by adding adversarial noise on the unlabelled ones. At the same time, with the goal to generate negative adversarial examples closer to the distribution of labeled example they apply a particular application of Adversarial Training. Instead of generating virtual adversarial perturbation for all unlabeled documents, the authors selectively generate them for difficult ones. Experiments show performance improvement on BPR, LambdaFM and IRGAN.

Differently from APR, they propose to add perturbations directly on the input vector and not on the embedding vector. 





we also explore\textbf{ virtual adversarial training} that can be promising for semi-supervised learning, which is not stud- ied in their work.

%%%%%
Cheng \textit{et al.}~\cite{DBLP:journals/tmm/DuFYXCT19} address the problem settings related to the ~\hltask{white box attacks} against collaborative filtering systems under which attackers have the knowledge of the target model. The authors use C\&W  attack~\cite{DBLP:conf/sp/Carlini017}, one of the strongest white-box attack methods, to show how adversary craft malicious user or item data to alter the performance of neural network-based collaborative filtering models. Due to the categorical nature of \textit{implicit feedback} prediction problem, they slightly change the adversarial goal of C\&W attack is 
\begin{equation}
    \label{eq:carlini_attack}
    \small
    \min _{\Delta_{u}, \Delta_{i}}\|\Delta_{u}\|+\|\Delta_{i}\|+c \cdot f(\mathbf{p}_{u}+\Delta_{u}, \mathbf{q}_{i}+\Delta_{i})
\end{equation}
where $c$ is a suitable constant and $f$ the neural collaborative filtering algorithm.
The author propose a novel student-teacher framework by adding extra noise layers before dense layers in the student model to improve its robustness to adversarial perturbations. The proposed model is named \hlmethod{feature-based neural collaborative filtering model} (FNCF) based on multi-layer perceptron model (MLP). The authors compare FNCF's vulnerability performance between MLP-based and Distillation-based training strategies. Results demonstrate that FNCF-MLP is less vulnerable than FNCF-Distilled.

Vagliano \textit{et al.}~\cite{DBLP:conf/recsys/VaglianoGMS18} and Tran \textit{et al.}~\cite{DBLP:conf/sigir/TranSL19} aim to solve the task of \hltask{automatic playlist continuation (APC)}~\cite{DBLP:journals/ijmir/SchedlZCDE18}. Where the system may generate a list of recommended tracks that can \textit{continue} the current playlist; specifically, the task is to \hltask{predict the missing tracks in a playlist}. 
\\The authors of~\cite{DBLP:conf/recsys/VaglianoGMS18}, inspired by AAE~\cite{DBLP:journals/corr/MakhzaniSJG15}, propose a GAN-based framework to ~\hlmethod{adversarially regularize} the autoencoder used to predict the next-track in a playlist. 
A binary classifier acts as the discriminator $D$ and the \textit{encoder} component of the autoencoder acts as the generator $G$. $D$ is trained to distinguish between the output of $G$ and a sample from a prior distribution, while $G$ is trained to generate a latent representation of its input capable to fool $D$. 
Let consider a playlist as a user $u$ and the track as an item $i$, then the objective function of $G$ and $D$ is Eqs.~\ref{equation:irgan_g} and~\ref{equation:irgan_d}.
The overall objective function is a combination between both the adversarial and the autoencoder training. 
As a result, the autoencoder is jointly optimized for for both matching the reconstruction of the input and a prior distribution, e.g. a Gaussian distribution. Note that the authors integrated also side information during the reconstruction phase of the input.
Experiments demonstrate the effectiveness of their model compared to Item Co-Occurrence(IC)~\cite{DBLP:journals/jasis/Small73}, Singular Value Decomposition for recommendation~\cite{Caragea:2013:CSF:2467696.2467743}, and a generic MLP and AE. The same approach has been proposed by the authors in~\cite{DBLP:conf/um/GalkeMVS18} on the citation recommendation task.
\\
The authors of~\cite{DBLP:conf/sigir/TranSL19} address the APC problem by modelling complex interactions among users, playlists, and songs using different model based on Mahalanobis distance~\cite{DBLP:journals/jmlr/WeinbergerS09}. Inspired by~\cite{DBLP:conf/sigir/0001HDC18} (see Section~\felice{XXX}), they apply an \hlmethod{adversarial training} step to further improve the robustness of their models. Through extensive experiments they show that all the proposed models using APR loss improve over the best baseline. 

Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} investigate \hltask{query recommendation systems} in order to improve the suggestion performance by understanding and modeling user search intents accurately. The authors propose a novel model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), that provides query suggestions considering the sequential search queries issued by the user and and his the history of clicks on last suggestions. Similarly to APR~\cite{DBLP:conf/sigir/0001HDC18}, they employ an adversarial training stage during the training of CFAE by injecting adversarial examples built by adding adversarial perturbations of item embeddings.~\felice{It is necessary to define in a Section the procedure user to create adversarial perturbations. They use FSGM}.
Experiments on a e-shopping domain dataset demonstrate that adversarial training on CFAN not only significantly \textit{improve the robustness} of the model but also outperforms the baseline methods for the task of query suggestion.


Chen et Li~\cite{DBLP:conf/recsys/ChenL19} propose \hlmethod{Adversarial Tensor Factorization} (ATF), Particularly, they combine tensor factorization and adversarial learning to improve the robustness of Pairwise Interaction Tensor Factorization (PITF)~\cite{DBLP:conf/wsdm/RendleS10} by injecting adversarial perturbations$\Delta$ on latent factors of PITF to quantify the loss of a tensor model under perturbations on its parameters. Comparison with standard tensor models in tag recommendations demonstrates that ATF outperforms existing baselines on tested datasets.

==> OLD_FILES/OLD_Sec4_C_Others.tex <==
\subsection{Others}\label{subsec:others}

Adversarial Machine Learning techniques are used also to address specific tasks which are independent of the recommender model.

\subsubsection{Privacy}
Attribute inference attacks are emerging issues to user privacy in recommender systems domain~\cite{DBLP:conf/recsys/WeinsbergBIT12, DBLP:conf/cikm/Otterbacher10}. The attacker aims to infer a user's private attributes (e.g., gender, sexual orientation, political and religion views) via leveraging its public data (e.g., in recommender systems, it could be the list of rated items).

Recognising existing defense methods against attribute inference attacks are either computationally intractable or computationally tractable - but they add a large amount of noise to a user's public data; Jia \textit{et al.}~\cite{jia2018attriguard} propose ~\hlmethod{AttriGuard} a computationally tractable defense mechanism that adds small noise. The proposed defense method works in two phases. Firstly, it finds such minimum adversarial noise to evade the attacker's classifier. through an optimized version of \textit{evasion attack} developed by Papernot \textit{et al.}~\cite{DBLP:conf/eurosp/PapernotMJFCS16}, named \hlmethod{Policy-Aware Noise Finding Algorithm} (PANDA). Then, AttriGuard randomly selects one of the adversarial noise found previously to mislead the attacker's inference. The authors evaluate AttriGuard and compare it with existing defenses using a real-world dataset. Results demonstrate that the proposed evasion attack outperforms existing ones (FGSM, JSMA~\cite{DBLP:conf/eurosp/PapernotMJFCS16} and C\&W), and the proposed defense mechanism, AttriGuard, is effective at defending against attribute inference attacks. Otherwise it adds significantly smaller noise to users' public data than existing defenses.

Resheff \textit{et al.}~\cite{DBLP:conf/icpram/ResheffESS19} addresses the problem setting of the \hltask{leakage of private information} in recommender systems. The proposed privacy-adversarial framework in addition to eliminating such leakage it helps to guarantee fairness of results.
Inspired by the Domain Adversarial Training~\cite{DBLP:series/acvpr/GaninUAGLLML17}, the proposed method points to construct a user representation from which the private information can not be read out. This is achieved by training the model with an additive loss for the privacy protection.
This is achieved by application of the gradient reversal trick~\cite{DBLP:series/acvpr/GaninUAGLLML17} which leads to the following update rule for user embedding $p_{u}$:
\begin{equation}
    \small  
    \label{eq:panda_optimization}
    p_{u} \leftarrow p_{u}-\alpha\left[\frac{\partial \mathcal{L}_{recsys}}{\partial p_{u}}
    - 
    \lambda \sum_{i} \frac{\partial \mathcal{L}_{private_{i}}}{\partial p_{u}}\right]
\end{equation}
where $\alpha$ is the learning rate, $\lambda$ is the adversarial learning rate, and $ \mathcal{L}_{recsys}$ and $\mathcal{L}_{private_{i}}$ are the loss function of the recommender model and the adversarial privacy-protection component appended to the recommender model. Experiments on movie recommendation domain show the effectiveness of the proposed method in reducing the leakage of user's personal data.


\subsubsection{Adversarial Machine Learning for Shilling Attacks}

\textbf{Adversarial Attacks on an Oblivious Recommender} by Konstantina Christakopoulou, Arindam Banerjee HAD BEEN ACCEPTED IN RECSYS2019. 
I am waiting for it because it is the long paper version of \textbf{Adversarial Recommendation: Attack of the Learned Fake Users}~\cite{DBLP:journals/corr/abs-1809-08336}.
They propose a framework for generating \hltask{shilling profiles} which, when incorporated in the training of a recommendation system, can achieve an adversarial intent, while remaining \textbf{indistinguishable from real user profiles}. The generation is mapped with a GAN-based framework where the Discriminator is the recommender model and the generator is the component that tries ot imitate the real distribution of users by looking to manipulate the recommendations.


\newpage



==> OLD_FILES/OLD_Sec4_Technical.tex <==
\section{ADVERSARIAL LEARNING BASED RECOMMENDATION: Technical Overview}\label{sec:TechnicalSection}
\felice{FIRST DRAFT VERSION}
In this section, we firstly introduce the application of adversarial machine learning based recommendation models and then highlight state-of-the-art research prototypes, aiming to identify the most notable and promising advancement in recent years.~\felice{Need paraphrasing}

We focus on technical and architectural solution in recommender systems looking at the application of adversarial learning in a GAN-based framework and the use of adversarial learning as a regularization parameters.    


\felice{Table Idea 1: A table where for each proposed model we can set:\\ TASK - Proposed Model - \textbf{Baseline} - \textbf{Metrics}}

\felice{Table Idea 2: At the end of the chapter we can Put a Table with:\\ Goal - Paper Name - Dataset - Public Available - Metrics }

\felice{Table Idea 3: Try to fix the Variable for the Formalism at create a TABLE with all the formula in a single table}


\subsection{GAN-based Recommender Systems}
This Section focus on different application of Generative Adversarial Network in recommendation domain. As there are different uses of GAN which depend from the type of recommendation, we present different proposed framework 



\subsection{Adversarial Regularization}

\subsection{Collaborative Filtering}\label{subsec:CF}
In this section we focus on technical overview of GAN-based approach and pre Adversarial-learning Approach in collaborative filtering recommender model.

\subsubsection{GAN-based Collaborative Filtering}

% IRGAN
\qquad\textit{IRGAN}~\cite{DBLP:conf/sigir/WangYZGXWZZ17} is the pioneering work that proposes a GAN-based method in Recommender Systems. The authors address the \hltask{rating prediction} and item \hltask{recommendations} proposing a \hlmethod{minimax game} to combine the rating \textit{generative} process and the learning to rank \textit{discriminative} process.
They model the minimax game between the generative and discriminative model in a GAN-based approach, named IRGAN, looking at the conditional GAN (CGAN)~\cite{DBLP:journals/corr/MirzaO14} , as both $G$ and $D$ are user-conditioned take \textbf{user-personalization} into account.

The \textit{Generator} tries to generate relevant items by approximating the true relevance distribution over items, $p_{\text { true }}(i | u, r)$, while the \textit{Discriminator} tries to distinguish between the generated and the ground-truth relevant items.
Formally:
\begin{equation}
     \small
     \label{equation:irgan}
     J(\theta, \phi)= \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
 \end{equation}
where $\theta$ parameterized the generator $p_{\theta}(\hat{i} | u_{n}, r)$ and $\phi$-parameterized the discriminator $D_{\phi}$. The generator maps a conditioned user vector $u_{z}$, to a generated relevant item. \\
The discriminator is trained to maximize such an objective with the fixed generator $G_{\theta}$
\begin{equation}
    \label{equation:irgan_max_d}
    \phi^{*}=\arg \max _{\phi} J(\theta, \phi) = \arg \max _{\phi} J^{D}
\end{equation}
\begin{equation}
    \label{equation:irgan_d}
    J^{D} = \mathbb{E}_{i \sim p_{\text { true }}(i | u, r)}[\log D_{\phi}(i | u)]+ \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
\end{equation}
while the generator is trained to minimize such an objective with the fixed discriminator $D_{\phi}$
\begin{equation}
    \small
    \theta^{*}=\arg \min _{\theta} J(\theta, \phi)=\arg \min _{\theta} \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}(\hat{i} | u)))]
\end{equation}
and, as claimed in the original GAN paper~\cite{DBLP:conf/nips/GoodfellowPMXWOCB14}
\begin{equation}
    \small
    \label{equation:irgan_min_g}
    \theta^{*} = \arg \min _{\theta} ( -  \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}(\hat{i} | u)))] ) = \arg \min _{\theta} J^{G}
\end{equation}
\begin{equation}
    \small
    \label{equation:irgan_g}
    J^{G} = - \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}(\hat{i} | u)))]
\end{equation}
Where $J_{D}$ and $J_{G}$ are the objective function~\footnote{We define the $J_{D}$ objective functions to be a maximization problem and $J_{G}$ a minimization problem.} of the GAN. \\
Note that they do not use the random noise variable $z$ like in classic GAN Eq.~\ref{equation:gan} since the goal is to generate a single, most plausible recommended item to a user rather than different relevant items.
As the sampling of $i$ is discrete, it cannot be directly optimised by gradient descent as in the original GAN formulation. Authors were the first to employ the \textit{policy-gradient based reinforcement learning} (REINFORCE)~\cite{DBLP:journals/ml/Williams92} to optimize the generator.
The authors empirically explores the effectiveness of the proposed method on the widely used matrix factorization~\cite{DBLP:journals/computer/KorenBV09} model in the movie domain with significant performance gains with respect to BPR~\cite{DBLP:conf/uai/RendleFGS09} and LambdaFM~\cite{DBLP:conf/cikm/YuanGJCYZ16}.
This work inspired a lot of new works to test GAN in Recommendation domain.

% CFGAN
\qquad Chae \textit{et al.} ~\cite{DBLP:conf/cikm/ChaeKKL18} address a qualitative problem in the IRGAN training algorithm. The authors identify the limitation of IRGAN and GraphGAN (see Section) in their \hltask{generation of discrete items} by verifying a worsening of recommendation performances when the number of epochs increase. As the training is further progressed, $G$ gets to sample frequently the items exactly same as those in ground truth. Since $D$ receives the same item index sometimes like a \textit{fake} element and sometimes like a \textit{ground-truth} one, it gets confused and, after few epochs, it starts to perform worse.
Beginning with such limitations, the authors propose a novel adversarial training, named \hlmethod{vector-wise training}, where $G$ \textit{generates real-valued vectors}. The proposed approach is named CFGAN, and it is based on a conditional GAN (CGAN). Formally, the important change compared to IRGAN overall objective function is in the $G$ Equation~\ref{equation:irgan_g}:
\begin{equation}
 \label{equation:cfgan_g}
 \small
 J^{G}=\mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}((\hat{i}\odot{e} ) | u))] = - \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (D_{\phi}((\hat{i}\odot{e} ) | u))]
 % J^{G}=\sum_{n=1}^{N} \log (1-D_{\phi}((\hat{i}\odot{e_{n}} ) | u_{n}))
\end{equation}

\begin{equation}
 \label{equation:cfgan_d}
 \small
 J^{D}= \mathbb{E}_{i \sim p_{\text { true }}(i | u_{n}, r)}[\log D_{\phi}(i | u_{n})] + \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u, r)}[\log (1-D_{\phi}((\hat{i}\odot{e} ) | u))]
 % J^{G}=\sum_{n=1}^{N} \log (1-D_{\phi}((\hat{i}\odot{e_{n}} ) | u_{n}))
\end{equation}
where $e$ in Eq.~\ref{equation:cfgan_g} is an $n$-dimensional vector specifying whether $u$ has purchased each item $\hat{i}$
% (eui =1) or not (eui =0),
and $\odot$ stands for element-wise multiplication. The main difference between CFGAN and the original GAN is element-wise multiplication in order to deal with the sparsity in ground-truth data that $G$ tries to mimic.
Experiments on different real-world datasets prove a significant improvement on different baseline methods ItemPop~\cite{DBLP:conf/recsys/CremonesiKT10}, BPR, FISM, CDAE and above all IRGAN and GraphGAN. 

\qquad Moreover, Chae \textit{et al.}~\cite{8525831, DBLP:journals/access/ChaeSK19} point out an issue regarding the employment of a linear model as the basic CF core of IRGAN because of non-ability to \hltask{capture non-linear interactions of users' and items'} latent factors to have better item-recommendations. Because of~\cite{DBLP:journals/access/ChaeSK19} is an extension of ~\cite{8525831} we deep in the extended one. Their main contribution is an advanced GAN-based CF framework, named \hlmethod{Collaborative Adversarial autoencoders} (CAAE), which is innovatively composed by three components: \textit{positive item generator} ($G$) , \textit{negative item generator} ($G^{\prime}$), and \textit{discriminator} ($D$). Generators are implemented with an autoencoder and the discriminator with BPR-MF~\cite{DBLP:conf/uai/RendleFGS09}.
Formally:
\begin{equation}
 \small
 \label{equation:cfgan2_d}
 J^{\mathcal{D}}= - \mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta} o r \hat{i} \sim p_{\theta^{\prime}}(\hat{i} | u)}[\log D_{\phi}(i, \hat{i} | u)]
\end{equation}
\begin{equation}
 \small
 \label{equation:cfgan2_g}
 J^{G}=\lambda \cdot \big( -\mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta}(\hat{i} | u)}[\log (1-D_{\phi}(i, \hat{i} | u))] \big) +(1-\lambda) \cdot  \mathcal{L}_{AE}
\end{equation}

\begin{equation}
 \small
 \label{equation:cfgan2_g_first}
 J^{G^{\prime}}=-\mathbb{E}_{i \sim p_{\text {true}}(i | u), \hat{i} \sim p_{\theta^{\prime}}(\hat{i} | u)}[\log {D}(i, \hat{i} | u)) ]
\end{equation}
where $\mathcal{L}_{AE}$ in Eq.~\ref{equation:cfgan2_g} is the loss function of the autoencoder of the positive example generator, $\lambda$ parameterized its importance regard to generative loss function and $\theta^{\prime}$ is the set of model parameters of the second generator ($G^{\prime}$).
Note that the objective of $G^{\prime}$ is to help $D$ to \hlmethod{correctly discriminate} $G^{\prime}$ \textit{real} items from \textit{fake} items coming from $G^{\prime}$ to help $D$ to capture the difference between positive and negative items and $G$ to decrease the likelihood of generating items that the user may not prefer. Experiments on recommendation accuracy of CAAE framework with some well-known baselines demonstrate significant improvement on IRGAN and comparable performances on CFGAN.

\qquad Inspired by CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18}, a \hlmethod{GAN-based Rating Augmentation framework with \textit{bias treatment}}, named $RAGAN^{BT}$, has been proposed by Kim \textit{et al.}~\footnote{The same group of Authors of CFGAN} to alleviate the \hltask{data sparsity} problem in collaborative filtering (CF) by generating additional labeled data, which is called data augmentation. They propose a bias treatment to avoid $G$ from being biased towards high ratings in rating augmentation. This challenge is addressed by training the GAN on a modified version of original rating matrix where they add low ratings to the negative items.  
Formally, the objective function of generator and discriminator are the same in Equations~\ref{equation:cfgan_g} and ~\ref{equation:cfgan_d}.
After training of GAN is completed, the generated ratings on unrated items are used to augment the original rating matrix. 
They validate the effectiveness of $RAGAN^{BT}$ on four real-world datasets. The results demonstrate that the proposed data augmentation strategy outperforms the state-of-the-art CF models not only under basic top-N recommendations, but also under (i) \hltask{long-tail item} recommendations and (ii) recommendations to cold-start users. Compared models are: ItemPop, Item\textit{k}NN, SVD~\cite{DBLP:journals/computer/KorenBV09}, SVD++~\cite{DBLP:conf/kdd/Koren08}, AutoRec, PureSVD~\cite{DBLP:conf/recsys/CremonesiKT10} and Zero-Injection~\cite{DBLP:conf/icde/HwangPKLL16}.

The \hltask{long-tail phenomenon} in recommender performance is addressed also by \textit{Krishnan et al.}~\cite{DBLP:conf/cikm/KrishnanSSS18}. They propose and GAN-based approach to augment Neural Collaborative Filtering training to levy penalties when the recommender fails to identify suitable niche items for users, given their history and global item co-occurrence. 
The discriminator learns the inter-item association structure in the feedback data and correlates the generated niche item recommendations with popular items in the user's history. The generator must produce synthetic niche item recommendations that are correlated with the user's history. The effectiveness of the proposed method is evaluated on VAE and CDAE by measuring performance gains in niche-item on two real-world datasets. Results demonstrate that the proposed approach outperforms long-tail performances on the same model without the adversarial training. 

\qquad Sun \textit{et al.}~\cite{DBLP:journals/eswa/SunWWY19} address the problem settings of the \hltask{unstable and slow convergence adversarial training on a huge number of items}~\cite{DBLP:conf/sigir/WangYZGXWZZ17}. They propose (i) a GAN-based recommendation method, namely \hlmethod{Adversarial Pairwise Learning} (APL), for improving the training process of the adversarial model, by accelerating the convergence and enhancing the stability; and (ii) a \hlmethod{differentiable procedure}~\cite{DBLP:conf/iclr/JangGP17} to imitate the discrete item generation process and optimize APL with gradient descent directly instead of REINFORCE~\cite{DBLP:journals/ml/Williams92} used in most works (see Table~\felice{TABLE WITH STATISTICS ON TECHNIQUES}). 
The generator $G$ tries to imitate the observed item generation process and generate personalized items for each user; while the discriminator $D$ aims at learning a pairwise ranking function and determining the preferences of each user in preferring real items on generated ones. The novel component is related to the adoption of a Gumbel-Softmax~\cite{DBLP:conf/iclr/JangGP17} module that works as a bridge between $G$ and $D$. This implies that the GAN model is entirely differentiable, and the generator can be optimized with a standard back-propagation algorithm. 
The experiments on real-world datasets showed that (i) APL substantially enhances the convergence and stability of the adversarial learning process; (i) the differentiable item sampling procedure improves the stability of APL; (i) APL achieves state- of-the-art performance with respect to analyzed baseline models. Compared models are ItemPop, UIEM~\cite{DBLP:journals/eswa/NilashiIB18}, BPRMF, LambdaMF, AOBPR~\cite{DBLP:conf/wsdm/RendleF14}, IRGAN.

\textit{Variational Autoencoder to Model Auxiliary Information.}

Lee \textit{et al.}~\cite{DBLP:conf/cikm/LeeSM17} and Zhang \textit{et al.}~\cite{8663730} propose for the first time the use of a Variational Autoencoder~\cite{DBLP:journals/corr/KingmaW13} as the generator in a GAN-based framework with the goal to take implicit feedback data into account for the top-\textit{n} recommendations.
Inspired by the adversarial process used in GAN, Lee \textit{et al.}~\cite{DBLP:conf/cikm/LeeSM17} propose a novel \hlmethod{VAE with Adversarial Regularization} (VAE-AR) framework to improve item recommendation. 
The basic idea is to merge two independent distributions of user-item interactions and auxiliary information in an unique model thanks to the capability of a Variational AutoEncoder to regularize another AutoEncoder through an adversarial \textit{minimax game}. Note that Variational AutoEncoders differ from Adversarial AutoEncoders, used for example in~\cite{DBLP:conf/webi/YiHQ18},. In fact, an AAE enforces prior knowledge on the latent variables of autoencoders, while a VAE regularize another VAE through its own inferred latent representations.  
The evaluation of recommendation performances on two publicly available datasets demonstrates a clear improvement on WRMF~\cite{DBLP:conf/icdm/HuKV08}, BPR~\cite{DBLP:conf/uai/RendleFGS09}, CDL~\cite{DBLP:conf/kdd/WangWY15}, CDAE~\cite{DBLP:conf/wsdm/WuDZE16}, CVAE~\cite{DBLP:conf/ijcnn/PandeyD17} and JMVAE~\cite{DBLP:conf/iclr/SuzukiNM17}. 

Tong \textit{et al.}~\cite{DBLP:conf/icde/TongLZSC19} implement the generator with a VAE in a collaborative scenario without implicit feedback.
They propose \hlmethod{Collaborative Generative Adversarial Network} (CGAN) model to enhance the recommendation performance and the robustness to adversarial examples by taking the advantage of the VAEs nonlinear nature in learning better aggregated posterior distribution from the given data and generate high-quality negative samples to fail the discriminator. Then, the author propose to alleviate the issue of unstable convergence and time-consuming training of classic GAN by using Improved Wasserstein GAN (WGAN-GP)~\cite{DBLP:conf/nips/GulrajaniAADC17}, which removes the log function and adds a gradient penalty term $ W_{pen}$ on the original critic loss. 
The objective functions of G and D are presented as follows:
\begin{equation}
    \label{eq:cf_vae_d}
    \small
    J^{D} = - \mathbb{E}_{i \sim p_{\text {true}}(i | u)}[D_{\phi}(i| u)] + \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u) }[D_{\phi}(\hat{i}| u)] + \lambda W_{pen}
\end{equation}

\begin{equation}
    \label{eq:cf_vae_g}
    \small
    J^{G}= \lambda \cdot \big(- \mathbb{E}_{\hat{i} \sim p_{\theta}(\hat{i} | u) }[D_{\phi}(\hat{i}| u)]\big) + (1 - \lambda) \cdot \mathcal{L}_{VAE}
\end{equation}
where $J^{D}$ is the WGAN-GP objective with the critic term, ${L}_{VAE}$ stands for the loss function of VAE, $\lambda$ parameterized its importance regard to generative loss function. Recommendations are built upon the reconstructed vector of user's ratings by the Variational AutoEncoder in the model.
Experimental evaluation on recommendation performances demonstrate advances on ItemPop, BPR-MF, CDAE, NeuMF~\cite{DBLP:conf/www/HeLZNHC17}, GraphGAN and IRGAN. Then, the authors demonstrate the effectiveness of the adversarial training by utilizing the Wasserstein distance with gradient penalty through an \textit{ablation study}.

\subsubsection{Adversarial Learning in Collaborative Filtering}

Under CF models there is a huge set of publications that starting from an assessment of model vulnerability to adversarial perturbations then they propose adversarial-based optimization framework to enhance the robustness of a recommender model and thus improve its generalization performance.
We identify in \hlmethod{Adversarial Personalized Ranking} (APR)~\cite{DBLP:conf/sigir/0001HDC18} the first fundamental work inside this field. Lots of publications have taken inspiration from APR. 

\qquad Xiangnan \textit{et al.}~\cite{DBLP:conf/sigir/0001HDC18}, inspired by advances on adversarial machine learning in failing many state-of-the-art classifiers with \textit{adversarial examples}~\felice{We should have defined in Chapter 2(Definition Reference)}, are the first authors that explore adversarial learning methods on item recommendation. 
\\Recognising the in-feasibility of generating adversarial perturbations directly on the discrete features of a recommender model (i.e., user-id, item-id, ratings and other categorical values) they start by investigating the robustness of BPR-MF at perturbations on embedding parameters.
For adversarial perturbations, they define it as the perturbations that aim to maximize the objective function of BPR:
\begin{equation}
    \small
    \label{eq:adv_perturbation}
    \Delta_{adv}=\arg \max _{\Delta, \| \Delta| | \leq \epsilon} \mathcal{L}_{BPR}(X | \Omega+\Delta)
\end{equation}
where $\epsilon$ controls the magnitude of adversarial perturbations, $|| \cdot ||$ denotes the $L_{2}$ norm, $\Omega$ is a constant set denoting the current model parameters, and $X$ denotes the set of pairwise training instances.
Inspired by the Fast Gradient Sign Method (FGSM) proposed in Goodfellow \textit{et al.}~\cite{DBLP:journals/corr/GoodfellowSS14}, they approximate the objective function by linearizing it round $\Delta$. With this approximation and the max-norm constraint, the adversarial perturbation is
\begin{equation}
    \small
    \label{eq:fgsm_adv_perturbations}
    \Delta_{adv}=\epsilon \frac{\Gamma}{\|\Gamma\|} \quad \text { where } \quad \Gamma=\frac{\partial \mathcal{L}_{BPR}(X | \Omega+\Delta)}{\partial \Delta}
\end{equation}
and $ \mathcal{L}_{BPR}$ is the objective function of BPR.
The authors verify the existence of vulnerability to adversarial perturbations and develop \hlmethod{Adversarial Personalized Ranking} (APR), a novel adversarial learning framework for personalized ranking that leads to robust recommender models that are insensitive to such adversarial perturbations.
\\The authors define the objective function of adversarial personalized ranking as follows
\begin{equation}
    \label{eq:j_apr}
    \small
    J_{APR}(X | \Omega)=\mathcal{L}_{BPR}(X | \Omega)+\lambda \mathcal{L}_{BPR}(X | \Omega+\Delta_{adv})
\end{equation}
where $\mathcal{L}_{BPR}(X | \Omega+\Delta_{adv})$ is the \textit{adversarial term} that can be seen as the \textit{regularizer term} of the model to stabilize the classification function in BPR.
looking at Equation~\ref{eq:j_apr}, the training process of APR can be expressed as playing the typical \textit{minimax game} where the
learning algorithm for model parameters $\Omega$ is the \textbf{minimizing} player, and the procedure for getting perturbations $\Delta$ acts as the \textbf{maximizing} player, which aims to build the worst-case perturbations against the current model. The minimax game evidences that APR is a general learning framework which is model independent.  Formally.
\begin{equation}
    \small
    \label{eq:minmax_apr}
    \Omega^{*}, \Delta^{*}=\arg \min _{\Omega} \max _{\Delta,| | \Delta| | \leq \epsilon} \mathcal{L}_{BPR}(X | \Omega)+\lambda \mathcal{L}_{B P R}(X | \Omega+\Delta_{adv})
\end{equation}
The authors employ APR on user and item embedding vectors of BPR-MF in a novel adversarial regularized model named Adversarial Matrix Factorization (AMF). The predicted  model with adversarial perturbations is defined as 
\begin{equation}
    \small
    \label{eq:amf_adv}
    \textbf{r}_{u i} = (\mathbf{p}_{u}+\Delta_{u})^{T}(\mathbf{q}_{i}+\Delta_{i})
\end{equation}
where $\Delta_{u} \in \mathbb{R}^{K}$ and $\Delta_{i} \in \mathbb{R}^{K}$ denote the perturbation vector for user $u$ and item $i$, respectively.
They evaluate the proposed model with three publicly available datasets and verify that, by training MF with APR, the model becomes less sensitive to adversarial perturbations compared to that the same model without adversarial regularization. Then, the performance evaluation show that AMF achieves the best results in most cases in comparing its TOP@\textit{k} recommendations ($k=50, k=100$) with ItemPop, BPR-MF, CDAE, NeuMF and IRGAN.

Inspired by ~\cite{DBLP:conf/sigir/0001HDC18}, Feng \textit{et al.}~\cite{advcol19sigir, DBLP:journals/corr/abs-1808-05361} address the problem setting related to the impact of \hltask{adversarial noises on the model non-linearity} by proposing \hlmethod{Fine-Grained Adversarial Collaborative AutoEncoder} (FG-ACAE).
The authors employ an adversarial training on a modified version of collaborative denoising auto-encoder (CDAE) model~\cite{DBLP:conf/wsdm/WuDZE16} by adding adversarial perturbations on different hidden weights of CDAE. Similarly to Equation~\ref{eq:j_apr}, th objective function is
\begin{equation}
    \small
    J_{FG-ACAE}= \mathcal{L}_{CAE}(X,\Omega)+\sum_{i=1}^{S} \lambda_{i} \mathcal{L}_{CAE}(X, \Omega + \alpha_{i} \Delta_{i} )
\end{equation}
where $S$ is the set of CAE layers where adversarial noises are added, $\alpha_{i}$ denotes the noise coefficient, $\Delta_{i}$ denotes the additive adversarial noise, $\lambda_{i}$ controls the adversarial regularization strength.
The authors show salient improvements on performance and robustness by carrying out standard experiments on three different datasets with respect to highly competitive state-of-the-art recommendation models, ItemPop, BPR-MF, CDAE, JRL~\cite{DBLP:conf/cikm/ZhangACC17}, NeuMF, ConvNCF~\cite{DBLP:conf/ijcai/0001DWTTC18} and AMF.

Adversarial regularization has been also proposed in multimedia recommendation by Tang \textit{et al.}~\cite{DBLP:journals/corr/abs-1809-07062}. The authors introduce an adversary which adds adversarial perturbations on multimedia content with the aim of maximizing the Visual Bayesian Personalized Ranking (VBPR)~\cite{DBLP:conf/aaai/HeM16} loss function, the image-based recommender model under their study. They propose \hlmethod{Adversarial Multimedia Recommendation} (AMR) likewise the Adversarial Personalized Recommendation~\cite{DBLP:conf/sigir/0001HDC18}.
Similar to Equation~\ref{eq:amf_adv}, the rating prediction of the perturbed model is formulated as
\begin{equation}
    \small
    \label{eq:amr_adv}
    \textbf{r}_{u i} = \mathbf{p}_{u}^{T} \big(\mathbf{q}_{i}+ E \cdot (c_{i} + \Delta_{i})\big)
\end{equation}
where $c_{i} $ denotes the visual feature vector for item $i$, and $E$ converts the visual feature vector to latent space. The overall objective function, the general learning framework and the learning of the adversarial perturbations are respectively the same in Equation~\ref{eq:j_apr}, ~\ref{eq:minmax_apr} and ~\ref{eq:fgsm_adv_perturbations}.
Experiments on two real-world datasets demonstrate performance advances of AMR with respect to ItemPop, BPR-MF, MF-eALS~\cite{DBLP:conf/sigir/HeZKC16}, DUIF~\cite{DBLP:conf/iccv/GengZBC15} and VBPR.


Park \textit{et al.}~\cite{DBLP:conf/www/ParkC19} address the vulnerability to adversarial examples by proposing and adversarial sampling-based training to build robust models. Differently from IRGAN, they do not use a GAN to generate examples, but they generate adversarial examples by adding adversarial noise on the unlabelled ones. At the same time, with the goal to generate negative adversarial examples closer to the distribution of labeled example they apply Selective Virtual Adversarial Training~\cite{miyato2015distributional}. Instead of generating virtual adversarial perturbation for all unlabeled documents, the authors selectively generate them for difficult ones. Experiments show performance improvement on BPR, LambdaFM and IRGAN.

Differently from APR, they propose to add perturbations directly on the input vector and not on the embedding vector. 





we also explore\textbf{ virtual adversarial training} that can be promising for semi-supervised learning, which is not stud- ied in their work.

%%%%%
Cheng \textit{et al.}~\cite{DBLP:journals/tmm/DuFYXCT19} address the problem settings related to the ~\hltask{white box attacks} against collaborative filtering systems under which attackers have the knowledge of the target model. The authors use C\&W  attack~\cite{DBLP:conf/sp/Carlini017}, one of the strongest white-box attack methods, to show how adversary craft malicious user or item data to alter the performance of neural network-based collaborative filtering models. Due to the categorical nature of \textit{implicit feedback} prediction problem, they slightly change the adversarial goal of C\&W attack is 
\begin{equation}
    \label{eq:carlini_attack}
    \small
    \min _{\Delta_{u}, \Delta_{i}}\|\Delta_{u}\|+\|\Delta_{i}\|+c \cdot f(\mathbf{p}_{u}+\Delta_{u}, \mathbf{q}_{i}+\Delta_{i})
\end{equation}
where $c$ is a suitable constant and $f$ the neural collaborative filtering algorithm.
The author propose a novel student-teacher framework by adding extra noise layers before dense layers in the student model to improve its robustness to adversarial perturbations. The proposed model is named \hlmethod{feature-based neural collaborative filtering model} (FNCF) based on multi-layer perceptron model (MLP). The authors compare FNCF's vulnerability performance between MLP-based and Distillation-based training strategies. Results demonstrate that FNCF-MLP is less vulnerable than FNCF-Distilled.

\subsubsection{Other Applications in CF}




\subsection{GAN-based Hybrid Filtering.}\label{subsec:GAN-based Hybrid}

\subsubsection{Graph-based methods.} 

GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18} is the first \hltask{graph representation learning} framework which \hltask{models} generative models, that learn the underlying connectivity distribution in the graph to generate \textit{fake vertex}, and discriminative models, that detect whether a sampled vertex is real or fake; in a GAN way. The authors accomplish the item-recommendation task with a graph representation learning by modeling users and items as vertices and by mapping user-item interaction, e.g. ratings and implicit feedback, with an edge. top-\textit{n} recommendation list is built upon this graph after the training of the model. Since the formulation of minimax problem is the same of IRGAN in Section~\ref{subsec:GAN-based CF} we identify a main contribution in the an alternative neighbor-aware softmax for the generator named \hlmethod{graph softmax} with the goal to overcome the limitations of traditional softmax function: (i) lacking of graph structure because of equal treats of all vertices and (ii) inefficiency due the evaluation of softmax on every vertex.
\\They demonstrate better recommendation performance of GraphGAN by comparing it with other graph representation learning methods: DeepWalk~\cite{DBLP:conf/kdd/PerozziAS14}, LINE~\cite{DBLP:conf/www/TangQWZYM15}, node2vec~\cite{DBLP:conf/kdd/GroverL16}, and struc2vec~\cite{DBLP:conf/kdd/RibeiroSF17}. 

Han \textit{et al.}~\cite{DBLP:conf/aaai/CaiHY18} address the problem of graph-based \hltask{citation recommendation} when heterogeneous content information is associated with each vertex of the network.
They model each paper and author ($i$) as a vertex, the citation as the link ($r$) between vertices and the recommendation task as a \hltask{link prediction problem}. Note that this work is not under collaborative settings with a user-item matrix, but under a content-based setting with an item-item matrix.
The authors propose a GAN-based model, named GAN-HBNR, \hlmethod{to learn an effective feature representation that preserves both vertex content information and network structure information}. 
% Then, this latent representation can be applied to address the  recommendation task.
They employ an energy-based formulation for generative adversarial training, called EBGAN~\cite{DBLP:conf/iclr/ZhaoML17}, where the ground truth is a vertex vector concatenated with its content vector, encoded with \textit{Doc2Vec}~\cite{DBLP:conf/icml/LeM14}.
The discriminator of an EBGAN is implemented with an auto-encoder architecture. The energy function, the MSE, is trained to push down on the reconstruction error of the autoencoder when the input is the ground truth, and to push up when the discriminator input is the generated one. 
The recommendations are made by mapping real-data into the latent space of the trained autoencoder and by producing the recommendation list by taking the most similar ones.
\\Experimental studies verify the effectiveness of the proposed approach compared to DeepWalk, Line, Doc2Vec, TriDNR~\cite{DBLP:conf/ijcai/PanWZZW16} and Node2Vec~\cite{DBLP:conf/kdd/GroverL16}.
% ~\felice{Here I am not inserting any formalism because I don't know how many papers use EBGAN. If I will find a lot of paper I will introduce here the formalism}.
~\futureworks{\textbf{What do you think if we use SemAuto in the Decoder? We should exploit its explainability properties for cold-item}}

% \vspace{5mm} 

\subsubsection{Content-based methods.}

In~\cite{DBLP:conf/icdm/LiH018}, the authors addresses the task of \hltask{Tag-Aware Recommendation}~\cite{DBLP:journals/jcst/ZhangZZ11}.
Formally, the overall loss function is a combination of three components:
\begin{equation}
    \label{equation:TDGAN}
    \small
    J(\theta, \phi, \eta) = \lambda_{1} \cdot f_{1}(R_{\eta}(x)) + \lambda_{2} \cdot f_{2}(G_{\theta}(R_{\eta}(x))) +  \lambda_{3} \cdot f_{3}D_{\phi}((G_{\theta}(R_{\eta}(x))))
\end{equation}
where $\theta, \phi, \eta$ are the model parameters of $G$, $D$ and $R$, $x$ is the input user or item vector, $f_{1}$ measures the relevance scores of items $i$ to a given user $u$, $f_{2}$ is the reconstruction error of the re-generated vector $x$ and $f_{3}$ measures the discrepancy between genuine input and generated one. 
After training, the proposed model predicts results for recommendation by combining linearly the similarity between the extracted abstract from the tag-based profiles of users and items, from $R$, and the tag-based profiles reconstructed by $G$.
Experiments on music domain show better top-\textit{n} recommendation performances compared to baseline methods: CFA~\cite{DBLP:journals/ijon/ZuoZGJ16} and DSPR~\cite{DBLP:conf/ijcai/XuLCMM17}. Furthermore, the authors explore the impact of the discriminator $D$ to implement the adversarial strategy by demonstrating that, without this component, accuracy metrics go down in a significance way.

\qquad The authors of ~\cite{DBLP:conf/webi/YiHQ18} focus on \hltask{solving the sparsity problem} in order to get \hltask{higher recommendation quality} by exploting both user-ratings and user-generated reviews on items. They propose a GAN-based recommendation method, named \hlmethod{aae-RS}, by employing the \textit{minimax game} between the rating relations and review relations of users and items in order to merge the user-item ratings and reviews by making them indistinguishable. The proposed model, inspired by AAE~\cite{DBLP:journals/corr/MakhzaniSJG15}, is composed by three autoencoders, namely $G_{rev}$, $G_{u}$, and $G_{i}$, a discriminator $D$ and a predictor $P$. autoencoders map users' vectors, items' vectors, and users' reviews in a common latent space. The discriminator tries to maximize its ability to distinguish between the user-item vector, the ground truth, and the review vector, the fake sample, while autoencoders try to minimize the difference of the two vectors in an adversarial manner. The prediction is trained to predict a real-value rating given auser-item vector. Formally, the overall objective function is a linear combination of six components:
\begin{equation}
    \label{equation:aae-RS}
    \small
    J = \lambda_{1} \cdot \mathcal{L}_{adv} 
    +  \lambda_{2} \cdot \mathcal{L}_{rec_{rev}} 
    +  \lambda_{3} \cdot \mathcal{L}_{rec_u}
    +  \lambda_{4} \cdot \mathcal{L}_{rec_i} 
    +  \lambda_{5} \cdot \mathcal{L}_{rec_{rev+u+i}}
    +  \lambda_{6} \cdot \mathcal{L}_{pred}
\end{equation}
where $\mathcal{L}_{adv}$ is the adversarial loss, $\mathcal{L}_{rec_{rev}}$ is the reconstruction loss of $G_{rev}$, $\mathcal{L}_{rec_u}$ and $J_{rec_i}$ are the reconstruction losses respective of $G_{u}$ and $G_{i}$, $\mathcal{L}_{rec_{rev+u+i}}$ is the reconstruction loss among the representations of different latent vectors of the same pair of user and item and $\mathcal{L}_{pred}$ is the square loss between the predicted ratings and the real ratings. $\lambda_{j}, j= 1,...,6$ are hyper parameters to weight objective functions. Experiments on e-commerce datasets validate the superiority of aae-RS over HFT~\cite{DBLP:conf/recsys/McAuleyL13}, mDA-CF~\cite{DBLP:conf/cikm/LiKF15}, ConvMF-~\cite{DBLP:conf/recsys/KimPOLY16} and ReDa~\cite{DBLP:journals/nn/ZhuangZQSXH17}.

\qquad Chen \textit{et al.}~\cite{DBLP:journals/tois/ChenZXQZ19} address computational inefficiency of baseline recommendation with external knowledge in practical scenario, i.e. review-based recommendation, by proposing a teacher-student model, named \textit{Generalized Distillation Framework} (GDF). Particularly the use an \hlmethod{adversarial adaption strategy} in order to guarantee the \hltask{effectiveness of the knowledge distillation} from the teacher to the student models of GDF for better \hltask{recommendation performances}.
The minimax-game is played by the user-item prediction network, which works as the generator $G$; and a discriminator $D$. 
$D$ tries to distinguish between the ground truth, the review-embedded vector produced by the Teacher, and the fake example, the user-item embedding vector generated by the Student for fooling $D$. At the end of the game, the user-item prediction network is able to encode review-based user-item relevant information and it achieves better rating prediction as show in the experimental evaluation.


\subsection{GAN-based Sequential Recommender System.}\label{subsec:GAN-based Sequential}
Sequence-aware Recommender Systems are mostly studied in these years to emphasize the significance of modeling short-term and long-term temporal profiles behind temporal evolution of user preference and item state to make relevant suggestions. Different solutions are proposed under the adversarial-framework.

\subsubsection{Model Dynamics of User and Item Interactions.}

\qquad Bharadhwaj \textit{et al.}~\cite{DBLP:conf/recsys/BharadhwajPL18} address the problem to improve the effectiveness of RS by accurately ~\hltask{modelling temporal dynamics of user and item} under the GAN framework. Inspired by Recurrent Recommender Networks~\cite{DBLP:conf/wsdm/WuABSJ17} and IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the authors propose a \hlmethod{Recurrent Generative Adversarial Networks for Recommendation Systems}, named RecGAN, in order to exploit in a single framework both the temporal modelling capabilities of RNN and the latent feature modelling power of the \textit{minimax game}.
They implement both the generator a the discriminator with the Gated Recurrent Unit (GRU)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}, a RNN cell, in order to make $G$ capable to generate ratings for each user-item pair denoted by $(r|u, j, t)$. The overall objective function is formally defined
\begin{equation}
     \small
     \label{equation:recgan}
     J(\theta, \phi)= \mathbb{E}_{r \sim p_{\text { true }}(r | i, u, t)}[\log D_{\phi}(r | i, u, t)]+ \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (1-D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}
where $p_{\theta}(\hat{r} | i, u, t)$ is the rating distribution learned by the generator and $D_{\phi}(r | i, u, t)$ refers to the discriminator's prediction of the likelihood of $(r|i, j, t)$ being sampled from the true distribution $p_{\text { true }}(r | i, u, t)$.
\\Similarly to Equations~\ref{equation:irgan_d} and~\ref{equation:irgan_g}
\begin{equation}
     \small
     \label{equation:recgan_d}
     J^{D} = \mathbb{E}_{r \sim p_{\text { true }}(r | i, u, t)}[\log D_{\phi}(r | i, u, t)]+ \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (1-D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}
 \begin{equation}
     \small
     \label{equation:recgan_g}
     J^{G}= - \mathbb{E}_{\hat{r} \sim p_{\theta}(\hat{r} | i, u, t)}[\log (D_{\phi}(\hat{r} | i, u, t))]
 \end{equation}

The authors demonstrate that RecGAN outperforms various baselines model dealing with temporal aspects in two different RS domains, movie and food. The baseline models include PMF~\cite{DBLP:conf/nips/SalakhutdinovM07}, TimeSVD++~\cite{DBLP:journals/cacm/Koren10}, AutoRec~\cite{DBLP:conf/iconip/OuyangLRX14} and RRN~\cite{DBLP:conf/wsdm/WuABSJ17}.  


\qquad Similar to~\cite{DBLP:conf/recsys/BharadhwajPL18}, Zhao \textit{et al.}~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, 8643032} address the ~\hltask{long and short-term preference modelling} by leveraging the MF~\cite{DBLP:conf/nips/SalakhutdinovM07} and RNN approaches for top-\textit{n} recommendation using a GAN framework. They propose ~\hlmethod{Prioritizes Long And Short-Term Information in top-\textit{n} reCommendation} (PLASTIC) model in order to incorporate long-term interactions modelling of MF and short-term interactions modelling of RNN in a unique recommendation framework. The discriminator $D$ is implemented via a \hlmethod{Siamese Network} that incorporates MF and LSTM~\cite{DBLP:conf/wsdm/WuABSJ17} cell in a pair-wise scenario and learns to distinguish the real high-rated items in the training data from the recommendation list generated by the generator $G$. While the generator $G$ learns to maximize the probability of $D$ making a mistake by  generating top-\textit{n} recommendations produced using a MF model and re-ranked with LSTM cell.
The discriminator and generator objective function are formally defined as
\begin{equation}
    \small
    \label{equation:plastic_d}
    J^{D} =  
    \mathbb{E}_{i_{+}, i_{-} \sim p_{true}(i_{+}, i_{-} |u, t)}[\log D_{\phi}(i_{+}, i_{-} |u, t)] + 
    \mathbb{E}_{i_{+} \sim p_{true}(i_{+} |u, t), \hat{i} \sim p_{\theta}(\hat{i} | u, t)}[\log (1-D_{\phi}(i_{+}, \hat{i} | u, t)]
\end{equation}
\begin{equation}
    \small
    \label{equation:plastic_g}
    J^{G} =  
    - 
    \mathbb{E}_{i_{+} \sim p_{true}(i_{+} |u, t), \hat{i} \sim p_{\theta}(\hat{i} | u, t)}[\log (D_{\phi}(i_{+}, \hat{i} | u, t)]
\end{equation}
where $i_{+}$ is a positive item, $i_{-}$ is a randomly chosen negative item and $\hat{i}$ is the generated item by $G$ at time $t$ for the user $u$. Experiments on movie domains demonstrate that PLASTIC outperforms recommendation performance of BPR~\cite{DBLP:conf/uai/RendleFGS09}, PRFM~\cite{DBLP:conf/cikm/QiangLY13}, LambdaFM~\cite{DBLP:conf/cikm/YuanGJCYZ16}, RRN and IRGAN.

\qquad Chen \textit{et al.}~\cite{DBLP:conf/icml/Chen0LJQS19} work on the challenging application of \hltask{reinforcement learning (RL)} to RS to take into account the long-term user interest evolution and the influence of the recommender action for improving, for instance, users' long-term engagement with an online platform. Model-free reinforcement learning techniques suffer from (i) manually designed reward function which may not reflect a user's preference, and (ii) the need for collecting lots of user-data in order to learn a good-policy. Starting from these limitations, the authors propose a model-based RL framework where user behavior model and the associated reward function are learnt by with a GAN-based approach, called \textbf{GAN user model}.
The generator $G$ learns to mimic the user model by generating the user's next action in order to maximize his reward function, that is to minimize the discriminator. The discriminator $D$ acts as the reward function by maximizing its ability to distinguish between the user's actual actions and those generated by $G$. On completion of the \textit{minimax game}, the authors use the user model and the reward function as the simulation environment to obtain a recommendation policy in the RL framework. Experiments show important advances of the proposed approach in an offline on realistic domains.
% Main contributions of this framework are: (i)the user model and the reward function are learned in a consistent way with the user model; (ii) the learned reward carries out the RL policy in a more principled way, rather than the manually designed one; (ii) the learned user model allows us to perform model-based RL and online adaptation for new users to achieve better results.


\subsubsection{Adversarial Negative Sampling.}

\qquad Wang \textit{et al.}~\cite{DBLP:conf/kdd/WangYHLWH18} and Tanielian \textit{et al.}~\cite{DBLP:journals/corr/abs-1805-08720}, address limitations of baseline \hltask{adaptive negative sampling} methods used to improve recommendations and optimize the training of multi-class models with a huge set of output classes.
Wang \textit{et al.}~\cite{DBLP:conf/kdd/WangYHLWH18} focus on this problem setting in their proposed streaming recommender system, called \hlmethod{Neural Memory Recommender Networks} (NMRN). Inspired by KBGAN~\cite{DBLP:conf/naacl/CaiW18}, the authors propose a novel \hlmethod{GAN-based adaptive negative sampling method} with the aim of improving training efficiency much more than classic random and popularity-biased sampling methods which are not able to dynamic negative items. At the end of the \textit{minimax game} the generator is able to generate adversarial negative samples for each user.
They validate their statements with extensive experiments which show clear improvements compared to the classic streaming recommendation models and the proposed model NRMN without the GAN sampling.
Tanielian \textit{et al.}~\cite{DBLP:journals/corr/abs-1805-08720} address the same issues in the task of basket completion with learned embedding representations. Inspired by MaliGAN~\cite{DBLP:journals/corr/CheLZHLSB17}, the authors propose to solve these issues with a GAN-based sampling method, called ~\hlmethod{Adversarial Negative Sampling} that draws negative samples from a dynamic distribution that is by design more informative than the fixed distribution used in standard negative sampling. They introduce the new method in a novel basket completion model, namely \textbf{GAN-Word2Vec}. 
Experiments on two e-commerce datasets show better top-\textit{1} recommendations when GAN-Word2Vec is compared to classical Word2Vec approaches.

\subsection{Context-aware Recommender System.}
We identify few works inside the class of Contextual Recommender Systems.

Zhou \textit{et al.}~\cite{DBLP:conf/www/0002YZTZW19} focuses on ~\hltask{location-based recommendation systems} to suggest point-of-interest (POI) to users. The authors address the ~\hltask{lack of formal models to understand user check-in behavior} which can lead to poor recommendation performance. They propose a novel GAN-based POI recommendation model, named \hlmethod{Adversarial POI Recommendation} (APOIR), for learning the user check-in model in a generative way, rather than extracting them with baseline approaches, such as MF, Context Embedding and Pairwise Ranking, in order to boost the recommendation performance.
The generative process is used to model the relationship between a user $u$ and the set of POIs, where a POI is $i$. The underlying distribution of the user preferences over POIs is learned by classical minimax game between a generator $G$ and a discriminator $D$ explained in Section~\ref{subsec:GAN-based CF}. Similarly to IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the authors employ a reward policy based on \textit{Geographical rewards}, e.g. the distance between POIs, and \textit{Social rewards}, e.g. the POIs visited by user's friends, which works as a regularizer to the recommended POIs from the generator $G$.
They evaluate APOIR on public location-based social network datasets and compare it to several state-of-the-art models. The results demonstrate the effectiveness of APOIR approach in improving POI recommendation.

Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} investigate \hltask{query recommendation systems} in order to improve the suggestion performance by understanding and modeling user search intents accurately. The authors propose a novel model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), that provides query suggestions considering the sequential search queries issued by the user and and his the history of clicks on last suggestions. Similarly to APR~\cite{DBLP:conf/sigir/0001HDC18}, they employ an adversarial training stage during the training of CFAE by injecting adversarial examples built by adding adversarial perturbations of item embeddings.~\felice{It is necessary to define in a Section the procedure user to create adversarial perturbations. They use FSGM}
Experiments on a e-shopping domain dataset demonstrate that adversarial training on CFAN not only significantly \textit{improve the robustness} of the model but also outperforms the baseline methods for the task of query suggestion.

\subsection{Recommender Models for Cross-Domain Recommendation}
Cross-domain recommendation (CDR) offers recommendations in a target domain by exploiting knowledge from source domains. This recommender category has received much attention because it is a potential solution to mitigate the cold-start and sparsity problem.
~\futureworks{I think that this field is quite not explored in the domain of adv-recommender systems. It can be intriguing to think on an adversarial-based model to move information from a movie domain (e.g. Netflix) to a music domain (e.g. Last.fm) in an unsupervised way. Another idea can be to use domin2domain translation also in music recommendation itslef for playlist building (ropose interesting playlist in another genre,...) }

Inspired by e Unsupervised Image-to-image Translation (UNIT)~\cite{DBLP:conf/nips/LiuBK17}, Nguyen and Ishigaki~\cite{DBLP:journals/corr/abs-1812-06229} address the problems relating to the ~\hltask{difficulty to obtain similar features among different domains} and to ~\hltask{transfer the knowledge on a denser target domain $A$ into a source one $B$} for cross-domain recommendation by proposing a \hlmethod{VAE-GAN-CC} network.
to (i) extract both homogeneous and divergent features among domains, (ii) translate one domain to another and (iii) apply an end-to-end deep learning approach for CF-RS which only uses the user interaction history as input.
The proposed model is composed by two generative adversarial networks $GAN_{A}$ and $GAN_{B}$. The generator of each GAN is a VAE.
In their model, $VAE_{A}$ is the generator for domain A, while $VAE_{B}$ is related to domain B. For an input click vector $u_{A}$ $\in$ A, the $VAE_{A}$ first maps $u_{A}$ to a code in a latent space $Z$ via its encoder component. It then decodes a randomly perturbed version of the code to reconstruct the input click vector via the decoder.
The authors enforce a weight-sharing constraint between some layers of VAEs in order to learn domain-to-domain translation, e.g. 
Because of the weight-sharing of between the two VAE of each GAN, each generator generates a reconstructed user vector that can come from the same domain, or a different one. For instance, it is possible to translate a click vector $u_{A}$ in domain A to a click vector in domain B through applying $G_{B}$.
$G_{A}$ generates click vector ${u}_{AA}$ and ${u}_{BA}$ where ${u}_{BA}$ is the translation vector of the user vector in domain B to the domain A, $G_{A}$ generates click vector ${u}_{BB}$ and ${u}_{AB}$ where ${u}_{AB}$ is the translated version of $u_{A}$ in the domain $B$. 
$D_{A}$ is trained to output true for real click vectors sampled from $A$ domain and to output false for click vectors generated from $G_{A}$, $D_{B}$ works in the same way for the $B$ domain.
The overall objective function is composed by six components:
\begin{equation}
    \label{equation:domain2domain}
    \small
    J = \mathcal{L}_{VAE_{A}} + \mathcal{L}_{GAN_{A}} + \mathcal{L}_{CC_{AB}} + \mathcal{L}_{VAE_{B}} + \mathcal{L}_{GAN_{B}} + \mathcal{L}_{CC_{BA}}
\end{equation}
where $\mathcal{L}_{VAE_{A}}$ and $\mathcal{L}_{CC_{BA}}$ are the loss function of the cycle-consistency constraint for weight-sharing.
The trained generator $G_{A}$ is used to predict the user click vector in the domain $D$ given the vector in a domain $A$ and viceversa. 
Experiments on real-world domains, i.e. movie and e-commerce, demonstrate an improvement of ranking based metrics on CDL~\cite{DBLP:conf/kdd/WangWY15}, CCCFNET~\cite{DBLP:conf/www/LianZXS17}, Multi-VAE~\cite{DBLP:conf/www/LiangKHJ18} and APR~\cite{DBLP:conf/sigir/0001HDC18}.
% ${u}_{AA}=G_{A}({z}_{A} \sim q_{A}({z}_{A} | {u}_{A}))$ and ${u}_{B A}=G_{A}({z}_{{B}} \sim q_{B}({z}_{B} | {u}_{B}))$, where $z_{A}$ and $z_{B}$ are the latent representation of the encoders of $G_{A}$ and $G_{B}$ respectively, $q_{A}$ and $q_{B}$ are the distributions of $z_{A}$ and $z_{B}$.

Wang \textit{et al.}~\cite{DBLP:journals/corr/abs-1903-10794} address \hltask{data sparsity and data imbalance} problem setting in cross-domain recommender systems. Inspired by the last advances in adversarial domain adaptation like ADDA~\cite{DBLP:conf/cvpr/TzengHSD17} and Bi-LSTM model~\cite{DBLP:journals/tomccap/WangYM18}, they propose a \hlmethod{Discriminative Adversarial Networks for Cross-Domain Recommendation (RecSys-DAN)} method to learn domain indistinguishable representations of users, items and user-item pairs across different product domains in a unsupervised way.~\felice{They claim that RecSys-DAN can be viewed as the first work which explores the power of GAN in the context of cross- domain recommender systems.} They perform domain adaptation going from a \textit{source domain with several user-item preference values} to a \textit{target domain with no user-item preferences}.~\felice{The minimax game objective function is a little bit complicated to insert because it is based on 6 generators and 3 discriminators.}
The authors evaluate RecSys-DAN on multiple sets on e-shopping domain with different item and user interactions such as review text, product images and ratings different tasks. Results demonstrates competitive performance compared to baseline supervised methods for the rating prediction, even without explicit preferences.

D. Perera and R. Zimmermann~\cite{DBLP:conf/www/PereraZ19} propose a solution to address the limit in applying \hltask{cross-domain recommendations} to apply a GAN based model to generate missing source network preferences for non-overlapped users. The authors propose \hlmethod{CnGAN}, a novel GAN based model which includes a content loss function and user-based pairwise loss (BPR) function for the \textit{generator} and \textit{recommender} tasks.
The generator task learns the corresponding mapping from target to source network user preferences and generates auxiliary preferences on the source network thanks. While classic GAN models are typically used to generate real-like samples from random noise vectors, CnGAN aims to \textit{learn} a specific mapping from target to source network encoding in order to 'move' the encoding of not-overlapped users in a latent space that encodes global implicit information of another domain (source network). The novel content-loss is used to provide additional guidance for G to map users in the source space.~\felice{Not simple to explain... need more accuracy}
The recommender task uses the synthetically generated preferences to provide recommendations for users who only have interactions on the target network (not overlapped users). Experimental evaluation of CnGAN against single network (TimePop:), cross-network (TBKNN~\cite{Campos:2010:STK:1869652.1869655}, TDCN~\cite{DBLP:conf/mm/PereraZ17}, linear factorization and GAN based baselines demonstrate advances in terms of accuracy, novelty and diversity.

Inspired by \hlmethod{adversarial negative sampling} techniques proposed in~\cite{DBLP:conf/kdd/WangYHLWH18}, Fan \textit{et al}~\cite{DBLP:journals/corr/abs-1905-13160} address the limitation of typical negative sampling in \hltask{social recommendation} domain to transfer users' information from social domain to item domain. The proposed framework, namely \hlmethod{Deep Adversarial SOcial recommendation} (DASO), harnesses the power of adversarial learning to dynamically generate 'difficult' negative samples of user-item pairs and user-user pairs, to guide the framework in learning better user and item representations.
The overall objective function of DASO is 
\begin{equation}
    \label{equation:daso}
    \small
    J = \mathcal{L}_{GAN_{I}} + \mathcal{L}_{GAN_{S}} +  \lambda \mathcal{L}J_{CC_{I,S}}
\end{equation}
where $\mathcal{L}_{GAN_{I}}$ is the objective function of the Item Domain Adversarial Learning used to learn better user and item representations in the item domain , $\mathcal{L}_{GAN_{U}}$ is the objective function of the Social Domain Adversarial Learning used to learn better user representations from the social perspective and $\lambda$ is the parameter to control the relative importance of cycle-reconstruction $\mathcal{L}_{CC_{I,S}}$ used to bidirectional map between the social and the item domain. To evaluate the performance, the authors compared DASO with BPR, SBPR~\cite{DBLP:conf/cikm/ZhaoMK14}, DeepSoR~\cite{DBLP:conf/aaai/FanLC18}, GraphRec~\cite{DBLP:conf/www/Fan0LHZTY19} and IRGAN. Comprehensive experiments on two real-world datasets show the effectiveness of their model

Transferability properties of GAN have been exploited also by Sang-Young Jo \textit{et al.}~\cite{DBLP:conf/bigcomp/JoJCJ19}. They focus on addressing \hltask{fashion recommendation} challenge by proposing a recommendation system that takes into account the styles and patterns of sceneries pictures. Inspired by style-transfer ability of DiscoGAN~\cite{DBLP:conf/icml/KimCKLK17}, the authors employ a GAN-based framework to generate new fashion images with the styles from the sceneries. ~\felice{I think we can remove the analysis of this article}.

\subsection{Recommender Models for Complementary Recommendation}
Complementary Recommendation (Com) is a novel challenging task that points to suggest complementary items to suggest new items to customers. A very intuitive application domain is the fashion domain. For instances, given a red top (i.e., upper garment), the recommender model may recommend a selection of bottoms (e.g., trousers) in a complementary way. 
\\Novel solutions have been proposed to address the problem of recommending complementary items by using adversarial-based approaches.


Huynh \textit{et al.}~\cite{DBLP:conf/eccv/HuynhCTA18} address the problem of ~\hltask{recommending complementary items} for a given item based on visual features. They develop an unsupervised learning approach for \hlmethod{Complementary Recommendation using Adversarial Feature Transform} (CRAFT), by learning the co-occurrence of item pairs in real images. The proposed method does not generate new images but it learns to generate features of the complementary items conditioned on the query item. 
\begin{figure}[h]
  \includegraphics[width=0.6\linewidth]{Pictures/CRAFT.png}
  \caption{Architecture for the CRAFT framework. The transformer component is trained to generate the target features conditioned on the source features and a sampled noise vector.}
  \label{fig:CRAFT}
\end{figure}

The generator $G$ acts like a feature transformer to transform the source feature $s_{q}$ into a complementary target feature $\hat{t_{q}}$ by playing a \textit{minimax game} with a discriminator $D$ that aims to classify feature pairs as real ($s_{i}$, $t_{i}$) or synthetic ($s_{q}$, $\hat{t_{q}}$).
Similar to Equation~\ref{equation:gan}, the objective function is
\begin{equation}
    \label{eq:craft}
    \small
    J(\theta, \phi) = \mathbb{E}_{(s_{i}, t_{i}) \sim p_{c}} \log D_{\phi}(s_{i}, t_{i})+\mathbb{E}_{z \sim p_{z}, s_{q} \sim p_{s}} \log (1-D_{\phi}(s_{q}, G_{\theta}(s_{q}, z)))
\end{equation}
where $p_{z}$ and $p_{s}$ are the probability distribution function of the random noise and the source feature.
Recommendation are built on a nearest neighbor search of $\hat{t_{q}}$ on the subspace with pre-indexed target features $t_{i}$.
CRAFT has been tested by experienced users whose who gave positive feedback on the goodness of complementary recommendations.

Inspired by advances in image generation by class labels or by texts, and image transformation between different domains, Kang \textit{et al.}~\cite{DBLP:conf/icdm/KangFWM17}, Shih \textit{et al.}~\cite{DBLP:conf/aaai/ShihCLS18}, Lin \textit{et al.}~\cite{Yang2018FromRT} and Kumar and Das Gupta~\cite{2019arXiv190605596K} propose GAN-based~\cite{DBLP:journals/corr/RadfordMC15} solutions for the \hltask{generation of compatible items} in the fashion domain.

\cite{DBLP:conf/icdm/KangFWM17} is the first publication where the Generative Adversarial Networks are used in Fashion Domain recommendation to \hltask{generate item images based on user preferences}. For instance, given a user and an item category, they propose a model to generate new images (i.e., clothing items) that are most consistent with user's preferences. In this paper, the authors adapt the Bayesian Personalized Ranking (BPR) to include item image content via a Siamese network in a \hlmethod{Deep Visually-aware Bayesian Personalized Ranking} method, called DVBPR. Then, this model is combined with a GAN-based framework to generate images that are consistent with user's personal taste. Iteratively, the generator learns a low dimensional latent code, which generates an item image that maximizes a personal objective value. 
Inspired by LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}, the overall objective function is
\begin{equation}
    \small
    \label{eq:dvbpr_gan_objective}
    J = \mathbb{E}_{\mathbf{x}, c \sim p_{true}(x, c)} [D(\mathbf{x}, c) - 1]^{2} + 
        \mathbb{E}_{c \sim p(c), z \sim p(z)} [D(G(z, c), c)]^{2}
\end{equation}
where $\mathbb{x}$ is a image of the training dataset, $c$ is the category of the image $\mathbb{x}$ a $z$ is a random noise vector. Given a user $u$ and a category $c$, the authors propose to synthesize personalized images by optimizing a user preference score
\begin{equation}
    \small
    \widehat{\delta}(u, c) = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} ( \widehat{r}_{u, e} )
    = \underset{e \in G(\cdot, c)}{\operatorname{argmax}} \big(r_{u, e}-\eta D(e, c) \big)
\end{equation}
where $r_{u,e}$ is the user score to a generated new image and $\eta$ controls the trade-off between preference score and image quality. Generated Images are quantitatively compared with real images using the preference score (mean objective value), inception score~\cite{DBLP:conf/nips/SalimansGZCRCC16} and Opposite SSIM~\cite{DBLP:conf/icml/OdenaOS17}. This comparison show above all improvement on preference score with respect to not-GAN based images. At the same time, the qualitative comparison demonstrates that the generated images are realistic and plausible, yet are quite different from any images in the original dataset—they have common shape and color profiles, but quite different styles. 

Shih \textit{et al.} propose a Compatibility Learning Framework by using a \hlmethod{Metric-regularized Conditional Generative Adversarial Network} (MrCGAN) to pursue the item generation task. The proposed model is composed of a compatibility learning component and a DCGAN~\cite{DBLP:journals/corr/RadfordMC15}-based component, MrCGAN, that is regularized on a compatibility metric learnt in the first component. Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18} they conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines. 
\\The authors of~\cite{Yang2018FromRT} addresses the same problem settings by proposing a novel fashion clothing framework composed of two parts: a clothing recommendation model based on BPR combined with visual features and a clothing complementary item generation based on DCGAN. Particularly, the generation component takes in input a piece of clothing recommended successfully in the recommendation model and generates clothing images of other categories (top, bottom or shoes) to build up a set of complementary items. They evaluate GAN performance with three index: Inception score related to the quality of the generated image~\cite{DBLP:conf/nips/SalimansGZCRCC16}, Opposite SSIM related to the diversity~\cite{DBLP:conf/icml/OdenaOS17}, and a proposed \textit{Compatibility index} to measure the compatibility of the generated set of complementary items. They compare the model with DCGAN as there are not baseline methods for such comparison. ~\futureworks{Can be interesting to focus on this field and try to propose new models a a baseline way to compare images?}.
A similar approach has been proposed also in~\cite{2019arXiv190605596K}, to generate bottom fashion item paired with a given top item.


\subsection{Others}\label{subsec:others}

Adversarial Machine Learning techniques are used also to address specific tasks which are independent of the recommender model.

\subsubsection{Privacy}
Attribute inference attacks are emerging issues to user privacy in recommender systems domain~\cite{DBLP:conf/recsys/WeinsbergBIT12, DBLP:conf/cikm/Otterbacher10}. The attacker aims to infer a user's private attributes (e.g., gender, sexual orientation, political and religion views) via leveraging its public data (e.g., in recommender systems, it could be the list of rated items).

Recognising existing defense methods against attribute inference attacks are either computationally intractable or computationally tractable - but they add a large amount of noise to a user's public data; Jia \textit{et al.}~\cite{jia2018attriguard} propose ~\hlmethod{AttriGuard} a computationally tractable defense mechanism that adds small noise. The proposed defense method works in two phases. Firstly, it finds such minimum adversarial noise to evade the attacker's classifier. through an optimized version of \textit{evasion attack} developed by Papernot \textit{et al.}~\cite{DBLP:conf/eurosp/PapernotMJFCS16}, named \hlmethod{Policy-Aware Noise Finding Algorithm} (PANDA). Then, AttriGuard randomly selects one of the adversarial noise found previously to mislead the attacker's inference. The authors evaluate AttriGuard and compare it with existing defenses using a real-world dataset. Results demonstrate that the proposed evasion attack outperforms existing ones (FGSM, JSMA~\cite{DBLP:conf/eurosp/PapernotMJFCS16} and C\&W), and the proposed defense mechanism, AttriGuard, is effective at defending against attribute inference attacks. Otherwise it adds significantly smaller noise to users' public data than existing defenses.

Resheff \textit{et al.}~\cite{DBLP:conf/icpram/ResheffESS19} addresses the problem setting of the \hltask{leakage of private information} in recommender systems. The proposed privacy-adversarial framework in addition to eliminating such leakage it helps to guarantee fairness of results.
Inspired by the Domain Adversarial Training~\cite{DBLP:series/acvpr/GaninUAGLLML17}, the proposed method points to construct a user representation from which the private information can not be read out. This is achieved by training the model with an additive loss for the privacy protection.
This is achieved by application of the gradient reversal trick~\cite{DBLP:series/acvpr/GaninUAGLLML17} which leads to the following update rule for user embedding $p_{u}$:
\begin{equation}
    \small  
    \label{eq:panda_optimization}
    p_{u} \leftarrow p_{u}-\alpha\left[\frac{\partial \mathcal{L}_{recsys}}{\partial p_{u}}
    - 
    \lambda \sum_{i} \frac{\partial \mathcal{L}_{private_{i}}}{\partial p_{u}}\right]
\end{equation}
where $\alpha$ is the learning rate, $\lambda$ is the adversarial learning rate, and $ \mathcal{L}_{recsys}$ and $\mathcal{L}_{private_{i}}$ are the loss function of the recommender model and the adversarial privacy-protection component appended to the recommender model. Experiments on movie recommendation domain show the effectiveness of the proposed method in reducing the leakage of user's personal data.


\subsubsection{Adversarial Machine Learning for Shilling Attacks}

\textbf{Adversarial Attacks on an Oblivious Recommender} by Konstantina Christakopoulou, Arindam Banerjee HAD BEEN ACCEPTED IN RECSYS2019. 
I am waiting for it because it is the long paper version of \textbf{Adversarial Recommendation: Attack of the Learned Fake Users}~\cite{DBLP:journals/corr/abs-1809-08336}.
They propose a framework for generating \hltask{shilling profiles} which, when incorporated in the training of a recommendation system, can achieve an adversarial intent, while remaining \textbf{indistinguishable from real user profiles}. The generation is mapped with a GAN-based framework where the Discriminator is the recommender model and the generator is the component that tries ot imitate the real distribution of users by looking to manipulate the recommendations.

\input{Plots/OpenChallenges.tex}
\input{Plots/Domain.tex}

\newpage

\subsection{~\felice{SOME EXAMPLE PLOTS/TABLES}}

\begin{figure}[h]
  \includegraphics[width=\linewidth]{Pictures/Challanges.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=\linewidth]{Pictures/Dataset.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=\linewidth]{Pictures/Trand.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=\linewidth]{Pictures/Metric.png}
\end{figure}

==> OLD_FILES/OLD_some_table.tex <==
\input{Sec4_A_GAN.tex}
\input{Sec4_B_AdvReg.tex}
\input{Sec4_C_Others.tex}


\subsection{~\felice{SOME EXAMPLE PLOTS/TABLES}}

\begin{figure}[h]
  \includegraphics[width=0.5\linewidth]{Pictures/Challanges.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=0.5\linewidth]{Pictures/Dataset.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=0.5\linewidth]{Pictures/Trand.png}
\end{figure}
\begin{figure}[h]
  \includegraphics[width=0.5\linewidth]{Pictures/Metric.png}
\end{figure}

==> OLD_FILES/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> OLD_FILES/Sec1_Introduction.tex <==
\section{Introduction}\label{sec:Introduction}

In the age of data deluge, where users are facing a new form of information explosion, recommender systems (RS) have emerged as a paradigm of information push to lessen decision anxieties and consumer confusion by over-choice. RS enhance users' decision-making process and support sales\footnote{It has been known that RS are an important monetization method of businesses. For instance, 80\% of hours streamed at Netflix derives from recommendation~\cite{DBLP:journals/tmis/Gomez-UribeH16}, 8\% of Amazon traffics derives from its recommendation engine~\cite{DBLP:journals/internet/SmithL17}.} by personalizing item recommendations for each user and helping them discover novel products. RS are pervasive part of user experience online today and serve as a principal choice of many consumer-oriented companies such as Amazon~\cite{DBLP:journals/internet/SmithL17, DBLP:conf/sigecom/SharmaHW15}, Netflix~\cite{DBLP:journals/tmis/Gomez-UribeH16}, Google (e.g., YouTube~\cite{DBLP:conf/imc/ZhouKG10}). Among different types of recommendation techniques, collaborative filtering (CF) methods have been the mainstream of recommendation research both in academia and industry due to their superb recommendation quality. CF builds on the fundamental assumption that users who have expressed similar interests in the past, will maintain similar choices in future~\cite{DBLP:journals/cacm/GoldbergNOT92}, and infers target user preference over unseen items by leveraging behavior data of other users and exploiting similarities in their behavior patterns. In the following, we discuss summary of the progress in CF-model developments over the last three decades.

\begin{figure}
    \centering
    \includegraphics[width = 0.94\linewidth]{Pictures/From_CF_to_SecureCF.pdf}
    \caption{Milestones of CF recommender models.}
    \label{fig:milestones}
\end{figure}

\subsection{Summary of the progress of CF models in the past decades}

Milestones in CF models over the past decades are summarized in Figure~\ref{fig:milestones}. The core idea of a recommending service can be traced back to cognitive science first described in a system named Grundy in 1972~\cite{DBLP:journals/cogsci/Rich79} in which the authors used stereotypes to build user models and suggest relevant books to individual users. Almost 20 years later, the idea of recommender systems started booming. In 1992, Belkin et. al.~\cite{DBLP:journals/cacm/BelkinC92} discussed the component of an \textit{information filtering} (IF) system in comparison with an \textit{information retrieval} (IR) system.\footnote{The work by Belkin et. al.~\cite{DBLP:journals/cacm/BelkinC92} used/assumed content-based filtering (CBF) system as the primary example of an IF system in which the CBF systems uses only textual information. Against this traditional view, modern RS nowadays utilize a variety of other information such as linked open data (LOD), multimedia (audio and visual) features, user-generated content (UGC) and heterogeneous information networks~\cite{DBLP:journals/umuai/LopsJMBK19}.} Afterwards, several works made attempts to \textit{automate} the idea of CF, notably, the first CF model made in 1992 by Goldberg et al. Tapestery~\cite{DBLP:journals/cacm/GoldbergNOT92} --- which consolidated the idea of like-minded users as the principal mechanism of CF --- Grouplens in 1994~\cite{DBLP:conf/cscw/ResnickISBR94}, the Bellcore's video recommender in 1995~\cite{DBLP:conf/chi/HillSRF95} and the music and album recommender Ringo in 1998~\cite{DBLP:conf/chi/ShardanandM95}.

We can identify two major eras in development of CF models based on their main objective:

\begin{enumerate}
    \item The era focused on maximizing/enhancing the recommendation accuracy and beyond-accuracy 
    \item The post neural era, the transition era from classical learning to adversarial machine learning
\end{enumerate}

\noindent \textbf{(1) Accuracy maximization and beyond-accuracy enhancement era:} 

In this era, the main effort of the research and practitioner-scholars was concentrated on the \dquotes{golden objective} of \textit{maximizing recommendation accuracy}. Consequently, machine-learned models tend to use any available signal in the data to reach this goal, even though some of the data contained noise as the results of user's misoperations. We distinguish between three classes of CF techniques in this era: (i) classical non-neural CF era, (ii) domain/task-dependent CF era and, (iii) deep neural CF era, each described in the following.

\begin{itemize} 
    \item \textbf{Classical non-neural CF}: The starting of this era dates back to the 1990s and is still progressing. Over these three decades, the study on CF methods has been the subject of active research by the RS community resulting in a diverse set of models and evaluation measures to assess the effectiveness of these models. We can classify these CF approaches based on various dimensions. For example, from a \textit{learning paradigm} perspective, CF models can be classified according to (i) \textit{memory-based CF} and (ii) \textit{model-based CF} models, in which the former category makes recommendation based on the similarity of users-user interactions (i.e., user-based neighborhood model) or item-item interactions (i.e., item-based neighborhood model) while the latter category predicts users' feedback of unseen items using latent factor model such as matrix-factorization (MF)~\cite{DBLP:journals/computer/KorenBV09}. From the \textit{model training} perspective, it is possible to categorize these models based on the loss functions employed according to: (i) \textit{point-wise} loss where the goal is to optimize towards a predefined ground-truth (e.g., matrix factorization approach based on SVD), (ii) \textit{pairwise ranking loss} where the goal is to optimize personalized ranking  (e.g., matrix factorization based on BPR) and (iii) \textit{list-wise} loss where the objective is to reflect the distance between the reference list and the output list ~\cite{DBLP:conf/recsys/ShiLH10}.
 
    
\item \textbf{Domain-dependent CF}: \dquotes{\textit{Recommendation is not a one-size-fits-all problem}}~\cite{ekstrand2011collaborative}. The research in this era has the main focus to integrate a wealth of side information data beyond the user rating matrix (URM) into the recommendation models to make RS adapted in specific domains. Such data consist of side information of users (e.g., demographics, personality traits, social-network information), items (e.g., item content, attributes) and the interplay between them (e.g., the time of interaction). For example, in~\cite{DBLP:conf/recsys/NingK12,DBLP:conf/recsys/VasileSC16} the authors use 
item description information such as textual metadata (e.g., movie cast, product review, artist information) and in ~\cite{DBLP:journals/umuai/DeldjooDCECSIC19,DBLP:conf/nips/OordDS13} features extracted directly from the signal (images or audio) in order to enhance recommendation. These approaches can be also used to alleviate cold-start issues such as data sparsity or new/item user problem, which impede the performance of CF models. Based on the unique nature of side information in different domains, different hybrid CF strategies have been developed~\cite{DBLP:conf/sigir/ScheinPUP02, DBLP:journals/csur/ShiLH14}. The survey~\cite{DBLP:journals/csur/ShiLH14} by Shi et al. provides a good frame of reference for CF methods leveraging rich side information.

\item \textbf{Deep neural CF}:  Another milestone that is booming is concerned with the success of deep learning (DL) or \dquotes{neural} technology
in machine learning (ML).  DNNs have shown to be capable of providing remarkable accuracy in several predictive tasks and domains such as image classification~\cite{DBLP:journals/spm/HanZCLX18} and speech recognition~\cite{DBLP:journals/ijar/SalakhutdinovH09} among others.

In the field of RS, DNNs have been shown useful for the recommendation in several ways such as extracting deep features (via using CNNs), to model item content in CF models by integrating side item information, building CF models by parameterizing latent factor models into layers of a DNN (deep CF), and modeling the sequential relations (via using RNNs). As for deep-CF approaches, while MF assumes that the \textit{linear interaction} between user and item latent factors can explain observed feedback, deep CF models can model a more complex representation of hidden latent factors by \textit{parametrization of MF via a DNN}.  Table~\ref{recommendermodels} summarizes the list of state-of-the-art deep CF approaches used in different recommendation tasks. 
\end{itemize}

\noindent \textbf{2. The post neural era, the transition era from classical learning to adversarial machine learning:}

Despite the significant success of DNNs to solve a variety of complex prediction tasks on non-structured data such as images, recently, they have been demonstrated to be vulnerable to \textit{adversarial examples}. Adversarial examples (or adversarial samples) are subtle but non-random perturbations \textit{designed} to dictate a ML model to produce erroneous outputs (e.g., to misclassify an input sample). The subject started booming after the pioneering work~\cite{DBLP:journals/corr/SzegedyZSBEGF13} by Szegedy et al. reported the vulnerability of DNNs against adversarial samples for the image classification task. It is shown that by adding a negligible amount of adversarial perturbation on an image (e.g., a panda), a CNN classifier could misclassify the image with another class (e.g., a gibbon) with high confidence.  These results were quite shocking since it was expected that state-of-the-art DNNs that generalize well on unknown data, do not change the label of a test image that is slightly perturbed and is human-imperceptible. Algorithms that aim to find such adversarial perturbations are referred to as \textit{adversarial attacks}. As ML models are involved in many consumer safety and security-intensive tasks such as autonomous driving, facial recognition, and camera surveillance, adversarial attacks pose significant concerns to the security and integrity of the deployed ML-models.

In the field of RS, numerous works have reported the failure of machine-learned recommendation models, i.e., latent-factor models (LFM) based on CF like MF and deep CF methods widely adopted in modern RS, against adversarial attacks. For instance, in~\cite{DBLP:conf/sigir/0001HDC18}  He et al. showed that by exposing
the model parameters of BPR~\cite{DBLP:conf/uai/RendleFGS09} to both adversarial and random perturbations of the BPR model parameters, the test NDCG is decreased by -21.2\% and -1.6\% respectively, which is equal to a staggering impact of approximately 13 times difference. One main explanation for such behavior is that adversarial attacks exploit the imperfections and approximations made by the ML model during the training phase to control the models' outcomes in an engineered way~\cite{DBLP:journals/corr/PapernotMG16}.


These examples underline the failure of classical ML. Adversarial machine learning (AML) is an emerging research field that combines the best practices in the areas of ML, robust statistics, and computer security~\cite{DBLP:journals/internet/Tygar11,DBLP:journals/ijon/XiaoBNXER15}. It is concerned with the design of learning algorithms that can resist adversarial attacks, studies the capabilities and limitations of the attacker and investigates suitable countermeasures to design more secure learning algorithms~\cite{DBLP:conf/ccs/HuangJNRT11}.
The pivotal distinguishing characteristic of AML is the notion of \dquotes{min-max} game, in which two competing players play a zero-sum differential game, one --- i.e., the attacker --- tries to \textit{maximize} the likelihood of the attack success, while the other --- i.e., the defender --- attempts to \textit{minimize} the risk in such a worst-case scenario. In the context of RS, the defender players can be a machine-learned model such as BPR or a neural network, while the attacker is the adversarial model.

To protect models against adversarial attacks, \textit{adversarial training} has been proposed. It is a defensive mechanism whose goal is not to detect adversarial examples, rather build models that perform equally well with adversarial and clean samples. Adversarial training consists of injecting adversarial samples --- generated via a specific attack model such as FGSM~\cite{DBLP:journals/corr/GoodfellowSS14} or BIM~\cite{DBLP:conf/iclr/KurakinGB17} --- into each step of the training process. It has been reported --- both in RS~\cite{8618394} and ML~\cite{DBLP:journals/corr/abs-1911-05268} --- that this process leads to robustness against adversarial samples (based on the specific attack type on which the model was trained on), and better generalization performance on clean samples. For instance, in~\cite{8618394}, the authors show that the negative impact of adversarial attacks measured in terms of NDCG is reduced from -8.7\% to -1.4\% when using adversarial training instead of classical training.

The above discussion highlights the failure of classical ML models (trained on clean data) in adversarial settings and advocates the importance of AML as a new paradigm of learning to design more secure models. Nevertheless, the attractiveness of AML that exploits the power of two adversaries within a \dquotes{min-max} game is not limited for security applications and has been exploited to build novel \textit{generative} models, namely generative adversarial networks (GANs). The key difference is as follows: the models used in AML for security (or attack and defense) focus only on a class of discriminative models (e.g., classifiers), whereas GANs build upon both discriminative and generative models.
A GAN is composed of two components: the generator $G$ and the discriminator $D$. The training procedure of a GAN is a min-max game between $G$,  optimized to craft fake samples such that $D$ cannot distinguish them from real ones, and $D$, optimized to correctly classify original samples from generated. 
Through the interplay between these two components, the model reaches the Nash equilibrium where $G$ has learned to mimic the ground-truth data distribution, e.g., a profile of a particular user. In the present survey, we identified different application for GAN-based RS including, improving negative sampling step in learning-to-rank objective function~\cite{DBLP:conf/kdd/WangYHLWH18, DBLP:conf/ijcai/FanD0WTL19}, fitting the generator to predict missing ratings by leveraging both temporal~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:conf/recsys/BharadhwajPL18} and side information~\cite{DBLP:conf/sigir/WangYZGXWZZ17, DBLP:conf/cikm/ChaeKKL18}, or to augment training dataset~\cite{DBLP:conf/www/ChaeKKC19, DBLP:journals/tmm/DuFYXCT19}.

\yashar{@Tommaso: everything that come below this part you may want to improve.}\\
The focus of this survey is on the following two studies both using the concept of \dquotes{min-max} in their formulation:
\begin{enumerate}
    \item \textit{AML for security of RS}: This is the \dquotes{principal application} of AML in RS, which focuses on adversarial attacks and defense models in RS, which we present in Section~\ref{sec:security}.
    \item \textit{Application of AML in GANs}: This is a \dquotes{derived topic} from AML, that is focused on \dquotes{generative} learning models. We identified four types of applications in this category, namely: \textit{improving CF recommendation}, \textit{context-aware recommendation},\textit{cross-domain recommendation} and \textit{complementary recommendation}, which we present in Section~\ref{sec:GAN}.
\end{enumerate}

Overall, AML-based recommendation scenarios are highly relevant to the field of RS. In recent years, a growing number of relevant research works have been proposed. Despite this success, research in AML-RS is overly scattered with each paper focusing on a particular task, domain, or architecture.
One major objective of this survey is to categorize state-of-the-art research in the field based on several identified dimensions to provide a richer understanding of the different facets of the AML-RS. 
Our ultimate motivation is to lay the foundation for a more standardized approach for reproducible research works in the field.

The practical outcome of the present survey includes:
\begin{enumerate}
    \item To the best of our knowledge this is the first work that provides a \textit{comprehensive understanding} of AML in RS domain, unifying the advances made in the communities of ML and RS;
    \item This survey sheds lights on two successful applications of AML, namely: adversarial attacks and defenses and GANs, both using the concept of \dquotes{min-max} game at their core. It provides an extensive literature review of the existing research, specifically:
    \begin{itemize}
        \item For AML-based RS focused on security: we present a unified problem formulation and discuss the existing adversarial attack studies on RS from various perspectives in particular attack and defense models, recommendation dimensions as well as evaluation and attack metrics used in different papers.
        \item For GAN-based RS: we provide a conceptual view of GAN-based Recommendation incorporating GAN to address the item recommendation task and review an extensive number of research, which we classify according the generator, discriminator type and training paradigm. We also categorize the existing research into several distinctive high-level goals (e.g., complementary recommendation in fashion domain, context-aware recommendation etc.).
     \end{itemize}
    \item We created an open-source repository\footnote{Table with AML-RS publications at \url{https://github.com/sisinflab/adversarial-recommender-systems-survey}} that includes all reviewed research articles and updated over time. The aim of this repository is to facilitate bench-marking AML in the RS field by proving the released codes links and datasets used for the evaluation.
\end{enumerate}

A preview of this survey has been presented at the WSDM'20 conference~\cite{DBLP:conf/wsdm/DeldjooNM20}.\footnote{Tutorial slides at ~\url{https://github.com/sisinflab/amlrecsys-tutorial}}

\subsection{How do we collect the papers?}\label{subsec:howCollect}

To identify the relevant publications that constitute the state-of-the-art on the topic of adversarial learning in recommender systems, we mainly relied on publications indexed in major computer science bibliography databases namely DBLP (\url{https://dblp.uni-trier.de/}) and Scopus (\url{https://www.scopus.com}). In addition, realizing the fact that many top-tiers venues also publish related works, which may not be necessarily indexed in the above databases, we also gathered a number of related publications by searching directly through Google Scholar (\url{https://scholar.google.it/}. Our search strategy was composed of two main stages: 
\begin{enumerate}
\item relevant publication collection, 
\item filtering and preparing the final list.
\end{enumerate} 
We collected also referenced publications in the yet selected ones.
As for the first stage, we queried the term \dquotes{adversarial recommend} in the above-mentioned indexing services. While search in DBLP returns publications containing the query term in the \textit{title}, the search results from Scopus and Google Scholar return publications containing the query \textit{both in the tile and the content}, thereby all-together forming a complete list of identified research works. We collected all resulting publications from DBLP, Scopus and Google Scholar search. In the second stage, we went through all the collected research works and removed all obviously irrelevant works. These for instance could include works that used AML for an application different than RS (e.g., in Computer Vision~\cite{DBLP:journals/corr/SzegedyZSBEGF13}, Speech Enhancement~\cite{DBLP:conf/interspeech/PascualBS17}).
We mostly turned our attention to conference-level and journal publications published in top conferences and to a lesser extent to workshop publications or works published in entry-level venues. Some of the considered journals and conferences include: the ACM Conference on Recommender Systems (RecSys), the International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR), the ACM International Conference on Web Search and Data Mining Conference (WSDM), the International World Wide Web Conference (TheWebConference), the International Joint Conferences on Artificial Intelligence (IJCAI), and the Knowledge Discovery and Data Mining conference (KDD).

In the subsequent core section of this survey, we present adversarial learning for attacking and defending RS in Section~\ref{sec:security}, AML for GAN-based RS in Section~\ref{sec:GAN}. Section~\ref{sec:conclusion} presents the open research directions and concludes the survey.

==> OLD_FILES/Sec2_Security.tex <==
\section{Adversarial Machine Learning for Security of RS}\label{sec:security}

For security concerns to be addressed appropriately in today's ML systems, there is a need to bridge the knowledge gap between the ML and computer security communities. Adversarial machine learning (AML) is a recently proposed and popularized approach that lies at the intersection of the above fields combining the best works of the two. The main goal of AML for security is to build systems can learn in normal conditions and when they are under attack --- in particular under \textit{adversarial attack} --- they can respond rapidly and
safeguard ML models against emerging adversaries' threats.

As the literature on AML for security emerged in the context of ML, in Section~\ref{sec:security} we first discuss the fundamentals on attack attacks on, and defenses of, ML models (cf. Section~\ref{subsec:AML_att_def}). We will then present AML-based RS focused on security applications in which we survey various identified literature in the field and classify them based on several methodological and evaluation-related dimensions (cf. Section~\ref{subsec:AML_RS}).

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\paperwidth]{Pictures/posion_evasion_attack.pdf}
    \caption{A schematic representation of the distinction between \textit{evasion} attacks and \textit{poisoning} attacks.}
    \label{figure:attack_scheme}
\end{figure}
\subsection{Foundations: Attack and Defense in ML and RS:}\label{subsec:AML_att_def}

\noindent \textbf{Task:} Throughout this section, we consider a supervising learning --- classification --- task. Assume a training dataset $\mathcal{D}$ of $n$ pairs $(x, y) \in \mathcal{X} \times \mathcal{Y}$, where $x$ is the input sample and $y$ is its corresponding class label. The problem of classification is formulated as finding a candidate function $f_\theta: \mathcal{X} \rightarrow \mathcal{Y}$  that can predict the class label around the input sample $x$, where $\theta$ is the model parameter.  This leads to solving an empirical risk minimization (ERM) problem of the form $\min_{\theta} \sum_{i \in \mathcal{D}} \ell(f(x_i;\theta),y_i)$ where $\ell(.)$ is the empirical risk function (the loss function). Various adversarial attacks aim to find a non-random perturbation $\delta$ to produce an adversarial example $x^{adv} = x + \delta$ that can cause an erroneous prediction (e.g., misclassfication).

\subsubsection{Attacks:}
In recent years, the advances made in deep learning (DL) have considerably advanced the intelligence of ML models in a unique number of predictive tasks such as visual classification of images and other unstructured data. Notwithstanding their great success, recent studies have shown that ML/DL models are not immune to security threats from adversarial use of AI. We can classify attacks along three main dimensions, attack \textit{timing} and \textit{goal}. 
\begin{itemize}
    
    \item \textbf{Attack timing}: As illustrated in Fig.~\ref{figure:attack_scheme}, an adversary can attack a ML model at two main stages of the learning pipeline, during \textit{training} or \textit{production}. These two categories of attacks are respectively known as (i) \textit{training-time attack} (aka causative or poisoning attack)~\cite{DBLP:conf/icml/BiggioNL12} and, ii) \textit{inference-time attack} (aka exploratory or evasion attack)~\cite{DBLP:journals/corr/SzegedyZSBEGF13}.
    \begin{itemize}
        \item \textit{Poisoning attack}: Data poisoning attacks are realized by injecting false data points into the training data with the goal that this can corrupt/degrade the model (e.g., the classifier). Poisoning attacks have been explored in the literature for a variety of tasks~\cite{DBLP:series/synthesis/2018Vorobeychik}, such as (i) attacks on binary classification tasks such as label flipping attack or attack against kernelized SVM, (ii) attacks on unsupervised learning such as clustering and anomaly detection and, (iii) attacks on matrix completion task in RS known as \textit{shilling attacks}~\cite{DBLP:conf/recsys/DeldjooNM19}. As an example, in the pioneering work~\cite{DBLP:conf/icml/BiggioNL12}, Biggio et al., propose a poisoning attack based on properties of the SVM optimal solution that could significantly degrade the classification test accuracy
     
        \item \textit{Evasion attack:} Unlike poisoning attacks, evasion attacks do not interfere with training data. They adjust malicious samples during the inference phase. These attacks are also named \textit{decision-time} attacks referring to their attempt to \textit{evade} the \textit{decision} made by the learned model at test  time. Evasive attacks are conducted by crafting \textit{adversarial examples} --- subtle but non-random perturbation --- added to original data to cause the learned model to produce erroneous output. Detailed information is presented in the following.
    \end{itemize}
    
    \item \textbf{Attack goal}: Attacks are conducted for different goals. We can distinguish between two main classes of attack goals: i) \textit{untargeted attack} and, ii) \textit{targeted attack}.
 \end{itemize}

\noindent{\textbf{Adversarial examples:}} Adversarial examples are additive perturbation of the input sample under a norm constraint whose goal is to fool the target model  (e.g., a classifier or a recommendation model). Perturbations are optimized by an attack algorithm known as \textit{adversarial attack} against the target model. To provide the reader with an intuitive insights of the mechanism behind adversarial attacks and defense strategies, we define them formally for a \textbf{classification} task~\cite{DBLP:series/synthesis/2018Vorobeychik}.

\begin{definition}[Untargeted adversarial attack]
    \label{def:untar_attack}
    \textit{The goal of the attacker in \textbf{untargeted adversarial attack} (misclassfication) is to add a minimal amount of perturbation $\delta$ on the input sample $x$ such that it can cause  incorrect classification}
    \begin{equation}
        \label{eq:att_untrg}
        \begin{aligned}
            & \min_{\delta}
            & & \left\lVert \delta \right\rVert \\
            & \text{s.t.:}
            & & f(x + \delta; \theta) \neq y , \ \ x + \delta \in [0,1]^n
        \end{aligned}
    \end{equation}
    \textit{where $y$ is the true class label. The second constraint $x + \delta \in [0,1]^n$ is a value-clipping constraint needed for images, to bound the adversarial samples into to a predefined range so that the images remain visible after adversarial attack. Alternatively, we can formulate this formulation into an \textbf{unconstrained optimization} problem where the goal of the attacker is to \textbf{maximize} the loss between the perturbed sample $x + \delta$ and true class $y$}
    \begin{equation}
        \label{eq:att_rel_gen}
        \begin{aligned}
            & \underset{\delta: \left\lVert \delta \right\rVert \leq \epsilon }{\text{max}}
            & &\ell(f(x+\delta; \theta),y) 
        \end{aligned}
    \end{equation}
    \textit{Obviously since adding an unbounded amount of noise on the input will eventually lead to a classification error, the goal of the attacker is to minimize a norm-constrained form of noise, that is $\left\lVert \delta \right\rVert \leq \epsilon$ for some exogenously given $\delta$. In the context of DNN, the above attacks are categorized based on the norm used to represent the magnitude of the noise according to the following norm types~\cite{DBLP:series/synthesis/2018Vorobeychik}: $l_0$, $l_1$ and $l_2$ and $l_{\infty}$.}
\end{definition}

\begin{definition}[Targeted adversarial attack]
    \label{def:untar_attack}
    \textit{The goal of the attacker in \textbf{targeted adversarial attack} is to perturb the input by adding a minimum amount of perturbation $\delta$ such that it can force the model to misclassify the perturbed sample into an illegitimate \textbf{target} class}
    \begin{equation}
        \label{eq:att_trg}
        \begin{aligned}
            & \underset{\delta}{\text{min}}
            & & \left\lVert \delta \right\rVert \\
            & \text{s.t.:}
            & & f(x + \delta; \theta) = y_t
        \end{aligned}
    \end{equation}
    \textit{\textit{where $y_t$ is the target class label; similarly the above problem can be expressed as a unconstrained optimization problem}}
    \begin{equation}
        \label{eq:att_rel_gen}
        \begin{aligned}
            & \underset{\delta: \left\lVert \delta \right\rVert \leq \epsilon }{\text{min}}
            & &\delta \ell(f(x+\delta; \theta), y_t) 
        \end{aligned}
    \end{equation}  
\end{definition}
The most common attack types so far exploited in the community of RS are fast gradient sign attack (FGSM)~\cite{DBLP:journals/corr/GoodfellowSS14} and Carlini and Wagner (C\&W) attacks, which belong to $l_{\infty}$-norm and $l_2$ and  attack types respectively. We provide the formal definition of the FGSM and C\&W attacks here.
\begin{definition}[FGSM attack]
    \textit{The fast gradient sign method (FGSM)~\cite{DBLP:journals/corr/GoodfellowSS14} utilizes the \textit{sign of the gradient} of the loss function to find perturbation that maximizes the training loss (for untargeted case)}
    \begin{equation}
        \label{eq:att_linf}
        \delta = \epsilon. \sign    (\bigtriangledown_x \ell(f(x;\theta),y))
    \end{equation}
    \textit{where $\bigtriangledown_x$ is the gradient of the loss function w.r.t. input sample $x$ and $\epsilon$ (perturbation level) represents the attack strength. The adversarial example is generated as $x^{adv} = x + \delta$. FGSM applies an $l_{\infty}$-bound constraint $||\delta||_{\infty} \leq \epsilon$ with the original idea to encourage perceptual similarity between original and perturbed sample. The unconstrained FGSM above aims to find perturbation that would increase/maximize the loss $\bigtriangledown_x$ value. The alternative approach for targeted FSGM was introduced by Kurakin et al.,~\cite{DBLP:conf/iclr/KurakinGB17}}
    \begin{equation}
        \label{eq:att_linf_targeted}
        \delta = - \epsilon. \sign    (\bigtriangledown_x \ell(f(x;\theta),y_t))
    \end{equation}
    \textit{where the goal is to maximize the conditional probability $p(y_t|x)$ for a given input $x$.}
\end{definition}

Several variants of the FGSM has been proposed in the literature~\cite{DBLP:journals/corr/abs-1911-05268,DBLP:journals/corr/abs-1810-00069}. For instance, the fast gradient value (FGV) method~\cite{DBLP:conf/cvpr/RozsaRB16}, which instead of using the sign of the gradient vector in FGSM, uses the actual value of the gradient vector to modify the adversarial change, or basic iterative method (BIM)~\cite{DBLP:conf/iclr/KurakinGB17}  (a.k.a iterative FGSM) that applies FGSM attack multiple times \textit{iteratively} using a small step size and within a total acceptable input perturbation level.


\begin{definition}[C\&W attack]
    \textit{The Carlini and Wagner (C\&W) attack~\cite{DBLP:conf/sp/Carlini017} is one of the most effective attack models against state-of-the-art adversarial defense strategies such as defensive distillation. The core idea of C\&W attack is to replace the standard loss function --- e.g., typically cross-entropy --- with an \textbf{empirically-chosen loss function} and use it in an \textit{unconstrained optimization formulation} given by $\underset{\delta}{\text{min}} \left\lVert \delta \right\rVert_p^p + c.h(x+\delta, y_t)$, where $h(\cdot)$ is the candidate loss function. The C\&W attack has been used with several norm-type constraint on perturbation $l_0$, $l_2$, $l_{\infty}$ among which the $l_2$-bound constraint has been reported to be most effective.}
\end{definition}

\textbf{Adversarial attacks on RS - challenges and differences with ML tasks}: In spite of the similarities between ML classification and recommendation learning tasks, there are considerable differences/challenges in adversarial attacks on RS compared with ML and the degree to which the subject has been studied in the respective communities:
\begin{itemize}
   
    \item \textit{Poisoning vs. adversarial attack:} The main focus of RS research community has been on \textit{hand-engineered} fake user profile (a.k.a shilling attacks) against rating-based CF. Given a URM with $n$ real users and $m$ items, the goal of a shilling attack is to augment a fraction of malicious users $\lfloor{\alpha n} \rfloor$ to URM ($\alpha \ll 1$) in which each malicious use profile can contain ratings to a maximum number of $C$ items. The ultimate goal is to harvest recommendation outcomes toward a illegitimate benefit, e.g., pushing some targeted items into the top-$K$ list of users for market penetration. Shilling attacks against RS have a established literature and their development face two main milestones: first, since the early of 2000s, where the focus of literature was focused on building hand-crafted fake profiles whose rating assignment follow different strategy according to random, popular, love-hate, bandwagon attacks among others~\cite{DBLP:journals/air/GunesKBP14}; the second research direction started in 2016 when the first ML-optimized attack was proposed by Li et al.,~\cite{DBLP:conf/nips/LiWSV16} on factorization-based RS. This  work reviews a novel type of data poisoning attack that applies the adversarial learning paradigm for generate poisoning input data. Nonetheless --- given their significant impact against modern recommendation models--- the research works focused on \textit{machine-learned adversarial attacks} against RS have recently received great attention by the research community.
    
    \item \textit{CF vs. classification models:} Attacks against classification tasks focus on enforcing wrong prediction of individual instances in the data. In RS however, the mainstream attacks rely on CF principles, i.e., mining similarity in opinions of like-minded users to compute recommendations. This interdependence between users and items can on one hand \textit{improve robustness} of CF, since predictions depend on a group of instances not on an individual one, and on other other hand may cause \textit{cascade effects}, where attack on individual user may impact other neighbor users~\cite{DBLP:conf/recsys/Christakopoulou19}.
   
    \item \textit{Attack granularity and application type:} Adversarial examples created for image classification task are empowered based on continuous real-valued representation of image data (i.e., pixel values), but in RS, the raw values are user, item IDs and ratings that are discrete in nature. Perturbing these discrete entities is infeasible since it may lead to changing the semantic of the input, e.g., loosely speaking $ID+\delta$ can result in a new user $ID$. Therefore, existing adversarial attacks in the field of ML are not transferable to the RS problems trivially. Furthermore, in the context of attacks against vision tasks, the perturbations often need to be \dquotes{human-imperceptible} or \dquotes{inconspicuous} (i.e., may be visible but not suspicious)~\cite{DBLP:journals/corr/abs-1911-05268}. How can we capture these nuances for designing attacks in RS remains as a challenge.
\end{itemize}

\subsubsection{Defense against adversarial attacks:}
From a broad perspective, defense mechanisms against adversarial attacks can be classified as \textit{detection} methods and methods seeking to increase the \textit{robustness} of the learning model. The goal of this section is to briefly review approaches that build \textit{robust ML} models in adversarial settings. The prominent methods used in RS are (i) the robust optimization and, (ii) the distillation method.

\textbf{Robust optimization against adversarial attacks:}
At the heart of robust optimization methods is the assumption that \textbf{every sample} in the training data $\mathcal{D}$ can be a source for adversarial behavior. It performs an ERM against a specific adversary on each sample in $\mathcal{D}$ and applies a zero sum-game between the prediction and attack adversaries
leading to the following \textbf{robust optimization} framework
\begin{equation}
    \begin{aligned}
        \label{eq:robust_opt_2}
         \min_{\theta}  \sum_{i \in \mathcal{D}_s} \max_{\delta: \left\lVert \delta \right\rVert \leq \epsilon} \ell(f(x_i+\delta; \theta),y_i)
    \end{aligned}
\end{equation}
\textit{where $\epsilon$ is an upper-bound on the adversarial perturbation's power $\delta$.} The ultimate goal in robust optimization is that the prediction model will perform equally well with adversarial and clean inputs.

\begin{definition}[Adversarial training]
\textit{The goal of adversarial training is to build a robust model from ground-up on a training set augmented with adversarial examples. Adversarial regularization is one of the mostly investigate techniques for adversarial training, which utilizes an approximation of the worst-case loss function --- i.e., $\max_{\delta: \left\lVert \delta \right\rVert \leq \epsilon} \ell(f(x + \delta; \theta),y_i)$ --- as the regularizer.}
\begin{equation}
    \label{eq:robust_opt_adv_reg}
        \ell_{T} = \underbrace{\min_{\theta}  \sum_{i \in \mathcal{D}} [\ell(f(x; \theta),y_i) + \lambda \underbrace{\max_{\delta: \left\lVert \delta \right\rVert \leq \epsilon} \ell(f(x + \delta; \theta),y_i)}_\text{optimal attack model}}_\text{optimal robustness-preserving prediction}]
\end{equation}
\textit{As it can be noted, the inner maximization finds the \textbf{strongest attack}  against the prediction model that is subject to adversarial perturbation. The other minimization  estimates the \textbf{strongest defensive} against a given attack by giving up a level of accuracy due the regularization The parameter $0<\lambda<1$ controls the trade-off between accuracy (on clean sample) and robustness (on perturbed data)}.
\end{definition}

\begin{exmp}[Adversarial training of BPR-MF]
BPR is the state-of-the-art method for personalized ranking  implicit feedbacks. It builds on the assumption that user would appreciated item consumed by them more than item not consumed. Given the training dataset $D$ composed of positive and negative item for each user $(u,i,j)$ (user $u$, a positive item $i$ and negative item $j$), the BPR objective function is defined as following
\begin{equation}
    \label{eq:BPR_loss}
    \ell_{BPR}(\mathcal{D} | \Theta) = \argmax_{\Theta} \sum_{(u,i,j) \in \mathcal{D}} ln \, \sigma(\hat{x}_{ui}(\Theta)-\hat{x}_{uj}(\Theta))-\lambda\left \| \Theta \right \|^2
\end{equation}
where $\sigma$ is the logistic function, and $\hat{x}_{ui}$ is the predicted score for user $u$ on item $i$ and $\hat{x}_{uj}$ is the predicted score for user $u$ on item $j$; $\lambda \left \| \Theta \right \|^2$ is a regularization method to prevent over-fitting.\footnote{As it can be noted, BPR can be viewed as a classifier on the triplet $(u,i,j)$, where the goal of the learner is to classify the difference $\hat{x}_{ui}-\hat{x}_{uj}$ as correct label +1 for a positive triplet sample and 0 for a negative instance.} Adversarial training of BPR-MF similar to Eq.~\ref{eq:robust_opt_adv_reg} can be formulated as
\begin{equation}
    \label{eq:robust_bpr_adv_reg}
    \ell_{APR} = \underbrace{\min_{\theta}  \sum_{(u,i,j) \in D} [\ell_{BPR}(\mathcal{D} | \Theta) + \lambda \underbrace{\max_{\delta: \left\lVert \delta \right\rVert \leq \epsilon} \ell_{BPR}(\mathcal{D} | \Theta + \delta)]}_\text{optimal attack model against BPR}}_\text{optimal robustness preserving defensive}
\end{equation}
\end{exmp}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\paperwidth]{Pictures/adversarial_framework_v2.pdf}
    \caption{A notional view of Adversarial Recommendation Framework integrating the adversarial perturbations on users and items, and their side information, model parameters.}
    \label{figure:adv_framework}
\end{figure}


\subsection{Adversarial Machine Learning for Attack and Defense on RS}\label{subsec:AML_RS}
In this section, we focus on state-of-the art approaches on the application of AML in RS research. RS which employ AML for security applications in recommendation tasks, follow the simplified steps sketched in Fig.~\ref{figure:adv_framework}. -- A short information to figure can go here--
In the following, in addition to providing concise summaries of the surveyed works, for a convenient overview, we categorize the reviewed research articles in Tables~\ref{tbl:adl_attack} according to the following dimensions:

\begin{itemize}
     \item \textbf{Model:} This column lists the model name and provides the reference to the main paper.
     
     \item \textbf{Attack and Defense Model:} This column represents the main \textit{attack} and \textit{defense} strategies applied on various recommendation models and the \textit{attack granularity} on the system.
     \begin{enumerate}
         \item \textit{Attack model:}
         Among all attacks strategies proposed in the community of MM~\cite{DBLP:journals/access/AkhtarM18}, in RS the most dominant attack approaches to date have been \textit{FGSM} and \textit{C\&W}, and attacks based on \textit{GANs}.
         \item \textit{Defense model:}  As for the best defensive strategy against attack, we have found the strategy \textit{adversarial training (aka adversarial regularization)} as the most commonly-adopted approach irrespective of the attack model, while the next defensive approach \textit{distillation} is adopted only by a single paper.
         \item \textit{Attack granularity:} This column represents the level of data on which the adversarial perturbation are added on. It is important to note that while in the computer vision domain, these perturbations are added on the raw data (e.g., pixel values), in RS they are applied on the model parameters of recommendation strategy, as illustrated in Fig.~\ref{figure:adv_framework}. In particular, adversarial perturbations are added to one of the following data: (i) directly on the \textit{user profile }(i.e., user rating profile), (ii) \textit{user and item latent factor model parameters} in a LFM, e.g., according to $\mathbf{p}'_u = \mathbf{p}_u + \delta$, $\mathbf{q}'_i = \mathbf{q}_i + \delta$ in which $\mathbf{p}_u, \mathbf{q}_i \in \mathbb{R}^F$ are $F$-dimensional embedding factors  whose linear interaction explains an unobserved preference; (iii) and (iv) \textit{embeddings representing side information of user and items} respectively.
    \end{enumerate}
     
     \item \textbf{Recommendation \& Learning:}
     The core recommendation models that we consider in this survey are CBF, CF and CA. We also consider hybrid system but do not specify a placeholder for hybrid systems; if an approach use both CBF+CF, we simply mark both corresponding columns, regardless of which hybridization technique it uses)~\cite{aggarwal2016ensemble}. Instead, given the ML (optimization)-based approach for most of the considered papers, we categorize papers based on the recommendation prediction model according to \textit{linear LFM} (e.g., MF or variations of that such as PMF), \textit{linear tensor factorization} (TF), \textit{non-linear models based on auto-encoder} (NL-AE) and \textit{neural network} (NL-NN); furthermore we classify the loss function used in the core optimization model of the attack and defense scenarios based on \textit{BPR}~\cite{DBLP:conf/uai/RendleFGS09} and \textit{cross-entropy}.

\end{itemize}

\felice{test}
We will now follow to provide a more detail analysis of each selected paper.
\input{Tables/table_security}

Looking at table~\ref{tbl:adl_attack} globally, we can note that adversarial personalized ranking (APR)~\cite{DBLP:conf/sigir/0001HDC18} by He et. al., which was published in SIGIR'18 was the first work that formally addressed AML to improve the robustness of BPR-MF. After this pioneering work, in the following years a growing number of works have considered application of AML for different recommendation tasks. Another interesting observation is the co-occurrence of the attack type FGSM and defense model adversarial training (AdReg). In fact, the adversarial training procedure based on FGSM is the first defense strategy proposed by Goodfellow et al.~\cite{DBLP:journals/corr/GoodfellowSS14} to train DNNs resistant to adversarial examples. The authors interpret the improvement in robustness to adversarial examples because the proposed procedure is based on the minimization of the error on adversarially perturbed data.

He et al.~\cite{DBLP:conf/sigir/0001HDC18} are the first to propose adversarial learning framework for recommendation. The proposed model, called \textit{adversarial personalized ranking (APR)}, examines the robustness of BPR-MF with respect to adversarial perturbation on users and items embedding of a BPR-MF~\cite{DBLP:conf/uai/RendleFGS09}. The authors firstly verify the success of using the \textbf{adversarial training} as a defence against adversarial perturbations and demonstrate the competitive results in applying adversarial training on BPR-MF.

Tang et al.~\cite{8618394} put under adversarial framework another BPR model, namely visual-BPR (VBPR). VBPR is built upon BPR and extends it by incorporating visual dimensions (originally based on deep CNN feature) by using an embedding matrix. In~\cite{8618394}, the authors first motivate the importance for adversarial training of VBPR conceptually by visually depicting how a surprisingly modest amount of adversarial perturbation ($\epsilon = 0.007$) added on raw image pixels \textemdash~where the noises added are barely perceivable to human eye \textemdash~can alter recommendation raking outcomes of VBPR and produce erroneous results. The proposed model by authors therefore consists of constructing adversarial perturbations under the FGSM attack model and adding them on the deep latent feature of items' images extracted by CNN (i.e., ResNet50~\cite{DBLP:conf/cvpr/HeZRS16}) with the goal to learn robust image embedding parameters. One of the key insights about this work is that it does not add perturbations directly on raw image pixels for two main reasons: (i) it would require the feature extractor (CNN) component and the recommender model to be trained end-to-end with overfitting issues on the CNN due to the sparsity of user-item feedback data, (ii) it would be a time consuming operation because at each update of the recommender model it is necessary to update all the CNN parameters.

In the above-mentioned works, the authors adopt several steps to validate the effectiveness of the proposed adversarial training framework, which can be summarized according to the following dimensions: (i) the \textit{generalization} capability, (ii) the comparison of \textit{adversarial noise v.s. random noise}, and (iii) the \textit{robustness of models}. Regarding (i), the key insight is that adversarial training approaches (i.e., AMF and AMR) can lead to learning model parameters, which can enhance model generalization capability \textemdash~in other words improvement of the general performance of recommendation while not being exposed to adversarial perturbation. Concerning (ii), it has been demonstrated that the impact adversarial perturbation on classical recommendation models (e.g., MF-BPR or VBPR) is significantly larger than their counter-part random noise under similar perturbation level. For instance,~\cite{8618394} show that by exposing MF to adversarial and random noise, the test NDCG is decreased by -21.2\% and -1.6\% respectively \textemdash~i.e., an impact of approximately 13 times difference. Dimension (iii) constitutes the core of the system validations in these works in which compelling evidence has been provided on the vulnerability of classical recommendation models to adversarial examples, or equivalently the robustness of the proposed training framework against adversarial samples. To provide an illustrating example, in~\cite{8618394} it has been shown for an experiment on Amazon dataset, that by changing the perturbation level from $\epsilon = 0.05$ to $\epsilon = 0.2$, the amount of decrease in NDCG ranges from -8.7\% to -67.7\% whereas for AMR it varies from -1.4\% to -20.2\%. These results suggest that approaches using adversarial learning instead of classical learning act significantly more robust against adversarial perturbations.

In~\cite{DBLP:conf/www/ParkC19}, the authors propose a system to address CF recommendation based on implicit feedbacks. The main issue in learning from implicit interaction is characterized by scarcity of negative feedbacks compared with positive ones, regarded as one-class problem. Sampling uniformly from unobserved data, known as \textit{negative sampling }has been introduced in prior work to address this issue. The proposed system in~\cite{DBLP:conf/www/ParkC19} is called AdvIR, which entails an adversarial sampling and training framework to learn recommendation models from implicit interactions. The system applies adversarial training on both positive and negative interaction separately, to create informative adversarial positive/negative samples. The proposed adversarial training approach works for both discrete and continuous input by adding the adversarial perturbation directly on the input vector (e.g., one-hot encoding user-id).

Yuan, F. et al.~\cite{DBLP:conf/sigir/YuanYB19, DBLP:conf/ijcnn/YuanYB19} use the adversarial training framework for a neural network-based recommendation model, namely collaborative denoising auto-encoder (CDAE)~\cite{DBLP:conf/wsdm/WuDZE16}, based on which the authors propose two variations, namely: i) the adversarial collaborative auto-encoder (ACAE) and (ii) fine-grained collaborative auto-encoder (FG-ACAE). ACAE applies adversarial noise on encoder and decoder parameters and trains adversarial training framework. FG-ACAE consider the impact of adversarial noise in a more fine-grained manner. In particular, in FG-ACAE adversarial noises are added on not only encoder and decoder, but also on the user's embedding matrix as well as hidden layers of the network. Furthermore, in order to increase the flexibility of training all the noise factors in ACAE and FG-ACAE are controlled by different parameters. The experimental results confirm the trend that AdReg may improve the model's robustness against adversarial perturbed input, as well as superior recommendation performance.

Chen and Li~\cite{DBLP:conf/recsys/ChenL19} combine tensor factorization and adversarial learning to improve the robustness of pairwise interaction tensor factorization (PITF)~\cite{DBLP:conf/wsdm/RendleS10} in context-aware recommendation. Comparison with standard tensor models in tag recommendations demonstrates that also the adversarial framework outperforms state-of-the-art tensor-based recommenders.

Du et al.~\cite{DBLP:journals/tmm/DuFYXCT19} approach security issues for \textbf{C\&W  attacks}~\cite{DBLP:conf/sp/Carlini017}, one of the most effective attack methods where adversaries have the full knowledge of the target model (i.e., white-box settings). The authors proposed to make more robust neural network-based collaborative filtering models (e.g., NCF~\cite{DBLP:conf/www/HeLZNHC17}) by using \textbf{knowledge distillation}~\cite{DBLP:journals/corr/HintonVD15} instead of the adversarial (re)training. The framework integrates the knowledge distillation-from a teacher network to a student one- with the injection of additive adversarial noise at training time. Experiments demonstrated that this system enhance the robustness of the treated recommender model.

Li R. \textit{et al.}~\cite{DBLP:conf/www/LiLWZW19} propose a novel recommender model, named ~\hlmethod{Click Feedback-Aware Network} (CFAN), to provide query suggestions considering the sequential search queries issued by the user and and his the history of clicks.
The authors employ additional adversarial (re)training epochs (i.e., adding adversarial perturbations on item embeddings) to improve the robustness of the model.

Di Noia \textit{et al.}~\cite{DBLP:conf/dsn/DiNoia20} explore the influence of targeted adversarial attacks (i.e., FGSM\cite{DBLP:journals/corr/GoodfellowSS14}, and PGD~\cite{DBLP:conf/iclr/MadryMSTV18}) against original product images used to extract deep features in state-of-the-art visual recommender models (i.e., VBPR~\cite{DBLP:conf/aaai/HeM16}, and AMR~\cite{8618394}). The authors verify that recommendation lists can be altered such that a low recommended product categories can be pushed by adding adversarial noise on product images in a human-imperceptible way.  

\input{Tables/table_security_datasets_metrics}

==> OLD_FILES/Sec3_Generative.tex <==
\section{Adversarial Learning for GAN-based Recommendation}~\label{sec:GAN}
What we presented in Section~\ref{sec:security} dealt with a class of statistical models referred to as \dquotes{discriminative} models. In the context of classification, a discriminative model is a model that seeks to find the mapping $x \rightarrow y$ for a given input-label pair $(x,y)$, by learning the conditional probability $p(y|x)$ from the training data. The focus of the current section is on a novel class of \dquotes{generative} models, named \textit{generative adversarial networks} (GANs). A generative model is a model that seeks to find the mapping $y \rightarrow x$ by learning the conditional probability $p(x|y)$ from the data. For example, if $y$ indicates whether an item is appealing to a user, $p(y|x)$ would measure the probability --- or whether or not --- the user would like the product; instead $p(x|y=1)$ looks into the distribution of product features appreciated by the user and $p(x|y=0)$, the distribution of irrelevant product features for the user. Loosely speaking, a generative model cares about the \textit{generative} process behind data --- or product features (in the example) ---  to categorize the data instances. A discriminative model disregards the information about how the data were generated, it merely focuses on how to \textit{categorize} given data instances.

GANs are a powerful class of generative models that use two networks --- trained simultaneously in zero-sum game --- with one network focused on data generation and the other centered on discrimination. The adversarial learning scheme --- or the the min-max game --- which lies in the heart of GANs empowers these ML models with phenomenal capabilities such as the ability to model high-dimensional distributions. As the result, these networks have been exploited to solve challenging problem in the computer vision. For instance in~\cite{DBLP:conf/cvpr/KarrasLA19}, a GAN model is proposed to transfer style plausible looking scenes. The research in RS community has used the generalization (or in technical term data distribution capturing) potential of GANs as an opportunity to solve variety of tasks relevant to RS.

In summary, it is important to distinguish between two different applications of AML in RS and in a general term:

\begin{enumerate}
    \item Adversarial learning to study attacks on, and defenses of machine-learned RS models. This aspect is centred on the \dquotes{security} of recommender models. We discussed this aspect in Section~\ref{sec:security}.
    \item  Adversarial learning scheme used in GANs, empowering them to generalize and learn the data distributions. We refer to this aspect the \dquotes{generative} potential of GANs, which have been exploited in the field of RS. The focus of the current section is on this aspect.
\end{enumerate}
As it can be noted the term \dquotes{adversarial} inside generative adversarial networks refers to the learning scheme used by these models and \textit{not the application}. In other words, the application of GANs for RS covers variety of aspects not limited to the security of RS, as we will see in the subsequent sections.

\subsection{Foundations of Generative Adversarial Networks (GANs)}

GAN are deep generative models proposed by Goodfellow et al.,~\cite{DBLP:journals/corr/GoodfellowPMXWOCB14} in 2014. A GAN is composed by two components, a generator $\mathcal{G}$, and a discriminator $\mathcal{D}$. The generator works to capture the real data distribution to generate adversarial examples and fool the discriminator,  while the discriminator endeavors to distinguish the fake examples from real ones.
This competition, known as adversarial learning, ends when the components reach the Nash equilibrium. The GAN architecture is shown in Figure~\ref{fig:gan_architecture}.

\begin{definition}[Conventional Vanilla GAN]
    \textit{Assume that we are given a dataset of $n$ input samples $x \in \mathcal{X}$, where $x \sim \mathbb{P}_{\mathcal{X}}$ and $\mathbb{P}_{\mathcal{X}}$ represents the probability distribution of the original data and suppose $z \in \mathcal{Z}$ denotes a sample from some latent space $\mathcal{Z}$. We are interested in sampling from $\mathbb{P}_{\mathcal{X}}$. The goal of GAN is to train the generator $\mathcal{G}$ to transform samples $z \sim \mathbb{P}_{\mathcal{Z}}$ into $g_{\theta}(z) \sim \mathbb{P}_{\theta}$ such that $ \mathbb{P}_{\theta} \approx \mathbb{P}_{\mathcal{X}}$. The role of the discriminator is to distinguish $\mathbb{P}_{\theta}$ and $\mathbb{P}_{\mathcal{X}}$ by training a classifier $f_{\phi}$. The training involves solving the following min-max objective}
    \begin{equation}
         \label{eq:gan_basic}
         \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z)))
    \end{equation}
    \textit{where $\theta$ and $\phi$ are model parameters of the discriminator and generator respectively, learned during the trained phase. Different distance measures $f_{\theta}$ lead to different GAN models, e.g., Vanilla GAN (based on Jensen-Shannon divergence)~\cite{DBLP:journals/corr/GoodfellowPMXWOCB14}, Wasserstein GAN (based on Wasserstein distance)~\cite{DBLP:journals/corr/ArjovskyCB17}, and Conditional GAN (based on class conditioning on both the generator and discriminator)~\cite{DBLP:journals/corr/MirzaO14}.}
\end{definition}

\begin{definition}[Conditional-GAN (CGAN)]
    \textit{Conditional GAN is proposed by Mirza et al.,~\cite{DBLP:journals/corr/MirzaO14} in which the model extends the conventional vanilla GAN presented in Def. 3.1, by incorporating $c$ --- an extra condition information term --- on both the input of the generator $\mathcal{G}$ and the discriminator $\mathcal{D}$, thus conditioning them on this extra term}
    \begin{equation}
         \label{eq:gan_basic}
         \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) =  \, \mathbb{E}_{x \sim \mathbb{P}_{\mathcal{X}}} \, \log f_{\phi}(x|c) + \mathbb{E}_{z \sim \mathbb{P}_{\mathcal{Z}}} \log (1-f_{\phi}(g_{\theta}(z|c)))
    \end{equation}
    \textit{where $c$ can represent any auxiliary information to the networks such as class labels, content features, data from other domains and so forth.}
\end{definition}

\begin{figure}
    \includegraphics[width=0.85\textwidth]{Pictures/GAN_joint.pdf}
  \caption{Schematic comparison of two well-known GAN models: (a) conventional vanilla GAN with filled color and (b) Conditional GAN (which includes the dashed blue entities)}
  \label{fig:gan_architecture}
\end{figure}

\subsection{GAN-based Recommendation Framework}\label{subsec:GAN_RF}

GANs have been successfully applied in start-of-the-at RS to learning recommendation models. Since the first pioneering GAN-based work IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} in 2017, we have witnessed a rapid adoption of these network architectures in many traditional and novel applications and domains. The attempt of this section is to provide a conceptual framework that will show how GANs are employed in RS domain and shed light on particularities and differences of GAN application in RecSys and ML. This section would continue by providing a survey of recent advances in GAN-based recommendation models.
\vspace{3mm}\\
\noindent {\textbf{Historical background:}} 
Among the pioneering works that proposed a GAN framework for improving the utility of item recommendation in a CF scenario, it is worth mentioning IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and GraphGAN~\cite{DBLP:conf/aaai/WangWWZZZXG18}. The former proposes a solution for CF based on MF whereas the second one proposed a graph-representation learning for the same problem. We discuss these two pioneering works in detail here (IRGAN) and in Section~\ref{subsec:GAN_CF_rec} (GraphGAN).

A fundamental question in IR is: \dquotes{Given a query $q$ and a document ($d$), what is the probability that $d$ is relevant to $q$?}. The answer to this basic question constitutes the basis for document ranking in IR and has been answered under two different perspectives, the generative model and the the discriminative one:

\begin{itemize}
    \item The \textbf{generative model} makes the underlying assumption that there exists a stochastic \textit{generative process} between $d$ and $q$. It then answers the above basic question in probabilistic sense, given by \dquotes{How to compute the probability of relevance $R$ for a given document $d$ with respect to a query $q$, or $p(R=r|d,q) = 1- p(R=\bar{r}|d,q)$?}. In text retrieval, two approaches are commonly adopted to estimate the probability $p \, (R=r|d,q)$, which are proven to be equivalent based on different parametrization of the likelihood under the Bayes rule. The first approach is the Robertson-Sparck Jones~\cite{DBLP:journals/ipm/Jones79} approach that models the probability of relevance in a forward manner $q \rightarrow d$ via factorization $p(R=r|d,q) = p(q|r) \,  p(d|q, r)$. It can be shown that this problem is equivalent to the naive Bayes model for classification in which for a given information need $q$, the goal is to classify the document into classes $r$ and $\bar{r}$. The second approach is based on language modeling paradigm~\cite{DBLP:conf/sigir/PonteC98}, that takes the reverse approach $d \rightarrow q$ via factorization $p(R=r|d,q) = p(d|r) p(q|d, r)$; it aims to generate query terms for a given document.
   
    \item The \textbf{discriminative model} uses a machine learning approach to answer the basic question in which documents and queries are jointly considered as features and the goal is to predict relevance in ML way by using a large amount of training data. Therefore the problem can be seen as $q + d \rightarrow d$. A prominent example of this approach is learning to rank (LTR) whose aim to is to learn the right ranking of documents (or items) given a representation of an information need (query or context).
\end{itemize}

Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} presented a unified theory of generative and discriminative methodologies in IR under the GAN framework named IRGAN. The proposed system is validated for different tasks including item recommendation in which the query is constructed from user's historical interactions. During adversarial learning --- the min-max game --- the generator learns true distribution of relevant items as much as possible.  It turns out that this novel training idea results in more satisfactory accuracy in recommendation than optimizing the traditional pure discriminate loss functions based on pointwise, or pairwise, objectives.\\

\noindent {\textbf{GAN-CF problem formulation and conceptual model:}}
The prominent recommendation models in the literature that successfully apply GAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17,DBLP:conf/aaai/WangWWZZZXG18} for CF task, utilize the two-player min-max game with objective function built on top of Eq.~\ref{eq:gan_basic}.
\begin{definition}[The GAN-CF model]
    \textit{Let $\mathcal{U}$ and $\mathcal{I}$ denote a set of users and items in a system, respectively. The training objective is given by}
    \begin{equation}
         \label{eq:irgan_basic}
          \min_{\theta} \max_{\phi} L(\mathcal{G}_\theta, \mathcal{D}_{\phi}) = \, \mathbb{E}_{i \sim \mathbb{P}_{\mathcal{X}}(i|u)} \, \log f_{\phi}(i|u) + \mathbb{E}_{\hat{i} \sim \mathbb{P}_{\theta}(\hat{i}|u)} \log \, (1-f_{\phi}(\hat{i} | u))
    \end{equation}
    \textit{where $i$ is an item receiving implicit (or explicit) feedback by user $u$ (e.g., purchased) and $\hat{i}$ is a generated item. In IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17}, the score functions in $\mathcal{G}$ and $\mathcal{D}$ are generally based on the \textit{sigmoid} function.}
\end{definition}
A few observations are important to be made here: (i) the output of generator $\mathcal{G}$ is a set of item indices deemed relevant to user $u$; (ii) both $\mathcal{G}$ and $\mathcal{D}$ are \textit{user-conditioned}, signifying that model parameters are learnt by considering \textbf{user's personalization}; (iii) the GAN-based CF works does use the noise term as input (to $\mathcal{G}$) as the goal is to generate one unique --- yet plausible --- item rather than a set of items. Figure~\ref{fig:GAN-CF} summarizes these aspects conceptually.

\noindent {\textbf{Discrete outcome and sampling strategies:}} 
The parameters in the GAN-CF model are learned in an end-to-end fashion. 
However, before we can take benefit of this training paradigm, the system needs to solve a critical issue that does not exist on original GAN presented in Def. 3.1. based on sampled noise signal. The generation of recommendation lists is a discrete sampling operation, i.e., performed over discrete candidate items, see Figure~\ref{fig:GAN-CF}. Thus, the gradients that are derived from the objective function in Eq.~\eqref{eq:irgan_basic} cannot be directly used to optimize the generator via gradient descent as happens in the original GAN formulation, where gradients are applied for differentiable values (e.g.,images and videos). To obtain differentiable sampling strategy in GAN-CF models, two sampling strategies are proposed in the literature based on reinforcement learning algorithm and the Gumbel-Softmax differentiable sampling procedure~\cite{DBLP:conf/nips/SuttonMSM99,DBLP:conf/iclr/JangGP17, DBLP:journals/eswa/SunWWY19}, summarized in Table~\ref{tbl:smple_strg}.

\input{Tables/sampling_strategy}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{Pictures/gan_cf_new2.pdf}
    \caption{A conceptual view of GAN-CF incorporating GAN to address item recommendation task.}
    \label{fig:GAN-CF}
\end{figure}

\subsection{GAN-based Recommendation Models: State of the Art}\label{subsec:Applications of GAN-based Recommendation}
In this section, we focus on the novel trend of AML research --- GAN-based Recommendation --- applied to various domains. We have identified a total of 47 papers that integrate GAN in order to accomplish a particular RS-related task. We can classify these tasks according to:
\input{Tables/gan_rs.tex}

\begin{enumerate}
    \item Collaborative Recommendation
    \item Context-aware Recommendation
    \item Cross-domain Recommendation
    \item Fashion Recommendation
\end{enumerate}
In the following, we review each of these application scenarios in detail. Table~\ref{tbl:gan-approaches} to summarize the proposed models providing insights about the constituting bulling bollocks of the GAN model.
\vspace{-2mm}
\subsubsection{Collaborative Recommendation}\label{subsec:GAN_CF_rec}
GANs have been shown powerful in generating relevant recommendations --- in particular using the CF approach --- and be able to successively compete with state-of-the-art models in the field of RS. We have identified the following reasons for the potential of GANs in RS: (i) they are able to generalize well and learn unknown user preference distributions and thus be able to model user preference in complex settings (e.g., IRGAN~\cite{DBLP:conf/sigir/WangYZGXWZZ17} and CFGAN~\cite{DBLP:conf/cikm/ChaeKKL18}); (ii) they are capable of generate more negative samples than random samples in pairwise learning tasks (e.g., APL~\cite{DBLP:journals/eswa/SunWWY19}, DASO~\cite{DBLP:conf/ijcai/FanD0WTL19}) and (iii) they can be used for data augmentation (e.g., AugCF~\cite{DBLP:conf/kdd/WangYWNHC19}  and RAGAN~\cite{DBLP:conf/www/ChaeKKC19}).

\setlength{\parindent}{15pt} [\textbf{IRGAN}] As presented in Section~\ref{subsec:GAN_RF}, IRGAN --- the work by Wang et. al.,~\cite{DBLP:conf/sigir/WangYZGXWZZ17} --- is presumably the first attempt to integrate generative and dicriminative approach to IR under the same roof by proposing a GAN-based IR model. The authors demonstrate the application of IRGAN for web search, item recommendation and question answering tasks. 

\setlength{\parindent}{15pt} [\textbf{GraphGAN}] In~\cite{DBLP:conf/aaai/WangWWZZZXG18}, H. Wang et al., propose GraphGAN --- a graph-based representation learning --- (a.k.a. network embedding) for CF recommendation. Graph-based analysis are a booming research in recent years due to their ubiquity in real-world problems such as modeling user preference for item recommendation as well as social graphs in social media (SM) networks, co-occurrence graph in linguistics, citation graph in research, knowledge graph and so forth. The central idea of network embedding is to represent each entity in a graph with a lower-dimensional latent representation to facilitate tasks within the network and prediction over entities. For example, such latent representation can allow to perform prediction for supervised tasks or the distance between node embedding vectors can serve as a useful measure in unsupervised tasks. GraphGAN can be viewed as a graph-based representation of IRGAN, where queries/items are \textit{nodes} of the graph. For a given node $v_c$, the objective of $\mathcal{G}$ is to learn the ground-truth connectivity distribution over vertices $p_{true}(v|v_c)$, whereas $\mathcal{D}$ aims to discern whether or not a connectivity should reside between vertex pairs $(v,v_c)$. GraphGan furthermore proposes the graph softmax as $\mathcal{G}$ --- instead of traditional softmax --- which appears to boost the computational efficiency of training (graph sampling and embedding learning) performed by  $\mathcal{G}$.

\setlength{\parindent}{15pt} [\textbf{GAN-HNBR}] From an application perspective, GAN-based graph representation have been also applied in more niche domains of RS including personalized citation recommendation. The goal is to recommend research articles for citation by using a content-based and author-based representation~\cite{DBLP:conf/ismis/ZhangYCD18} or learning heterogeneous bibliographic network representation (HBNR). In~\cite{DBLP:conf/aaai/CaiHY18} Cai et al., propose GAN-HNBR --- a GAN-based citation recommendation model --- that can learn the optimal representation of a bibliographic network consisting of heterogeneous vertex content features such as papers and authors into a common shared latent space and provide personalized citation recommendation.

\setlength{\parindent}{15pt} [\textbf{CFGAN}] CFGAN is introduced in~\cite{DBLP:conf/cikm/ChaeKKL18}, to address a problem with \textit{discrete items} in IRGAN, where $\mathcal{G}$ produces at each iteration a single item index, which is a discrete entity in nature. This is different from the original GAN in the CV domain in which the output of $\mathcal{G}$ is an image (i.e., a vector). The generation of discrete item indices by $\mathcal{G}$ results in a poor sampling of items from the pool of available alternatives (i.e., samples identical to ground-truth) deteriorating the performance of $\mathcal{G}$ and $\mathcal{D}$ --- instated of improvement --- during the min-max training iteration. CFGAN introduces \textit{vector-wise
training} in which $\mathcal{G}$ generates continuous-valued vectors to avoid misleading $\mathcal{D}$, which in turn improves the performance of both $\mathcal{G}$ and $\mathcal{D}$. The authors show the improvement of CFGAN over IRGAN and GraphGAN baselines. As an example, with regards to P@20 on the Ciao dataset, the improvement is $100\%$  for CFGAN vs. IRGAN (0.45 v.s. 0.23) and $160\%$ for CFGAN vs. GraphGAN (0.45 v.s. 0.17), which turns to be a significant improvement of the recommendation accuracy.

\setlength{\parindent}{15pt} [\textbf{Chae et al.,}] In ~\cite{8525831}, Chae et al. propose an auto-encoder-based GAN, in which an auto-encoder(AE), as $\mathcal{G}$ models the underlying distribution of user preference over items. The primary motivation behind this work is the conventional GAN-based MF-based approaches are linear. Instead, the proposed system can generate non-linear latent factor model and uncover more complex relationships in the underlying use item interaction matrix.

\setlength{\parindent}{15pt} [\textbf{VAE-GAN]} An adversarial variational auto-encoder (VAE) is adopted in~\cite{8663730}, where the authors propose the usage of a GAN to regularize VAE by imposing an arbitrary prior on the latent representation (based on implicit feedback). A similar work can be found in~\cite{DBLP:conf/icde/TongLZSC19, DBLP:conf/cikm/LeeSM17}, which exploits a VAE to enhance the robustness of adversarial examples. The author furthermore present the Wasserstein Distance with gradient penalty.

\setlength{\parindent}{15pt} [\textbf{CALF]} Other issues of IRGAN such as sparsity causing gradient vanishing and update instability and discrete value preventing a training to optimize using gradient descent are addressed in~\cite{DBLP:conf/flairs/CostaD19}. The proposed solution is named convolutional adversarial latent factor model (CALF), which employ a CNN to learn correlations between embeddings and Rao-Blackwell sampling to deal with discrete values optimizing CALF.

\setlength{\parindent}{15pt} [\textbf{PD-GAN]} The authors of~\cite{DBLP:conf/ijcai/WuLMZZG19} propose a solution to improve diversity of CF-based recommendation with GAN based on personalized diversification.

\setlength{\parindent}{15pt} [\textbf{LambdaGAN]} In~\cite{DBLP:conf/ijcnn/WangZC019}, the authors Wang et al., propose LambdaGAN --- a GAN model with lambda ranking strategy --- that improves the recommendation performance in a pairwise ranking setting by proposing lambda rank~\cite{DBLP:conf/cikm/YuanGJCYZ16} function into the adversarial learning of the proposed GAN-based CF framework.

\setlength{\parindent}{15pt} [\textbf{VAEGAN]} A variant of VAE is introduced in~\cite{DBLP:conf/ijcai/YuZCX19} to address the limited expressiveness of the inference model and latent features, which reduces the generalization performance of the model. The proposed solution, named adversarial variational autoencoder GAN (VAEGAN), is a more expressive, and flexible model that better approximates the posterior distribution by combining VAEs and GAN. This work is one of first work to propose the application of adversarial variational Bayes (AVB)~\cite{DBLP:conf/icml/MeschederNG17} to perform the adversarial training.


\subsubsection{Context-aware Recommendation}
Although long-term preference modeling has proven to be effective in several domains~\cite{DBLP:conf/kdd/BerkovskyF15}, recent research indicates that users' preferences are highly variable based on the user's context, e.g., time, location, and mood~\cite{DBLP:conf/recsys/KompanKB17}. Context provides the background of \textit{user objective} for using the system and can be used to generate more relevant recommendations.

\noindent \textbf{Temporal-aware Recommendation:}
In real applications, users' preferences change over time and modeling such \textit{temporal evolution} is needed for effective recommendation. While long-term preferences of users change slowly, their \textit{short-term preferences} can be seen as more dynamic and changing more rapidly. Predicting short-term user preference has been recently studied in the context of \textit{session-based} and \textit{sequential recommendations}. A temporal extension of SVD++ towards the modeling of temporal dynamic,  named TimeSVD++, has been proposed by Koren~\cite{DBLP:journals/cacm/Koren10} in 2010. It has also been reported that the structure of time-aware inputs (e.g., click-logs, session) are effectively modelled by recurrent neural network (RNN).
For instance, Hidasi et al.~\cite{DBLP:journals/corr/HidasiKBT15} proposed to model the sequential user clicks to output session-based recommendation with a GRU-gated recurrent unit; while Wu et al.~\cite{DBLP:conf/wsdm/WuABSJ17} proposed to integrate an LSTM model, to capture both the user and the item temporal evolution, and MF to model stationary preferences. Inspired by the accuracy improvements of IRGAN, GAN-based models have been combined in temporal frameworks to boost the recommendation performance in sequence-aware recommendation tasks. 

\setlength{\parindent}{15pt} [\textbf{RecGAN}] In~\cite{DBLP:conf/recsys/BharadhwajPL18}, the authors propose to incorporate in a single framework both the temporal modeling capabilities of RNN and the latent feature modeling power of the \textit{min-max  game}. The proposed framework, named RecGAN, implements both the generator and the discriminator with the Gated Recurrent Unit (GRU)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}, in order to make $\mathcal{G}$ capable of predicting a sequence of relevant items based on the dynamic evolution of user's preferences.

\setlength{\parindent}{15pt} [\textbf{PLASTIC \& LSIC}] Differently from RecGAN that implements only a RNN cell to capture the dynamic evolution of user's behaviour, Zhao et al.~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, 8643032} propose to combine MF and RNN in an adversarial recommendation framework to model respectively long and short-term user-item associations. The proposed framework, named PLASTIC, adopts MF and LSTM cells into $\mathcal{G}$ to account for varying aspect of both users and item,  while a two-input Siamese network --- built manually by using a MF and RNN --- as $\mathcal{D}$ encodes both the \textit{long-term} and \textit{session-based information} in the pair-wise scenario.

\setlength{\parindent}{15pt} [\textbf{NMRN-GAN}] Recent studies have endorsed creating close-to-observed negatives samples adversarially are capable of improving the user and item representation. In~\cite{DBLP:conf/kdd/WangYHLWH18}, Wang et al., introduce \textit{GAN-based negative sampling} for streaming recommendation. Instead of using a random sampling strategy, which is static and hardly contributes towards the training of the recommender model, adversarially generated negative samples are more informative. NMRN-GAN uses a key-value memory network~\cite{DBLP:conf/www/ZhangSKY17} to keep the model's long-term and short-term memory combined with a GAN-based negative sampling strategy to create more instructive negative samples and improve the training effectiveness and the quality of the recommendation model.

\setlength{\parindent}{15pt} [\textbf{GAN-CQDN}] GAN-based solution for sequence-aware recommendation has been proposed in conjunction with reinforcement learning (RL), to model the dynamic of user's status and long-term performance. In~\cite{DBLP:conf/icml/Chen0LJQS19}, the authors Chen et al., propose GAN-CQDN, an RL-based recommender system that exploits GAN to model user behavior dynamics and learn her reward function. The advantages of using GAN is that it improves the representation of the user profile, improves the reward function according to the learned user profile and accommodates online changes for new users. 

\noindent \textbf{Geographical-aware Recommendation:}  A relevant application of contextual information is point-of-interest (POI) recommendation. \yashar{add a few more words here}

\setlength{\parindent}{15pt} [\textbf{Geo-ALM}] In~\cite{DBLP:conf/ijcai/0061W0Y19}, the authors propose Geo-ALM, a GAN-based POI recommender that integrates geographical features (POI and region features) with a GAN to achieve (better) POI recommendation. In the proposed system, $\mathcal{G}$ improves the random negative sampling approach in the pairwise POI recommendation scenario that leads to better representation of user and items and enhances recommendation quality with respect to state of the art models.

\setlength{\parindent}{15pt} [\textbf{APOIR}] Inspired by the advances of POI recommendation performance under GAN-based framework, Zhou et al., propose adversarial point-of-interest recommendation (APOIR)~\cite{DBLP:conf/www/0002YZTZW19} to learn user-latent representations in a generative manner. The main novelty of the proposed framework is the use of POIs' geographical features and the users' social relations into the reward function used to optimize the $\mathcal{G}$. The reward function acts like a contextual-aware regularizer of $\mathcal{G}$, that is the component of APOIR in the proposed POI recommendation model.

\subsubsection{Cross-domain Recommendation}
\yashar{To make it balanced with previous section, this introduction could be a bit shortened by Tommaso}
Cross-domain recommender models are designed to compute recommendations for items belonging to a single domain; for example, in media streaming platforms, Netflix recommends movies/TV series to its consumers while Lasts.Fm offers songs and music-album recommendations. Items belonging to a specific domain share characteristics and attributes, which are intrinsically similar and domain-specific recommendation models allow the designer to study these characteristics individually. However, \textit{single-domain} recommendation face numerous challenges. First, refers to the well-known \textit{cold-start} problem, when insufficient interactions exist in the considered domain. Second, users' interests and needs span across different application areas and large e-commerce sites, like Amazon or Ebay, store users' preference scores related to products/services of various domains - from books and products to online movies and music. As companies strive to increase the diversity of products or services to users, cross-domain recommendation can help such companies to increase sale productivity by offering personalized cross-selling or bundle recommendations for items from multiple domains~\cite{cantador2015cross}. The third aspect is a novel research idea related to discovering relationships between item (e.g., images) of two different domains. For example, can machine achieve a human-level understanding to recommend a fashion item (domain A) consistent with user taste/style in another domain such as media or visual scenery (domain B)? The central problem here is to find a mapping function from one domain to another domain~\cite{DBLP:journals/corr/abs-1812-06229}. Recently, the generative power of GANs has been used to tackle this problem as a conditional image generation problem, i.e., to generate an image in one domain given another image in the other domain~\cite{DBLP:conf/cvpr/IsolaZZE17}. In the following we review different research works applying GAN-based approaches to various cross-domain recommendations tasks: 

\setlength{\parindent}{15pt} [\textbf{FR-DiscoGAN}]
In~\cite{DBLP:conf/bigcomp/JoJCJ19}, the authors propose a cross-domain GAN to generate fashion designs from the sceneries. In the proposed hypothetical scenario, the user can specify via a query her POI to visit (e.g., mountain, beach) together with keywords describing a season (i.e., spring, summer, fall, and winter). The core idea is to automatically generate fashion items (e.g., clothes, handbags, and shoes) whose useful features (i.e., style) match the the natural scenery specified by the user. For instance, the system can recommend a collection of fashion items that look cool/bright for visiting a beach in summer even though the true preference of the user is black-style clothes. The role of GAN is to learn associations between scenery and fashion images. In the field of ML and Computer Vision, the problem is termed as \dquotes{style transfer} or \dquotes{image to image translation} problem~\cite{DBLP:conf/cvpr/GatysEB16}. 

\setlength{\parindent}{15pt} [\textbf{VAE-GAN-CC}]
An effective cross-domain recommendation system relies on \textit{capturing both similarities and differences} among features of domains and exploiting them for improving recommendation quality in multiple domains. Single-domain algorithms have difficulty in uncovering the specific characteristics of each domain. To solve this problem, some approaches extract latent features of the domains by a separate network~\cite{DBLP:conf/www/LianZXS17,DBLP:journals/tmm/MinBXH15}. Although these approaches might be successful in capturing characteristic features of each domain, they do not establish the similarity between features of multiple domains. To extract both homogeneous and divergent features in multiple domains, in~\cite{DBLP:journals/corr/abs-1812-06229} Nguyen et al., propose a generic cross-domain recommendation system that takes as input the user interaction history (click vector) in each domain,  maps the vectors to a shared latent space using two AEs and then uses $\mathcal{G}$ to remap the underlying latent representation to click vectors. The main novelty of this work lies in building/linking shared latent space between domains, which in turn facilitates \textit{domain-to-domain} translation. In particular, the former is realized by enforcing a weight-sharing constraint related to variational auto-encoders, i.e., the encoder-generator pair $\{\mathcal{E}_A, \mathcal{G}_A\}$ and $\{\mathcal{E}_B, \mathcal{G}_B\}$ and using cycle-consistency (CC) as a weight-sharing constraint. Finally, two separate adversarial discriminators are employed to determine whether the translated vectors are realistic. The final system is called VAE-GAN-CC network, which extends the unsupervised image-to-image translation network in the CV domain~\cite{DBLP:conf/nips/LiuBK17} for RS applications and is thus named domain-to-domain translation model (D2D-TM).

\setlength{\parindent}{15pt} [\textbf{DASO}]
Inspired by the efficacy of \textit{adversarial negative sampling} techniques proposed in~\cite{DBLP:conf/kdd/WangYHLWH18}, Fan et al.~\cite{DBLP:conf/ijcai/FanD0WTL19} address the limitation of typical negative sampling in the \textit{social recommendation} domain in transferring users' information from social domain to item domain. The proposed deep adversarial social recommendation (DASO) system, harnesses the power of adversarial learning to dynamically generate difficult negative samples for \textit{user-item} and \textit{user-user pairs}, to guide the network to learn better user and item representations. The authors validate the effectiveness of the system compared with the state of the art pairwise ranking and GAN-based models.

\setlength{\parindent}{15pt} [\textbf{CnGAN}]
Perera et al., in~\cite{DBLP:conf/www/PereraZ19}, propose GAN for cross-network (CnGAN) to address one of the significant shortcomings of cross-network recommendation concerning \textit{non-overlapping users}  missing preference scores. These users exist in the source domain but not in the target domain, and thus, their preferences about items in the target domain are not available. In the proposed work, $\mathcal{G}$ learns the mapping of user preferences from \textit{target to source} and generate more \textit{informative preferences} on the source domain. $\mathcal{D}$ uses the synthetically generated preferences (generated from $\mathcal{G}$) to provide recommendations for users who only have interactions on the target network (not overlapped users). The authors also propose two novel loss functions --- a content-wise and a user-wise loss function --- to guide the min-max training process better. The author validate the effectiveness of the system against state-of-the-art models both in terms of accuracy and beyond-accuracy measures (novelty, diversity).
\vspace{-5mm}


\subsubsection{Fashion Recommendation}
Most conventional RS --- such as CF or CBF --- are not suitable for application in the fashion domain due to unique characteristics hidden in this domain. For instance, people do not follow the crowd blindly when buying clothes or do not buy a fashion item twice~\cite{DBLP:conf/waim/ShaWZFZY16}. Furthermore, each person --- in particular women ---  would like to look different than the others. Another aspect is related to notion of \textit{complementary} relationship for recommending a personalized fashion outfit. It is natural for humans to establish a sense of relationship between products based on their visual appearance. Traditional visual CBF (and hybrid) models are centered around the notion of similarity (or alternativeness), e.g., seeking to answer the question \dquotes{which shirt matches this shirt more?}. Instead, complementary relationship seeks to answer the question \dquotes{given a red top (upper garment), which pairs of trousers (bottom garment) matches it --- as an outfit --- in a complementary way?}. Recently, GAN-based models have shown promising performance for outfit recommendation, being able to compete with state-of-the-art fashion recommendation models in the field, such as Siamese-base networks~\cite{DBLP:journals/mms/GaoLWZ19}. Finally, another exciting application of GANs are related to exploit the \textit{generative power of GANs} to synthesize real-looking fashion clothes. This aspect can inspire the aesthetic appeal/curiosity of costumer and designers and motivates them to explore the space of
potential fashion styles.

\setlength{\parindent}{15pt} [\textbf{CRAFT}] Huynh et al.,~\cite{DBLP:conf/eccv/HuynhCTA18} address the problem of recommending complementary fashion items for a given fashion based on visual features by using an adversarial process that resembles GAN and uses a conditional feature transformer as $\mathcal{G}$ and a discriminator, $\mathcal{D}$. One main distinction between this work and the prior literature is that the <input, output> pair for $\mathcal{G}$ are both features (here features are extracted using pre-trained CNNs~\cite{DBLP:conf/aaai/SzegedyIVA17}), instead of <image, image> or hybrid types such as <image, features> explored in numerous previous works~\cite{DBLP:conf/iccv/ZhuFULL17,DBLP:conf/cvpr/VolpiMSM18}. This would allow the network to learn the relationship between items directly on the feature space, spanned by the features extracted. The proposed system is named complementary recommendation using adversarial feature transform (CRAFT) since in the model, $\mathcal{G}$ acts like a feature transformer that --- for a given query product image $q$ --- it maps the source feature $s_{q}$ into a complementary target feature $\hat{t}_{q}$ by playing a min-max game with $\mathcal{D}$ that aims to classify fake/real features. For training, the system relies on learning the co-occurrence of item pairs in real images. In summary, the proposed method does not generate new images; instead it learns how to generate features of the complementary items conditioned on the query item. CRAFT has been tested by experienced users who gave positive feedback on the goodness of complementary recommendations.

\setlength{\parindent}{15pt} [\textbf{DVBPR}] Deep visual Bayesian personalized ranking (DVBPR)~\cite{DBLP:conf/icdm/KangFWM17} is presumably one of the first works that exploit the \textit{visual generative power of the GAN} in the fashion recommendation domain. It aims to generate clothing images based on user preferences. Given a user and a fashion item category (e.g., tops, t-shirts, and shoes), the proposed system generates new images --- i.e., clothing items --- that are consistent with the user's preferences. The contributions of this work are two-fold: first, it builds and end-to-end learning framework based on the Siamese-CNN framework. Instead of using the features extracted in advance, it constructs an end-to-end system that turns out to improve the visual representation of images. Second, it uses a GAN-based framework to generate images that are consistent with the user's personal taste. Iteratively, $\mathcal{G}$ learns to generate a product image integrating a \textit{user preference maximization objective}, while $\mathcal{D}$ tries to distinguish crafted images from real ones. Generated images are quantitatively compared with real images using the preference score (mean objective value), inception score~\cite{DBLP:conf/nips/SalimansGZCRCC16}, and opposite SSIM~\cite{DBLP:conf/icml/OdenaOS17}. This comparison shows improvement in preference prediction in comparison with non-GAN based images. At the same time, the qualitative comparison demonstrates that the generated images are realistic and plausible, yet they are quite different from any images in the original dataset --they have standard shape and color profiles, but quite different styles.

\setlength{\parindent}{15pt} [\textbf{MrCGAN}] Shih et al.,~\cite{DBLP:conf/aaai/ShihCLS18} propose a compatibility learning framework that allows the user to visually explore candidate \textit{compatible prototypes} (e.g., a white T-shirt and a pair of blue-jeans). The system uses metric-regularized conditional GAN (MrCGAN) to pursue the item generation task. It takes as the input a projected prototype (i.e., the transformation of a query image in the latent "Compatibility Space") and produces as the output a synthesized image of a compatible item (the authors consider a compatibility notions based on the complementary of the query item across different catalogue categories.). Similar to the evaluation protocol in~\cite{DBLP:conf/eccv/HuynhCTA18}, the authors conduct online user surveys to evaluate whether their model could produce images that are perceived as compatible. The results show that MrCGAN can generate compatible and realistic images under compatibility learning setting compared to baselines.

\setlength{\parindent}{15pt} [\textbf{Yang et al.,} \& \textbf{$c^+$GAN}] Yang et al., in~\cite{Yang2018FromRT} address the same problem settings of MrCGAN~\cite{DBLP:conf/aaai/ShihCLS18} by proposing a fashion clothing framework composed of two parts: a clothing recommendation model based on BPR combined with visual features and a clothing complementary item generation based GAN. Notably, the generation component takes in input a piece of clothing recommended in the recommendation model and generates clothing images of other categories (i.e., top, bottom, or shoes) to build up a set of complementary items. The authors follow a similar qualitative and quantitative evaluation procedure as DVBPR~\cite{DBLP:conf/icdm/KangFWM17} and further propose a \textit{compatibility index} to measure the compatibility of the generated set of complementary items. A similar approach has also been proposed also in $c^+$GAN~\cite{DBLP:journals/corr/abs-1906-05596}, to generate bottom fashion item paired with a given top item.

==> OLD_FILES/Sec4_Domain.tex <==
\section{Domain and Datasets}\label{sec:domain_catag}

Figure~\ref{plt:domain} shows in which application domain adversarial-based recommenders have been proved. In the following, we explain a meaningful example of a publications in each domain.
% \input{Tables/GoalBasedCategorization.tex}
\input{Plots/Domain.tex}\label{plt:domain}

\qquad\textit{Media \& Entertainment} is the most examined domain with a huge amount of works on the movie domain, e.g., in ~\cite{DBLP:conf/sigir/WangYZGXWZZ17, DBLP:conf/ijcai/ZhaoWYGYC18} and ~\cite{DBLP:conf/cikm/ChaeKKL18}, where the general goal seems to be voted in improving the personalized recommendation. The consumption of M\&E content is also based on both long-term and short-term preferences. Such constraints are pursued by ~\cite{DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:conf/recsys/BharadhwajPL18, DBLP:conf/kdd/WangYHLWH18}.
Interesting publications on the challenge of automatic playlist continuation~\cite{DBLP:conf/recsys/VaglianoGMS18, DBLP:journals/corr/abs-1906-03450} and content-based rating prediction~\cite{DBLP:conf/webi/YiHQ18} are addressed in this domain. Challenging work on long-term user behavior modelling  has been presented in ~\cite{DBLP:conf/icml/Chen0LJQS19}.


\qquad\textit{E-Products} is another mostly investigated domain of adversarial-based recommenders. A common problem settings is related on the generation of complementary recommendation in Fashion domain, e.g., ~\cite{DBLP:conf/eccv/HuynhCTA18, DBLP:journals/corr/abs-1711-02231, 2019arXiv190605596K } and~\cite{DBLP:journals/corr/abs-1711-02231} propose new frameworks.
E-Products websites sell generally products in different categories, e.g., Home \& Kitchen and Office Products~\cite{DBLP:journals/corr/abs-1903-10794}. In ~\cite{DBLP:journals/corr/abs-1903-10794,DBLP:journals/corr/abs-1812-06229, DBLP:conf/bigcomp/JoJCJ19}, authors mitigates the cold-start and sparsity problem by leveraging the knowledge from different domains. Other problem in the e-commerce domain is the next-basket recommendation~\cite{DBLP:journals/corr/abs-1805-08720}.

\qquad\textit{Social Computing} is a challenging application area with lots of interest from the industry, i.e., one of the most important conference in rec-sys community propose a challenge on this domain~\footnote{https://recsys.acm.org/recsys19/challenge/}. 
AML has been applied to predict the next location in POI recommendations~\cite{DBLP:conf/www/0002YZTZW19}, to improve image-based recommendation task in a Social Network like Pinterest~\footnote{} ~\cite{DBLP:journals/corr/abs-1809-07062}. Another problem setting is to improve recommendation by transferring preferences between different Social-network. For example,  ~\cite{DBLP:conf/www/PereraZ19,} proposes a adversarial-based solutions by generating user preferences on the Twitter source network for recommendations on the YouTube target network for not-overlapped users; and ~\cite{ DBLP:journals/corr/abs-1905-13160} works on transferring users' information from social domain to item domain.

\qquad\textit{Information-based} domain is mostly investigated in personalized citation-recommendations~\cite{DBLP:conf/aaai/CaiHY18, DBLP:conf/um/GalkeMVS18, DBLP:conf/ismis/ZhangYCD18}.
Other publications concern to query prediction during online search~\cite{DBLP:conf/www/LiLWZW19}, the improvement of long-tail performance in the question-info domain~\cite{DBLP:conf/cikm/KrishnanSSS18} and news-recommendations~\cite{DBLP:conf/icml/Chen0LJQS19}.
    

==> OLD_FILES/Sec4_SummaryFuture.tex <==
\section{Summary and Future Directions}\label{sec:conclusion}
In this paper, we have surveyed the use of a wide variety of tasks in which adversarial machine learning (AML) is important to train a secure recommendation model, improve the generalization performance of the model or synthesize plausible-looking images, for instance in the fashion and retail domain. This broad range of applications can be categorized into two --- objective-wise distinct --- technologies, (i) AML for improving security (cf. Section~\ref{sec:security}) and, (ii) AML used in generative adversarial networks (GANs) exploited for numerous tasks such as better CF recommendation, context-aware recommendation, cross-domain system, or visually-aware fashion item/outfit recommendation (cf. Section~\ref{sec:GAN}). The common point of both technologies is the joint min-max optimization used for training models, in which two competing players play a zero-sum differential game until they reach a Nash equilibrium. In the literature review, we have reviewed and categorized the state of the art over the past 3 years. To the best of our knowledge, this practice is the first work that sums up the advances of AML application in recommendation settings, and proposes a clear taxonomy to classify such applications.\yashar{I feel it better not to mention 3 years. Will ask Tommaso}

We put forward what is better to invest in AML-RS research and introduce the following open research directions:

\emph{Bridging the gap between attack/defense models in the ML/CV and RS domain.} 
As the prior literature of AML for security emerged in the field of machine learning (ML) and computer vision (CV), there remains a large gap between advances made in those fields and that in RS. Consider the questions: \dquotes{\textit{Attacks for images are designed to be human-imperceptible or inconspicuous (i.e., may be visible but not suspicious).  How can we capture these notions for designing attacks in RS?}}; furthermore \dquotes{\textit{Images are continuous-valued data while a user profile is a discrete data. Modifying users' profiles completely change the semantic of their behaviors. What is the best approach to treat these nuances in RS attack designs?}} \yashar{I have left some reference in section 2 (page 11), please add 1-2 ref here.}~\felice{?}

\emph{Choice of recommendation models.} Modern recommendation models exploit a
wealth of side-information beyond the user-item matrix such as as social-connections \yd{[xxx]}, multimedia content, semantic data among others  \yd{[xxx]}. However, most of the attacks against recommendation system are designed and validated against CF systems. Investigating the impact of adversarial attacks again these --- heterogeneous in nature --- data types remains as an open highly interesting challenges, e.g, adversarial attacks against, music, image and video recommendation models leveraging multimedia content. In this regard, we also recognize attack against state of the art deep and graph-based models another highly-valued research direction. \yashar{I will fix xxx}

\emph{Definition of attack threat model.} The research in RS community misses a common evaluation approach for attacking/defending scenarios such as the one introduced by Carlini at el., in~\cite{DBLP:journals/corr/abs-1902-06705}. For instance, it is important to define a common attacker threat model to establish in advance the attacker knowledge and capabilities to make the attack (or defense) reproducible and comparable with novel proposals.

\emph{Move the attention towards beyond accuracy goal in recommendation.}
According to our survey, most of the identified research work focus on accuracy metrics such as HR and nDCG. Consider the question: \dquotes{\textit{What is the impact of adversarial attacks and defenses in other evaluation objectives of RS, for instance diversity, novelty, and fairness of recommendations?}}.\yashar{@Tommaso: please check and improve this one. Thanks}

\emph{Scalability and stability of learning.} We identify the need to further explore the stability learning problems in the discrete item sampling strategy to train the generator, which have been already identified as a big problem when GAN-based RS are applied in real scenarios with huge catalogue. A point of study may be the study of novel GAN models proposed in computer vision (e.g., WGAN~\cite{DBLP:journals/corr/ArjovskyCB17}, LSGAN~\cite{DBLP:conf/iccv/MaoLXLWS17}, and BEGAN~\cite{DBLP:journals/corr/BerthelotSM17}).

\emph{Users preferences learning with GANs.} An interesting already established application if AM-RS is to exploit the generative power of GANs to produce more plausible user-rating profiles that can be used to improve recommendations in the cold-user scenario or improve the prediction performance in warm-start settings. We consider extremely interesting such applications, and we promote further research in this direction in resolving the well-known cold-start obstacle of recommender models.

\emph{Strengthen the difference between AML for security and GANs.} We think that the application of AML in RS needs a unified view and categorization. In this work, we have raised up the \textit{misunderstanding} of the application of AML in GAN-based recommender models and in attack/defense scenario. We deem important to remark such division.\yashar{@Tommaso, you may want to improve this part. Thanks}
d

==> Plots/Domain.tex <==
\begin{figure}
\begin{center}
    \begin{tikzpicture}
        \small
          \begin{axis}[
            width=0.6\linewidth,
            height=6cm,
            ybar,
            enlargelimits=0.20,
            legend style={at={(0.5,-0.2)}, anchor=north,legend columns=-1},
            ylabel={\# publications},
            symbolic x coords={Media \& Ent.,E-Products, Social Computing, Information-based},
            xtick=data,
            bar width= 15,
            nodes near coords, 
            nodes near coords align={vertical},
            x tick label style={rotate=45,anchor=east}
            ][black]
            
            
            \addplot[ thick,
                color=black,fill=lightgray] 
                coordinates {
                (Media \& Ent.,     33)
                (E-Products,                14)
                (Social Computing,          10)
                (Information-based,         7)
    
                };
          \end{axis}
    \end{tikzpicture}
\end{center}
        \caption{Distribution of publications per application domain.}\label{plt:domain}

\end{figure}

==> Plots/OpenChallenges.tex <==
\begin{figure}
\begin{center}
    \begin{tikzpicture}
        \small
        \centering
          \begin{axis}[
            width=0.7\linewidth,
            height=6cm,
            ybar,
            enlargelimits=0.15,
            legend style={at={(0.5,-0.2)}, anchor=north,legend columns=-1},
            ylabel={\# publications},
            symbolic x coords={Collaborative, Content, Sequences,Complementary,Cross-Domain,Context,Cold-Start, Diversity \& Novelty, Fairness \& Privacy, Efficiency},
            xtick=data,
            nodes near coords, 
            nodes near coords align={vertical},
            x tick label style={rotate=45,anchor=east},
            bar width= 12
            ][black]
            
            
            \addplot[ thick,
                color=black,fill=lightgray] 
                coordinates {
                (Collaborative,           16)
                (Content,                   10)
                (Sequences,                 8)
                (Complementary,             4)
                (Cross-Domain,              5)
                (Context,                   3)
                (Cold-Start,                3)   
                (Diversity \& Novelty,      2) 
                (Fairness \& Privacy,       3)
                (Efficiency,   2)

                };
          \end{axis}
    \end{tikzpicture}
\end{center}
    \caption{Distribution of publication per challenges.}\label{plt:openchallenge} 

\end{figure}

==> Tables/CategoryChallangeDomainBase.tex <==
\begin{table}
    \tiny
    \centering
    \caption{Categorization of publication regarding Task Type, Open Challenge and Domain. ~\felice{DRAFT}}
    \label{tab:CatTaskChalDom}
    \begin{threeparttable}
        \begin{tabular}{@{} c @{}}
             \begin{tabular}{lllll}
                \toprule
            \textbf{Paper} & \(  \textbf{Challenge}\)  & \(  \textbf{Domain}\) & \( \textbf{Data Source} \) \\
                
                \midrule
                \cite{DBLP:conf/bigcomp/JoJCJ19}      & CD     &     EP      &   Fashion       \\
                \cite{DBLP:conf/eccv/HuynhCTA18}    &  Com   &     EP      &   Fashion   \\
                \cite{DBLP:journals/corr/abs-1906-05596} &  Com   &     EP      &   Fashion \\
                % \cite{DBLP:journals/corr/abs-1711-02231}& H  &      EP      &   Fashion     \\
                \cite{Yang2018FromRT} & Com   &   EP      &   Fashion      \\
                \cite{DBLP:conf/aaai/ShihCLS18}  &  Com  & EP      &   Fashion       \\
                \cite{DBLP:journals/corr/abs-1812-06229}  & CD & EP, M\&E &   Fashion, Product, Movie, Image    \\
                \cite{DBLP:journals/corr/abs-1903-10794}   &    CD  &   EP    & Product          \\
                \cite{DBLP:conf/ijcai/FanD0WTL19}   &    CD  &   SC    & Social Network          \\
                \cite{DBLP:journals/tois/ChenZXQZ19}    &  H & EP    & Product          \\
                \cite{DBLP:journals/corr/abs-1805-08720}    & Seq   &  EP    & Product \\
                \cite{8663730}  & CF   & M\&E &    Music, Movie      \\
                \cite{DBLP:conf/icdm/LiH018} &  H &  M\&E, SC & Music, Food          \\
                \cite{DBLP:conf/recsys/VaglianoGMS18}  &  Seq     &  M\&E & Music          \\
                (No)~\textsuperscript{waiting}  &  Seq     &  ?? &  ??          \\
                \cite{DBLP:conf/icml/Chen0LJQS19}  &  Seq     &  All & Movie, Music, Products, Business, News          \\
                \cite{DBLP:conf/sigir/TranSL19}  &  Seq     &  M\&E & MOvie          \\
                \cite{DBLP:conf/5gwn/HanH19}  & Con  &  M\&E & Music        \\
                \cite{DBLP:journals/eswa/SunWWY19} & CF& M\&E, SC & Music, Image, Social Network, Business          \\
                \cite{DBLP:conf/sigir/WangYZGXWZZ17}    &   CF  &   M\&E   &  Movie        \\
                \cite{DBLP:conf/cikm/ChaeKKL18}    &   CF   &   M\&E   &     Movie     \\
                \cite{DBLP:journals/access/ChaeSK19}   &   CF &       M\&E     &     Movie     \\
                \cite{8525831}  &   CF&   M\&E     &     Movie        \\
                \cite{DBLP:conf/kdd/WangYHLWH18}& Seq   & M\&E     &     Movie          \\

                \bottomrule
                \end{tabular}
    
             \begin{tabular}{lllll}
                \toprule
            \textbf{Paper} &\(  \textbf{Challenge}\)  & \(  \textbf{Domain}\) & \( \textbf{Data Source} \) \\
                
                \midrule
                \cite{DBLP:conf/ijcai/ZhaoWYGYC18}    & Seq  & M\&E     &     Movie         \\
                \cite{DBLP:conf/recsys/BharadhwajPL18}   & Seq &  M\&E, SC     &     Movie, Food         \\
                \cite{DBLP:conf/www/PereraZ19}  & CD & M\&E, SC &   Movie, Social Network       \\
                \cite{DBLP:conf/www/ChaeKKC19}   & CF  & M\&E     &     Movie    \\

                \cite{DBLP:journals/corr/abs-1807-03521}   &  CF  &  M\&E     &     Movie \\
                \cite{DBLP:conf/aaai/WangWWZZZXG18}   & CF  &    M\&E     &     Movie  \\
                \cite{DBLP:conf/cikm/KrishnanSSS18}    & CF  &  M\&E, I     &     Movie, Question Info \\
                \cite{DBLP:conf/webi/YiHQ18}   & H   &     M\&E  &   Entertainment      \\
                \cite{DBLP:conf/www/0002YZTZW19}   &  Con &   SC   &  Tourism, Social Network         \\

                \cite{DBLP:conf/aaai/CaiHY18}   & Graph   &  I & Citation          \\
                \cite{DBLP:conf/um/GalkeMVS18}     & H    &  I & Citation   \\
                \cite{DBLP:conf/ismis/ZhangYCD18}  & Graph   &    I & Citation  \\
                \cite{DBLP:conf/www/LiLWZW19}  & Con  &  I    &      Query    \\

                \cite{DBLP:conf/www/ParkC19}~\textsuperscript{def}  & CF&  M\&E     &     Movie \\
                \cite{DBLP:conf/ijcnn/YuanYB19}~\textsuperscript{def, att}  & CF  & M\&E     &     Movie    \\
                \cite{DBLP:journals/corr/abs-1809-07062}~\textsuperscript{def, att}   & CF  &  M\&E     &     Movie\\
                \cite{DBLP:journals/tmm/DuFYXCT19}~\textsuperscript{def, att}  & CF&  M\&E     &     Movie \\
                \cite{DBLP:journals/corr/abs-1809-08336}~\textsuperscript{att} & CF  &    SC   & Food  \\

                \cite{DBLP:journals/corr/abs-1809-07062}~\textsuperscript{def, att} &  H   & EP, SC      &   Fashion, Social Network      \\
                \cite{DBLP:conf/sigir/0001HDC18}~\textsuperscript{def, att}   & CF &   SC   &  Tourism, Social Network\\

                % \hdashline
                \cite{DBLP:journals/corr/abs-1807-03521}   &  Privacy, CF  &  M\&E     &     Movie \\
                \cite{jia2018attriguard}  &  Privacy  & M\&E  & Movie          \\
                \cite{DBLP:conf/icpram/ResheffESS19}  &  Privacy  & EP & Apps          \\


                
                \bottomrule
                \end{tabular}

        \end{tabular}

        %  \hline

         \begin{tablenotes}[para,flushleft]
                \footnotesize 
                \textbf{Challenge} CF: Collaborative Filtering, H: Hybrid, G: Graph-based , Seq: Sequence-aware, Con: Context-aware, CD: Cross-Domain, Com: Complementray \\
                \textbf{Domain} EP: E-Prodcuts, M\&E: Media \& Entertainment, SC: Social Computing, I: Information-based
         \end{tablenotes}

    \end{threeparttable}

\end{table}


==> Tables/DomainTable.tex <==
\begin{table}[h!]
    \label{tab:DomainCategorization}
    \caption{Domain-based Categorization of Publications.}
    \begin{tabular}{|c|c|l|}
        \hline
        \textbf{Domain} &\textbf{ Data Source} & \textbf{Publications} \\ \hline
        
        \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Media \\ \&\\ Entertainment\end{tabular}} 
        
        & Music &  
        \cite{8663730, DBLP:conf/icdm/LiH018, DBLP:conf/recsys/VaglianoGMS18, DBLP:conf/5gwn/HanH19, DBLP:journals/eswa/SunWWY19}
        \\ \cline{2-3} 
        
         & Movie & 
         \cite{DBLP:journals/corr/abs-1812-06229, 8663730, DBLP:conf/sigir/WangYZGXWZZ17, DBLP:conf/cikm/ChaeKKL18, DBLP:journals/access/ChaeSK19, 8525831, DBLP:conf/kdd/WangYHLWH18, DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:conf/recsys/BharadhwajPL18, DBLP:conf/www/PereraZ19, DBLP:conf/www/ChaeKKC19, DBLP:journals/corr/abs-1808-05361, DBLP:conf/sigir/YuanYB19, DBLP:journals/tmm/DuFYXCT19, DBLP:conf/www/ParkC19, DBLP:journals/corr/abs-1807-03521, DBLP:conf/cikm/KrishnanSSS18, DBLP:conf/aaai/WangWWZZZXG18}
         \\ \cline{2-3} 
         
         & Image &  
         \cite{DBLP:journals/eswa/SunWWY19}
         \\ \cline{2-3} 
         
         & Entertainment &
         \cite{DBLP:journals/corr/abs-1812-06229, DBLP:conf/webi/YiHQ18}
         \\ \hline
        
            \multirow{3}{*}{E-Products}
            
            & Fashion & 
            \cite{DBLP:conf/bigcomp/JoJCJ19, DBLP:conf/eccv/HuynhCTA18, DBLP:journals/corr/abs-1711-02231, Yang2018FromRT, DBLP:journals/corr/abs-1809-07062, DBLP:conf/aaai/ShihCLS18, DBLP:journals/corr/abs-1812-06229, 2019arXiv190605596K}
            \\ \cline{2-3} 
            
             & Products & 
             \cite{DBLP:journals/corr/abs-1812-06229, DBLP:journals/corr/abs-1903-10794, DBLP:journals/tois/ChenZXQZ19, DBLP:journals/corr/abs-1805-08720}
             \\ \cline{2-3} 
             
             & Mobile Apps &  
             \cite{jia2018attriguard}
             \\ \hline
             
         
        \multirow{4}{*}{Social Computing}
        
        & Social Media & 
        \cite{DBLP:journals/corr/abs-1809-07062, DBLP:journals/eswa/SunWWY19, DBLP:conf/www/PereraZ19, DBLP:conf/www/0002YZTZW19, DBLP:conf/sigir/0001HDC18}
        \\ \cline{2-3} 
        
         & Tourism &  
         \cite{DBLP:conf/www/0002YZTZW19, DBLP:conf/sigir/0001HDC18}
         \\ \cline{2-3} 
         
         & Food & 
         \cite{8663730, DBLP:conf/recsys/BharadhwajPL18, DBLP:journals/corr/abs-1809-08336}
         \\ \cline{2-3} 
         
         & Business &
         \cite{DBLP:journals/eswa/SunWWY19}
         \\ \hline
         
         
        \multirow{3}{*}{Information-based} 
        
        & Questions Info &
        \cite{DBLP:conf/cikm/KrishnanSSS18}
        \\ \cline{2-3} 
        
         & Query &
         \cite{DBLP:conf/www/LiLWZW19}
         \\ \cline{2-3} 
         
         & Citation &
         \cite{DBLP:conf/aaai/CaiHY18, DBLP:conf/um/GalkeMVS18, DBLP:conf/ismis/ZhangYCD18}
         \\ \hline
         
    \end{tabular}
\end{table}

==> Tables/GoalBasedCategorization.tex <==
\begin{table}[h!]
\label{table:task}
    \caption{Goal-based categorization of AML in RS.}

\centering
 \begin{tabular}{|c|l|l|}

        \hline
        \multicolumn{2}{|c|}{\textbf{Goals}} & \textbf{Publications} \\ \hline
        \multicolumn{2}{|c|}{Adversarial Attack} & \cite{DBLP:conf/sigir/0001HDC18, DBLP:journals/corr/abs-1808-05361, advcol19sigir, DBLP:journals/tmm/DuFYXCT19, DBLP:journals/corr/abs-1809-07062, DBLP:journals/corr/abs-1809-08336} \\ \hline
        \multicolumn{2}{|c|}{Defense Mechanism} & \cite{DBLP:conf/sigir/0001HDC18, DBLP:journals/corr/abs-1808-05361, advcol19sigir,DBLP:journals/tmm/DuFYXCT19, DBLP:conf/www/ParkC19, DBLP:journals/corr/abs-1809-07062, DBLP:conf/spawc/TruongKE18}  \\ \hline
        \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Improve\\ Recommendation\end{tabular}} & 
        
        Collaborative Filtering, \textit{CF} & 
        \cite{DBLP:conf/sigir/0001HDC18, DBLP:journals/corr/abs-1808-05361, advcol19sigir, DBLP:journals/tmm/DuFYXCT19, DBLP:conf/www/ParkC19, DBLP:conf/www/ChaeKKC19, DBLP:journals/corr/abs-1807-03521,DBLP:conf/cikm/KrishnanSSS18, DBLP:journals/eswa/SunWWY19, DBLP:journals/corr/abs-1809-08336, DBLP:conf/sigir/WangYZGXWZZ17, DBLP:conf/cikm/ChaeKKL18, DBLP:journals/access/ChaeSK19, 8525831, 8663730} \\ \cline{2-3} 
        
         & Hybrid, \textit{H} & 
         \cite{DBLP:journals/corr/abs-1809-07062, DBLP:conf/um/GalkeMVS18, DBLP:journals/corr/abs-1711-02231, DBLP:conf/icdm/LiH018, DBLP:journals/tois/ChenZXQZ19, DBLP:conf/webi/YiHQ18} \\ \cline{2-3} 
         
         & Graph-based, \textit{G} & 
         \cite{DBLP:conf/ismis/ZhangYCD18, DBLP:conf/aaai/WangWWZZZXG18, DBLP:conf/aaai/CaiHY18}
         \\ \cline{2-3} 
         
         & Session-based, \textit{S} & 
         \cite{DBLP:conf/recsys/BharadhwajPL18, DBLP:journals/corr/abs-1805-08720, DBLP:conf/ijcai/ZhaoWYGYC18, DBLP:conf/kdd/WangYHLWH18, DBLP:conf/recsys/VaglianoGMS18}
         \\ \cline{2-3} 
         
         & Context-aware, \textit{C} &
         \cite{DBLP:conf/www/0002YZTZW19, DBLP:conf/5gwn/HanH19, DBLP:conf/www/LiLWZW19}
         \\ \cline{2-3} 
         & Cross-Domain Recommendation, \textit{CD} & 
         \cite{DBLP:conf/bigcomp/JoJCJ19, DBLP:journals/corr/abs-1812-06229, DBLP:journals/corr/abs-1903-10794, DBLP:conf/www/PereraZ19}
         \\ \cline{2-3} 
         
         & Complementary Recommendation, \textit{Com} & 
         \cite{DBLP:conf/eccv/HuynhCTA18, Yang2018FromRT, DBLP:conf/aaai/ShihCLS18}
         \\ \hline
    \end{tabular}

\end{table}

==> Tables/Old_Categorization.tex <==
\begin{table}
    \centering
    \caption{Categorization of publication regarding Task Type, Open Challenge and Domain.}
    \label{tab:CatTaskChalDom}
    \begin{threeparttable}
        \begin{tabular}{@{} c @{}}
             \begin{tabular}{lllll}
                \toprule
            \textbf{Paper} & \( \textbf{Task} \)& \(  \textbf{Challenge}\)  & \(  \textbf{Domain}\) & \( \textbf{Data Source} \) \\
                
                \midrule
                \cite{DBLP:conf/bigcomp/JoJCJ19}   & ImpR    & CD     &     EP      &   Fashion       \\
                \cite{DBLP:conf/eccv/HuynhCTA18}    &    ImpR   &  Com   &     EP      &   Fashion   \\
                \cite{DBLP:journals/corr/abs-1711-02231}    &   ImpR & H  &      EP      &   Fashion     \\
                \cite{Yang2018FromRT}    &  ImpR  & Com   &   EP      &   Fashion      \\
                \cite{DBLP:conf/aaai/ShihCLS18}    & ImpR   &  Com  & EP      &   Fashion       \\
                \cite{DBLP:journals/corr/abs-1812-06229}    & ImpR  & CD & EP, M\&E &   Fashion, Product, Movie, Image    \\
                \cite{DBLP:journals/corr/abs-1903-10794}    & ImpR &    CD  &   EP    & Product          \\
                \cite{DBLP:journals/tois/ChenZXQZ19}    & ImpR   &  H & EP    & Product          \\
                \cite{DBLP:journals/corr/abs-1805-08720}    &  ImpR  & Seq   &  EP    & Product \\
                \cite{8663730}    & ImpR & CF   & M\&E &    Music, Movie      \\
                \cite{DBLP:conf/icdm/LiH018}    &  ImpR  &  H &  M\&E, SC & Music, Food          \\
                \cite{DBLP:conf/recsys/VaglianoGMS18}    &   ImpR  &  Seq     &  M\&E & Music          \\
                \cite{DBLP:conf/5gwn/HanH19}    & ImpR & Con  &  M\&E & Music        \\
                \cite{DBLP:journals/eswa/SunWWY19}    &   ImpR  & CF& M\&E, SC & Music, Image, Social Network, Business          \\
                \cite{DBLP:conf/sigir/WangYZGXWZZ17}    &   ImpR     &   CF  &   M\&E   &  Movie        \\
                \cite{DBLP:conf/cikm/ChaeKKL18}    & ImpR     &   CF   &   M\&E   &     Movie     \\
                \cite{DBLP:journals/access/ChaeSK19}    & ImpR     &   CF &       M\&E     &     Movie     \\
                \cite{8525831}    & ImpR     &   CF&   M\&E     &     Movie        \\

            %     \bottomrule
            %     \end{tabular}
    
            %  \begin{tabular}{lllll}
            %     \toprule
            % \textbf{Paper} & \( \textbf{Task} \)& \(  \textbf{Challenge}\)  & \(  \textbf{Domain}\) & \( \textbf{Data Source} \) \\
                
            %     \midrule
                \cite{DBLP:conf/kdd/WangYHLWH18}    &  ImpR  & Seq   & M\&E     &     Movie          \\
                \cite{DBLP:conf/ijcai/ZhaoWYGYC18}    &  ImpR  & Seq  & M\&E     &     Movie         \\
                \cite{DBLP:conf/recsys/BharadhwajPL18}    & ImpR  & Seq &  M\&E, SC     &     Movie, Food         \\
                \cite{DBLP:conf/www/PereraZ19}    &  ImpR & CD & M\&E, SC &   Movie, Social Network       \\
                \cite{DBLP:conf/www/ChaeKKC19}    & ImpR & CF  & M\&E     &     Movie    \\

                \cite{DBLP:journals/corr/abs-1807-03521}    & ImpR  &  CF  &  M\&E     &     Movie \\
                \cite{DBLP:conf/aaai/WangWWZZZXG18}    & ImpR   & CF  &    M\&E     &     Movie  \\
                \cite{DBLP:conf/cikm/KrishnanSSS18}    &  ImpR   & CF  &  M\&E, I     &     Movie, Question Info \\
                \cite{DBLP:conf/webi/YiHQ18}    &  ImpR  & H   &     M\&E  &   Entertainment      \\
                \cite{DBLP:conf/www/0002YZTZW19}    & ImpR   &  Con &   SC   &  Tourism, Social Network         \\

                \cite{DBLP:conf/aaai/CaiHY18}    &  ImpR  & Graph   &  I & Citation          \\
                \cite{DBLP:conf/um/GalkeMVS18}    & ImpR   & H    &  I & Citation   \\
                \cite{DBLP:conf/ismis/ZhangYCD18}    &  ImpR  & Graph   &    I & Citation  \\
                \cite{DBLP:conf/www/LiLWZW19}    &   ImpR  & Con  &  I    &      Query    \\

                \cite{DBLP:conf/www/ParkC19}    & Def, ImpR   & CF&  M\&E     &     Movie \\
                \cite{DBLP:journals/corr/abs-1809-07062}    &  Att, Def  &  H   & EP, SC      &   Fashion, Social Network      \\
                \cite{DBLP:conf/sigir/0001HDC18}    & Att, Def, ImpR   & CF &   SC   &  Tourism, Social Network\\
                \cite{DBLP:journals/corr/abs-1809-08336}    & Att, ImpR   & CF  &    SC   & Food  \\
                \cite{DBLP:conf/ijcnn/YuanYB19}    & Att, Def, ImpR   & CF  & M\&E     &     Movie    \\
                \cite{advcol19sigir}    & Att, Def, ImpR   & CF  &  M\&E     &     Movie\\
                \cite{DBLP:journals/tmm/DuFYXCT19}    & Att, Def, ImpR   & CF&  M\&E     &     Movie \\
                
                \cite{jia2018attriguard}    &  Privacy  &  X  & EP & Apps          \\

                
                \bottomrule
                \end{tabular}

        \end{tabular}

        %  \hline

         \begin{tablenotes}[para,flushleft]
                \footnotesize 
                \felice{I think we can remove the column with Task and Set a symbol (e.g. *) to represent papers with attack/defense strategies}
                \textbf{Task} Att: Attack, Def: Defense, ImpR: Improve Recommendation      \\
                \textbf{Challenge} CF: Collaborative Filtering, H: Hybrid, G: Graph-based , Seq: Sequence-aware, Con: Context-aware, CD: Cross-Domain, Com: Complementray \\
                \textbf{Domain} EP: E-Prodcuts, M\&E: Media \& Entertainment, SC: Social Computing, I: Information-based
                \textbf{Data Source}
         \end{tablenotes}

    \end{threeparttable}

\end{table}


==> Tables/Recommender_Models.tex <==
\begin{table}[!t]
\caption{Collaborative-based Recommender Models.}~\felice{ \textbf{@Yashar: }I think that we can remove this table putting the specification directly in the text in order to solve also the R1.3 comment and also gain half-page} \yashar{completely agree, beside this list is not complete nor related to the core part of the survey, if we wanted to make such a list it should have gone to appendix. I would just remove it to gain space.}
\label{tbl:recommender_models}
\centering
{
\scalebox{0.80}{
\begin{tabular}{L{3.5cm}|L{14cm} |}
\toprule
\multicolumn{1}{l}{\textbf{Recommender Abbr.}} &\multicolumn{1}{c}{\textbf{Description}} \\
\bottomrule
\textbf{Classical RS} & \\    \hline \myrowcolour

MF~\cite{DBLP:journals/computer/KorenBV09} & Matrix Factorization (MF) is the state-of-the-art recommendation model for implicit datasets. \\    \hline

BPR-MF~\cite{DBLP:conf/uai/RendleFGS09}  & Bayesian Personalized Ranking (BPR-MF) is a highly competitive MF-model for item recommendation optimized with a pairwise objective function (BPR). \\    \hline \myrowcolour

FM~\cite{DBLP:conf/icdm/Rendle10} & Factorization Machine (FM) is a generalized MF model that encodes (users, items, features)-interactions into a joint dot-product space. \\  \hline

VBPR~\cite{DBLP:conf/aaai/HeM16} & Visual Bayesian Pairwise Ranking (VBPR) model integrates items' visual features --- extracted by a CNN --- in the BPR-MF preference prediction. \\  \hline 

\textbf{Deep-Learning RS} & \\    \hline \myrowcolour

CDL~\cite{DBLP:conf/kdd/WangWY15} & Collaborative Deep Learning (CDL) is a hybrid model combines the extraction of deep items' features with the collaborative user-item feedbacks.  \\  \hline

AutoRec~\cite{DBLP:conf/www/SedhainMSX15}& AutoRec reconstructs partial user profiles (i.e., item recommendation) based on the reconstruction power of auto-encoders .  \\  \hline \myrowcolour

% CDAE~\cite{DBLP:conf/wsdm/WuDZE16}& Collaborative Denoising Auto-Encoder (CDAE) generalizes latent factor models by learning full-users preferences thanks to the reconstruction from a sub-set of preferences.   \\  \hline

CVAE~\cite{DBLP:conf/kdd/LiS17} & Collaborative Variational Auto-Encoder (CVAE) performs recommendations by learning both deep user-item latent representations from content data and implicit user-item relationships from both content and ratings.  \\  \hline 

RRN~\cite{DBLP:conf/wsdm/WuABSJ17} & Recurrent Recommender Networks (RRN) predicts future user preferences by integrating MF with a Long Short-Term Memory (LSTM) model to capture dynamics.\\  \hline \myrowcolour

NCF~\cite{DBLP:conf/www/HeLZNHC17} & Neural Collaborative Filtering (NCF) learns user-item preference function by replacing the inner product of MF with a neural architecture to extract non-linear relations. \\  

\bottomrule
\end{tabular}}}
\end{table}


==> Tables/gan_basic.tex <==
% \begin{table}
% \small
% \centering
% \caption{Conceptual goals, inputs, and outputs of XXX \yashar{Please improve and define the variables shortly e.g., $d$, $q$, ...}\felice{*I think that the input of the generator is important because the CFGAN has a conditioned input}}
% \label{tbl:MMRS}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Appr} & \textbf{Input} of Gen?* & \begin{tabular}[c]{@{}c@{}} \textbf{Type of $G$ and $D$ } \\\textbf{models}\end{tabular} & \textbf{Goal/Output of $G$ and $D$} \\ \hline



% \begin{tabular}[c]{@{}c@{}} IRGAN \\\cite{DBLP:conf/sigir/WangYZGXWZZ17}\end{tabular} & \begin{tabular}[c]{@{}c@{}} queries/users \\ docs/items\end{tabular} &
% \begin{tabular}[c]{@{}c@{}} $G$: MF \\ $D$: BPR \end{tabular} & 

% \begin{tabular}[c]{@{}c@{}}  
% $G$: generate $p_{\theta}(d|q,r) \simeq p_{true}(d|q,r)$; \\ \yashar{one/more items index/ices?}\\ \felice{Generate relevant items given a user} \\ 
% $D$: discriminate well/ill-matched ($q$,$d$); \\ a scalar representing the rel of ($q$,$d$) 
% \end{tabular} 


% \\ \hline


% \begin{tabular}[c]{@{}c@{}} GraphGAN \\\cite{DBLP:conf/aaai/WangWWZZZXG18}\end{tabular}& \begin{tabular}[c]{@{}c@{}} nodes/edges \end{tabular} & 
% \begin{tabular}[c]{@{}c@{}} $G$: MF 
% % \yashar{xxx}  
% \\
% $D$: BPR ~\felice{[cite?]}
% % \yashar{xxx} 
% \end{tabular} &
% \begin{tabular}[c]{@{}c@{}}  $G$: generate $p_{\theta}(v|v_c) \simeq p_{true}(v|v_c)$; \\ \felice{Generate most similar nodes given a node}
% \\ $D$: discriminate the connectivity for vertex \\ pair ($v$,$v_c$);  a scalar representing the prob \\ of an edge existing btw vertex  pair ($v$,$v_c$) 

% \end{tabular} 
% \\ \hline



% \begin{tabular}[c]{@{}c@{}} CFGAN \\\cite{DBLP:conf/cikm/ChaeKKL18}\end{tabular}& \begin{tabular}[c]{@{}c@{}} nodes/edges \end{tabular} & 
% \begin{tabular}[c]{@{}c@{}} $G$: MF \\ $D$: BPR \end{tabular} & 
% \begin{tabular}[c]{@{}c@{}}  $G$: \felice{Generate "plausible purchase vector"} \\
% \felice{starting from real-valued elements}\\ 

% $D$: discriminate the generated vector \\with the real-one   \end{tabular} \\ \hline

% \end{tabular}
% \end{table}

==> Tables/old_table_security_datasets_metrics.tex <==
\begin{table}[!t]
\caption{Evaluation and domain comparison of adversarial machine learning approaches for attack and defense on RS  (ML: Movielens, FL: FilmTrust, EM: EachMovie, CD: CiaoDVD, Yelp: YE, LFM: LastFM, PI: Pinterest, AM: Amazon, 30M: 30Music , YA: Yahoo, AotM: Art of the Mix)
\tommaso{Put a list of the baselines together with a reference. As far as I can see, some of them are not metioned anywhere within the paper. In case, we can also put them in Table \ref{tbl:recommender_models}}\yashar{This is true, we should add it.}
}
\label{tbl:adl_evaluation}
{\scalebox{0.70}{\begin{tabular}{p{1.70cm} c c|p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm} p{0.13cm}|c c c|}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Model \\  Name\end{tabular}}
&\multicolumn{1}{c}{\textbf{Authors}}
&\multicolumn{1}{c}{\textbf{Year}} & \multicolumn{9}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Evaluation \end{tabular}}} 
& \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Domain \& Dataset\end{tabular}}} \\ 
\cmidrule(r){1-1}\cmidrule(r){2-2}\cmidrule(r){3-3}\cmidrule(r){4-12}\cmidrule(r){13-15}
&
&
& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}pref. \\ type\end{tabular}} 
& \multicolumn{7}{c|}{\begin{tabular}[c]{@{}c@{}}evaluation \\ metric \end{tabular}}
&
domain
&baselines &datasets \\
\cmidrule(lr){4-5}\cmidrule(lr){6-12}
&
&
&\rotatebox{90}{\small{implicit}} &\rotatebox{90}{\small{explicit}}  &\rotatebox{90}{\small{NDCG}}  &\rotatebox{90}{\small{HR}} 
&\rotatebox{90}{\small{SR}} 
& \rotatebox{90}{\small{F1}} 
&\rotatebox{90}{\small{$L_2$-dist.}}
&\rotatebox{90}{\small{Precision}}
&\rotatebox{90}{\small{MAP}}
& & &
\\
\bottomrule
\small{APR~\cite{DBLP:conf/sigir/0001HDC18}} &He at al. &2018 &\cmark & &\cmark &\cmark & & & & & &\small{tourism, SM/SN} &\begin{tabular}[c]{@{}c@{}} \small{ItemPop, MF-BPR, CDAE,} \\ \small{NeuMF, IRGAN}\end{tabular} &\begin{tabular}[c]{@{}c@{}} \small{YE, PI, GO} \end{tabular}  \\
\myrowcolour
\small{ACAE~\cite{DBLP:conf/ijcnn/YuanYB19}} &Yuan et al. &2019 &\cmark & & &\cmark & & & & & &\small{movie} &\begin{tabular}[c]{@{}c@{}} \small{ItemPop, MF-BPR, CDAE,} \\ \small{NeuMF, AMF} \end{tabular} &\begin{tabular}[c]{@{}c@{}} \small{ML 1M, CD, FT}\end{tabular} \\
\small{FGACAE~\cite{DBLP:conf/sigir/YuanYB19}} &Yuan et al. &2019 &\cmark & & &\cmark & & & & & &\small{movie}  &\begin{tabular}[c]{@{}c@{}}\small{ItemPop, MF-BPR, CDAE,} \\ \small{JRL, NeuMF, ConvNCF, AMF}\end{tabular} &\begin{tabular}[c]{@{}c@{}} \small{ML 1M, CD, FT} \end{tabular}\\
\myrowcolour
\small{AMR~\cite{8618394}} &Tang et al. &2019 &\cmark & &\cmark &\cmark & & & & & &\small{fashion}  &\begin{tabular}[c]{@{}c@{}} \small{ItemPop, MF-BPR, MF-eALS,} \\ \small{DUIF, VBPR}\end{tabular} &\small{PI, AM}   \\
\small{FNCF~\cite{DBLP:journals/tmm/DuFYXCT19}} &Du et al. &2019 &\cmark & &\cmark &\cmark &\cmark & &\cmark & & &\small{movie}  &\begin{tabular}[c]{@{}c@{}}  \small{FNCF-Distill, FNCF-Single,} \\ \small{FNCF-Multi}\end{tabular} &\small{ML (100k, 1M)} \\
\myrowcolour
\small{ATF~\cite{DBLP:conf/recsys/ChenL19}} &Chen et al. &2019 & \cmark &  & & & &\cmark & & & &\small{movie, music} &\begin{tabular}[c]{@{}c@{}} \small{CANDECOMP/PARAFAC (CP),} \\ \small{HOSVD, PITF}\end{tabular} &\small{ML, LFM}  \\
\small{GANAtt~\cite{DBLP:conf/recsys/Christakopoulou19}} & Christ. et al. & 2019 & &\cmark  & & & & & & & &\small{movie} & low-rank recommenders & ML 1M \\ [5pt]
\myrowcolour
\small{AdvIR~\cite{DBLP:conf/www/ParkC19}} &Park et al. &2019 & \cmark & & & & & & &  \cmark & &\small{movie} & MF-BPR, LambdaFM, IRGAN & ML 100K  \\
\small{AMASR~\cite{DBLP:conf/sigir/TranSL19}} &Tran et al. &2019  & \cmark & &\cmark &\cmark & & & & & &\small{music} &\begin{tabular}[c]{@{}c@{}} MF-BPR, CML, NeuMF, FISM, \\ CMN, PRME, Transrec, Caser \end{tabular}& 30M, AotM  \\
\myrowcolour
\small{ATMBPR~\cite{DBLP:journals/access/WangH20a}} &Wang et al. &2020 & \cmark & &\cmark &\cmark & & & &\cmark & &\begin{tabular}[c]{@{}c@{}}\small{tourism,}\\\small{SM/SN, movie} \end{tabular} &\begin{tabular}[c]{@{}c@{}}MF-BPR, CDAE, MPR, AMF \\ MLP, NeuMF, LRML, JRL\end{tabular} &\begin{tabular}[c]{@{}c@{}} ML (100k, 1M), \\ YA, YE, PI\end{tabular} \\
\small{SACRA~\cite{DBLP:conf/wsdm/LiW020}} &Li et al. &2020 & \cmark & & & & & & & &\cmark &\begin{tabular}[c]{@{}c@{}} \small{tourism,} \\ \small{SM/SN,} \\ \small{business}\end{tabular} & \begin{tabular}[c]{@{}c@{}} WRMF, MMMF, MF-BPR, CofiRank,  \\ CLiMF, USG, GeoMF, Rank-GeoMF, \\ ASMF, ARMF, CORALS, SAE-NAD \end{tabular}& YE, FS  \\
\myrowcolour
\small{RAP~\cite{DBLP:conf/wsdm/BeigiMGAN020}} & Beigi et al. & 2020 & \cmark & & \cmark & &  & & & & &\small{movie} & \begin{tabular}[c]{@{}c@{}}Privacy preservation models:  \\ LDP-SH, BlurME \end{tabular}& ML 100k \\
\small{TAaMR~\cite{DBLP:conf/dsn/DiNoia20}} & Di Noia et al. & 2020 & \cmark & & & \cmark &  & & & & &\small{fashion} & \begin{tabular}[c]{@{}c@{}}VBPR, AMR \end{tabular}& \begin{tabular}[c]{@{}c@{}} AM Men, \\ AM Women  \end{tabular} \\
\bottomrule
\end{tabular}}}
\end{table}

